Ontology Reasoning with Deep Neural Networks

The ability to conduct logical reasoning is a fundamental aspect of intelligent human behavior, and thus an important problem along the way to human-level artificial intelligence. Traditionally, logic-based symbolic methods from the field of knowledge representation and reasoning have been used to equip agents with capabilities that resemble human logical reasoning qualities. More recently, however, there has been an increasing interest in using machine learning rather than logic-based symbolic formalisms to tackle these tasks. In this paper, we employ state-of-the-art methods for training deep neural networks to devise a novel model that is able to learn how to effectively perform logical reasoning in the form of basic ontology reasoning. This is an important and at the same time very natural logical reasoning task, which is why the presented approach is applicable to a plethora of important real-world problems. We present the outcomes of several experiments, which show that our model is able to learn to perform highly accurate ontology reasoning on very large, diverse, and challenging benchmarks. Furthermore, it turned out that the suggested approach suffers much less from different obstacles that prohibit logic-based symbolic reasoning, and, at the same time, is surprisingly plausible from a biological point of view.

==> map.tex <==
\newcommand{\Europe}{

    % //////// ALBANIA /////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (352.7484,311.4419) .. controls (353.1384,310.7759) and
    (353.4684,309.9919) .. (353.1884,309.2109) .. controls (354.2384,309.3799) and
    (353.6984,306.9599) .. (353.9184,306.1759) .. controls (354.0884,305.5709) and
    (353.1484,305.5409) .. (353.4884,304.7699) .. controls (353.7384,304.1919) and
    (353.9484,303.5839) .. (354.0784,302.9639) .. controls (354.2984,301.9079) and
    (354.0784,300.7349) .. (352.7484,301.0739) .. controls (352.2284,299.4759) and
    (352.2484,297.3319) .. (353.2584,295.9839) .. controls (354.0884,294.8889) and
    (354.2284,293.1449) .. (355.3884,295.1859) .. controls (356.1184,296.4789) and
    (357.2384,293.6599) .. (358.3284,295.7449) .. controls (358.5584,296.1779) and
    (358.5184,296.4929) .. (358.8784,296.8389) .. controls (359.5684,297.5059) and
    (360.0284,296.8189) .. (361.0784,298.2819) .. controls (361.2484,298.5289) and
    (361.5384,300.0769) .. (361.4684,301.2839) .. controls (360.3284,302.0079) and
    (361.7284,303.1589) .. (360.5484,303.7199) .. controls (360.6484,304.1549) and
    (360.9784,304.4889) .. (361.1684,304.8569) .. controls (361.1684,305.1739) and
    (361.2984,305.3409) .. (361.0684,305.6089) .. controls (360.9284,306.3039) and
    (361.4984,307.2239) .. (361.9684,307.5969) .. controls (362.5184,308.0349) and
    (362.3584,309.1249) .. (363.3684,309.0069) .. controls (364.3584,308.8909) and
    (364.2984,309.4879) .. (364.6084,310.1839) .. controls (365.8184,312.8859) and
    (363.8884,312.2549) .. (363.1984,313.9649) .. controls (362.9684,314.5399) and
    (362.3784,315.8699) .. (361.7284,316.2139) .. controls (360.0584,317.1009) and
    (360.1184,317.0319) .. (360.7784,318.6409) .. controls (359.2784,318.4619) and
    (361.2384,319.5399) .. (359.2584,319.8659) .. controls (358.1084,320.0549) and
    (357.7884,319.4229) .. (357.6484,318.5049) .. controls (357.2684,316.1149) and
    (354.0884,315.2589) .. (352.7084,313.3849) .. controls (353.1884,313.4649) and
    (353.5284,313.7239) .. (353.7184,314.1769) .. controls (354.4384,313.3439) and
    (353.0484,312.8169) .. (353.8184,312.5209) .. controls (353.3784,312.2419) and
    (353.0184,311.8809) .. (352.7384,311.4419);
    
    
    % //////// ANDORRA /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]

        \path[country]
        (1287.4900,391.3180) .. controls (1288.0400,390.6020) and (1289.3400,390.9530)
        .. (1289.7900,391.6060) .. controls (1289.3000,392.2530) and
        (1288.4800,392.5930) .. (1287.7000,392.6860) .. controls (1287.7000,392.2250)
        and (1287.5900,391.7690) .. (1287.4900,391.3180);

    \end{scope}
    
    
    % //////// AUSTRIA /////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country, we]
    (284.2784,254.9229) .. controls (284.9884,253.6849) and
    (284.8384,254.0349) .. (284.4984,252.9169) .. controls (284.3784,252.5319) and
    (289.8884,252.6949) .. (288.5984,254.9229) .. controls (290.1584,254.8729) and
    (290.1984,253.4119) .. (290.5484,252.2569) .. controls (291.2084,252.8519) and
    (292.7884,252.8579) .. (293.6184,252.7789) .. controls (292.9384,253.1279) and
    (294.8184,253.7229) .. (295.0484,253.6459) .. controls (295.5384,253.8789) and
    (296.2684,253.2079) .. (296.9484,252.9779) .. controls (298.3084,252.1539) and
    (300.5884,251.5529) .. (302.1384,252.0599) .. controls (302.1384,251.7909) and
    (302.1384,251.5089) .. (302.0184,251.2499) .. controls (302.7884,251.3499) and
    (304.0384,251.9899) .. (304.8084,251.6259) .. controls (306.4084,250.8639) and
    (306.2284,252.6439) .. (307.2184,253.0169) .. controls (308.0184,253.3229) and
    (308.3484,251.3669) .. (307.6584,251.2719) .. controls (306.7584,251.1479) and
    (307.3084,250.1199) .. (307.1984,249.6569) .. controls (307.0584,249.0339) and
    (306.5084,248.8549) .. (306.2484,248.2999) .. controls (305.5884,246.8819) and
    (309.2484,246.3949) .. (309.9784,245.9009) .. controls (310.6084,245.4739) and
    (310.1184,243.6199) .. (311.2984,244.0649) .. controls (312.8784,244.6649) and
    (311.9584,243.0229) .. (312.3284,241.5909) .. controls (313.4584,241.8889) and
    (314.7884,243.6859) .. (316.0684,243.8529) .. controls (318.3984,243.2669) and
    (318.6084,243.8229) .. (318.8384,243.9029) .. controls (318.8384,243.2069) and
    (319.2284,242.5259) .. (319.9184,242.3019) .. controls (320.8184,242.0109) and
    (320.7084,241.3819) .. (320.7784,240.2309) .. controls (322.2684,240.1009) and
    (324.0584,240.7929) .. (325.4584,241.2579) .. controls (325.9284,241.0089) and
    (328.2084,242.7929) .. (329.9084,242.3879) .. controls (331.2384,242.0719) and
    (333.8084,241.9339) .. (334.0084,243.5079) .. controls (334.0084,243.6999) and
    (334.0084,244.4519) .. (334.2084,245.1269) .. controls (334.3884,245.8689) and
    (334.2084,246.9319) .. (334.6384,247.4769) .. controls (335.1684,248.2219) and
    (335.9084,248.3549) .. (335.8384,248.8319) .. controls (335.7384,249.3099) and
    (334.9084,250.1229) .. (334.5484,251.0589) .. controls (333.8784,252.8189) and
    (333.0584,250.5779) .. (331.4184,251.2349) .. controls (330.7084,251.5199) and
    (334.0084,252.2059) .. (332.0484,253.2019) .. controls (330.5184,253.9819) and
    (330.9184,256.0429) .. (331.3684,257.2219) .. controls (330.2684,256.9889) and
    (327.4484,258.6479) .. (328.3484,260.1019) .. controls (326.7784,259.1109) and
    (326.0484,260.2459) .. (324.5684,260.3809) .. controls (323.4984,260.4809) and
    (322.7584,259.9729) .. (321.7484,260.1769) .. controls (320.9884,260.3319) and
    (319.3384,261.9249) .. (318.7384,262.2389) .. controls (317.6084,262.8279) and
    (314.6984,261.4859) .. (313.5684,261.3229) .. controls (310.6584,260.9009) and
    (308.0984,261.2629) .. (305.1084,260.3229) .. controls (304.1984,260.0379) and
    (300.7584,257.6159) .. (302.4984,256.5729) .. controls (301.5084,256.3659) and
    (300.6984,257.0869) .. (299.7584,257.2209) .. controls (298.3884,257.4179) and
    (297.2184,257.2309) .. (295.8384,257.6229) .. controls (295.0184,257.8549) and
    (294.3584,259.3389) .. (293.5084,259.0909) .. controls (292.6484,258.8399) and
    (291.8684,258.6439) .. (290.9984,258.4289) .. controls (290.2884,258.2509) and
    (290.6684,257.4209) .. (290.1984,257.3449) .. controls (289.6484,257.2549) and
    (289.2784,257.7799) .. (288.9484,258.1879) .. controls (288.3384,258.9349) and
    (286.6084,257.8739) .. (286.1284,257.3539) .. controls (285.5984,256.7899) and
    (284.8284,256.7059) .. (284.5284,256.7009) .. controls (284.8184,256.0419) and
    (284.6484,255.4429) .. (284.2784,254.9189);
    

    % //////// BELARUS /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}
    
        \path[shift={(-12.49595,1.66613)}, country]
        (373.6284,212.9909) .. controls (374.0984,211.7529) and
        (374.7584,210.5809) .. (376.2084,210.3169) .. controls (377.6384,210.0559) and
        (378.0684,208.9639) .. (377.9184,207.6349) .. controls (377.5484,204.5159) and
        (374.8484,202.3409) .. (374.3484,199.2659) .. controls (375.9784,199.6829) and
        (378.0884,199.3839) .. (379.7884,199.5789) .. controls (380.3084,199.6389) and
        (381.0884,199.2419) .. (381.5884,199.1169) .. controls (382.5884,198.8649) and
        (382.3384,198.4029) .. (383.0584,197.7909) .. controls (383.5084,197.4129) and
        (384.0684,197.7709) .. (384.5384,197.5459) .. controls (384.9184,197.3679) and
        (385.0984,196.9509) .. (385.4884,196.7679) .. controls (386.2384,196.4179) and
        (387.7884,196.3169) .. (387.3084,197.6099) .. controls (387.7284,197.7469) and
        (388.3984,197.6999) .. (388.6684,197.2829) .. controls (389.2484,196.3829) and
        (387.6284,196.0749) .. (387.1684,195.8829) .. controls (388.8084,194.0989) and
        (387.5284,192.1959) .. (389.8284,190.9869) .. controls (390.8984,190.4249) and
        (391.0084,189.2779) .. (392.4184,189.4039) .. controls (393.9584,189.5409) and
        (393.2084,188.7459) .. (394.3684,188.1779) .. controls (392.7584,187.7499) and
        (391.1184,187.0499) .. (392.7784,185.1289) .. controls (393.8384,183.9029) and
        (396.1784,183.5429) .. (397.6484,183.9869) .. controls (399.4384,184.5219) and
        (399.4884,182.1159) .. (401.1184,181.5159) .. controls (401.9884,181.1969) and
        (403.3184,182.1029) .. (403.7484,181.7519) .. controls (405.3784,181.6069) and
        (409.9084,181.8119) .. (410.2884,182.9419) .. controls (410.6584,183.2859) and
        (410.0484,184.0269) .. (410.4784,184.4449) .. controls (411.0584,185.0079) and
        (413.0684,184.2299) .. (413.6784,183.9379) .. controls (415.8184,182.9109) and
        (416.6384,183.4879) .. (418.5584,184.8469) .. controls (419.0784,185.2159) and
        (420.4584,185.3629) .. (420.4184,186.4619) .. controls (420.4184,187.7849) and
        (420.3184,188.0699) .. (421.0084,189.2649) .. controls (421.4384,190.0519) and
        (421.6384,190.3159) .. (420.8584,190.8839) .. controls (419.7884,191.6549) and
        (421.5184,192.7899) .. (422.1584,193.4079) .. controls (423.5384,194.7329) and
        (423.9784,196.8469) .. (426.1384,197.5959) .. controls (426.7684,197.8109) and
        (427.7884,198.0109) .. (428.0584,198.7139) .. controls (428.4184,199.6209) and
        (427.3684,200.5219) .. (428.2784,200.5229) .. controls (428.6584,200.4729) and
        (429.1484,200.4829) .. (429.4984,200.3479) .. controls (429.9984,200.2459) and
        (430.5884,200.5549) .. (431.0884,200.6169) .. controls (432.7584,200.8279) and
        (431.7284,201.2079) .. (432.4084,201.9819) .. controls (432.7584,202.3849) and
        (433.7984,202.6399) .. (434.2684,203.2739) .. controls (435.2484,204.5889) and
        (433.7084,204.7019) .. (433.2684,204.9959) .. controls (432.4684,205.5219) and
        (432.2184,205.8689) .. (430.9884,206.1689) .. controls (429.4584,206.5419) and
        (428.5884,205.1639) .. (427.2484,205.4439) .. controls (423.9084,206.1409) and
        (426.0284,207.4329) .. (427.1484,208.3189) .. controls (427.8884,208.8819) and
        (427.7384,210.0479) .. (427.9384,210.8589) .. controls (428.2684,212.1879) and
        (429.2684,213.2889) .. (429.9784,214.4359) .. controls (428.3684,214.4359) and
        (429.0384,214.0329) .. (426.1984,214.9319) .. controls (425.0184,214.2499) and
        (423.0284,215.4419) .. (422.3884,217.5049) .. controls (422.1084,218.4169) and
        (422.6584,219.0969) .. (422.8084,220.5259) .. controls (422.9684,222.1309) and
        (420.9684,220.7499) .. (420.5684,220.2609) .. controls (419.3984,218.8429) and
        (418.1884,220.4989) .. (416.7584,219.6899) .. controls (413.4484,221.4949) and
        (414.3484,219.2149) .. (412.8084,218.7249) .. controls (411.8884,218.2439) and
        (410.3784,219.1579) .. (410.5184,220.2199) .. controls (409.9684,219.9719) and
        (409.9484,219.1359) .. (409.4384,218.9249) .. controls (408.9084,218.7049) and
        (408.2484,219.3209) .. (407.7884,218.9849) .. controls (407.1484,218.5199) and
        (406.5084,218.5569) .. (405.7684,218.6399) .. controls (404.7684,218.7519) and
        (404.3084,218.0769) .. (404.1784,219.2779) .. controls (403.5584,219.1199) and
        (403.1084,218.5519) .. (402.4684,218.4859) .. controls (401.7484,218.4159) and
        (400.9384,219.0459) .. (400.3584,218.2499) .. controls (399.1384,216.5599) and
        (397.2884,217.2339) .. (395.5684,216.8739) .. controls (393.7984,216.5049) and
        (391.7584,215.6319) .. (389.9584,215.9529) .. controls (387.5684,216.0329) and
        (385.6384,216.1519) .. (383.6184,216.1819) .. controls (381.4484,216.1819) and
        (381.5284,217.1129) .. (380.0584,218.3069) .. controls (379.2684,218.9389) and
        (378.5584,218.4289) .. (377.7184,218.2669) .. controls (376.5984,218.0479) and
        (376.8084,218.7269) .. (376.5584,219.3729) .. controls (375.7984,220.5199) and
        (376.6584,215.9929) .. (376.6584,215.6679) .. controls (376.7584,213.2029) and
        (373.9584,214.6199) .. (373.6484,212.9629);
    
    \end{scope}[draw, fill, red]
    
    
    % //////// BELGIUM /////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country, we, query]
    (238.2084,222.9819) .. controls (239.9884,222.0559) and
    (242.1384,221.1219) .. (244.0884,220.6049) .. controls (243.1684,221.5859) and
    (245.3684,221.3489) .. (246.1184,221.5329) .. controls (246.7584,221.6869) and
    (247.0784,221.9599) .. (247.7784,221.7709) .. controls (248.6484,221.5369) and
    (249.6384,220.0769) .. (249.9384,221.4409) .. controls (249.8284,221.1339) and
    (249.7284,220.8219) .. (249.6484,220.5039) .. controls (250.3084,220.6489) and
    (251.1084,220.6129) .. (251.0184,219.7129) .. controls (251.5384,220.1089) and
    (252.3984,220.3469) .. (252.8184,219.6429) .. controls (253.1684,220.5059) and
    (254.4284,220.2269) .. (254.8984,219.6429) .. controls (255.4484,221.6699) and
    (258.4184,221.6639) .. (260.1584,222.3779) .. controls (259.2284,223.4679) and
    (258.2484,224.7869) .. (259.9084,225.6179) .. controls (260.4784,225.8999) and
    (260.8384,225.7649) .. (261.2284,225.6879) .. controls (260.9384,226.4139) and
    (263.3184,226.7029) .. (262.3184,227.7079) .. controls (263.3084,227.5409) and
    (263.2584,228.6859) .. (263.5484,229.2919) .. controls (262.3984,229.4999) and
    (262.5084,230.1349) .. (261.7984,230.7259) .. controls (261.5084,230.9649) and
    (260.7784,230.3559) .. (260.1284,231.3799) .. controls (259.5784,232.2459) and
    (259.1384,232.6709) .. (259.2784,233.4279) .. controls (259.4484,234.1979) and
    (260.6184,235.1669) .. (259.2784,236.0859) .. controls (259.0084,236.0559) and
    (258.1684,236.0759) .. (257.2984,235.9759) .. controls (257.1884,235.7899) and
    (256.6784,234.9609) .. (256.1184,234.6319) .. controls (255.3684,234.1829) and
    (253.8284,234.0549) .. (253.3484,233.4689) .. controls (253.0284,233.0789) and
    (253.2484,231.1449) .. (253.2084,230.5879) .. controls (252.5384,230.8519) and
    (252.3484,231.4099) .. (251.8784,231.8719) .. controls (251.0084,232.7209) and
    (249.6384,232.3459) .. (248.5984,232.1719) .. controls (248.8184,231.2929) and
    (249.2184,229.9089) .. (248.4884,229.4369) .. controls (247.6184,228.8749) and
    (246.2584,228.8979) .. (245.6484,229.2919) .. controls (245.7584,227.9359) and
    (244.8684,228.2539) .. (243.8784,227.8389) .. controls (242.7184,227.3479) and
    (243.0184,227.3259) .. (242.3684,226.3139) .. controls (242.1384,225.9449) and
    (239.9384,226.0099) .. (239.4684,225.7279) .. controls (238.1284,224.9149) and
    (239.3084,223.3549) .. (238.2284,222.9739);
    
    
    % //////// BOSNIA //////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (326.8984,273.5699) .. controls (326.7984,271.2259) and
    (328.7784,272.8909) .. (329.6784,273.6299) .. controls (330.6584,274.4259) and
    (331.3384,273.7549) .. (331.7284,272.7469) .. controls (332.0984,271.7789) and
    (333.5784,272.4299) .. (334.2484,272.5659) .. controls (334.3684,271.6239) and
    (338.3184,273.2139) .. (339.2184,273.2139) .. controls (339.8384,273.2139) and
    (340.9684,273.8439) .. (341.4684,273.4909) .. controls (342.6284,272.6779) and
    (342.3284,273.6559) .. (343.3484,273.4309) .. controls (344.6084,273.1539) and
    (345.6984,273.4709) .. (346.8684,273.9379) .. controls (347.8484,274.3329) and
    (347.2384,275.2799) .. (348.4984,275.3489) .. controls (349.2784,275.3889) and
    (350.3484,274.5489) .. (351.0384,274.8919) .. controls (352.1384,275.4449) and
    (351.2184,276.9659) .. (350.7584,277.5799) .. controls (349.2384,279.6219) and
    (350.9184,280.3179) .. (352.4084,281.4509) .. controls (354.9784,283.4059) and
    (351.6684,282.4389) .. (351.2884,282.9809) .. controls (351.2884,283.0509) and
    (353.0584,285.3159) .. (353.0684,285.8729) .. controls (353.0684,286.3589) and
    (349.6484,287.0129) .. (349.0784,286.8229) .. controls (348.9384,287.7309) and
    (350.0684,288.0979) .. (349.6584,289.0549) .. controls (349.0984,287.2129) and
    (346.4384,289.5489) .. (347.2784,291.0709) .. controls (344.4584,290.4479) and
    (348.0584,295.0109) .. (346.3184,294.9789) .. controls (345.2084,294.9589) and
    (343.2584,293.6189) .. (342.4084,292.9369) .. controls (341.9584,292.5769) and
    (341.8984,292.1439) .. (341.2684,292.0619) .. controls (340.6884,291.9819) and
    (340.5284,292.5569) .. (339.9384,291.7189) .. controls (341.8184,291.6889) and
    (338.2484,288.7049) .. (337.9184,288.2949) .. controls (336.2284,286.1949) and
    (334.9784,285.4879) .. (333.4384,283.7599) .. controls (332.6484,282.8729) and
    (331.6084,282.4099) .. (330.7984,281.5749) .. controls (329.8584,280.5929) and
    (330.4684,279.0119) .. (329.5684,277.9169) .. controls (328.8884,277.0849) and
    (328.0084,276.8699) .. (327.1684,276.2829) .. controls (326.7484,275.9899) and
    (326.9684,274.2139) .. (326.8984,273.5759);
    
    
    % //////// BULGARIA ////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (372.8384,284.5859) .. controls (372.8384,283.4089) and
    (373.7984,281.7989) .. (374.5284,280.9179) .. controls (374.7684,280.6359) and
    (376.7484,281.5939) .. (376.8684,281.8509) .. controls (377.1884,282.5529) and
    (375.8184,283.2519) .. (376.2284,283.9669) .. controls (376.8384,285.0099) and
    (380.1784,284.0169) .. (381.2084,284.2309) .. controls (382.8984,284.5829) and
    (384.7484,285.7739) .. (386.4684,285.1569) .. controls (387.8484,284.6599) and
    (389.5884,285.0459) .. (391.0584,285.1569) .. controls (393.2284,285.3299) and
    (394.3884,286.3029) .. (396.3884,284.7779) .. controls (397.9384,283.5979) and
    (399.0084,282.6469) .. (400.9984,282.3029) .. controls (402.8084,281.9889) and
    (404.7484,280.9799) .. (406.5184,281.9049) .. controls (407.6484,282.4939) and
    (409.2684,282.9689) .. (410.5284,282.7369) .. controls (410.9684,282.6569) and
    (412.5984,284.4169) .. (413.2284,284.6669) .. controls (414.0684,285.0039) and
    (415.5584,284.3269) .. (415.7084,285.5429) .. controls (415.8584,286.8559) and
    (416.0484,287.8649) .. (414.4584,287.7419) .. controls (412.8684,287.6189) and
    (412.1384,288.7829) .. (411.4984,290.0949) .. controls (410.9384,291.2249) and
    (411.4984,292.4889) .. (410.8584,293.7269) .. controls (410.6484,294.1059) and
    (410.3984,294.4679) .. (410.1784,294.8379) .. controls (409.8084,295.4369) and
    (409.0684,295.0319) .. (408.6984,295.7429) .. controls (410.6584,296.1879) and
    (411.0284,297.6019) .. (412.2884,298.9129) .. controls (413.8384,300.5269) and
    (410.4284,300.5089) .. (409.4084,300.2219) .. controls (408.3084,299.9109) and
    (408.1984,298.7789) .. (406.8084,299.1779) .. controls (405.7784,299.4749) and
    (404.9584,299.7589) .. (403.8884,300.1019) .. controls (402.2884,300.6189) and
    (403.3584,300.8139) .. (403.0084,300.9979) .. controls (402.4084,301.3089) and
    (401.1884,301.8929) .. (401.8484,302.3659) .. controls (396.9484,301.3959) and
    (402.5884,304.4789) .. (399.6584,305.5679) .. controls (398.3484,306.0579) and
    (398.6884,305.2309) .. (394.9184,306.0369) .. controls (393.8284,306.2699) and
    (392.9584,305.0959) .. (391.9884,305.1509) .. controls (390.7284,305.2209) and
    (390.6284,305.6729) .. (389.4384,304.1389) .. controls (388.7484,303.2399) and
    (387.9784,303.4219) .. (386.9584,303.5859) .. controls (385.5584,303.8139) and
    (384.6784,305.4509) .. (383.1884,305.4189) .. controls (381.2484,305.3789) and
    (380.3884,305.3289) .. (379.7884,305.8499) .. controls (379.4584,306.1369) and
    (378.4584,305.8599) .. (377.5584,305.5889) .. controls (378.2884,304.7729) and
    (377.5584,303.5769) .. (377.5584,302.3469) .. controls (377.6584,301.1089) and
    (376.3484,299.9399) .. (375.4784,299.2269) .. controls (374.5984,298.7029) and
    (373.8384,297.4829) .. (373.1384,296.7599) .. controls (376.4584,295.7749) and
    (373.0384,294.9959) .. (373.9684,292.7089) .. controls (374.2884,291.9199) and
    (375.0584,292.4799) .. (375.5884,292.1409) .. controls (376.2484,291.7249) and
    (377.0884,290.3239) .. (377.3984,289.6229) .. controls (375.4684,289.0089) and
    (373.0584,286.4409) .. (372.7884,284.5799);
    
    
    % //////// CROATIA /////////////////////////////////////////////////////////////////////////////

    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path4066
        \path[country]
        (1371.4400,366.7700) .. controls (1371.9300,366.8850) and (1372.4200,367.0140)
        .. (1372.9200,367.1210) .. controls (1373.5600,367.2590) and
        (1374.0700,366.6380) .. (1374.4200,366.5170) .. controls (1374.5900,366.4570)
        and (1376.0400,367.8530) .. (1378.1400,365.1680) .. controls
        (1379.4500,366.4460) and (1380.5100,365.9840) .. (1381.9200,366.7700) ..
        controls (1383.7700,367.7970) and (1382.8600,365.5300) .. (1383.6800,365.3300)
        .. controls (1383.3200,365.2500) and (1383.0200,364.9420) ..
        (1382.6700,364.8260) .. controls (1385.5200,362.7790) and (1386.2000,364.9370)
        .. (1385.1600,361.0410) .. controls (1385.0300,360.5450) and
        (1387.5300,360.0990) .. (1387.9400,359.7070) .. controls (1388.5700,359.1060)
        and (1387.9400,359.3160) .. (1388.5700,358.8870) .. controls
        (1388.5700,358.8870) and (1389.5600,359.1340) .. (1389.7300,359.1390) ..
        controls (1387.8300,356.9720) and (1391.4000,357.8370) .. (1392.1100,358.5520)
        .. controls (1392.6200,359.0560) and (1395.3300,360.6860) ..
        (1395.6900,361.1780) .. controls (1397.1400,362.8060) and (1399.2500,363.6030)
        .. (1401.5100,364.3390) .. controls (1406.8900,364.6390) and
        (1404.4500,363.2260) .. (1406.8300,362.8980) .. controls (1406.8300,362.3790)
        and (1407.2100,363.4800) .. (1407.5200,364.1290) .. controls
        (1407.9700,365.0650) and (1407.5200,366.2830) .. (1408.9500,366.3390) ..
        controls (1406.6600,367.9320) and (1411.7000,368.8430) .. (1411.1700,369.1730)
        -- (1408.9500,369.7230) .. controls (1409.6700,370.9140) and
        (1408.7400,372.8720) .. (1407.2300,371.6980) .. controls (1406.2300,369.9280)
        and (1406.2600,370.8620) .. (1405.7600,370.3810) .. controls
        (1404.8200,370.0380) and (1403.9600,369.8410) .. (1403.0200,370.0890) ..
        controls (1401.9900,370.3590) and (1402.0600,369.5700) .. (1401.0500,370.1190)
        .. controls (1400.3100,370.5270) and (1399.8100,370.0990) ..
        (1399.1000,369.9350) .. controls (1397.4100,369.8950) and (1395.9200,369.3540)
        .. (1394.3300,368.9000) .. controls (1393.1600,369.0060) and
        (1394.7900,369.5000) .. (1392.9700,369.0060) .. controls (1391.6400,368.6450)
        and (1391.5300,368.9860) .. (1391.0800,369.8090) .. controls
        (1390.1000,371.5800) and (1389.9500,370.8010) .. (1388.2600,369.5440) ..
        controls (1386.0700,367.9280) and (1386.3700,370.8890) .. (1386.5100,371.9920)
        .. controls (1386.6100,372.6740) and (1386.3800,372.7980) ..
        (1387.0900,373.1020) .. controls (1387.7200,373.3750) and (1388.7900,374.0500)
        .. (1389.2300,374.6690) .. controls (1390.1600,375.9560) and
        (1389.2300,377.7560) .. (1391.1800,378.9170) .. controls (1393.0800,380.0270)
        and (1394.1500,381.8780) .. (1395.9100,383.1920) .. controls
        (1397.3300,384.2500) and (1397.9800,385.5610) .. (1399.2000,386.6280) ..
        controls (1400.6800,387.9150) and (1399.9400,389.3970) .. (1398.2700,387.4470)
        .. controls (1396.5400,385.4300) and (1392.2300,382.4740) ..
        (1389.4400,383.5130) .. controls (1388.7100,383.7850) and (1388.3300,383.5130)
        .. (1387.8600,382.8960) .. controls (1387.2800,382.1410) and
        (1387.6400,381.9390) .. (1386.5300,381.3920) .. controls (1384.9300,380.5930)
        and (1382.7200,378.7820) .. (1382.0900,377.0640) .. controls
        (1383.0900,376.8920) and (1383.9900,377.0340) .. (1384.9800,377.2090) ..
        controls (1383.6800,376.2570) and (1382.0800,375.5440) .. (1381.1800,374.1470)
        .. controls (1380.4200,372.9800) and (1380.9200,371.4850) ..
        (1380.1900,370.3280) .. controls (1379.5400,369.3110) and (1378.1000,368.3390)
        .. (1376.9400,368.0220) .. controls (1376.0900,367.7890) and
        (1375.3100,370.2460) .. (1375.4700,370.8730) .. controls (1375.1000,370.7210)
        and (1374.9700,370.8330) .. (1374.6800,370.5130) .. controls
        (1374.5700,371.3370) and (1374.3700,372.2190) .. (1373.7400,372.8170) ..
        controls (1373.2300,372.4220) and (1371.5700,370.3780) .. (1372.3700,369.7210)
        .. controls (1371.4600,369.9320) and (1371.0200,367.4340) ..
        (1370.7900,366.6970) .. controls (1371.0000,366.7170) and (1371.2200,366.7470)
        .. (1371.4400,366.7670);

        % path4068
        \path[country]
        (1400.0200,388.8700) .. controls (1400.7600,388.2130) and (1401.6800,389.2100)
        .. (1402.7000,390.1100) .. controls (1403.9800,391.2330) and
        (1406.8300,391.4680) .. (1405.9300,392.5420) .. controls (1404.7700,392.3810)
        and (1402.7600,390.7480) .. (1401.8500,390.0170) .. controls
        (1401.0500,389.3770) and (1400.0100,389.4740) .. (1399.0900,389.1580) ..
        controls (1398.0900,388.8160) and (1397.2600,387.9310) .. (1396.1300,388.0790)
        .. controls (1397.3100,387.1730) and (1399.5900,388.5770) ..
        (1400.5300,389.3030) .. controls (1400.3600,389.1580) and (1400.1900,389.0140)
        .. (1400.0200,388.8700);

        % path4070
        \path[country]
        (1376.7700,370.8700) .. controls (1376.3600,370.4330) and
        (1376.2400,369.9300) .. (1376.4100,369.3570) .. controls (1377.2400,370.7290)
        and (1377.3900,372.3170) .. (1377.8500,373.8210) .. controls
        (1376.8900,373.6780) and (1375.9600,371.5750) .. (1376.7700,370.8700);

        % path4072
        \path[country]
        (1377.9900,375.3300) .. controls (1377.6000,374.8320) and
        (1377.2000,374.3520) .. (1376.7700,373.8900) .. controls (1377.2800,374.2580)
        and (1377.7200,374.7550) .. (1377.9900,375.3300);

        % path4074
        \path[country]
        (1378.6400,370.8700) .. controls (1377.9900,370.8000) and
        (1376.8400,369.4760) .. (1377.9200,369.1410) .. controls (1378.6700,368.9080)
        and (1379.2500,370.5840) .. (1379.7900,370.8700) .. controls
        (1379.4000,371.2680) and (1379.0100,371.2680) .. (1378.6400,370.8700);

        % path4076
        \path[country]
        (1379.1400,372.3100) .. controls (1379.3800,372.4540) and
        (1379.6200,372.5980) .. (1379.8600,372.7420) .. controls (1379.2100,373.0480)
        and (1378.9700,372.9040) .. (1379.1400,372.3100);

        % path4078
        \path[country]
        (1380.5800,377.7100) .. controls (1380.3400,377.5180) and
        (1380.1000,377.3260) .. (1379.8600,377.1340) .. controls (1380.1800,377.2340)
        and (1380.4200,377.4260) .. (1380.5800,377.7100);

        % path4080
        \path[country]
        (1381.3000,375.6200) .. controls (1380.6000,374.9480) and
        (1379.9000,374.2500) .. (1379.4300,373.3880) .. controls (1380.3100,374.6080)
        and (1381.8600,375.0500) .. (1382.7400,376.2680) .. controls
        (1382.0400,376.8050) and (1381.6200,376.1520) .. (1381.3000,375.6200);

        % path4082
        \path[country]
        (1381.3700,379.0100) .. controls (1381.1300,378.7940) and
        (1380.9000,378.5770) .. (1380.6600,378.3620) .. controls (1381.5900,378.4320)
        and (1381.8100,379.5270) .. (1382.5300,379.9460) .. controls
        (1381.9800,379.8340) and (1381.5900,379.5220) .. (1381.3700,379.0100);

        % path4086
        \path[country]
        (1383.0300,380.4500) .. controls (1383.5900,380.7620) and
        (1384.0900,381.1450) .. (1384.5400,381.6020) .. controls (1383.9700,381.3400)
        and (1383.3800,380.9870) .. (1383.0300,380.4500);

        % path4088
        \path[country]
        (1383.0300,379.2200) .. controls (1382.7900,379.0520) and
        (1382.5500,378.8840) .. (1382.3100,378.7160) .. controls (1382.6700,378.7260)
        and (1382.9100,378.8960) .. (1383.0300,379.2200);

        % path4090
        \path[country]
        (1385.7700,382.1700) .. controls (1386.0300,382.2900) and
        (1386.2900,382.4100) .. (1386.5600,382.5300) .. controls (1386.2800,382.4400)
        and (1386.0200,382.3210) .. (1385.7700,382.1700);

        % path4092
        \path[country]
        (1389.8700,383.6100) .. controls (1390.1100,383.5900) and
        (1390.3500,383.5600) .. (1390.5900,383.5400) .. controls (1390.3500,383.6400)
        and (1390.1100,383.6600) .. (1389.8700,383.6100);

        % path4094
        \path[country]
        (1391.0200,385.1300) .. controls (1390.7800,385.0100) and
        (1390.5400,384.8900) .. (1390.3000,384.7700) .. controls (1390.6100,384.7690)
        and (1390.8500,384.8890) .. (1391.0200,385.1300);

        % path4096
        \path[country]
        (1393.1800,385.7000) .. controls (1392.4400,385.7000) and
        (1391.5000,385.5140) .. (1391.3800,384.6200) .. controls (1392.3800,384.5900)
        and (1393.3800,384.7200) .. (1394.3300,385.0520) .. controls
        (1394.0300,385.4170) and (1393.6400,385.6330) .. (1393.1800,385.7000);

        % path4098
        \path[country]
        (1394.5500,388.8000) .. controls (1394.0500,388.6830) and
        (1393.5500,388.6120) .. (1393.0400,388.5840) .. controls (1393.9300,387.8090)
        and (1395.8200,387.9350) .. (1396.7800,388.5140) .. controls
        (1396.0300,388.7490) and (1395.2500,388.3490) .. (1394.5500,388.8020);

        % path4100
        \path[country]
        (1395.8500,386.9300) .. controls (1394.3700,386.9800) and
        (1392.8700,386.8500) .. (1391.4500,386.4260) .. controls (1393.1400,385.8700)
        and (1394.8600,386.7720) .. (1396.5700,386.7140) .. controls
        (1396.3300,386.7840) and (1396.0900,386.8580) .. (1395.8500,386.9300);

        % path4102
        \path[country]
        (1400.6700,390.5300) .. controls (1399.9500,390.2790) and
        (1399.1800,390.1800) .. (1398.4400,390.0260) .. controls (1399.2000,389.8590)
        and (1400.0300,390.1360) .. (1400.6700,390.5300);

    \end{scope}
    
    
    % //////// CZECH REPUBLIC //////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (301.2684,229.2899) .. controls (302.0084,229.2899) and
    (302.5984,229.9079) .. (302.7784,230.5859) .. controls (303.0384,227.9939) and
    (306.7784,228.6609) .. (307.4984,228.1089) .. controls (310.0884,226.1369) and
    (313.4584,225.1479) .. (316.2484,224.1789) .. controls (316.0184,223.9559) and
    (315.7684,223.7409) .. (315.5284,223.5309) .. controls (316.1584,223.3849) and
    (316.8884,223.1569) .. (317.3784,223.7129) .. controls (317.8084,224.2069) and
    (318.1984,225.1369) .. (318.9884,224.8629) .. controls (319.5284,224.6749) and
    (320.2084,224.7829) .. (320.3184,224.1519) .. controls (320.4384,223.3929) and
    (320.7584,223.5439) .. (321.2584,223.6719) .. controls (322.0984,223.8859) and
    (322.3284,224.0139) .. (322.5684,224.8049) .. controls (323.2784,226.7059) and
    (327.0984,224.6269) .. (327.1884,226.9149) .. controls (327.5584,226.5169) and
    (328.4884,226.3779) .. (329.0384,226.4859) .. controls (330.8284,226.8409) and
    (329.0384,227.9059) .. (328.4184,228.4279) .. controls (329.6684,228.8619) and
    (330.0984,229.5279) .. (330.8084,230.5249) .. controls (331.6884,231.7449) and
    (333.1084,230.3169) .. (333.8884,229.7959) .. controls (333.4184,229.4009) and
    (333.1484,228.8979) .. (333.0984,228.2839) .. controls (334.9584,228.7709) and
    (336.6884,230.1869) .. (338.7084,229.5799) .. controls (338.7084,230.5099) and
    (338.5984,232.0579) .. (339.6684,231.9749) .. controls (340.8084,231.8849) and
    (341.2184,231.6769) .. (342.4284,232.2439) .. controls (343.7184,232.8509) and
    (344.0184,232.4129) .. (344.6784,233.8159) .. controls (343.5484,233.0479) and
    (346.0284,234.0579) .. (347.0484,236.3189) .. controls (345.7384,236.8049) and
    (343.7684,237.0409) .. (342.6084,237.9099) .. controls (341.7684,238.5349) and
    (341.7684,239.9149) .. (340.8884,240.3499) .. controls (339.9984,240.7929) and
    (338.8884,241.9349) .. (336.9284,241.8999) .. controls (335.6384,241.8799) and
    (334.7084,241.8999) .. (333.9584,243.5479) .. controls (333.2984,241.1469) and
    (329.9684,242.8649) .. (328.4684,242.3479) .. controls (327.2384,241.9219) and
    (326.0184,241.4299) .. (324.7784,241.0259) .. controls (323.7584,240.6989) and
    (321.8284,240.1619) .. (320.7784,240.2359) .. controls (320.8784,240.9209) and
    (320.5684,241.5689) .. (320.6384,242.2519) .. controls (319.6184,242.1109) and
    (318.8484,242.9199) .. (318.8384,243.9079) .. controls (317.3284,243.3049) and
    (317.2984,243.9579) .. (315.8084,243.8179) .. controls (314.8184,243.7279) and
    (313.9984,242.6659) .. (313.2284,242.1439) .. controls (312.2284,241.4739) and
    (311.1684,240.9119) .. (310.1284,240.3089) .. controls (309.1584,239.7459) and
    (308.0584,238.3489) .. (307.0284,237.9439) .. controls (305.3084,237.2699) and
    (304.9084,234.8849) .. (303.3584,234.0439) .. controls (305.5384,232.1239) and
    (301.4684,231.9989) .. (301.2684,229.2899);
    
    
    % //////// DENMARK /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path4494
        \path[country]
        (1345.0100,286.9200) .. controls (1345.5100,287.2480) and
        (1345.9900,289.0140) .. (1346.9600,288.3590) .. controls (1347.9700,287.6800)
        and (1345.7200,286.5080) .. (1345.0100,286.9200);

        % path4548
        \path[country]
        (1335.2200,274.3900) .. controls (1335.3200,274.1500) and (1335.4100,273.9110)
        .. (1335.5100,273.6700) .. controls (1335.9300,274.1320) and
        (1337.1800,274.8790) .. (1337.8200,274.4620) .. controls (1338.0900,275.6730)
        and (1338.9000,275.2330) .. (1339.1000,274.3580) .. controls
        (1339.5800,272.2490) and (1342.5500,273.1980) .. (1340.9800,273.9590) ..
        controls (1341.6300,274.0190) and (1342.6200,273.8370) .. (1342.5700,274.8220)
        .. controls (1342.8000,273.9160) and (1342.8100,273.5010) ..
        (1341.8500,273.5980) .. controls (1341.8500,272.8600) and (1341.6000,271.7620)
        .. (1342.2600,271.2040) .. controls (1342.6900,270.9280) and
        (1343.1600,270.8180) .. (1343.6700,270.8730) .. controls (1344.4800,270.9230)
        and (1344.9400,270.5750) .. (1345.6500,270.5750) .. controls
        (1346.5100,270.5750) and (1347.0500,270.6150) .. (1347.8600,270.9360) ..
        controls (1348.8500,271.3300) and (1348.5500,272.5610) .. (1349.0500,273.3090)
        .. controls (1348.0400,273.2190) and (1347.0900,273.5230) ..
        (1346.1700,273.8850) .. controls (1347.1000,273.9050) and (1347.7500,273.1910)
        .. (1348.7100,273.6010) .. controls (1349.2700,273.8440) and
        (1348.1400,274.9170) .. (1348.1100,275.3250) .. controls (1348.3600,273.9710)
        and (1351.9600,274.6830) .. (1352.6700,275.2450) .. controls
        (1353.2700,275.7250) and (1352.0700,277.5860) .. (1351.4600,277.5840) ..
        controls (1350.8400,277.5840) and (1350.5800,277.5240) .. (1350.3400,278.2750)
        .. controls (1349.5900,278.1050) and (1349.4500,277.5950) ..
        (1349.9800,277.0500) .. controls (1348.6000,276.5930) and (1348.6600,277.7580)
        .. (1348.6000,278.7320) .. controls (1348.5000,280.3060) and
        (1347.3000,280.0000) .. (1346.1700,280.2910) .. controls (1346.5900,280.3310)
        and (1347.4200,280.7970) .. (1346.9300,281.3460) .. controls
        (1346.3200,282.0400) and (1345.0500,281.4500) .. (1344.2900,281.5870) ..
        controls (1344.8200,281.7770) and (1345.3500,281.9690) .. (1345.8800,282.1630)
        .. controls (1344.6200,283.4490) and (1344.0600,282.7070) ..
        (1344.9100,284.6320) .. controls (1345.4300,285.7980) and (1343.3200,285.7650)
        .. (1343.3600,286.9150) .. controls (1344.3500,286.8040) and
        (1345.5500,287.3990) .. (1345.3000,288.5720) .. controls (1344.5700,288.5220)
        and (1344.6500,287.7860) .. (1343.9600,288.3220) .. controls
        (1343.2200,288.8970) and (1342.4100,288.7350) .. (1341.6100,288.4850) ..
        controls (1340.5100,288.1410) and (1337.7800,288.3730) .. (1338.3900,286.4830)
        .. controls (1337.8100,286.7020) and (1337.3600,286.3790) ..
        (1337.1700,285.8360) .. controls (1340.5400,285.8360) and (1336.4300,283.0470)
        .. (1336.2300,282.5230) .. controls (1336.0700,284.1000) and
        (1335.2400,282.5930) .. (1335.1600,281.8910) .. controls (1335.0600,281.0060)
        and (1335.2600,280.0880) .. (1335.0600,279.2120) .. controls
        (1335.1600,279.8730) and (1336.3400,281.0670) .. (1336.7200,279.9320) ..
        controls (1336.9000,279.3940) and (1334.8200,277.1010) .. (1335.1300,278.9960)
        .. controls (1334.5200,277.8080) and (1334.8200,275.6110) ..
        (1335.2300,274.3870);

        % path4492
        \path[country]
        (1338.4600,273.6700) .. controls (1339.4700,273.4360) and
        (1340.1400,272.3830) .. (1339.9000,271.3660) .. controls (1339.5200,271.6380)
        and (1339.1000,271.8360) .. (1338.6400,271.9580) .. controls
        (1338.1900,272.0940) and (1338.3000,272.8970) .. (1337.7400,273.0940) ..
        controls (1337.9600,273.3140) and (1338.2000,273.5060) ..
        (1338.4600,273.6700);

        % path4496
        \path[country]
        (1345.0900,283.1000) .. controls (1345.0900,284.3120) and
        (1346.7100,285.0760) .. (1346.9600,286.2680) .. controls (1346.9600,285.2190)
        and (1347.6500,285.7420) .. (1347.8300,286.3700) .. controls
        (1347.9800,286.8910) and (1350.1600,286.9560) .. (1350.5200,286.8910) ..
        controls (1352.4000,286.5550) and (1352.6800,283.8870) .. (1350.7000,283.4600)
        .. controls (1350.9400,283.3220) and (1351.1800,283.1790) ..
        (1351.4200,283.0280) .. controls (1351.2500,282.7250) and (1351.0400,282.4620)
        .. (1350.7800,282.2350) .. controls (1350.7800,282.9560) and
        (1350.3300,283.6390) .. (1349.5500,283.5320) .. controls (1350.9700,281.9530)
        and (1345.6700,283.0660) .. (1345.0900,283.1000);

        % path4498
        \path[country]
        (1349.5500,288.7200) .. controls (1349.6500,287.9490) and
        (1348.6100,287.6900) .. (1348.1100,287.4240) .. controls (1348.5500,287.9030)
        and (1349.0300,288.3350) .. (1349.5500,288.7200);

        % path4500
        \path[country]
        (1350.1300,287.2800) .. controls (1350.4200,287.3500) and
        (1350.7000,287.4240) .. (1350.9900,287.4950) .. controls (1350.9900,286.6580)
        and (1350.5800,286.8890) .. (1350.1300,287.2800);

        % path4502
        \path[country]
        (1351.1400,280.0100) .. controls (1350.7100,279.9400) and
        (1350.4200,279.6990) .. (1350.2700,279.2900) .. controls (1350.6900,279.7910)
        and (1350.6600,280.2700) .. (1350.1700,280.7290) .. controls
        (1350.7400,280.8720) and (1351.0800,280.5950) .. (1351.1100,280.0100);

        % path4504
        \path[country]
        (1351.4900,287.7800) .. controls (1350.9400,288.2820) and
        (1350.9300,288.9980) .. (1351.5900,289.4350) .. controls (1351.9100,288.5460)
        and (1352.9700,287.5070) .. (1352.5200,286.4830) .. controls
        (1352.3200,287.0210) and (1351.9800,287.4530) .. (1351.5100,287.7800);

        % path4506
        \path[country]
        (1353.0800,269.2100) .. controls (1353.4800,269.0960) and
        (1353.7200,268.8320) .. (1353.8000,268.4180) .. controls (1353.2400,268.3980)
        and (1352.7600,268.5920) .. (1352.3600,268.9930) .. controls
        (1352.6000,269.0630) and (1352.8400,269.1380) .. (1353.0800,269.2100);

        % path4508
        \path[country]
        (1353.8700,284.4000) .. controls (1354.5300,284.6350) and
        (1354.6200,285.3350) .. (1355.1300,285.5950) .. controls (1355.5900,285.8320)
        and (1356.3900,285.6350) .. (1356.8900,285.5950) .. controls
        (1358.3100,285.4790) and (1358.6300,287.0660) .. (1357.4000,286.6350) ..
        controls (1357.7100,286.6950) and (1358.7400,287.0070) .. (1358.7800,287.4230)
        .. controls (1358.6000,287.6410) and (1358.3600,287.6900) ..
        (1358.0500,287.5700) .. controls (1358.0500,288.1590) and (1358.9600,290.2560)
        .. (1359.2700,290.7380) .. controls (1359.4700,290.1930) and
        (1360.4700,289.1310) .. (1360.4600,288.6260) .. controls (1360.4600,288.0030)
        and (1359.3500,287.8340) .. (1359.1300,287.2830) .. controls
        (1359.6800,287.5060) and (1360.2300,287.5060) .. (1360.7800,287.2830) ..
        controls (1359.9300,286.0900) and (1360.9000,285.6370) .. (1361.9200,285.2640)
        .. controls (1363.1600,284.8120) and (1361.7900,284.1660) ..
        (1361.3400,283.7190) .. controls (1360.3600,282.7370) and (1362.2500,282.2820)
        .. (1362.7900,281.9060) .. controls (1364.0400,281.0410) and
        (1362.3100,279.6820) .. (1363.4500,278.8590) .. controls (1362.0700,277.4900)
        and (1360.5100,278.5660) .. (1359.0600,279.1470) .. controls
        (1360.1200,279.5740) and (1360.7200,281.8800) .. (1359.1600,281.9560) ..
        controls (1359.5700,281.3610) and (1359.9700,280.6730) .. (1359.5900,279.9390)
        .. controls (1359.2900,280.1380) and (1358.4900,282.0110) ..
        (1358.0800,281.7520) .. controls (1357.4200,281.3290) and (1357.6200,279.8510)
        .. (1357.9800,279.7950) .. controls (1357.3900,279.3160) and
        (1356.3700,279.4270) .. (1355.6800,279.5070) .. controls (1356.0500,279.4170)
        and (1356.2900,279.5270) .. (1356.4000,279.8170) .. controls
        (1356.0900,281.1040) and (1353.6700,281.3570) .. (1352.7300,281.3070) ..
        controls (1353.1900,281.8280) and (1355.9100,284.2740) ..
        (1353.8800,284.4020);

        % path4510
        \path[country]
        (1353.2200,288.9300) .. controls (1354.1800,289.6100) and
        (1357.6600,291.0760) .. (1358.6200,289.8750) .. controls (1359.7100,288.5230)
        and (1357.5500,288.4720) .. (1356.8600,288.5650) .. controls
        (1355.5200,288.7490) and (1354.8700,286.9970) .. (1353.5100,287.9940) ..
        controls (1353.6700,288.2360) and (1353.8400,288.4750) .. (1354.0100,288.7140)
        .. controls (1353.7500,288.7840) and (1353.4800,288.8580) ..
        (1353.2200,288.9300);

        % path4512
        \path[country]
        (1360.8600,287.3500) .. controls (1360.7600,287.6380) and
        (1360.7100,287.9260) .. (1360.6400,288.2140) .. controls (1360.9300,288.1240)
        and (1363.2600,287.6450) .. (1363.0300,287.2060) .. controls
        (1362.7700,286.7350) and (1361.2500,287.3190) .. (1360.8600,287.3500);

        % path4514
        \path[country]
        (1362.9400,282.1700) .. controls (1363.2800,282.9830) and
        (1363.5400,282.9340) .. (1363.7400,282.0250) .. controls (1363.4700,282.0750)
        and (1363.2000,282.1250) .. (1362.9400,282.1700);

        % path4516
        \path[country]
        (1378.7800,285.6900) .. controls (1377.8100,284.9260) and
        (1376.1600,285.7900) .. (1377.3400,286.6730) .. controls (1379.2300,288.0890)
        and (1380.4000,285.8700) .. (1378.7800,285.6900);

        % path4550
        \path[country]
        (1336.9500,273.6700) .. controls (1335.4900,272.7550) and
        (1336.7400,271.1440) .. (1337.7000,270.4430) .. controls (1339.0500,269.4590)
        and (1341.2800,269.9610) .. (1342.8400,269.8050) .. controls
        (1344.2400,269.6660) and (1344.9600,268.1880) .. (1345.7600,267.2380) ..
        controls (1346.6500,266.1800) and (1349.2700,265.4770) .. (1350.6300,265.0310)
        .. controls (1349.0100,266.4720) and (1350.9200,267.4460) ..
        (1350.0800,269.0940) .. controls (1349.1400,270.9160) and (1348.1400,270.9960)
        .. (1346.2900,270.4310) .. controls (1345.4100,270.1600) and
        (1344.6200,270.3510) .. (1343.7300,270.5870) .. controls (1342.7400,270.8460)
        and (1341.9400,270.4420) .. (1340.9900,270.6270) .. controls
        (1340.1500,270.7930) and (1338.9800,271.0450) .. (1338.4000,271.7330) ..
        controls (1338.0200,272.1760) and (1337.6900,273.5570) .. (1336.9500,273.5250)
        .. controls (1337.5700,273.4210) and (1337.9200,273.7630) ..
        (1337.8200,274.3890) .. controls (1337.5100,274.1720) and (1337.2200,273.9320)
        .. (1336.9500,273.6680);

    \end{scope}
    
    
    % //////// ESTONIA /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path5944
        \path[country]
        (1421.8400,263.6600) .. controls (1422.9500,263.2460) and
        (1422.6600,262.3130) .. (1423.2800,261.5720) .. controls (1423.7100,261.0540)
        and (1424.5400,261.2280) .. (1425.1000,260.9990) .. controls
        (1425.4400,261.0190) and (1425.7600,261.0690) .. (1426.0900,261.1400) ..
        controls (1426.4100,260.9080) and (1426.7200,260.6540) .. (1427.0100,260.3790)
        .. controls (1427.6800,260.0140) and (1428.2400,259.1930) ..
        (1429.1100,259.4830) .. controls (1427.8800,258.3200) and (1426.7200,258.1340)
        .. (1425.0800,258.2590) .. controls (1424.2000,258.3290) and
        (1423.7000,258.1350) .. (1422.9800,258.7920) .. controls (1422.4200,259.3020)
        and (1421.2100,258.8920) .. (1420.5400,258.9790) .. controls
        (1421.4700,259.7290) and (1420.4300,260.4720) .. (1421.6800,261.2700) ..
        controls (1423.1400,262.1990) and (1420.9600,262.7720) ..
        (1421.8400,263.6600);

        % path5946
        \path[country]
        (1424.7200,254.3000) .. controls (1423.7000,255.2300) and
        (1422.5000,255.3180) .. (1421.1900,255.4520) .. controls (1422.1600,255.9500)
        and (1423.4700,255.4320) .. (1424.0000,256.6610) .. controls
        (1424.3900,257.5580) and (1425.1800,257.4180) .. (1425.5900,256.6310) ..
        controls (1425.7700,256.2790) and (1427.1500,256.3960) .. (1426.8600,255.5870)
        .. controls (1426.5800,254.8020) and (1425.1900,254.9120) ..
        (1424.7200,254.3000);

        % path5948
        \path[country]
        (1428.3200,258.4800) .. controls (1428.8000,258.7200) and
        (1429.2100,258.6250) .. (1429.5400,258.1920) .. controls (1429.2000,257.6610)
        and (1428.6200,257.4210) .. (1428.0300,257.6880) .. controls
        (1428.1300,257.9510) and (1428.2200,258.2160) .. (1428.3200,258.4800);

        % path5950
        \path[country]
        (1428.1800,254.5900) .. controls (1428.1800,254.8060) and
        (1428.1800,255.0220) .. (1428.1800,255.2370) .. controls (1428.4500,255.0820)
        and (1428.6900,254.8890) .. (1428.9000,254.6610) .. controls
        (1428.6600,254.6410) and (1428.4200,254.6110) .. (1428.1800,254.5910);

        % path5970
        \path[country]
        (1430.4100,258.4000) .. controls (1429.8700,256.9310) and (1431.7500,257.1640)
        .. (1432.5700,256.8160) .. controls (1431.9700,256.6580) and
        (1430.7500,257.1510) .. (1430.2600,256.7460) .. controls (1429.4000,256.0370)
        and (1431.0000,255.4260) .. (1430.4800,254.5860) .. controls
        (1430.2300,254.7220) and (1429.9900,254.8650) .. (1429.7600,255.0180) ..
        controls (1429.9100,254.5440) and (1429.6600,253.8170) .. (1430.0500,253.4230)
        .. controls (1430.8800,252.4710) and (1432.3900,252.7440) ..
        (1433.5000,252.7140) .. controls (1433.3200,252.4430) and (1433.1800,252.1550)
        .. (1433.0700,251.8500) .. controls (1434.1400,252.4540) and
        (1434.6100,251.0490) .. (1435.6400,251.2160) .. controls (1436.1700,251.3060)
        and (1437.8200,251.9950) .. (1437.6100,250.8420) .. controls
        (1438.2400,250.8720) and (1442.5600,251.5260) .. (1441.7800,249.9780) ..
        controls (1443.3700,250.5140) and (1445.5100,250.2760) .. (1447.1900,250.4770)
        .. controls (1448.6800,250.6530) and (1449.9300,251.2790) ..
        (1451.3800,251.4660) .. controls (1452.7800,251.6480) and (1458.0700,250.5670)
        .. (1458.6300,252.1390) .. controls (1457.2400,252.1190) and
        (1457.0300,252.8560) .. (1456.7100,254.0010) .. controls (1456.3400,255.2930)
        and (1454.6800,255.7040) .. (1454.7000,256.8270) .. controls
        (1454.7000,257.6830) and (1455.3100,258.2490) .. (1455.5300,259.0480) ..
        controls (1455.7300,259.7630) and (1455.1400,260.3360) .. (1455.3900,261.0510)
        .. controls (1455.5700,261.5640) and (1456.2700,261.9490) ..
        (1456.6300,262.3050) .. controls (1457.1800,262.8560) and (1456.6300,263.3400)
        .. (1457.7700,263.8740) .. controls (1456.7700,264.9880) and
        (1455.3500,265.5040) .. (1455.7700,266.6820) .. controls (1454.8800,266.7120)
        and (1453.7000,266.1860) .. (1452.8400,266.0670) .. controls
        (1451.8700,265.9320) and (1451.2200,266.8710) .. (1450.2800,266.6830) ..
        controls (1448.2600,266.2800) and (1446.6600,264.5300) .. (1444.7700,263.7470)
        .. controls (1444.2300,263.5220) and (1443.2700,263.0020) ..
        (1442.6800,263.0440) .. controls (1441.9200,263.0940) and (1441.4800,262.5140)
        .. (1440.8100,262.5230) .. controls (1439.2000,262.5430) and
        (1437.6400,264.4120) .. (1436.0200,263.9480) .. controls (1436.1600,263.1980)
        and (1436.4000,261.2570) .. (1436.7700,260.6700) .. controls
        (1437.2400,259.9250) and (1436.1100,259.5710) .. (1435.7200,260.3260) ..
        controls (1434.5600,262.6070) and (1431.3000,258.4260) ..
        (1430.4100,258.4010);

    \end{scope}
    
    
    % //////// FINLAND /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path4630
        \path[country]
        (1405.4900,244.5800) .. controls (1404.9200,245.2140) and
        (1404.9200,245.3450) .. (1405.7800,245.5160) .. controls (1405.7800,245.1770)
        and (1405.6700,244.8650) .. (1405.4900,244.5800);

        % path4632
        \path[country]
        (1407.2200,246.0900) .. controls (1408.1900,246.2490) and
        (1408.2500,245.3170) .. (1407.8000,244.7220) .. controls (1408.2700,244.5920)
        and (1408.8200,245.5670) .. (1409.3300,245.3220) .. controls
        (1410.3600,244.8250) and (1407.2400,243.7640) .. (1406.7200,243.8590) ..
        controls (1407.2400,244.2870) and (1407.2600,244.8940) .. (1406.8200,245.3710)
        .. controls (1406.8200,244.7800) and (1406.4200,244.4130) ..
        (1405.8100,244.6500) .. controls (1406.0500,245.3100) and (1406.2800,246.3680)
        .. (1407.2500,246.0900);

        % path4634
        \path[country]
        (1407.9400,246.4500) .. controls (1410.6100,247.4730) and
        (1408.8500,245.6390) .. (1407.9400,246.4500);

        % path4636
        \path[country]
        (1409.9600,246.9600) .. controls (1410.2200,247.0870) and
        (1410.4900,247.0870) .. (1410.7500,246.9600) .. controls (1410.4800,246.9600)
        and (1410.2200,246.9600) .. (1409.9600,246.9600);

        % path4638
        \path[country]
        (1413.6300,222.1900) .. controls (1415.1100,222.0170) and
        (1414.0400,220.5970) .. (1412.9100,221.5430) .. controls (1413.1200,221.7850)
        and (1413.3600,222.0010) .. (1413.6300,222.1900);

        % path4642
        \path[country]
        (1416.0100,242.7100) .. controls (1416.2700,242.6900) and
        (1416.5400,242.6600) .. (1416.8000,242.6400) .. controls (1416.2500,242.1490)
        and (1415.9900,242.1730) .. (1416.0100,242.7100);

        % path4644
        \path[country]
        (1418.3800,220.5300) .. controls (1418.1200,220.6300) and
        (1417.8500,220.7210) .. (1417.5900,220.8170) .. controls (1417.9000,220.8470)
        and (1418.1600,220.7470) .. (1418.3800,220.5300);

        % path4646
        \path[country]
        (1419.3200,220.8200) .. controls (1419.0800,220.8400) and
        (1418.8400,220.8700) .. (1418.6000,220.8900) .. controls (1419.3100,221.5560)
        and (1419.5500,221.5320) .. (1419.3200,220.8200);

        % path4648
        \path[country]
        (1419.9000,243.7900) .. controls (1419.6500,243.5440) and
        (1419.3900,243.3280) .. (1419.1000,243.1420) .. controls (1418.5100,244.1180)
        and (1419.6900,244.4290) .. (1420.4000,244.2220) .. controls
        (1420.2500,244.1720) and (1419.8800,243.7790) .. (1419.9000,243.7900);

        % path4650
        \path[country]
        (1419.6800,245.5900) .. controls (1419.4800,245.4770) and
        (1419.2700,245.3340) .. (1419.0300,245.3020) .. controls (1419.2500,245.4020)
        and (1419.4600,245.4940) .. (1419.6800,245.5900);

        % path4652
        \path[country]
        (1419.9700,245.5200) .. controls (1420.4500,245.7300) and
        (1420.6900,245.6340) .. (1420.6900,245.2320) .. controls (1420.4500,245.3320)
        and (1420.2100,245.4240) .. (1419.9700,245.5200);

        % path4660
        \path[country]
        (1422.9200,217.0100) .. controls (1422.6600,217.0300) and
        (1422.3900,217.0600) .. (1422.1300,217.0800) .. controls (1422.3700,217.2680)
        and (1422.6300,217.4120) .. (1422.9200,217.5130) .. controls
        (1423.0200,217.1980) and (1423.2600,216.8770) .. (1422.9200,217.0090);

        % path4662
        \path[country]
        (1422.2700,244.4400) .. controls (1422.5100,244.4600) and
        (1422.7500,244.4900) .. (1422.9900,244.5100) .. controls (1422.6600,243.9130)
        and (1422.6500,244.1670) .. (1422.2700,244.4400);

        % path4664
        \path[country]
        (1422.7000,246.9600) .. controls (1423.2700,246.9000) and
        (1423.8500,246.9600) .. (1424.4300,246.9200) .. controls (1425.5500,246.8500)
        and (1425.1500,245.2090) .. (1426.0100,244.7270) .. controls
        (1425.1800,245.2450) and (1423.8800,245.5170) .. (1422.9200,245.3030) ..
        controls (1424.5800,245.9340) and (1422.3300,245.6810) ..
        (1422.7000,246.9600);

        % path4666
        \path[country]
        (1425.2200,246.9600) .. controls (1425.6100,247.6290) and
        (1426.9000,248.1720) .. (1426.9500,246.9600) .. controls (1426.3700,247.1170)
        and (1425.7900,247.1170) .. (1425.2200,246.9600);

        % path4670
        \path[country]
        (1431.7000,208.1500) .. controls (1433.0900,208.8630) and
        (1433.0100,207.5590) .. (1434.0100,207.9340) .. controls (1433.5700,207.2730)
        and (1431.9500,207.3080) .. (1431.7000,208.1500);

        % path4682
        \path[country]
        (1406.0000,177.9800) .. controls (1406.8300,177.0680) and (1407.9800,178.0880)
        .. (1408.9500,177.5480) .. controls (1408.7000,177.3370) and
        (1408.4600,177.1210) .. (1408.2300,176.9000) .. controls (1410.8900,175.3060)
        and (1413.4100,177.2570) .. (1415.3700,179.1910) .. controls
        (1416.7500,180.5490) and (1419.4400,181.4410) .. (1421.4100,180.8620) ..
        controls (1422.4800,180.5490) and (1423.1700,180.3960) .. (1424.0400,179.7550)
        .. controls (1424.8300,179.1650) and (1427.0300,180.0810) ..
        (1427.8800,180.3240) .. controls (1429.1000,180.6710) and (1429.1800,181.3490)
        .. (1430.4200,181.1260) .. controls (1431.4800,180.9320) and
        (1431.7100,179.1050) .. (1433.1600,179.0050) .. controls (1433.8900,178.9550)
        and (1434.5600,178.8720) .. (1434.4000,177.9730) .. controls
        (1434.1100,176.4290) and (1434.7200,174.9960) .. (1435.0900,173.5170) ..
        controls (1435.9700,172.3480) and (1437.6700,171.1060) .. (1439.4000,171.5060)
        .. controls (1441.0000,171.8740) and (1441.9900,171.2640) ..
        (1443.4400,170.6510) .. controls (1445.0300,169.9800) and (1446.1900,171.3670)
        .. (1447.5900,171.8850) .. controls (1449.0600,172.4250) and
        (1450.5200,172.7370) .. (1452.0100,173.1020) .. controls (1456.5500,174.2110)
        and (1450.5800,176.4760) .. (1453.1000,178.0710) .. controls
        (1451.9500,178.6990) and (1450.4900,178.7960) .. (1449.4900,179.1340) ..
        controls (1450.0400,179.2040) and (1452.3800,179.3210) .. (1451.3000,180.4040)
        .. controls (1450.2200,181.4770) and (1449.8400,182.2710) ..
        (1451.2000,183.3890) .. controls (1452.4800,184.4480) and (1454.1400,184.5080)
        .. (1455.5600,185.2710) .. controls (1456.8100,185.9430) and
        (1458.0800,186.7650) .. (1459.2600,187.5630) .. controls (1462.0900,189.4740)
        and (1454.3800,192.0350) .. (1455.8700,194.1310) .. controls
        (1458.0500,197.1780) and (1461.7300,199.0080) .. (1463.0300,202.8210) ..
        controls (1462.2600,202.8610) and (1461.4900,203.1040) .. (1460.7500,203.2380)
        .. controls (1461.7200,203.5130) and (1461.2700,205.0310) ..
        (1460.7500,205.7320) .. controls (1460.3600,206.2610) and (1461.9100,206.5860)
        .. (1462.1400,207.1100) .. controls (1460.7800,207.4030) and
        (1460.7100,208.4670) .. (1461.6200,209.2860) .. controls (1462.5100,210.0860)
        and (1463.9700,209.0970) .. (1464.6000,210.5260) .. controls
        (1461.8300,211.7730) and (1465.7600,213.1280) .. (1466.8700,213.6810) ..
        controls (1469.3100,214.9060) and (1465.6900,217.1920) .. (1464.5500,217.7670)
        .. controls (1467.9400,219.3260) and (1471.1400,221.1400) ..
        (1474.1700,223.2740) .. controls (1475.1700,224.1450) and (1474.6700,224.5680)
        .. (1474.2700,225.7160) .. controls (1473.5400,227.6530) and
        (1472.2900,228.4790) .. (1470.7700,229.6720) .. controls (1467.2500,233.5850)
        and (1464.1000,236.7190) .. (1458.8300,239.6530) .. controls
        (1457.9000,240.3120) and (1456.9500,240.9960) .. (1456.0900,241.7420) ..
        controls (1455.6700,242.0400) and (1455.2700,242.3910) .. (1455.0000,242.8280)
        .. controls (1454.5100,243.5450) and (1453.4700,242.9920) ..
        (1452.8000,243.0540) .. controls (1451.8400,243.1440) and (1451.7800,242.2840)
        .. (1450.7000,242.7900) .. controls (1449.8900,243.1770) and
        (1449.1200,243.4950) .. (1448.1900,243.4980) .. controls (1447.8000,243.5180)
        and (1447.4500,243.4280) .. (1447.1300,243.2150) .. controls
        (1447.0300,243.5500) and (1446.8300,243.7700) .. (1446.5100,243.8740) ..
        controls (1445.7100,244.1220) and (1444.6900,243.7070) .. (1444.0300,243.2870)
        .. controls (1444.6500,243.9930) and (1444.3000,244.2370) ..
        (1443.6000,244.2950) .. controls (1443.7000,244.5370) and (1443.7800,244.7760)
        .. (1443.8900,245.0150) .. controls (1443.1400,245.2060) and
        (1442.2900,244.8980) .. (1442.3100,244.0070) .. controls (1441.5900,245.2070)
        and (1439.5300,245.2120) .. (1438.3200,245.4600) .. controls
        (1437.6400,245.5990) and (1437.0400,245.8660) .. (1436.3900,246.0800) ..
        controls (1435.9000,246.2390) and (1435.8500,246.8440) .. (1435.3500,246.9800)
        .. controls (1434.4300,247.2290) and (1434.1600,246.4100) ..
        (1433.1900,246.6600) .. controls (1431.7200,247.0390) and (1430.0900,247.8240)
        .. (1428.5500,247.5360) .. controls (1428.8500,247.3620) and
        (1429.1400,247.1700) .. (1429.4200,246.9600) .. controls (1428.2200,247.4090)
        and (1427.3600,248.3560) .. (1426.0300,248.4720) .. controls
        (1426.4900,248.2060) and (1427.0900,247.9320) .. (1427.3700,247.4350) ..
        controls (1427.9800,246.3320) and (1426.1400,247.3350) .. (1427.8400,246.6000)
        .. controls (1427.1600,246.7000) and (1426.6300,246.3940) ..
        (1426.1100,246.0180) .. controls (1425.2100,245.3740) and (1426.1100,244.7590)
        .. (1426.7500,244.1520) .. controls (1426.1400,244.3410) and
        (1421.9600,245.7160) .. (1423.3600,243.9360) .. controls (1422.0300,243.6560)
        and (1420.6600,243.6690) .. (1419.5000,242.8610) .. controls
        (1419.0200,242.5200) and (1417.6200,241.4590) .. (1417.8900,242.8610) ..
        controls (1417.4800,242.5410) and (1416.3600,242.1650) .. (1416.5100,241.7550)
        .. controls (1416.8000,241.0140) and (1415.9000,239.1340) ..
        (1415.5100,238.4700) .. controls (1417.9600,238.5000) and (1415.0400,233.5900)
        .. (1417.4600,234.8700) .. controls (1416.4100,234.1570) and
        (1415.1100,232.2850) .. (1414.7600,231.0680) .. controls (1414.4700,230.0810)
        and (1415.2000,229.4330) .. (1414.5500,228.3600) .. controls
        (1414.0700,227.5740) and (1413.5700,226.4730) .. (1413.0600,226.3740) ..
        controls (1413.6200,225.6960) and (1414.9500,222.6450) .. (1416.1600,223.2060)
        .. controls (1415.6000,222.7680) and (1415.1100,221.9850) ..
        (1415.5100,221.2620) .. controls (1416.5900,222.4860) and (1419.1700,221.7260)
        .. (1420.3400,221.0460) .. controls (1420.0200,220.7800) and
        (1418.8000,219.0790) .. (1420.3400,220.1820) .. controls (1420.1100,219.9400)
        and (1419.8700,219.7010) .. (1419.6200,219.4620) .. controls
        (1420.5100,220.4050) and (1421.0600,217.7990) .. (1422.7900,218.5980) ..
        controls (1422.4500,217.1000) and (1424.8200,216.6290) .. (1425.8100,216.3660)
        .. controls (1425.7100,216.1010) and (1425.6700,215.8370) ..
        (1425.5900,215.5740) .. controls (1426.5600,215.5340) and (1427.0200,215.0070)
        .. (1427.5800,214.3030) .. controls (1428.4800,213.1640) and
        (1429.8700,212.7150) .. (1430.8500,211.6860) .. controls (1431.4900,211.0170)
        and (1431.7700,210.1260) .. (1432.5300,209.4770) .. controls
        (1433.6900,208.4820) and (1435.0700,209.1970) .. (1436.3200,209.4570) ..
        controls (1436.1400,209.2260) and (1435.9800,208.9850) .. (1435.8200,208.7360)
        .. controls (1436.2100,208.6030) and (1436.5500,208.3860) ..
        (1436.8300,208.0880) .. controls (1436.4400,207.6170) and (1435.2900,207.2660)
        .. (1435.4200,206.7910) .. controls (1435.6400,206.0180) and
        (1436.0500,205.0710) .. (1435.3200,204.4620) .. controls (1434.2300,203.5220)
        and (1431.0700,203.7160) .. (1430.8300,202.1120) .. controls
        (1429.7700,202.7760) and (1428.7900,202.1820) .. (1428.1000,201.3060) ..
        controls (1427.2900,200.2600) and (1426.5000,199.6930) .. (1425.5800,198.7850)
        .. controls (1424.0800,197.3260) and (1427.7200,195.1340) ..
        (1425.5800,193.3070) .. controls (1425.1900,192.9780) and (1423.8600,192.0240)
        .. (1424.1300,191.4660) .. controls (1424.3100,191.0980) and
        (1425.4200,190.1100) .. (1424.6300,189.8050) .. controls (1423.5400,189.3900)
        and (1423.1200,189.8250) .. (1423.0200,188.3210) .. controls
        (1423.0200,187.8550) and (1423.0200,187.3690) .. (1422.9200,186.9080) ..
        controls (1422.8200,186.4460) and (1423.7800,186.5210) .. (1423.7400,186.2710)
        .. controls (1423.5900,185.3510) and (1421.6100,184.8870) ..
        (1420.9700,184.5120) .. controls (1420.3400,184.1490) and (1420.2800,183.4070)
        .. (1419.4900,183.0970) .. controls (1418.6900,182.7860) and
        (1417.8200,182.7680) .. (1416.9900,182.6000) .. controls (1415.5200,182.3030)
        and (1413.9400,181.5790) .. (1412.5500,181.0240) .. controls
        (1410.4300,180.1750) and (1408.2500,178.2510) .. (1405.9600,177.9870);

        % path4688
        \path[country]
        (1421.5500,244.8700) .. controls (1421.2900,244.6840) and
        (1421.0100,244.6120) .. (1420.6900,244.6530) .. controls (1421.1500,244.4470)
        and (1421.8600,244.3020) .. (1422.2700,244.7230) .. controls
        (1422.0300,244.7730) and (1421.7900,244.8230) .. (1421.5500,244.8680);

        % path4690
        \path[country]
        (1422.4100,244.0800) .. controls (1422.5100,243.9210) and
        (1422.6100,243.8500) .. (1422.7800,243.8650) .. controls (1422.6500,243.9350)
        and (1422.5300,244.0090) .. (1422.4100,244.0800);

    \end{scope}


    % //////// FRANCE //////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path2166
        \path[country, we]
        (1258.5400,351.4300) .. controls (1258.2200,351.0940) and
        (1257.8600,350.8050) .. (1257.4600,350.5660) .. controls (1257.5600,351.1320)
        and (1257.9300,351.5270) .. (1258.5400,351.4300);
        
        % path2168
        \path[country, we]
        (1264.7400,354.6700) .. controls (1264.5400,354.2110) and
        (1264.5400,354.0420) .. (1263.9400,354.1660) .. controls (1264.2000,354.3340)
        and (1264.4700,354.5020) .. (1264.7400,354.6700);

        % path2172
        \path[country, we]
        (1270.2100,361.0060) .. controls (1269.9400,360.4340) and
        (1269.1700,360.5580) .. (1268.7000,360.6460) .. controls (1269.2200,360.6660)
        and (1269.7300,360.7840) .. (1270.2100,361.0060);

        % path2174
        \path[country, we]
        (1270.4900,363.9580) .. controls (1270.9800,363.2530) and
        (1270.3900,362.0470) .. (1269.4900,362.5180) .. controls (1269.9400,362.9160)
        and (1270.2700,363.3960) .. (1270.4900,363.9580);
        
        % path2182
        \path[country, we]
        (1247.9600,345.0940) .. controls (1248.8500,344.6720) and (1249.9200,344.4080)
        .. (1250.9100,344.5900) .. controls (1251.2500,343.0760) and
        (1249.2400,344.1170) .. (1248.8200,343.0780) .. controls (1249.7400,342.7710)
        and (1250.8200,342.8840) .. (1251.7800,342.9330) .. controls
        (1251.0300,342.8040) and (1250.0100,343.0710) .. (1250.5500,342.1410) ..
        controls (1249.9700,342.1110) and (1248.0000,343.2200) .. (1247.7600,342.2490)
        .. controls (1247.4400,340.9240) and (1249.4600,340.1240) ..
        (1250.4200,339.9340) .. controls (1251.7100,339.6780) and (1252.9300,339.5740)
        .. (1254.2400,339.6100) .. controls (1256.0900,339.6600) and
        (1257.2800,337.8600) .. (1259.3400,338.1090) .. controls (1259.1000,338.7740)
        and (1261.5700,341.0960) .. (1262.2600,340.8170) .. controls
        (1262.7300,340.5910) and (1263.1700,340.3330) .. (1263.6000,340.0450) ..
        controls (1264.5400,339.5240) and (1264.4800,340.1970) .. (1265.2600,340.3470)
        .. controls (1266.0300,340.4950) and (1266.6300,339.8850) ..
        (1266.6800,341.1340) .. controls (1267.1800,340.7870) and (1266.4400,340.3720)
        .. (1266.8500,339.8070) .. controls (1267.2800,339.2300) and
        (1267.5000,340.1060) .. (1267.8700,340.2040) .. controls (1268.7500,340.4360)
        and (1269.8900,340.2040) .. (1270.7800,340.0540) .. controls
        (1268.8900,339.5010) and (1269.5800,336.8350) .. (1269.7400,335.4460) ..
        controls (1269.8400,334.7700) and (1268.7900,334.0920) .. (1268.4400,333.6200)
        .. controls (1267.8400,332.8070) and (1268.4400,331.5710) ..
        (1267.5400,330.9090) .. controls (1268.1900,331.0230) and (1268.7900,331.3430)
        .. (1269.4400,331.4780) .. controls (1270.1500,331.6260) and
        (1271.0200,330.9290) .. (1271.6500,331.2430) .. controls (1272.6200,331.7310)
        and (1271.4100,333.1970) .. (1272.7500,333.9670) .. controls
        (1273.1400,334.1890) and (1273.8400,333.7940) .. (1274.2400,333.7900) ..
        controls (1275.4100,333.7800) and (1276.5300,334.1750) .. (1277.6700,334.3910)
        .. controls (1278.7800,334.6020) and (1279.7500,334.5700) ..
        (1280.7400,334.0010) .. controls (1281.6400,333.4860) and (1282.8500,333.5050)
        .. (1283.6700,332.9260) .. controls (1283.0200,333.1820) and
        (1281.9200,333.3120) .. (1281.2900,332.9560) .. controls (1280.0200,332.2250)
        and (1282.9600,330.4270) .. (1283.4400,330.2080) .. controls
        (1284.9900,329.5140) and (1286.7500,329.5970) .. (1288.3200,328.9670) ..
        controls (1289.2300,328.6020) and (1290.4500,326.5140) .. (1291.5800,327.0980)
        .. controls (1290.5900,326.4590) and (1291.2000,322.0340) ..
        (1292.0200,321.2050) .. controls (1292.8300,320.3910) and (1296.9600,318.9190)
        .. (1298.0300,319.8140) .. controls (1298.5700,320.2700) and
        (1297.5100,322.0240) .. (1299.0900,322.4150) .. controls (1300.7200,322.8180)
        and (1300.3400,322.4550) .. (1301.5000,322.7980) .. controls
        (1302.5800,323.1230) and (1302.2400,323.9540) .. (1303.0700,324.3580) ..
        controls (1304.1600,324.8850) and (1305.2600,324.2580) .. (1305.1200,325.9440)
        .. controls (1305.7700,325.5250) and (1306.9000,325.6220) ..
        (1307.5800,325.8640) .. controls (1308.8800,326.3080) and (1308.3300,327.9030)
        .. (1308.0700,328.8290) .. controls (1308.9400,328.9740) and
        (1309.9200,329.2430) .. (1310.7800,328.8990) .. controls (1311.6300,328.5580)
        and (1311.8300,327.5850) .. (1312.6800,327.2450) .. controls
        (1312.7800,327.7810) and (1312.5300,330.1780) .. (1313.2600,330.2040) ..
        controls (1314.3300,330.2440) and (1316.4900,331.6550) .. (1316.8200,332.6820)
        .. controls (1316.7200,332.3860) and (1320.8900,333.0600) ..
        (1321.1000,333.0780) .. controls (1322.1200,333.1680) and (1322.8700,332.9560)
        .. (1323.6800,333.7930) .. controls (1324.3100,334.4530) and
        (1324.7500,335.4900) .. (1325.7100,335.7410) .. controls (1325.9200,335.6410)
        and (1326.0800,335.4970) .. (1326.2100,335.3030) .. controls
        (1326.5200,334.9820) and (1326.6700,335.4080) .. (1327.0000,335.4530) ..
        controls (1327.1900,335.5230) and (1327.2400,335.6490) .. (1327.1500,335.8300)
        .. controls (1327.0500,336.2220) and (1328.0100,336.0080) ..
        (1328.1600,336.0210) .. controls (1329.1900,336.1110) and (1329.7700,335.4830)
        .. (1330.7200,336.2040) .. controls (1331.7300,336.9720) and
        (1333.8100,337.1140) .. (1335.0700,337.3250) .. controls (1333.5300,338.6900)
        and (1332.1000,340.1880) .. (1331.6000,342.2160) .. controls
        (1331.3600,343.2020) and (1330.7700,344.1080) .. (1330.6100,345.1020) ..
        controls (1330.5100,345.7520) and (1330.7300,346.0160) .. (1330.4700,346.8510)
        .. controls (1330.1600,347.8600) and (1330.9300,348.7010) ..
        (1330.2500,349.3270) .. controls (1329.6700,349.8550) and (1329.2300,350.3640)
        .. (1328.3700,350.2870) .. controls (1327.6500,350.2270) and
        (1327.5900,349.1560) .. (1326.7200,349.6390) .. controls (1326.1000,349.9880)
        and (1326.0400,351.1020) .. (1327.0800,350.9350) .. controls
        (1326.3000,351.7610) and (1325.6000,352.7420) .. (1324.7000,353.4550) ..
        controls (1324.1500,353.8130) and (1323.6100,354.1890) .. (1323.0900,354.5830)
        .. controls (1322.6600,354.9730) and (1322.7000,355.7370) ..
        (1322.3300,356.1910) .. controls (1321.7100,356.9650) and (1320.5000,357.3290)
        .. (1320.3100,358.4230) .. controls (1320.4500,358.7960) and
        (1320.5500,359.1800) .. (1320.6000,359.5740) .. controls (1320.4500,360.2830)
        and (1319.7900,360.5360) .. (1319.5200,361.1580) .. controls
        (1320.7100,361.0090) and (1321.1500,360.6030) .. (1321.4600,359.4670) ..
        controls (1321.7700,358.3490) and (1323.8300,358.4350) .. (1324.6700,358.6700)
        .. controls (1325.6700,358.9530) and (1324.9900,360.5970) ..
        (1325.7100,361.3980) .. controls (1326.9800,362.7900) and (1326.2000,363.3120)
        .. (1325.0600,364.2550) .. controls (1325.6700,365.1120) and
        (1327.9400,366.7000) .. (1327.3200,367.9560) .. controls (1326.8900,368.7990)
        and (1323.7500,369.9560) .. (1323.7600,370.1000) .. controls
        (1323.7600,371.0940) and (1325.7300,371.9410) .. (1326.3900,372.5080) ..
        controls (1327.3500,373.3280) and (1325.0600,374.7890) .. (1325.3900,375.8730)
        .. controls (1325.7900,377.1890) and (1328.3100,378.6810) ..
        (1329.6400,378.1480) .. controls (1331.3100,377.4790) and (1331.0600,378.4520)
        .. (1330.4300,379.5650) .. controls (1328.9100,382.2460) and
        (1326.0000,383.5980) .. (1323.4000,385.3510) .. controls (1323.5700,385.5950)
        and (1323.7400,385.8350) .. (1323.9100,386.0710) .. controls
        (1322.9400,386.2100) and (1322.1300,386.7080) .. (1321.2200,387.0260) ..
        controls (1320.2500,387.3690) and (1319.6200,386.8290) .. (1318.7000,386.9020)
        .. controls (1317.3000,387.0120) and (1316.4400,385.8460) ..
        (1314.7700,385.9990) .. controls (1315.4400,384.2680) and (1312.5700,385.5950)
        .. (1312.5400,384.5890) .. controls (1312.7200,384.2770) and
        (1313.0100,384.1950) .. (1313.4000,384.3430) .. controls (1313.4000,383.7760)
        and (1313.0300,383.4560) .. (1312.4600,383.4790) .. controls
        (1312.9400,384.2130) and (1312.5600,384.3210) .. (1311.8700,384.3540) ..
        controls (1310.7800,384.4040) and (1310.6700,384.3440) .. (1310.3700,383.0470)
        .. controls (1310.7600,385.6300) and (1310.1000,383.9830) ..
        (1308.4300,383.9830) .. controls (1307.4600,383.9830) and (1306.6700,383.3730)
        .. (1305.7300,383.3270) .. controls (1304.5800,383.2670) and
        (1303.3100,384.5760) .. (1302.2800,385.0460) .. controls (1301.4800,385.4130)
        and (1298.6600,386.4570) .. (1298.8400,387.5460) .. controls
        (1298.8400,387.9030) and (1298.7100,388.2350) .. (1298.5200,388.5420) ..
        controls (1298.0700,388.9420) and (1298.1100,389.2980) .. (1298.6300,389.6100)
        .. controls (1299.0300,390.8620) and (1298.7700,391.4890) ..
        (1299.5000,392.6960) .. controls (1298.8100,392.8930) and (1298.2100,392.5470)
        .. (1297.5300,392.5880) .. controls (1296.8300,392.6280) and
        (1296.4700,393.1930) .. (1295.8400,393.3650) .. controls (1294.3200,393.7800)
        and (1293.3900,392.2050) .. (1291.9300,393.2650) .. controls
        (1291.8300,393.3350) and (1289.8100,392.3930) .. (1289.5900,392.2300) ..
        controls (1289.0200,391.8070) and (1290.3200,391.8610) .. (1289.4100,391.2520)
        .. controls (1288.8800,390.8990) and (1287.9300,390.7440) ..
        (1287.4800,391.3220) .. controls (1287.2700,390.0330) and (1285.8400,390.5720)
        .. (1285.0700,389.9600) .. controls (1284.0000,389.1150) and
        (1281.8100,388.5730) .. (1282.1500,390.6030) .. controls (1280.9500,390.4300)
        and (1279.6000,390.1280) .. (1278.3900,390.3500) .. controls
        (1277.7200,390.4730) and (1277.2700,390.6630) .. (1276.7000,390.1470) ..
        controls (1275.6800,389.2330) and (1275.7600,389.6090) .. (1274.7300,389.5950)
        .. controls (1273.7000,389.5850) and (1268.7600,386.3350) ..
        (1268.2500,387.6510) .. controls (1267.3100,387.2650) and (1267.9800,386.5850)
        .. (1268.0400,385.9300) .. controls (1268.1400,385.1510) and
        (1265.8400,385.5060) .. (1265.3700,384.9150) .. controls (1268.2300,383.8560)
        and (1268.4700,379.8920) .. (1268.9900,377.3140) .. controls
        (1269.2000,376.3020) and (1269.3800,374.7070) .. (1270.2200,373.9850) ..
        controls (1271.4500,372.9330) and (1269.8000,372.7850) .. (1269.6900,373.9750)
        .. controls (1269.5200,371.5390) and (1270.0100,368.5540) ..
        (1271.0600,366.3430) .. controls (1272.0700,366.9120) and (1273.0800,367.5870)
        .. (1273.5100,368.7190) .. controls (1273.6100,369.2230) and
        (1273.7000,369.7270) .. (1273.8000,370.2310) .. controls (1274.0300,370.8720)
        and (1274.6700,370.9600) .. (1274.6600,371.7430) .. controls
        (1274.9500,370.7360) and (1273.9300,369.9610) .. (1273.8300,369.0070) ..
        controls (1273.6900,367.5410) and (1273.1700,366.5480) .. (1271.8700,365.8350)
        .. controls (1271.3300,365.5370) and (1270.7200,365.1300) ..
        (1270.2700,364.6930) .. controls (1269.5300,363.9810) and (1271.4600,364.3360)
        .. (1271.8500,364.6930) .. controls (1270.9400,364.2520) and
        (1270.8900,360.3990) .. (1271.4200,359.6530) .. controls (1270.2300,360.4880)
        and (1267.4200,358.8450) .. (1266.8700,357.7380) .. controls
        (1266.3800,356.7590) and (1265.2700,356.2500) .. (1265.0500,355.1070) ..
        controls (1264.8500,354.0640) and (1266.7600,352.9220) .. (1264.3600,352.8140)
        .. controls (1264.6400,352.4810) and (1264.7000,351.8760) ..
        (1265.0600,351.6220) .. controls (1265.9800,350.9840) and (1266.8200,352.0570)
        .. (1267.6800,352.1660) .. controls (1266.1500,351.1570) and
        (1265.5500,351.4920) .. (1263.9500,351.7000) .. controls (1263.1500,351.8050)
        and (1261.5900,350.6200) .. (1263.0700,350.4380) .. controls
        (1262.6600,350.0310) and (1262.8300,349.7670) .. (1263.5700,349.6460) ..
        controls (1262.4400,349.3640) and (1260.8200,350.2880) .. (1259.9000,349.2860)
        .. controls (1260.4100,349.2860) and (1260.8900,349.1590) ..
        (1261.3400,348.9260) .. controls (1260.4400,348.3220) and (1258.7700,348.5670)
        .. (1258.5300,349.7900) .. controls (1258.5300,348.9900) and
        (1257.6100,348.2420) .. (1258.4300,347.5590) .. controls (1258.0800,348.4350)
        and (1256.5100,348.3780) .. (1257.4900,347.2710) .. controls
        (1255.5000,349.0010) and (1252.8200,345.0620) .. (1250.8000,347.2010) ..
        controls (1249.9900,346.0840) and (1249.3200,345.3980) ..
        (1247.9300,345.1090);

        % path2184
        \path[country, we]
        (1337.1700,393.1180) .. controls (1337.5800,392.7030) and
        (1337.6600,391.8610) .. (1338.2100,391.5840) .. controls (1339.3100,391.0340)
        and (1340.5600,390.8920) .. (1341.6000,390.1990) .. controls
        (1342.5300,389.5800) and (1341.8700,387.8350) .. (1343.1400,387.9330) ..
        controls (1343.2900,390.1290) and (1344.3400,393.2940) .. (1343.8200,395.4210)
        .. controls (1343.2700,397.6650) and (1342.1700,399.8100) ..
        (1341.2000,401.9000) .. controls (1340.8200,401.3070) and (1337.2900,400.0180)
        .. (1339.1800,399.2360) .. controls (1338.6700,399.1170) and
        (1338.1900,398.9250) .. (1337.7400,398.6610) .. controls (1338.2300,398.3490)
        and (1338.5800,397.8280) .. (1338.5300,397.2210) .. controls
        (1337.5200,397.4580) and (1337.3800,396.3340) .. (1337.9600,395.7820) ..
        controls (1337.1000,395.5660) and (1336.5600,394.4400) .. (1337.7400,394.1980)
        .. controls (1337.4900,393.8660) and (1337.3000,393.5070) ..
        (1337.1700,393.1180);
    
    \end{scope}
    
    
    % //////// GERMANY /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path3832
        \path[country, we]
        (1337.7400,289.8700) .. controls (1337.9000,289.1070) and
        (1337.6400,289.0590) .. (1337.0200,289.7250) .. controls (1337.2600,289.7750)
        and (1337.5000,289.8250) .. (1337.7400,289.8700);

        % path3834
        \path[country, we] (1354.0100,292.0300) .. controls (1354.4400,292.0800) and
        (1354.8800,292.0800) .. (1355.3100,292.0300) .. controls (1355.0100,291.2700)
        and (1354.2400,291.0030) .. (1353.5100,291.3090) .. controls
        (1353.6700,291.5500) and (1353.8400,291.7900) .. (1354.0100,292.0300);

        % path3884
        \path[country, we]
        (1336.6800,287.2600) .. controls (1336.0000,287.5360) and (1335.9300,288.4950)
        .. (1336.0700,289.0740) .. controls (1336.0700,288.6820) and
        (1336.4300,288.3410) .. (1336.8800,288.1670) .. controls (1336.5600,288.0600)
        and (1336.3900,287.7480) .. (1336.6800,287.2600) -- cycle(1337.5800,288.0660)
        .. controls (1337.3700,288.0650) and (1337.1800,288.1060) ..
        (1336.9800,288.1670) .. controls (1337.3600,288.2570) and (1337.8900,288.1970)
        .. (1338.1900,288.1670) .. controls (1337.9900,288.0870) and
        (1337.8000,288.0670) .. (1337.5800,288.0660) -- cycle(1339.3300,287.9590) ..
        controls (1338.7000,287.8990) and (1338.9200,288.1030) .. (1338.2900,288.1670)
        .. controls (1338.7100,288.3790) and (1339.1600,289.6790) ..
        (1339.4000,290.0820) .. controls (1339.6100,290.4370) and (1340.5900,291.1280)
        .. (1340.3100,291.5940) .. controls (1339.8400,292.3610) and
        (1338.5200,291.9360) .. (1337.9900,292.9040) .. controls (1338.6900,293.2020)
        and (1339.3900,293.0710) .. (1340.1000,292.9040) .. controls
        (1338.5000,293.6400) and (1340.2300,294.1450) .. (1340.5100,295.0210) ..
        controls (1339.8300,294.9910) and (1339.5800,295.4130) .. (1340.1000,295.9280)
        .. controls (1340.6800,296.4890) and (1341.5100,296.3150) ..
        (1342.2200,296.5320) .. controls (1342.9700,296.7630) and (1343.3500,297.3640)
        .. (1343.8300,297.9440) .. controls (1344.4100,298.6390) and
        (1345.1800,298.7220) .. (1345.8500,299.2540) .. controls (1344.1100,299.0650)
        and (1343.6500,297.6200) .. (1342.3200,296.8350) .. controls
        (1341.4500,296.3210) and (1340.4300,296.9250) .. (1339.5000,296.8350) ..
        controls (1338.4100,296.7270) and (1337.3500,296.3740) .. (1337.1800,297.8430)
        .. controls (1337.0800,298.4290) and (1337.5900,298.8900) ..
        (1337.5800,299.4550) .. controls (1337.4200,299.8760) and (1337.3600,300.3230)
        .. (1337.2800,300.7660) .. controls (1337.1800,300.0380) and
        (1337.3900,299.3410) .. (1336.5800,298.9520) .. controls (1335.6200,298.4960)
        and (1335.2800,299.3980) .. (1335.8700,300.0600) .. controls
        (1335.3400,300.1930) and (1334.8900,300.0800) .. (1334.4600,299.7580) ..
        controls (1336.8300,298.1580) and (1330.4100,297.9060) .. (1329.7200,298.0440)
        .. controls (1328.9300,298.2020) and (1327.5900,299.4720) ..
        (1327.6100,300.3630) .. controls (1327.6100,301.1020) and (1330.3800,301.4930)
        .. (1329.9200,301.2700) .. controls (1328.8000,300.7220) and
        (1328.0400,304.9540) .. (1327.8100,305.9060) .. controls (1327.5100,307.1330)
        and (1326.4700,306.2210) .. (1325.5900,306.8130) .. controls
        (1324.2100,307.7360) and (1326.7800,308.1680) .. (1327.1200,308.7410) ..
        controls (1328.1100,310.3820) and (1324.6900,310.8720) .. (1325.7600,312.0960)
        .. controls (1326.7900,313.2920) and (1322.1500,313.0130) ..
        (1321.5200,312.6890) .. controls (1321.9300,313.8420) and (1321.1700,312.8340)
        .. (1320.3500,313.3650) .. controls (1320.4500,313.6320) and
        (1320.1400,313.6990) .. (1320.3500,314.0710) .. controls (1321.2700,314.3870)
        and (1322.3900,316.5470) .. (1321.8800,317.5160) .. controls
        (1321.4300,318.3840) and (1319.6700,319.6560) .. (1320.5200,320.8420) ..
        controls (1320.9800,321.4770) and (1320.6200,322.3570) .. (1320.7100,322.5900)
        .. controls (1320.9800,323.3010) and (1322.6400,323.3360) ..
        (1321.8600,324.3510) .. controls (1322.8500,324.1840) and (1322.7600,325.3230)
        .. (1323.0500,325.9280) .. controls (1320.0800,325.8980) and
        (1319.5800,328.2490) .. (1322.4200,329.6330) .. controls (1324.4100,330.6070)
        and (1322.4200,332.4840) .. (1323.1400,333.3360) .. controls
        (1323.2500,333.4660) and (1325.1800,335.8400) .. (1325.6600,335.7610) ..
        controls (1326.3500,335.6470) and (1325.8000,335.2220) .. (1326.8200,335.3560)
        .. controls (1327.3600,335.4260) and (1326.8200,336.3160) ..
        (1327.7400,336.0790) .. controls (1328.0900,335.9890) and (1328.5700,336.0790)
        .. (1328.9300,336.0490) .. controls (1330.2100,335.6050) and
        (1330.3400,336.2990) .. (1331.5200,336.6710) .. controls (1332.5900,337.0060)
        and (1333.9200,337.1500) .. (1335.0300,337.3350) .. controls
        (1334.1300,338.1300) and (1333.2800,338.9160) .. (1332.5400,339.8730) ..
        controls (1331.7100,340.9690) and (1331.4200,342.6370) .. (1330.8600,343.8510)
        .. controls (1330.4900,344.6630) and (1329.0900,350.5230) ..
        (1331.1800,348.7600) .. controls (1330.4600,349.5990) and (1334.0900,349.0100)
        .. (1334.7600,349.0450) .. controls (1336.0600,349.1150) and
        (1337.2000,349.0650) .. (1337.4800,348.2380) .. controls (1335.9200,348.8190)
        and (1336.4500,346.7210) .. (1338.2900,347.6340) .. controls
        (1339.5900,348.2790) and (1342.7400,348.6730) .. (1344.0600,349.4430) ..
        controls (1344.8700,349.9150) and (1349.2000,349.6240) .. (1348.0700,351.5650)
        .. controls (1349.6300,351.5150) and (1349.7400,350.0990) ..
        (1350.0800,348.9440) .. controls (1350.7500,349.5390) and (1352.2700,349.5270)
        .. (1353.1100,349.4480) .. controls (1352.3800,349.8060) and
        (1354.2500,350.3460) .. (1354.6200,350.3550) .. controls (1355.4800,350.3750)
        and (1356.0200,349.6300) .. (1356.8400,349.5490) .. controls
        (1358.4100,349.3910) and (1359.9300,348.1740) .. (1361.6700,348.7420) ..
        controls (1361.6700,348.4730) and (1361.6700,348.1950) .. (1361.5700,347.9360)
        .. controls (1362.3800,348.0360) and (1363.1700,348.4400) ..
        (1363.9900,348.4400) .. controls (1364.3900,348.3040) and (1364.7900,348.2180)
        .. (1365.2000,348.1380) .. controls (1365.6500,348.1880) and
        (1365.8400,349.0620) .. (1366.2100,349.3470) .. controls (1367.3300,350.2080)
        and (1367.3200,349.7710) .. (1367.6200,348.7420) .. controls
        (1367.9200,347.7160) and (1366.6400,348.1120) .. (1366.7100,347.2310) ..
        controls (1366.8100,346.1560) and (1366.8400,346.2020) .. (1366.0100,345.3150)
        .. controls (1365.3800,344.6470) and (1365.8100,344.1290) ..
        (1366.5100,343.8040) .. controls (1367.3200,343.4330) and (1369.9400,342.9850)
        .. (1369.9400,341.7880) .. controls (1369.9400,339.6810) and
        (1371.3800,341.5140) .. (1372.1600,340.5780) .. controls (1373.5600,338.8780)
        and (1371.1100,337.6940) .. (1370.0400,337.0500) .. controls
        (1368.7800,336.2970) and (1367.7200,335.2550) .. (1366.4100,334.5310) ..
        controls (1364.7700,333.6200) and (1364.4400,331.5470) .. (1362.8800,330.7000)
        .. controls (1364.1100,329.7220) and (1363.5400,328.9180) ..
        (1362.3800,328.2810) .. controls (1361.4800,327.7880) and (1361.2800,326.8960)
        .. (1360.8700,326.1650) .. controls (1361.5200,326.0650) and
        (1362.0300,326.3300) .. (1362.2800,327.2730) .. controls (1362.5300,324.6180)
        and (1365.9400,325.6520) .. (1367.3200,324.5520) .. controls
        (1369.5100,322.7960) and (1373.1700,321.8270) .. (1375.7800,320.8230) ..
        controls (1375.5500,320.6010) and (1375.3200,320.4280) .. (1375.0800,320.2180)
        .. controls (1376.0800,319.9820) and (1376.3200,319.6950) ..
        (1377.1800,320.8290) .. controls (1379.3000,323.5630) and (1380.6500,318.5010)
        .. (1379.6000,317.1890) .. controls (1379.4600,316.3730) and
        (1378.1600,316.3320) .. (1378.0900,315.6820) .. controls (1377.9900,314.7990)
        and (1378.0900,314.4960) .. (1377.4000,313.7670) .. controls
        (1376.9500,313.2790) and (1377.6200,312.8860) .. (1377.8000,312.4220) ..
        controls (1378.8400,309.7570) and (1376.1800,309.0410) .. (1376.8800,308.2410)
        .. controls (1378.2800,306.6370) and (1374.4100,306.0790) ..
        (1373.8800,304.5710) .. controls (1374.5900,304.0130) and (1376.8400,300.5650)
        .. (1375.3800,300.3620) .. controls (1375.0800,299.2530) and
        (1374.7500,298.0780) .. (1373.5700,297.6400) .. controls (1372.8400,297.3710)
        and (1371.6500,297.1740) .. (1371.5500,296.2290) .. controls
        (1371.5500,295.7370) and (1371.2800,294.2130) .. (1370.5400,294.2130) ..
        controls (1370.1000,294.2130) and (1369.1900,294.2130) .. (1369.4300,294.7170)
        .. controls (1368.6300,294.2460) and (1366.8800,292.1660) ..
        (1366.1100,292.0970) .. controls (1364.4900,291.9520) and (1363.3900,292.0870)
        .. (1362.1800,293.3060) .. controls (1361.9800,291.9510) and
        (1364.2500,291.8550) .. (1365.1000,291.9960) .. controls (1363.4500,291.3800)
        and (1363.2100,291.8550) .. (1361.9800,292.8020) .. controls
        (1361.3900,293.2500) and (1360.1200,293.7490) .. (1360.4600,294.7170) ..
        controls (1360.6200,293.0830) and (1357.3800,294.5390) .. (1356.6300,295.0200)
        .. controls (1358.1000,294.3050) and (1356.4700,295.5040) ..
        (1356.2300,296.2290) .. controls (1355.6300,295.6670) and (1352.1300,294.8860)
        .. (1352.9000,296.2290) .. controls (1352.7600,295.7120) and
        (1352.4000,295.4330) .. (1351.9000,295.3220) .. controls (1352.8700,294.3210)
        and (1353.7500,293.6570) .. (1354.0100,292.1970) .. controls
        (1352.6900,292.4600) and (1351.9000,292.9910) .. (1350.5900,292.3990) ..
        controls (1349.7700,292.0300) and (1348.4700,291.5300) .. (1348.0700,292.7010)
        .. controls (1347.9600,292.1810) and (1347.9400,292.1510) ..
        (1348.2700,291.6930) .. controls (1347.6000,291.3940) and (1346.8100,291.4230)
        .. (1346.1500,291.6930) .. controls (1346.6500,291.4570) and
        (1347.8000,289.9490) .. (1346.5500,289.9800) .. controls (1348.5500,289.0730)
        and (1341.7600,288.4670) .. (1342.0300,288.6160) .. controls
        (1341.4300,288.2850) and (1339.9900,288.0260) .. (1339.3300,287.9580) --
        cycle;

        % path3892
        \path[country, we]
        (1366.9000,292.6800) .. controls (1367.9800,292.5440) and
        (1367.4700,291.5160) .. (1367.1200,290.9520) .. controls (1367.8800,290.8820)
        and (1368.6000,291.1590) .. (1369.2800,291.4560) .. controls
        (1368.9600,290.5690) and (1367.1000,290.8280) .. (1368.5600,289.8720) ..
        controls (1368.4600,291.3320) and (1370.0500,290.0520) .. (1370.2900,290.9150)
        .. controls (1370.4000,291.3380) and (1369.6700,291.8780) ..
        (1370.1800,292.2040) .. controls (1370.5600,292.4440) and (1370.8700,292.4760)
        .. (1370.8600,293.0390) .. controls (1370.1500,292.9180) and
        (1369.5200,292.4900) .. (1368.9100,293.0190) .. controls (1368.3800,293.4780)
        and (1367.2100,293.3470) .. (1366.9000,292.6850);

        % path3894
        \path[country, we]
        (1371.3700,295.0500) .. controls (1371.3700,294.7060) and
        (1371.3700,294.3700) .. (1371.2200,294.0420) .. controls (1371.9100,294.9170)
        and (1373.3500,294.9030) .. (1373.9700,295.8630) .. controls
        (1374.5800,296.8000) and (1372.0400,296.8050) .. (1371.5800,296.5620) ..
        controls (1372.6000,296.3780) and (1371.6800,295.3350) .. (1372.8100,295.2660)
        .. controls (1372.3100,295.3060) and (1371.8300,295.2360) ..
        (1371.3700,295.0500);

    \end{scope}
    
    
    % //////// GREECE //////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path6492
        \path[country]
        (1417.6600,416.3740) .. controls (1418.1800,416.4940) and (1418.8700,416.5970)
        .. (1419.3800,416.3540) .. controls (1420.4700,415.8330) and
        (1418.6800,415.1280) .. (1420.3300,415.2960) .. controls (1419.7500,413.8550)
        and (1419.3500,413.9070) .. (1420.7300,413.1590) .. controls
        (1421.6000,412.6880) and (1422.1900,412.0330) .. (1422.5000,411.0840) ..
        controls (1422.9300,409.7740) and (1423.4100,409.8890) .. (1424.2400,408.9520)
        .. controls (1425.0500,408.0480) and (1423.8000,406.9460) ..
        (1423.8500,406.0180) .. controls (1424.4600,406.4180) and (1425.4100,405.8670)
        .. (1426.4200,405.8890) .. controls (1428.6500,405.9390) and
        (1429.8000,404.5980) .. (1431.6500,403.7720) .. controls (1432.8400,403.2420)
        and (1434.2400,403.9520) .. (1435.5600,403.5050) .. controls
        (1436.4000,403.2190) and (1435.8600,402.1060) .. (1437.0400,402.1290) ..
        controls (1437.8200,402.1490) and (1438.7400,402.9150) .. (1439.4300,402.4290)
        .. controls (1440.3600,401.7780) and (1441.7600,402.1730) ..
        (1442.8100,402.0310) .. controls (1443.8600,401.8890) and (1444.8600,400.7270)
        .. (1445.8600,400.4090) .. controls (1446.6500,400.1580) and
        (1447.9900,399.7150) .. (1448.6700,400.4290) .. controls (1449.2700,401.0530)
        and (1449.7400,402.2190) .. (1450.8300,401.8720) .. controls
        (1452.0200,401.4970) and (1452.7400,402.4210) .. (1453.8500,402.6400) ..
        controls (1454.8500,402.8350) and (1455.7500,402.2130) .. (1456.7500,402.2530)
        .. controls (1457.6500,402.2930) and (1458.8800,402.5570) ..
        (1459.6600,401.9560) .. controls (1460.6300,401.2070) and (1459.5600,400.2690)
        .. (1459.2800,399.4960) .. controls (1458.7800,398.1100) and
        (1461.8000,399.1120) .. (1462.1200,399.2910) .. controls (1463.1400,399.8570)
        and (1462.9500,400.7790) .. (1463.3300,401.7780) .. controls
        (1461.1100,402.7310) and (1461.6800,403.2940) .. (1461.5700,404.6950) ..
        controls (1461.4700,405.7890) and (1460.8400,406.6580) .. (1459.4900,407.3040)
        .. controls (1459.9100,406.1540) and (1454.6300,405.9210) ..
        (1453.8100,405.5970) .. controls (1452.2200,404.9670) and (1452.2400,405.2850)
        .. (1450.8200,406.2240) .. controls (1449.8300,406.8710) and
        (1448.9200,405.0300) .. (1447.9900,405.4930) .. controls (1446.6800,406.1430)
        and (1446.6300,407.8870) .. (1444.6500,407.1630) .. controls
        (1443.1700,406.6210) and (1443.2700,407.3230) .. (1443.6600,408.3120) ..
        controls (1443.8700,408.8470) and (1444.6500,408.4500) .. (1444.2200,409.2190)
        .. controls (1443.9300,409.7410) and (1444.5600,410.3600) ..
        (1444.9600,409.9340) .. controls (1445.7700,409.0670) and (1447.8200,411.8480)
        .. (1448.2600,412.3440) .. controls (1447.1200,412.9660) and
        (1445.6700,410.5200) .. (1444.5000,410.4210) .. controls (1441.7800,410.1950)
        and (1445.3900,412.8730) .. (1445.5300,413.6400) .. controls
        (1444.2600,414.0510) and (1442.9300,411.8270) .. (1441.8800,411.4050) ..
        controls (1441.0000,411.0520) and (1440.8900,411.6130) .. (1441.2200,412.2750)
        .. controls (1441.7100,413.2420) and (1442.6700,413.4840) ..
        (1443.4400,414.1440) .. controls (1441.5800,414.9210) and (1441.1300,413.2900)
        .. (1440.5900,412.1260) .. controls (1439.9900,410.8130) and
        (1438.0300,410.6390) .. (1437.1800,409.5360) .. controls (1437.7400,409.3730)
        and (1438.0200,408.9670) .. (1437.9000,408.3840) .. controls
        (1433.8800,408.9350) and (1435.7300,413.4040) .. (1437.2100,415.3510) ..
        controls (1438.0000,416.3850) and (1443.1800,421.1230) .. (1439.4800,421.4870)
        .. controls (1441.0600,420.9350) and (1439.5800,418.7680) ..
        (1438.4000,419.1110) .. controls (1436.8700,419.5590) and (1438.1900,422.4050)
        .. (1439.4100,421.9200) .. controls (1438.6300,422.9200) and
        (1437.3500,423.5220) .. (1436.0900,423.1440) .. controls (1436.9100,423.5670)
        and (1439.1900,424.1930) .. (1439.5400,425.0000) .. controls
        (1439.8200,425.6480) and (1440.6100,424.5970) .. (1441.0500,425.2570) ..
        controls (1441.4700,425.8800) and (1440.4100,425.9450) .. (1441.8700,426.3560)
        .. controls (1443.4000,426.7890) and (1444.3500,427.6730) ..
        (1445.8000,428.3240) .. controls (1446.8700,428.8050) and (1446.8100,429.7050)
        .. (1446.6700,430.7120) .. controls (1446.5200,431.8220) and
        (1447.4700,432.8120) .. (1446.9000,433.8730) .. controls (1445.6800,432.9040)
        and (1444.6200,431.2360) .. (1442.9800,430.9290) .. controls
        (1441.7800,430.7050) and (1440.6200,431.6550) .. (1439.4800,431.5680) ..
        controls (1439.4800,432.5630) and (1440.3700,431.6680) .. (1440.4400,432.7300)
        .. controls (1440.4400,433.4210) and (1441.6600,435.8940) ..
        (1441.8600,434.0890) .. controls (1442.1100,434.5830) and (1443.4000,435.1220)
        .. (1442.9300,435.8170) .. controls (1443.0400,435.6560) and
        (1440.7700,436.8170) .. (1441.1300,436.8250) .. controls (1440.1100,436.8050)
        and (1440.8000,435.7710) .. (1440.0200,435.4600) .. controls
        (1439.2600,435.1530) and (1438.3200,435.0830) .. (1437.6800,434.5210) ..
        controls (1437.5500,436.2960) and (1439.2300,437.8640) .. (1439.8100,439.4510)
        .. controls (1440.1600,440.3950) and (1440.6200,441.2120) ..
        (1440.3700,442.2150) .. controls (1440.1400,443.1000) and (1441.4900,443.3580)
        .. (1441.3000,444.1870) .. controls (1441.2000,444.5550) and
        (1438.6700,441.9910) .. (1438.4500,441.6480) .. controls (1437.1800,439.6300)
        and (1436.0700,442.8470) .. (1436.4500,444.0250) .. controls
        (1435.3600,444.1800) and (1434.9800,441.1070) .. (1434.1900,440.5560) ..
        controls (1433.6900,440.2030) and (1433.8900,439.2270) .. (1433.0700,439.3090)
        .. controls (1432.0000,439.4160) and (1432.1800,440.7760) ..
        (1432.2800,441.5050) .. controls (1430.1200,441.1380) and (1429.3700,438.6490)
        .. (1430.2400,436.8670) .. controls (1430.9400,435.4180) and
        (1426.6900,432.6360) .. (1426.0100,431.6400) .. controls (1426.8600,431.3710)
        and (1427.2900,430.1690) .. (1427.9000,429.5950) .. controls
        (1428.5000,429.0360) and (1429.2000,429.6350) .. (1429.8600,429.0640) ..
        controls (1430.3100,428.6690) and (1430.8100,427.7610) .. (1431.5300,427.9000)
        .. controls (1432.8500,428.1550) and (1433.7500,429.5120) ..
        (1435.2100,429.6430) .. controls (1436.3600,429.7450) and (1437.1100,430.5810)
        .. (1438.0300,431.1370) .. controls (1438.7700,431.5780) and
        (1439.1200,430.7010) .. (1439.8900,430.2410) .. controls (1440.5000,429.8690)
        and (1441.3300,429.3200) .. (1439.9900,429.1500) .. controls
        (1439.2400,429.0600) and (1438.6000,429.1700) .. (1437.9200,428.7430) ..
        controls (1437.1300,428.2550) and (1436.9700,427.3880) .. (1436.3400,428.4000)
        .. controls (1435.9700,427.8780) and (1435.5400,427.4210) ..
        (1435.0400,427.0320) .. controls (1435.1500,428.9030) and (1432.4700,427.4240)
        .. (1431.7100,427.5950) .. controls (1429.7600,428.0320) and
        (1428.5100,428.6420) .. (1427.4800,426.8170) .. controls (1427.3400,427.4720)
        and (1426.7400,427.9560) .. (1426.1900,428.2570) .. controls
        (1425.8200,427.0690) and (1425.5200,425.7700) .. (1424.4700,424.9920) ..
        controls (1423.9200,424.5810) and (1422.3600,423.4660) .. (1423.1600,422.6400)
        .. controls (1423.4600,422.3280) and (1427.4100,423.5720) ..
        (1425.6100,421.9200) .. controls (1425.0500,421.4110) and (1422.9500,421.2850)
        .. (1423.0900,422.5670) .. controls (1422.5000,420.8220) and
        (1420.8800,420.5730) .. (1419.7400,419.4450) .. controls (1418.9500,418.6530)
        and (1419.0700,416.4970) .. (1417.6900,416.3750);

        % path3608
        \path[country]
        (1468.3500,442.2940) .. controls (1467.1800,441.1900) and
        (1470.0900,440.2210) .. (1470.8700,440.4220) .. controls (1470.2500,440.9120)
        and (1468.4000,441.3470) .. (1468.3500,442.2940);

        % path6518
        \path[country]
        (1417.5200,418.3180) .. controls (1417.7800,418.4860) and
        (1418.0400,418.6540) .. (1418.3100,418.8220) .. controls (1416.9100,419.0920)
        and (1415.0700,416.6980) .. (1415.1400,415.4380) .. controls
        (1417.9400,415.1620) and (1415.5500,417.6840) .. (1417.5200,418.3180);

        % path6520
        \path[country]
        (1421.7000,427.6060) .. controls (1421.7000,427.3660) and
        (1421.7000,427.1270) .. (1421.7000,426.8860) .. controls (1422.2200,427.3150)
        and (1421.9600,428.0770) .. (1422.4500,428.4700) .. controls
        (1422.9900,428.9040) and (1423.5100,429.3600) .. (1423.7100,430.0540) ..
        controls (1423.0800,430.2990) and (1421.3500,430.0940) .. (1421.4100,429.1180)
        .. controls (1421.1700,429.2650) and (1420.9300,429.4090) ..
        (1420.6900,429.5500) .. controls (1419.9900,428.2510) and (1421.2400,428.4640)
        .. (1421.7000,427.6060);

        % path6522
        \path[country]
        (1422.7000,423.6460) .. controls (1423.0700,424.0910) and
        (1422.9900,426.1950) .. (1422.1200,425.5620) .. controls (1421.6200,425.1950)
        and (1421.9400,423.4970) .. (1422.7000,423.6460);

        % path6524
        \path[country]
        (1423.0600,428.1820) .. controls (1422.7000,427.7540) and
        (1422.4300,427.2740) .. (1422.2700,426.7420) .. controls (1422.6300,427.1650)
        and (1422.9000,427.6450) .. (1423.0600,428.1820);

        % path6526
        \path[country]
        (1424.1400,433.8700) .. controls (1423.4400,433.4390) and
        (1422.5400,432.8010) .. (1422.6300,431.8530) .. controls (1424.1500,431.8530)
        and (1425.0400,432.6530) .. (1424.1400,433.8700);

        % path6528
        \path[country]
        (1439.7700,444.8140) .. controls (1440.2600,445.3930) and
        (1440.9800,446.4960) .. (1439.7700,446.7580) .. controls (1439.6100,446.1800)
        and (1439.0300,445.2880) .. (1439.7700,444.8140);

        % path6530
        \path[country]
        (1442.9300,430.8460) .. controls (1443.4000,431.6010) and
        (1443.0300,431.7900) .. (1442.3600,431.7830) .. controls (1442.3600,431.3680)
        and (1442.5700,431.0560) .. (1442.9300,430.8460);

        % path6532
        \path[country]
        (1443.0100,433.6540) .. controls (1442.8100,433.4060) and
        (1442.6400,433.1420) .. (1442.5000,432.8630) .. controls (1443.3100,432.6300)
        and (1443.4800,432.8930) .. (1443.0100,433.6540);

        % path6534
        \path[country]
        (1443.4400,426.8140) .. controls (1443.7700,425.3320) and
        (1439.7500,422.6050) .. (1438.5400,423.6460) .. controls (1439.1200,422.9960)
        and (1439.7700,421.9660) .. (1440.7600,421.9380) .. controls
        (1441.9000,421.9080) and (1442.3200,423.2290) .. (1443.0000,423.8830) ..
        controls (1444.0100,424.8640) and (1445.4900,424.4710) .. (1446.6800,425.0150)
        .. controls (1448.0700,425.6500) and (1447.4000,427.4920) ..
        (1448.1500,428.5490) .. controls (1448.7500,429.3970) and (1450.0100,429.1100)
        .. (1450.4900,430.1810) .. controls (1451.1400,431.6470) and
        (1448.8800,430.4590) .. (1448.5600,430.1810) .. controls (1447.8300,429.5050)
        and (1447.3600,427.9000) .. (1446.5100,427.4810) .. controls
        (1445.5900,427.0300) and (1444.0700,427.9050) .. (1443.4400,426.8230);

        % path6536
        \path[country]
        (1444.0100,421.6300) .. controls (1443.7500,421.4320) and
        (1443.5100,421.2150) .. (1443.2900,420.9820) .. controls (1443.8300,420.8420)
        and (1444.1400,421.0420) .. (1444.0100,421.6300);

        % path6538
        \path[country]
        (1448.7000,454.9660) .. controls (1447.7400,455.1750) and
        (1445.7200,455.0460) .. (1444.8100,454.6530) .. controls (1443.8800,454.2500)
        and (1444.4800,452.7300) .. (1444.5200,452.0140) .. controls
        (1444.7500,452.1620) and (1444.9900,452.3060) .. (1445.2400,452.4460) ..
        controls (1445.5000,451.9740) and (1445.6000,451.4700) .. (1445.5300,450.9340)
        .. controls (1446.1100,452.7020) and (1447.5500,451.9590) ..
        (1448.9100,451.7980) .. controls (1447.5600,452.3230) and (1448.5500,452.5590)
        .. (1449.1200,453.0780) .. controls (1449.9800,453.8670) and
        (1450.7800,453.7180) .. (1451.8200,453.3460) .. controls (1453.9700,452.5770)
        and (1456.2200,453.9260) .. (1458.3800,454.0310) .. controls
        (1458.9900,454.0610) and (1460.1400,453.4380) .. (1460.1700,454.5010) ..
        controls (1460.1700,454.9400) and (1459.8800,455.5190) .. (1460.5500,455.4770)
        .. controls (1461.5600,455.4170) and (1462.7000,454.5160) ..
        (1463.7000,454.7070) .. controls (1464.1800,454.7970) and (1464.3100,455.8440)
        .. (1464.0200,456.1670) .. controls (1463.6400,456.6010) and
        (1462.8500,456.5830) .. (1462.3300,456.5800) .. controls (1460.2500,456.5700)
        and (1458.2400,456.7780) .. (1456.2000,457.1790) .. controls
        (1455.4500,457.3250) and (1454.4800,457.6180) .. (1453.7600,457.2090) ..
        controls (1453.1400,456.8510) and (1453.2500,456.0750) .. (1452.6000,455.7680)
        .. controls (1451.3900,455.1900) and (1449.9800,455.2810) ..
        (1448.7000,454.9690);

        % path6540
        \path[country]
        (1448.7700,434.9500) .. controls (1448.4800,434.3670) and
        (1448.7700,433.8880) .. (1449.3400,433.6530) .. controls (1449.4400,434.2140)
        and (1449.2400,434.6470) .. (1448.7700,434.9500);

        % path6542
        \path[country]
        (1449.4900,442.5100) .. controls (1449.4900,442.2460) and
        (1449.4900,441.9820) .. (1449.4900,441.7180) .. controls (1449.9900,442.2150)
        and (1450.5900,442.1480) .. (1451.0000,441.5750) .. controls
        (1451.0000,442.5230) and (1450.1100,442.3470) .. (1449.4900,442.5100);

        % path6544
        \path[country]
        (1449.7800,408.7410) .. controls (1448.7700,408.4600) and
        (1448.6700,406.6220) .. (1449.9200,406.8690) .. controls (1451.0400,407.0940)
        and (1450.8200,408.5910) .. (1449.7800,408.7410);

        % path6546
        \path[country]
        (1450.1300,424.2940) .. controls (1450.0300,423.4800) and
        (1448.9600,423.4520) .. (1449.2700,422.5650) .. controls (1450.1600,422.6250)
        and (1450.4600,423.5460) .. (1450.7800,424.2210) .. controls
        (1450.5600,424.2410) and (1450.3400,424.2710) .. (1450.1300,424.2910);

        % path6548
        \path[country]
        (1452.0800,440.2790) .. controls (1451.9600,440.0390) and
        (1451.8400,439.7990) .. (1451.7200,439.5580) .. controls (1452.5400,439.5570)
        and (1452.6600,439.7980) .. (1452.0800,440.2790);

        % path6550
        \path[country]
        (1453.3000,413.6380) .. controls (1454.1100,413.5150) and
        (1454.9000,413.9920) .. (1455.6800,413.5680) .. controls (1455.4000,414.0350)
        and (1455.2600,414.5390) .. (1455.2500,415.0810) .. controls
        (1454.1400,414.4740) and (1452.4500,415.7880) .. (1453.3000,413.6400);

        % path6552
        \path[country]
        (1453.4500,433.5820) .. controls (1452.7900,432.8750) and
        (1452.2400,432.0470) .. (1451.4300,431.4930) .. controls (1451.6300,431.2520)
        and (1451.8700,431.0600) .. (1452.1500,430.9180) .. controls
        (1452.4900,432.0630) and (1454.3000,432.0640) .. (1453.4500,433.5820);

        % path6554
        \path[country]
        (1453.7400,433.6540) .. controls (1454.4000,433.8530) and
        (1455.4200,433.7810) .. (1455.4600,434.7340) .. controls (1454.7100,434.8750)
        and (1453.9600,434.3530) .. (1453.7400,433.6540);

        % path6556
        \path[country]
        (1453.9500,443.0140) .. controls (1453.6800,442.8700) and
        (1453.4200,442.7260) .. (1453.1600,442.5820) .. controls (1453.6900,442.5220)
        and (1453.6200,442.7540) .. (1453.9500,443.0140);

        % path6558
        \path[country]
        (1455.4600,439.7020) .. controls (1454.8300,439.2080) and
        (1454.8800,438.6130) .. (1455.6100,438.2620) .. controls (1456.0400,438.7390)
        and (1455.9500,439.3140) .. (1455.4600,439.7020);

        % path6560
        \path[country]
        (1456.4000,435.9580) .. controls (1455.8500,435.2090) and
        (1456.0100,434.9920) .. (1456.9000,435.3100) .. controls (1456.7300,435.5260)
        and (1456.5600,435.7420) .. (1456.4000,435.9580);

        % path6562
        \path[country]
        (1456.8300,442.5100) .. controls (1456.5900,442.3180) and
        (1456.3500,442.1260) .. (1456.1100,441.9340) .. controls (1456.6500,441.6140)
        and (1457.1800,441.8840) .. (1456.8300,442.5100);

        % path6564
        \path[country]
        (1456.9000,409.3900) .. controls (1456.9000,409.6300) and
        (1456.9000,409.8690) .. (1456.9000,410.1100) .. controls (1456.3200,410.2230)
        and (1455.8800,409.9120) .. (1455.8200,409.3180) .. controls
        (1456.1800,409.2160) and (1456.5400,409.2380) .. (1456.9000,409.3880);

        % path6566
        \path[country]
        (1457.3300,440.2060) .. controls (1457.0600,439.8460) and
        (1456.5100,439.1780) .. (1456.7800,438.6640) .. controls (1456.9300,438.3850)
        and (1457.7100,437.7390) .. (1458.0300,437.9910) .. controls
        (1458.5900,438.4280) and (1457.8000,439.9770) .. (1457.3300,440.2060);

        % path6568
        \path[country]
        (1459.8600,441.5020) .. controls (1460.1400,440.7040) and
        (1460.9300,440.3470) .. (1461.7300,440.3500) .. controls (1461.0400,440.6310)
        and (1460.5200,441.1850) .. (1459.8600,441.5020);

        % path6570
        \path[country]
        (1460.7200,429.5500) .. controls (1459.1200,428.9340) and
        (1461.0600,427.0730) .. (1459.2800,426.3820) .. controls (1461.1600,423.9440)
        and (1462.5700,428.3880) .. (1460.7200,429.5500);

        % path6572
        \path[country]
        (1460.8600,435.0940) .. controls (1460.9600,433.7940) and
        (1462.5100,433.9870) .. (1463.3800,433.5820) .. controls (1462.9600,434.5150)
        and (1461.8200,435.0190) .. (1460.8600,435.0940);

        % path6574
        \path[country]
        (1463.1700,422.5660) .. controls (1462.3500,422.4760) and
        (1461.6100,422.0710) .. (1460.9300,421.6300) .. controls (1461.1600,421.4500)
        and (1461.4100,421.2820) .. (1461.6600,421.1260) .. controls
        (1460.9900,421.0660) and (1460.1600,421.4250) .. (1459.5700,421.0040) ..
        controls (1458.4600,420.2200) and (1459.6900,419.8600) .. (1460.4000,419.6660)
        .. controls (1462.6300,419.0620) and (1463.3200,419.9150) ..
        (1464.5300,422.0620) .. controls (1463.9500,421.7070) and (1463.4400,422.0120)
        .. (1463.1700,422.5660);

        % path6576
        \path[country]
        (1466.7000,433.9420) .. controls (1466.5700,433.8040) and
        (1463.9700,433.0380) .. (1465.5600,432.6070) .. controls (1466.4100,432.3770)
        and (1467.3100,433.0290) .. (1468.1300,432.7910) .. controls
        (1467.9000,433.4040) and (1467.3500,433.8650) .. (1466.7000,433.9420);

        % path6578
        \path[country]
        (1467.3400,438.6220) .. controls (1467.1000,438.4060) and
        (1466.8600,438.1890) .. (1466.6200,437.9740) .. controls (1467.1900,437.9740)
        and (1467.1700,438.1770) .. (1467.3400,438.6220);

        % path6580
        \path[country]
        (1468.2100,440.1340) .. controls (1467.6600,439.4320) and
        (1467.8100,439.1920) .. (1468.6400,439.4140) .. controls (1468.4900,439.6550)
        and (1468.3500,439.8940) .. (1468.2100,440.1340);

        % path6582
        \path[country]
        (1470.2200,453.3100) .. controls (1469.9300,451.9490) and
        (1469.9800,450.9350) .. (1470.5100,449.6380) .. controls (1470.7000,450.4140)
        and (1470.9300,452.8770) .. (1470.2200,453.3100);

        % path6584
        \path[country]
        (1475.4800,448.1260) .. controls (1474.7500,450.1050) and
        (1474.1300,447.8950) .. (1474.0300,447.1190) .. controls (1473.8300,445.6260)
        and (1476.0900,444.5480) .. (1477.3500,444.3090) .. controls
        (1477.5600,445.1840) and (1477.0600,446.0000) .. (1476.8200,446.8020) ..
        controls (1476.3900,448.2480) and (1476.2700,447.0480) ..
        (1475.4800,448.1260);

    \end{scope}
    
    
    % //////// HUNGARY /////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (328.7784,258.3059) .. controls (329.4584,257.5839) and
    (330.3284,256.9959) .. (331.3684,257.2259) .. controls (331.0384,256.3529) and
    (330.8084,255.1809) .. (331.0884,254.2659) .. controls (331.3284,253.4909) and
    (332.3084,253.2369) .. (332.5584,252.4539) .. controls (332.7584,251.8079) and
    (330.4284,251.5709) .. (331.7084,251.0879) .. controls (332.6884,250.7219) and
    (333.7184,252.3569) .. (334.4384,251.1479) .. controls (334.9484,250.2959) and
    (335.3984,249.1409) .. (335.8284,248.7449) .. controls (336.2484,248.3479) and
    (336.6384,248.7049) .. (337.8084,249.6149) .. controls (340.6984,251.8519) and
    (343.6284,250.7189) .. (346.9884,250.3089) .. controls (345.1284,248.8269) and
    (347.7884,248.7689) .. (348.9284,248.6589) .. controls (349.4784,248.6089) and
    (350.9184,248.1119) .. (351.0684,247.4159) .. controls (351.3084,246.2269) and
    (352.2984,247.1689) .. (353.1584,247.5059) .. controls (354.3284,247.9649) and
    (356.1684,247.4859) .. (357.0084,246.6789) .. controls (357.6284,246.0919) and
    (357.3984,244.4299) .. (358.1584,244.1259) .. controls (359.6584,243.5359) and
    (361.4684,244.3999) .. (362.9784,244.5459) .. controls (363.6284,243.5079) and
    (364.5384,244.2009) .. (365.1284,244.8049) .. controls (366.0084,245.7109) and
    (366.8784,246.0649) .. (368.0584,245.5759) .. controls (370.1084,244.7249) and
    (371.1184,247.1789) .. (373.0484,247.8639) .. controls (375.1984,248.6229) and
    (373.7184,249.7819) .. (373.1684,250.2849) .. controls (372.2684,251.1099) and
    (370.7684,250.3649) .. (370.1484,251.3249) .. controls (369.6684,252.0589) and
    (368.3584,253.0629) .. (368.3384,253.7789) .. controls (368.3384,254.5429) and
    (366.7884,257.0249) .. (365.7084,258.9279) .. controls (365.2284,259.7769) and
    (364.2384,260.5149) .. (363.9884,261.4899) .. controls (363.7984,262.2439) and
    (363.9884,262.9479) .. (362.3484,263.3729) .. controls (361.5284,263.5889) and
    (360.8284,263.1929) .. (360.2984,263.9699) .. controls (359.7084,264.8479) and
    (358.9784,264.1679) .. (358.2384,264.4119) .. controls (357.1384,264.7679) and
    (355.8684,264.4619) .. (354.7684,264.3519) .. controls (353.9884,264.2719) and
    (352.7484,263.8239) .. (352.0984,264.4419) .. controls (351.3484,265.1499) and
    (351.1284,265.7489) .. (350.0084,265.8009) .. controls (348.9784,265.8509) and
    (347.8784,265.9529) .. (346.9184,266.3529) .. controls (346.0284,266.7269) and
    (345.7784,267.6139) .. (344.7084,267.7489) .. controls (342.9284,267.9739) and
    (340.6284,267.5329) .. (339.1584,266.5999) .. controls (338.3184,266.0649) and
    (337.5284,266.1839) .. (336.8584,265.2719) .. controls (336.0284,264.1419) and
    (334.8584,263.4849) .. (333.6984,262.7239) .. controls (332.6484,262.0259) and
    (331.8184,261.4139) .. (331.1784,260.3199) .. controls (330.6584,259.4549) and
    (330.0084,258.0819) .. (328.7784,258.3009);
    
    
    % //////// IRELAND /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path5352
        \path[country]
        (1228.5900,287.2800) .. controls (1228.7300,287.3900) and
        (1228.4900,287.7560) .. (1228.7700,287.4240) .. controls (1229.0300,287.0880)
        and (1228.7700,287.3940) .. (1228.5900,287.2800);

        % path5348
        \path[country]
        (1218.1500,296.2800) .. controls (1219.3100,295.7820) and
        (1217.1900,295.4100) .. (1216.6400,295.7040) .. controls (1217.2200,295.7040)
        and (1217.7200,295.8870) .. (1218.1500,296.2800);

        % path5402
        \path[country]
        (1215.7800,315.2900) .. controls (1215.5400,315.3100) and (1215.3000,315.3400)
        .. (1215.0600,315.3600) .. controls (1216.0100,314.5010) and
        (1217.0200,313.4400) .. (1218.3700,313.2720) .. controls (1217.1100,313.0600)
        and (1215.0300,314.8400) .. (1213.8800,313.8650) .. controls
        (1212.5900,312.7690) and (1216.8000,310.6860) .. (1217.6500,310.9680) ..
        controls (1216.3900,310.4060) and (1214.6700,310.8880) .. (1213.4000,311.1840)
        .. controls (1213.0600,310.1680) and (1214.1300,310.0110) ..
        (1214.8700,309.9140) .. controls (1215.2600,309.8640) and (1215.7000,309.8340)
        .. (1216.0500,309.6470) .. controls (1216.3800,309.4690) and
        (1217.0900,310.1070) .. (1217.8600,309.9600) .. controls (1217.6900,309.4090)
        and (1217.4200,308.9050) .. (1217.0700,308.4470) .. controls
        (1218.4400,308.4470) and (1218.8500,307.1960) .. (1220.2800,307.2160) ..
        controls (1221.9400,307.2360) and (1223.4300,306.5820) .. (1225.0600,306.4320)
        .. controls (1224.5100,306.4120) and (1224.0300,306.0880) ..
        (1223.8400,305.5680) .. controls (1221.7500,306.9090) and (1220.1500,306.8600)
        .. (1217.7200,307.2970) .. controls (1218.3800,306.8330) and
        (1221.6700,305.2090) .. (1221.2600,304.1170) .. controls (1220.6800,302.5590)
        and (1223.8800,302.5980) .. (1224.5600,301.8960) .. controls
        (1223.3100,301.8160) and (1222.1300,301.7730) .. (1220.8800,301.7830) ..
        controls (1220.2700,301.7830) and (1219.2200,301.1290) .. (1218.4400,301.0320)
        .. controls (1218.5800,300.7910) and (1218.7200,300.5520) ..
        (1218.8700,300.3120) .. controls (1218.1400,300.0930) and (1217.5700,300.7920)
        .. (1216.8600,300.3820) .. controls (1217.1000,300.2190) and
        (1217.3400,300.0510) .. (1217.5800,299.8780) .. controls (1217.3400,299.7080)
        and (1217.1000,299.5400) .. (1216.8600,299.3740) .. controls
        (1217.7100,299.2360) and (1217.3800,299.1350) .. (1217.9800,298.7530) ..
        controls (1218.4700,298.4440) and (1219.2100,298.7830) .. (1219.7400,298.7230)
        .. controls (1218.9900,298.8230) and (1218.1500,298.1600) ..
        (1218.9700,297.5040) .. controls (1219.3100,297.2340) and (1220.0300,297.2870)
        .. (1220.4300,297.1570) .. controls (1222.4500,296.5040) and
        (1218.5000,296.2460) .. (1218.6700,296.5070) .. controls (1218.4000,296.1020)
        and (1219.2900,296.0810) .. (1219.4500,296.2040) .. controls
        (1218.9900,295.4640) and (1219.7500,294.2370) .. (1218.5100,294.9070) ..
        controls (1218.8500,294.4760) and (1218.8200,294.0680) .. (1218.4100,293.6830)
        .. controls (1218.2000,293.9080) and (1218.0000,294.1480) ..
        (1217.8300,294.4030) .. controls (1217.9400,293.8770) and (1218.1600,293.3970)
        .. (1218.4800,292.9640) .. controls (1218.5900,294.0980) and
        (1220.1700,292.9140) .. (1221.3100,292.8390) .. controls (1222.3800,292.7690)
        and (1223.7500,293.0420) .. (1223.8800,294.3320) .. controls
        (1224.4200,291.9790) and (1226.8900,294.3820) .. (1228.1300,293.1800) ..
        controls (1227.8600,293.0430) and (1227.6000,292.8990) .. (1227.3400,292.7480)
        .. controls (1228.1300,291.7110) and (1230.3100,291.8160) ..
        (1230.5000,290.5880) .. controls (1229.2800,290.3510) and (1227.9600,290.7330)
        .. (1226.8300,290.0840) .. controls (1227.0900,289.2300) and
        (1228.0100,289.0070) .. (1228.7800,289.2920) .. controls (1228.4900,288.6680)
        and (1228.4700,288.2420) .. (1229.4200,288.5730) .. controls
        (1228.8400,287.8140) and (1229.4200,286.5770) .. (1230.1800,286.1780) ..
        controls (1231.5100,285.4660) and (1232.6900,286.0690) .. (1233.9600,285.9070)
        .. controls (1233.3800,284.9030) and (1234.3400,284.8200) ..
        (1234.6600,285.3930) .. controls (1235.2400,286.4130) and (1234.6600,286.4090)
        .. (1234.3900,287.2760) .. controls (1235.4800,287.2960) and
        (1235.9100,286.1210) .. (1235.1100,285.4030) .. controls (1236.6800,284.3130)
        and (1237.2600,284.9060) .. (1238.7900,285.1870) .. controls
        (1237.9600,286.1130) and (1236.1300,286.3160) .. (1235.7200,287.5990) ..
        controls (1235.3600,288.7280) and (1234.0100,290.2870) .. (1232.5200,289.6510)
        .. controls (1232.8100,289.9360) and (1233.1300,290.2010) ..
        (1233.4600,290.4440) .. controls (1232.1400,291.2730) and (1229.9000,291.0760)
        .. (1231.6300,292.6680) .. controls (1232.3900,293.3630) and
        (1233.4900,293.7790) .. (1234.3800,294.0630) .. controls (1235.2300,294.3320)
        and (1235.8900,294.6570) .. (1236.2900,293.3070) .. controls
        (1236.5000,292.5930) and (1236.1900,291.9120) .. (1237.7500,292.3030) ..
        controls (1238.7900,292.5650) and (1239.2800,293.8070) .. (1239.8600,293.9700)
        .. controls (1239.8600,295.3720) and (1240.8100,294.9770) ..
        (1241.5200,294.9060) .. controls (1242.1500,294.8460) and (1242.1300,294.3480)
        .. (1243.0300,295.1950) .. controls (1242.5300,295.4500) and
        (1241.9000,295.4730) .. (1241.4600,295.8640) .. controls (1241.3200,295.9930)
        and (1242.1100,296.9990) .. (1242.0400,297.5540) .. controls
        (1241.9400,298.3340) and (1243.9200,300.3570) .. (1241.9400,300.7380) ..
        controls (1243.2600,302.7660) and (1242.6900,303.9750) .. (1241.8400,306.0050)
        .. controls (1241.4200,307.0580) and (1240.8200,309.1910) ..
        (1239.3200,309.0180) .. controls (1240.9600,309.2410) and (1239.8800,310.6410)
        .. (1238.6800,310.4210) .. controls (1237.7300,310.2450) and
        (1236.2600,311.0080) .. (1236.0100,309.5940) .. controls (1236.6300,311.4420)
        and (1233.2200,310.7510) .. (1232.2700,311.0870) .. controls
        (1231.3900,311.4000) and (1231.9700,312.2440) .. (1230.5900,312.2440) ..
        controls (1229.5200,312.2440) and (1228.9800,313.7210) .. (1227.5900,313.6260)
        .. controls (1228.4200,312.4060) and (1226.9100,312.7430) ..
        (1226.2900,312.9780) .. controls (1227.4000,313.2950) and (1227.0200,313.8250)
        .. (1226.2900,314.2470) .. controls (1225.9600,314.3770) and
        (1225.7000,314.5820) .. (1225.4900,314.8630) .. controls (1225.2400,315.3550)
        and (1224.8200,314.9230) .. (1224.3700,315.1100) .. controls
        (1223.3100,315.5430) and (1222.1800,315.5250) .. (1221.0800,315.8810) ..
        controls (1219.8500,316.2780) and (1218.4400,315.8810) .. (1217.2900,316.4340)
        .. controls (1217.6000,315.9120) and (1218.0300,315.5280) ..
        (1218.5900,315.2830) .. controls (1218.0600,315.3630) and (1217.5500,315.5030)
        .. (1217.0700,315.7150) .. controls (1217.7000,315.1470) and
        (1218.4900,314.8580) .. (1219.3000,314.6350) .. controls (1218.3600,314.1370)
        and (1216.5100,314.6950) .. (1215.7100,315.2840);

    \end{scope}
    
    
    % //////// ITALY ///////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]

        % path2906
        \path[country]
        (1323.6900,369.5990) .. controls (1324.7000,368.5240) and (1327.3600,369.4320)
        .. (1327.2400,367.1950) .. controls (1327.2400,366.2930) and
        (1326.5300,365.8970) .. (1325.9600,365.2790) .. controls (1325.6500,364.9600)
        and (1325.2900,364.5920) .. (1325.0200,364.2370) .. controls
        (1325.8700,363.7540) and (1326.7200,362.6880) .. (1326.2000,362.1100) ..
        controls (1327.1000,362.3500) and (1328.0900,363.2260) .. (1329.0600,362.8890)
        .. controls (1330.2800,362.4650) and (1330.8300,362.6700) ..
        (1331.9900,362.7570) .. controls (1332.7600,362.8170) and (1333.6900,361.8880)
        .. (1334.0400,361.2960) .. controls (1334.3200,360.8420) and
        (1334.3600,360.4390) .. (1334.0400,360.0190) .. controls (1334.8600,359.7970)
        and (1335.4700,359.1480) .. (1335.9800,358.5060) .. controls
        (1336.8700,359.0580) and (1336.5200,359.7790) .. (1337.0100,360.5610) ..
        controls (1337.4700,361.3070) and (1338.1800,361.5070) .. (1338.8200,362.1260)
        .. controls (1339.0700,362.3650) and (1339.1300,363.0790) ..
        (1340.0700,363.6570) .. controls (1340.3700,363.8430) and (1340.2400,361.8040)
        .. (1340.9100,361.1810) .. controls (1341.6600,360.4730) and
        (1341.9100,360.0130) .. (1342.0000,358.8640) .. controls (1342.1700,356.9050)
        and (1342.8200,358.2950) .. (1343.2500,358.7590) .. controls
        (1343.9900,359.5360) and (1344.2500,359.6520) .. (1345.1800,359.3350) ..
        controls (1346.6800,358.8210) and (1346.6800,359.9240) .. (1347.7200,360.4500)
        .. controls (1347.8200,359.7910) and (1348.3300,359.1250) ..
        (1347.4900,358.7430) .. controls (1346.7400,358.4010) and (1347.7400,357.0550)
        .. (1348.2200,356.9590) .. controls (1348.6900,356.8590) and
        (1349.2100,357.5650) .. (1349.6600,357.6860) .. controls (1350.6300,357.9530)
        and (1349.7600,356.3650) .. (1349.8200,356.0450) .. controls
        (1350.0100,355.4230) and (1350.1000,355.2180) .. (1350.2000,354.9300) ..
        controls (1350.8300,354.9900) and (1352.4100,355.4760) .. (1352.7700,355.6620)
        .. controls (1353.7300,356.1510) and (1354.3800,354.8930) ..
        (1354.9400,354.3910) .. controls (1355.6800,353.7220) and (1356.8500,353.9120)
        .. (1357.7600,353.9650) .. controls (1359.2200,354.0550) and
        (1360.6300,352.9530) .. (1362.0500,353.2490) .. controls (1360.4700,354.1920)
        and (1363.6700,356.6490) .. (1364.5500,356.9300) .. controls
        (1367.2100,357.7740) and (1369.0800,356.9300) .. (1371.7400,357.6940) ..
        controls (1371.6300,358.7010) and (1370.5500,359.3910) .. (1370.0400,360.0180)
        .. controls (1370.6300,360.3550) and (1371.2300,360.7310) ..
        (1371.9100,360.8820) .. controls (1371.3300,361.5580) and (1370.4500,362.5330)
        .. (1371.7000,362.8980) .. controls (1370.9600,363.8610) and
        (1372.1600,364.2220) .. (1372.5600,364.3020) .. controls (1373.5100,364.4910)
        and (1373.7800,366.0570) .. (1372.3400,365.7780) .. controls
        (1373.3400,363.7010) and (1370.6200,364.8670) .. (1370.1100,365.0580) ..
        controls (1369.8900,363.6250) and (1368.1500,364.9300) .. (1367.6400,365.2480)
        .. controls (1367.0900,365.5970) and (1366.5100,365.9200) ..
        (1365.9200,366.2140) .. controls (1365.5300,366.4090) and (1362.2400,367.4730)
        .. (1364.2800,366.4240) .. controls (1363.7300,366.5370) and
        (1363.0000,366.4640) .. (1362.5500,366.8570) .. controls (1362.2200,367.1360)
        and (1362.3800,368.2870) .. (1361.7600,368.1530) .. controls
        (1361.7600,368.4860) and (1362.9800,370.1970) .. (1363.1000,370.2300) ..
        controls (1364.9200,370.7320) and (1363.7700,373.3850) .. (1362.7000,372.1850)
        .. controls (1360.6100,375.8710) and (1365.2900,379.3730) ..
        (1367.8200,380.9840) .. controls (1369.0600,381.7730) and (1371.0600,382.3280)
        .. (1371.9200,383.5650) .. controls (1373.1900,385.3660) and
        (1373.8600,387.7350) .. (1374.6000,389.7900) .. controls (1375.5500,392.4280)
        and (1379.0100,395.1270) .. (1381.4800,396.2610) .. controls
        (1383.3100,397.1010) and (1384.2800,397.3600) .. (1386.3100,397.0880) ..
        controls (1387.0700,396.9870) and (1390.4200,396.4940) .. (1390.0100,398.2330)
        .. controls (1389.8100,399.0630) and (1387.4400,399.8350) ..
        (1388.3000,400.8500) .. controls (1389.2400,401.9450) and (1391.7300,402.5680)
        .. (1393.0000,403.0220) .. controls (1395.0300,403.7470) and
        (1396.8600,404.4640) .. (1398.5500,405.8180) .. controls (1400.2900,407.1990)
        and (1402.4200,407.6090) .. (1404.1100,409.1340) .. controls
        (1405.2400,410.1590) and (1406.7600,411.2330) .. (1406.4700,412.9410) ..
        controls (1406.3700,413.3290) and (1406.3300,415.0750) .. (1405.7500,415.1330)
        .. controls (1404.9500,415.2130) and (1403.9700,414.7400) ..
        (1403.5500,414.0500) .. controls (1402.6300,412.5440) and (1402.6900,410.8000)
        .. (1400.4200,411.0290) .. controls (1398.5900,411.2130) and
        (1398.2200,410.0200) .. (1397.9700,409.3370) .. controls (1396.0400,409.6620)
        and (1395.6100,409.6430) .. (1394.4000,411.4350) .. controls
        (1393.6500,412.5460) and (1393.1000,413.9400) .. (1392.8300,415.2550) ..
        controls (1392.5100,416.7620) and (1394.4300,417.1290) .. (1395.4700,417.6070)
        .. controls (1397.1400,418.3740) and (1397.4400,419.5670) ..
        (1397.6100,421.2550) .. controls (1397.8800,424.1050) and (1392.9500,422.0560)
        .. (1393.4200,425.4970) .. controls (1393.6400,427.1800) and
        (1393.1900,427.3120) .. (1392.1100,428.4550) .. controls (1391.2000,429.4230)
        and (1390.5000,430.6170) .. (1389.4200,431.4110) .. controls
        (1388.4000,432.1580) and (1387.5400,431.7380) .. (1387.0300,430.6490) ..
        controls (1386.2500,428.9910) and (1388.6600,428.2220) .. (1388.7800,426.7140)
        .. controls (1388.7800,426.2020) and (1388.5700,425.5850) ..
        (1388.9200,425.1280) .. controls (1389.5100,424.3640) and (1390.6700,424.9350)
        .. (1390.9900,423.9520) .. controls (1391.2600,423.0960) and
        (1390.1800,422.1250) .. (1389.9700,421.3430) .. controls (1389.6500,420.1280)
        and (1389.5400,419.0600) .. (1388.8800,417.9500) .. controls
        (1388.1000,416.6200) and (1387.9800,414.6270) .. (1386.9400,413.5030) ..
        controls (1386.3100,412.8340) and (1385.8800,412.9930) .. (1385.2900,413.4830)
        .. controls (1384.5900,414.0680) and (1383.8600,412.8800) ..
        (1383.4000,412.5100) .. controls (1382.8800,412.0920) and (1382.0300,412.2020)
        .. (1381.8700,411.3610) .. controls (1381.7400,410.6680) and
        (1382.1900,410.4610) .. (1381.8700,409.6090) .. controls (1381.0700,407.7700)
        and (1379.0000,407.7270) .. (1377.4900,408.6890) .. controls
        (1378.2600,407.5100) and (1378.0200,406.4040) .. (1376.4200,406.5650) ..
        controls (1375.2300,406.6840) and (1374.5500,404.9250) .. (1374.1200,404.1030)
        .. controls (1373.3600,402.6420) and (1372.4500,403.4920) ..
        (1371.2000,403.1240) .. controls (1370.5300,402.9280) and (1369.9100,402.6140)
        .. (1369.1900,402.7850) .. controls (1367.6900,403.1420) and
        (1368.6600,402.9440) .. (1367.6200,402.0990) .. controls (1366.5900,401.2620)
        and (1365.3000,401.0320) .. (1364.2800,400.1080) .. controls
        (1363.1400,399.0830) and (1362.4800,397.5670) .. (1361.2400,396.7020) ..
        controls (1360.1600,395.9500) and (1359.7400,396.1410) .. (1359.0200,394.9670)
        .. controls (1358.2800,393.7410) and (1356.3500,392.3010) ..
        (1354.8900,393.2090) .. controls (1355.7300,391.8020) and (1352.3000,388.1700)
        .. (1351.0300,388.3500) .. controls (1351.1800,388.3300) and
        (1349.1600,382.5930) .. (1349.0800,382.2200) .. controls (1348.3900,378.8430)
        and (1346.0900,379.2200) .. (1343.6600,377.5850) .. controls
        (1341.1500,375.8940) and (1337.9500,374.9750) .. (1335.8500,377.7040) ..
        controls (1335.1000,378.6730) and (1334.4800,379.7910) .. (1333.3600,380.3930)
        .. controls (1332.9600,380.6070) and (1329.3500,381.7540) ..
        (1329.6000,380.8280) .. controls (1329.7800,380.1480) and (1332.4800,377.1530)
        .. (1329.2600,378.2900) .. controls (1327.3400,378.9700) and
        (1323.7200,375.9380) .. (1326.1000,373.9700) .. controls (1326.9600,373.2640)
        and (1326.8000,372.6800) .. (1325.7900,372.1690) .. controls
        (1324.1200,371.3260) and (1323.6400,370.0440) .. (1323.8600,369.9560);

        % path2910
        \path[country]
        (1335.6000,409.9870) .. controls (1335.3500,409.4120) and
        (1334.8600,409.0470) .. (1334.5200,408.5420) .. controls (1333.8800,407.6110)
        and (1334.3800,406.7390) .. (1334.2400,405.7390) .. controls
        (1336.1400,407.8850) and (1338.5800,405.3180) .. (1340.0700,404.0350) ..
        controls (1340.6100,403.5700) and (1341.3700,402.7700) .. (1342.1500,403.2640)
        .. controls (1342.6600,403.5870) and (1343.0100,404.4480) ..
        (1343.7400,404.0820) .. controls (1343.4800,404.6410) and (1343.7400,404.9880)
        .. (1344.3100,405.0190) .. controls (1344.0700,405.2130) and
        (1343.8400,405.4060) .. (1343.6000,405.5960) .. controls (1345.0700,405.5360)
        and (1345.7000,408.9610) .. (1345.3900,409.9870) .. controls
        (1345.1200,410.8810) and (1343.7800,411.3600) .. (1344.6100,412.4060) ..
        controls (1345.4300,413.4440) and (1344.7100,416.0840) .. (1344.6100,417.3360)
        .. controls (1344.6100,418.2740) and (1344.6100,420.2160) ..
        (1343.7100,420.8070) .. controls (1342.8500,421.3530) and (1341.4100,420.2690)
        .. (1340.4500,420.3550) .. controls (1339.9500,421.1190) and
        (1340.1200,423.2350) .. (1338.6300,422.9860) .. controls (1337.2200,422.7490)
        and (1337.1900,423.1250) .. (1336.4900,421.7230) .. controls
        (1336.3000,421.9640) and (1336.1000,422.2040) .. (1335.9100,422.4430) ..
        controls (1335.6700,422.2400) and (1335.4800,422.0000) .. (1335.3300,421.7230)
        .. controls (1336.5800,421.4730) and (1335.7900,420.6890) ..
        (1335.7500,419.6170) .. controls (1335.7500,418.2980) and (1335.8900,416.9870)
        .. (1335.9800,415.6750) .. controls (1336.2200,415.8650) and
        (1336.4600,416.0580) .. (1336.7000,416.2510) .. controls (1336.7000,415.7970)
        and (1336.8900,415.3190) .. (1336.7000,414.8680) .. controls
        (1336.5400,414.3780) and (1335.8100,414.5560) .. (1335.7100,413.9720) ..
        controls (1335.6100,413.4470) and (1336.2600,412.7420) .. (1336.2500,412.1390)
        .. controls (1336.2500,411.3520) and (1335.3900,410.7260) ..
        (1335.5700,409.9870);

        % path2912
        \path[country]
        (1349.8600,390.4030) .. controls (1349.1500,389.9690) and
        (1348.3100,390.3530) .. (1347.6300,389.8270) .. controls (1348.3600,389.4870)
        and (1349.2100,389.5660) .. (1349.8600,389.0350) .. controls
        (1349.9600,389.4910) and (1349.9600,389.9470) .. (1349.8600,390.4030);

        % path2920
        \path[country]
        (1367.2100,434.5390) .. controls (1366.3300,434.5090) and
        (1365.0600,434.2350) .. (1364.5200,433.4670) .. controls (1363.3500,431.8000)
        and (1365.7300,430.5520) .. (1366.2700,429.4990) .. controls
        (1367.3400,431.0620) and (1368.0400,430.1690) .. (1369.2800,429.4790) ..
        controls (1371.1800,428.4240) and (1372.5300,431.3330) .. (1374.7100,430.8720)
        .. controls (1375.9600,430.6070) and (1377.2000,430.8220) ..
        (1378.4600,430.5920) .. controls (1379.6200,430.3830) and (1380.7000,429.2000)
        .. (1381.8300,429.2090) .. controls (1382.8300,429.2090) and
        (1383.0200,429.9550) .. (1383.9700,429.2790) .. controls (1384.5900,428.8430)
        and (1386.2800,428.0610) .. (1387.0100,428.4840) .. controls
        (1386.0900,429.6290) and (1385.1800,430.9920) .. (1384.5900,432.3440) ..
        controls (1384.1900,433.2860) and (1382.9800,435.1730) .. (1383.2500,436.1950)
        .. controls (1383.4900,437.0880) and (1385.1000,438.4240) ..
        (1384.6000,439.4330) .. controls (1384.1900,440.2860) and (1383.0600,440.9280)
        .. (1383.6300,442.0200) .. controls (1382.4900,442.2860) and
        (1381.1200,442.1690) .. (1380.0100,441.8280) .. controls (1378.4500,441.3480)
        and (1378.5300,439.5140) .. (1377.0200,438.8950) .. controls
        (1375.4200,438.2410) and (1373.7200,438.1530) .. (1372.1700,437.2930) ..
        controls (1370.5800,436.4140) and (1369.1500,434.5750) ..
        (1367.2100,434.5320);

    \end{scope}
    
    
    % //////// LATVIA //////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (356.7784,178.3139) .. controls (356.8784,178.5539) and
    (356.9684,178.7929) .. (357.0684,179.0339) .. controls (356.9684,177.7839) and
    (356.6784,176.4669) .. (357.5484,175.4059) .. controls (357.9284,174.9509) and
    (358.5984,174.6289) .. (358.7584,174.0139) .. controls (358.9484,173.2419) and
    (358.7584,172.5739) .. (359.1384,171.8119) .. controls (359.9284,170.3409) and
    (360.8984,169.6649) .. (362.4784,169.2739) .. controls (363.2484,169.0859) and
    (365.2984,167.8619) .. (365.8984,168.5929) .. controls (366.8484,169.7529) and
    (367.8884,170.2579) .. (368.9684,171.2519) .. controls (370.1984,172.3809) and
    (370.6984,173.8779) .. (372.4284,174.4289) .. controls (373.7784,174.8639) and
    (375.1084,174.2959) .. (376.2184,173.5099) .. controls (377.8184,172.3719) and
    (377.5884,171.0079) .. (376.9084,169.3739) .. controls (376.6384,168.7279) and
    (376.3584,168.0159) .. (376.5084,167.2979) .. controls (377.1184,167.4719) and
    (377.7384,167.0279) .. (378.2184,166.7449) .. controls (379.1884,166.1829) and
    (381.0584,165.3759) .. (382.0784,166.0219) .. controls (382.7484,166.4499) and
    (384.0484,166.3269) .. (384.9284,166.8159) .. controls (386.2484,167.5449) and
    (387.3584,167.7459) .. (388.5284,168.8029) .. controls (389.4784,169.6669) and
    (390.3684,170.1819) .. (391.5784,169.5639) .. controls (392.9384,168.8749) and
    (394.4484,169.9089) .. (395.8784,169.9589) .. controls (396.8784,169.9989) and
    (399.5284,172.1229) .. (399.3284,172.9219) .. controls (399.2084,173.3609) and
    (398.6084,175.0809) .. (398.2584,175.4329) .. controls (400.3984,175.1739) and
    (399.5484,176.0569) .. (400.4884,176.4139) .. controls (401.5984,176.8339) and
    (402.6184,180.6809) .. (402.8184,181.7239) .. controls (402.3784,181.9219) and
    (401.6784,181.2209) .. (400.9084,181.6159) .. controls (400.3184,181.9159) and
    (399.8384,182.6649) .. (399.4684,183.1829) .. controls (399.2484,183.4749) and
    (399.3384,183.9469) .. (398.9784,184.1439) .. controls (397.8284,184.7749) and
    (396.3884,183.4179) .. (395.0984,184.0639) .. controls (393.6184,184.8109) and
    (392.9284,185.5559) .. (391.1984,184.5999) .. controls (389.7784,183.8139) and
    (388.4984,182.7949) .. (387.1584,181.8789) .. controls (385.8784,180.9949) and
    (384.2484,181.4419) .. (382.9784,180.6449) .. controls (381.8784,179.9479) and
    (381.6484,178.4519) .. (380.1484,179.3379) .. controls (378.8384,180.1079) and
    (378.3884,180.0779) .. (376.9484,180.2179) .. controls (375.6584,180.3429) and
    (374.1184,179.4999) .. (372.7084,179.5209) .. controls (371.2484,179.5409) and
    (371.0284,179.7889) .. (369.5984,179.2959) .. controls (368.7384,178.9979) and
    (366.4784,179.2359) .. (365.5484,179.2359) .. controls (364.0884,179.2359) and
    (362.7984,179.4689) .. (361.3984,179.8099) .. controls (360.4984,180.0259) and
    (359.0784,180.2319) .. (358.6884,181.2319) .. controls (358.4384,181.8889) and
    (357.6984,182.2169) .. (357.2484,181.6609) .. controls (356.4584,180.6969) and
    (356.6984,179.4629) .. (356.7784,178.3129);
    
    
    % //////// LIECHTENSTEIN ///////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}, country, we]
    
        \path[fill]
        (1343.3600,353.3740) .. controls (1343.3600,352.7460) and (1343.5200,352.1460)
        .. (1343.7900,351.5750) .. controls (1344.2500,352.2200) and
        (1344.7300,353.6670) .. (1343.3600,353.3740);

    \end{scope}
    
    
    % //////// LITHUANIA ///////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (357.2884,181.8409) .. controls (358.3084,182.0049) and
    (358.5484,180.9449) .. (359.2284,180.4739) .. controls (359.9784,179.9599) and
    (361.2984,179.7909) .. (362.1584,179.5899) .. controls (364.3984,179.0679) and
    (367.0184,179.0469) .. (369.3084,179.1769) .. controls (370.6584,179.7689) and
    (372.3184,179.2569) .. (373.5484,179.6169) .. controls (375.0384,179.7439) and
    (378.2084,180.4279) .. (379.6384,179.5029) .. controls (381.5884,178.2389) and
    (381.6684,179.6129) .. (382.8784,180.5729) .. controls (383.6084,181.1559) and
    (384.5684,181.0469) .. (385.4584,181.1809) .. controls (386.6584,181.3599) and
    (387.7284,181.8679) .. (388.4984,182.7449) .. controls (388.9884,183.2929) and
    (392.0484,185.3129) .. (392.7384,184.9399) .. controls (392.2484,187.0969) and
    (392.4184,187.6569) .. (394.3684,188.1769) .. controls (393.1684,188.7649) and
    (394.0484,189.7539) .. (392.3784,189.4249) .. controls (391.0984,189.1719) and
    (390.9484,190.3889) .. (390.0184,190.9299) .. controls (387.7284,192.2499) and
    (389.0784,193.8419) .. (387.1684,195.8819) .. controls (387.6484,196.0779) and
    (388.6184,196.1569) .. (388.7484,196.8169) .. controls (388.8984,197.6129) and
    (387.8384,197.7809) .. (387.3084,197.6089) .. controls (387.8584,196.1339) and
    (385.5884,196.5739) .. (385.4684,196.8709) .. controls (384.8984,198.2489) and
    (383.1584,197.2719) .. (382.4884,198.6649) .. controls (382.2584,199.1509) and
    (381.0484,199.1579) .. (380.5384,199.4399) .. controls (379.6684,199.9159) and
    (378.0584,199.3899) .. (377.0884,199.4799) .. controls (376.6084,199.5199) and
    (374.4684,199.8119) .. (374.3084,198.9999) .. controls (374.1084,198.0349) and
    (373.1284,196.7159) .. (372.1884,196.2899) .. controls (370.8884,192.8649) and
    (371.8284,193.1379) .. (372.3384,191.7929) .. controls (372.4384,191.5109) and
    (370.5184,189.9829) .. (370.1984,189.9749) .. controls (369.4284,189.9549) and
    (365.4284,190.1899) .. (364.1484,189.1639) .. controls (362.7384,188.0459) and
    (360.7584,187.6609) .. (360.5084,188.7599) .. controls (360.5084,187.6929) and
    (358.7984,186.3019) .. (358.2584,185.3959) .. controls (357.5884,184.2889) and
    (357.6884,183.0299) .. (357.2884,181.8409);
    
    
    % //////// LUXEMBURG ///////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]

        \path[country, we, neighbor]
        (1318.7500,329.5800) .. controls (1318.7500,329.3620) and (1319.3000,329.7060)
        .. (1318.7500,329.5600) .. controls (1319.2300,328.2930) and
        (1319.3400,327.7700) .. (1320.3200,327.4510) .. controls (1321.4400,327.0860)
        and (1321.0200,328.1320) .. (1321.4000,328.7140) .. controls
        (1321.9000,329.4940) and (1322.9600,329.7520) .. (1323.5300,330.4830) ..
        controls (1324.1500,331.2760) and (1323.0300,332.4760) .. (1323.1400,333.3920)
        .. controls (1322.4400,333.0500) and (1319.6700,333.0200) ..
        (1318.7300,332.7260) .. controls (1320.0100,331.8450) and (1319.1600,331.1040)
        .. (1318.7300,330.1510);

    \end{scope}
    
    
    % //////// MACEDONIA ///////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (360.5284,303.5939) .. controls (361.4284,303.4619) and
    (360.8284,302.7319) .. (360.8184,302.1939) .. controls (360.8184,301.4469) and
    (362.1184,301.0729) .. (362.3084,300.1569) .. controls (362.4584,299.3579) and
    (363.1384,298.9669) .. (363.8084,298.6449) .. controls (365.2884,297.9349) and
    (365.0184,298.8699) .. (366.3584,298.9139) .. controls (366.0684,297.8299) and
    (366.8384,298.2339) .. (367.3684,297.6899) .. controls (367.6784,297.5349) and
    (367.9784,297.5399) .. (368.2884,297.7099) .. controls (369.0284,297.9229) and
    (369.0984,297.2269) .. (369.7384,297.1179) .. controls (370.4584,296.9949) and
    (371.9484,297.2819) .. (372.5284,296.8429) .. controls (373.2584,296.2899) and
    (374.0384,297.9189) .. (374.4984,298.3419) .. controls (376.2084,299.9169) and
    (377.6984,300.3839) .. (377.6884,303.1559) .. controls (377.6884,303.7339) and
    (378.0784,304.6919) .. (377.7884,305.3489) .. controls (377.5984,305.7239) and
    (376.8984,305.2989) .. (376.9584,305.9299) .. controls (377.0584,306.8069) and
    (375.3684,307.4139) .. (374.3684,307.1129) .. controls (373.2384,306.7759) and
    (372.1084,307.0629) .. (371.1384,307.7669) .. controls (369.2184,309.1639) and
    (367.6984,309.1709) .. (365.3384,309.5489) .. controls (364.0784,309.7519) and
    (364.6184,308.8819) .. (363.5484,309.1549) .. controls (362.2384,309.4909) and
    (362.8784,308.3529) .. (362.1884,307.8149) .. controls (360.7984,306.7329) and
    (361.1284,305.1379) .. (360.5784,303.5979);
    
    
    % //////// MOLDOVA /////////////////////////////////////////////////////////////////////////////

    \begin{scope}[shift={(-1072.0076,-94.98601)}]

        \path[country]
        (1458.5600,343.2940) .. controls (1459.2500,342.8900) and (1459.2100,343.1900)
        .. (1459.4900,342.5290) .. controls (1459.6800,342.0830) and
        (1460.4000,342.1350) .. (1460.7700,342.1590) .. controls (1461.8700,342.2290)
        and (1463.2100,342.3230) .. (1464.1700,341.6010) .. controls
        (1466.1700,340.1030) and (1467.6900,344.9270) .. (1469.7400,343.9620) ..
        controls (1469.9800,345.2080) and (1470.7800,343.6340) .. (1471.0100,344.9260)
        .. controls (1471.2700,343.6890) and (1472.5300,344.1860) ..
        (1473.1200,344.8760) .. controls (1473.4100,345.2150) and (1474.1800,346.1590)
        .. (1474.5700,345.7860) .. controls (1475.1800,345.1980) and
        (1475.3100,346.0030) .. (1475.7700,346.6090) .. controls (1476.8900,348.0710)
        and (1476.3700,348.4640) .. (1477.4100,349.8090) .. controls
        (1477.7300,350.1660) and (1477.6500,351.0520) .. (1477.9900,351.3860) ..
        controls (1478.3900,351.8330) and (1478.5000,350.8350) .. (1478.8900,351.3160)
        .. controls (1479.6400,352.2520) and (1477.9100,355.3320) ..
        (1478.3000,354.0780) .. controls (1478.9800,351.8390) and (1484.0300,356.9370)
        .. (1481.8900,357.6960) .. controls (1482.5500,357.9700) and
        (1482.6600,358.6330) .. (1483.3600,358.8480) .. controls (1481.7500,360.5520)
        and (1478.7800,356.8480) .. (1477.7100,359.0640) .. controls
        (1477.5300,358.6360) and (1477.3600,358.2050) .. (1477.2100,357.7680) ..
        controls (1474.6200,358.7090) and (1476.7200,360.6120) .. (1475.3000,362.4950)
        .. controls (1474.4700,363.5840) and (1473.9500,364.3560) ..
        (1473.3900,365.5450) .. controls (1473.2600,365.8030) and (1473.2900,366.3680)
        .. (1472.9500,366.4610) .. controls (1472.4300,366.5920) and
        (1471.4600,366.1400) .. (1471.3700,367.0570) .. controls (1470.4100,366.2370)
        and (1470.7500,365.8380) .. (1470.3800,364.8140) .. controls
        (1469.2700,361.6960) and (1470.8500,359.6930) .. (1470.4800,357.5480) ..
        controls (1470.2300,356.2240) and (1468.6200,353.7640) .. (1467.7400,352.9600)
        .. controls (1465.7200,351.1010) and (1464.6700,349.9760) ..
        (1463.2700,347.5800) .. controls (1462.1400,345.6670) and (1461.1300,343.4300)
        .. (1458.6000,343.2980);
    
    \end{scope}
    
    
    % //////// MONTENEGRO //////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        \path[country]
        (1405.7100,391.6060) .. controls (1407.5900,391.2960) and (1403.8200,387.0850)
        .. (1406.7900,387.7180) .. controls (1405.9400,386.1960) and
        (1408.6100,383.8600) .. (1409.1700,385.7020) .. controls (1409.5700,384.7450)
        and (1408.4500,384.3770) .. (1408.5900,383.4700) .. controls
        (1409.7900,383.8680) and (1410.1000,384.5910) .. (1411.1100,385.4670) ..
        controls (1412.4900,386.6580) and (1412.9200,387.2010) .. (1414.5500,388.0220)
        .. controls (1415.1800,388.3420) and (1417.0500,388.1300) ..
        (1417.4400,388.8220) .. controls (1418.0400,389.8780) and (1416.4800,389.8010)
        .. (1416.3200,389.9350) .. controls (1415.8200,390.3420) and
        (1417.6300,391.4330) .. (1416.7200,391.8930) .. controls (1416.1100,392.2050)
        and (1415.3600,392.5960) .. (1414.8400,391.8630) .. controls
        (1414.5600,391.4630) and (1414.3600,390.6240) .. (1413.7300,391.3440) ..
        controls (1412.1100,393.1750) and (1411.5600,395.2090) .. (1412.3300,397.5810)
        .. controls (1411.1600,396.9150) and (1409.9400,395.7240) ..
        (1409.1600,394.6390) .. controls (1408.9200,394.3070) and (1406.9200,392.6330)
        .. (1406.5100,392.6890) .. controls (1407.2200,392.3730) and
        (1407.0700,392.4340) .. (1407.8700,392.8290) .. controls (1407.9700,391.6110)
        and (1405.3500,393.6480) .. (1405.7100,391.6060);

    \end{scope}
    
    
    % //////// NETHERLANDS /////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        \begin{scope}
        
            % path6448
            \path[country, we]
            (1306.4900,314.1300) .. controls (1306.2500,314.1500) and
            (1306.0200,314.1800) .. (1305.7800,314.2000) .. controls (1306.5400,314.5170)
            and (1307.4500,315.5900) .. (1308.2900,314.7760) .. controls
            (1307.8000,314.3400) and (1307.1600,314.0480) .. (1306.4900,314.1280);

            % path6450
            \path[country, we]
            (1306.7800,313.7700) .. controls (1307.9800,313.3150) and
            (1308.7200,315.3520) .. (1309.8800,314.4900) .. controls (1308.9800,314.0630)
            and (1307.7500,312.6810) .. (1306.7800,313.7700);

            % path6452
            \path[country, we]
            (1312.9000,303.7700) .. controls (1313.5200,303.5300) and
            (1313.9500,302.9610) .. (1313.4800,302.3300) .. controls (1312.9500,302.6280)
            and (1312.6300,303.1670) .. (1312.9000,303.7700);

            % path6454
            \path[country, we]
            (1314.5600,301.4600) .. controls (1314.3100,301.6060) and
            (1314.0300,301.7420) .. (1313.8400,301.9640) .. controls (1314.0800,301.7960)
            and (1314.3200,301.6280) .. (1314.5600,301.4600);

            % path6456
            \path[country, we]
            (1315.8600,300.8100) .. controls (1316.6100,300.5770) and
            (1317.4000,300.4290) .. (1318.0900,300.0180) .. controls (1317.3100,300.1510)
            and (1316.5300,300.3660) .. (1315.8600,300.8100);

            % path6458
            \path[country, we]
            (1319.0200,300.1700) .. controls (1319.5500,300.1600) and
            (1320.0500,300.0370) .. (1320.5300,299.8100) .. controls (1319.9900,299.8100)
            and (1319.4900,299.9230) .. (1319.0200,300.1700);

            % path6482
            \path[country, we]
            (1303.3300,317.6600) .. controls (1303.4500,316.3250) and
            (1308.1700,317.3750) .. (1309.0900,317.3720) .. controls (1308.2700,318.1990)
            and (1306.9500,318.8190) .. (1305.8200,318.2910) .. controls
            (1305.0900,317.9450) and (1303.6000,318.3410) .. (1303.3300,317.6600);

            % path6484
            \path[country, we]
            (1324.8900,299.8600) .. controls (1322.3700,300.1800) and (1319.3600,300.3710)
            .. (1317.5300,302.2790) .. controls (1316.6900,303.1550) and
            (1315.4300,303.9970) .. (1314.2000,304.1940) .. controls (1313.4000,304.3230)
            and (1312.5900,304.5490) .. (1312.2900,305.4030) .. controls
            (1311.2400,308.3170) and (1310.4100,310.1410) .. (1308.1500,312.3580) ..
            controls (1307.2800,313.2160) and (1309.4600,313.9090) .. (1309.9700,314.0710)
            .. controls (1311.1800,314.4560) and (1312.6900,313.4820) ..
            (1313.0900,314.3740) .. controls (1311.5300,314.0740) and (1309.8700,315.5400)
            .. (1308.3600,314.8780) .. controls (1309.7100,315.7390) and
            (1308.1400,315.1030) .. (1307.5500,315.4820) .. controls (1308.1100,315.8760)
            and (1309.1700,315.6800) .. (1309.2600,316.5910) .. controls
            (1308.1500,316.9390) and (1307.5100,315.8420) .. (1306.7400,315.2810) ..
            controls (1305.7900,315.2810) and (1304.6000,314.9730) .. (1304.0200,315.9860)
            .. controls (1304.7500,316.9490) and (1306.1100,316.7520) ..
            (1307.1500,316.6920) .. controls (1308.0000,316.6420) and (1310.7400,318.0980)
            .. (1310.5700,316.3900) .. controls (1311.1000,316.7870) and
            (1311.8600,316.9950) .. (1312.2900,316.2890) .. controls (1312.6400,317.1520)
            and (1313.9400,316.8730) .. (1314.4000,316.2890) .. controls
            (1314.9500,318.3160) and (1317.9000,318.2950) .. (1319.6400,319.0100) ..
            controls (1318.4600,320.3790) and (1317.3100,322.3990) .. (1320.3500,322.4370)
            .. controls (1321.6600,322.4570) and (1320.1300,320.3970) ..
            (1320.3500,320.0180) .. controls (1321.0400,318.8460) and (1322.4400,317.6130)
            .. (1321.9600,316.0870) .. controls (1321.7200,315.3090) and
            (1321.1900,314.3600) .. (1320.3500,314.0710) .. controls (1320.2500,312.3040)
            and (1322.1600,314.1410) .. (1321.6600,312.7610) .. controls
            (1322.2500,313.0600) and (1325.6700,313.4100) .. (1325.8900,312.4590) ..
            controls (1326.0000,312.0310) and (1325.2700,311.4860) .. (1325.8900,311.1480)
            .. controls (1326.1700,311.0580) and (1326.3600,310.9060) ..
            (1326.6000,310.7450) .. controls (1329.1700,308.1810) and (1324.6800,308.2030)
            .. (1325.3900,307.0160) .. controls (1325.9200,306.1280) and
            (1327.7300,307.1500) .. (1327.8100,306.3100) .. controls (1327.9200,305.1870)
            and (1328.5600,304.3580) .. (1328.8200,303.2860) .. controls
            (1329.2200,301.6370) and (1326.4900,299.6560) .. (1324.8900,299.8600) --
            cycle(1318.5400,307.0160) .. controls (1318.7800,306.9860) and
            (1319.0600,306.9960) .. (1319.3400,307.1170) .. controls (1320.1800,307.4840)
            and (1319.8200,308.0420) .. (1319.3400,308.4270) .. controls
            (1318.8700,308.8040) and (1318.4100,309.2660) .. (1317.9300,309.6360) ..
            controls (1317.2200,310.1910) and (1316.0800,309.1010) .. (1315.3100,309.1320)
            .. controls (1315.5500,308.6190) and (1316.0800,308.2890) ..
            (1316.6200,308.1250) .. controls (1317.2900,307.7750) and (1317.8100,307.1000)
            .. (1318.5400,307.0160) -- cycle;

        \end{scope}
  
    \end{scope}
    
    
    % //////// NORWAY //////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]

        % path6606
        \path[country]
        (1317.0800,238.1000) .. controls (1316.8400,237.8550) and
        (1316.5800,237.6400) .. (1316.2900,237.4530) .. controls (1316.0300,238.2940)
        and (1316.2900,238.5100) .. (1317.0800,238.1000);

        % path6608
        \path[country]
        (1317.3700,244.2200) .. controls (1317.0600,243.9780) and
        (1316.7400,243.7380) .. (1316.4300,243.5000) .. controls (1316.6100,244.0130)
        and (1316.7100,244.5410) .. (1316.7200,245.0840) .. controls
        (1317.3200,245.1140) and (1317.5700,244.7940) .. (1317.3700,244.2200);

        % path6610
        \path[country]
        (1316.7200,242.7800) .. controls (1316.9800,242.9710) and
        (1317.2500,243.1640) .. (1317.5100,243.3550) .. controls (1317.3300,243.0390)
        and (1317.0600,242.8470) .. (1316.7200,242.7800);

        % path6614
        \path[country]
        (1318.0100,231.6200) .. controls (1318.2400,230.9260) and
        (1317.7000,230.9400) .. (1317.2200,231.1160) .. controls (1317.4800,231.2840)
        and (1317.7500,231.4520) .. (1318.0100,231.6200);

        % path6616
        \path[country]
        (1317.6600,252.3600) .. controls (1317.2400,252.9300) and
        (1317.4600,253.4750) .. (1318.0900,253.7280) .. controls (1318.3700,253.0850)
        and (1318.4000,252.2050) .. (1317.8000,251.7120) .. controls
        (1317.8000,251.9280) and (1317.7000,252.1440) .. (1317.6600,252.3600);

        % path6618
        \path[country]
        (1318.0900,248.4000) .. controls (1317.0300,248.3700) and
        (1317.5500,249.4360) .. (1317.4400,250.0560) .. controls (1317.6000,249.4470)
        and (1318.0600,249.1120) .. (1318.6600,249.4800) .. controls
        (1318.6600,249.0460) and (1318.4200,248.6860) .. (1318.0900,248.4000);

        % path6620
        \path[country]
        (1318.6600,247.2400) .. controls (1318.3000,247.7620) and
        (1318.4300,249.0150) .. (1319.2400,249.0410) .. controls (1320.3300,249.0710)
        and (1319.3400,247.3290) .. (1318.6600,247.2400);

        % path6624
        \path[country]
        (1319.6000,246.9600) .. controls (1319.3600,247.0100) and
        (1319.1200,247.0600) .. (1318.8800,247.1040) .. controls (1319.5800,247.1540)
        and (1320.1400,247.9340) .. (1320.6900,247.1440) .. controls
        (1321.1800,246.4390) and (1319.9000,246.5270) .. (1319.6000,246.9570);

        % path6626
        \path[country]
        (1322.1900,228.9600) .. controls (1321.6900,228.8140) and
        (1321.1900,228.7910) .. (1320.6800,228.8900) .. controls (1320.6800,230.0340)
        and (1321.8600,229.7220) .. (1322.1900,228.9600);

        % path6628
        \path[country]
        (1323.4100,228.0900) .. controls (1323.1700,228.0400) and
        (1322.9400,227.9900) .. (1322.7000,227.9460) .. controls (1322.6000,228.4250)
        and (1322.5900,228.9050) .. (1322.5500,229.3850) .. controls
        (1323.0500,229.1370) and (1323.4200,228.6730) .. (1323.4100,228.0900);

        % path6630
        \path[country]
        (1324.8600,227.5900) .. controls (1324.6200,227.5400) and
        (1324.3800,227.5200) .. (1324.1400,227.5200) .. controls (1324.3800,227.5400)
        and (1324.6200,227.5700) .. (1324.8600,227.5900);

        % path6632
        \path[country]
        (1324.3500,227.8100) .. controls (1324.6100,227.9100) and
        (1324.8800,228.0020) .. (1325.1400,228.0980) .. controls (1324.9400,227.8450)
        and (1324.6700,227.7490) .. (1324.3500,227.8100);

        % path6634
        \path[country]
        (1328.3800,225.5000) .. controls (1328.1200,225.5000) and
        (1327.8500,225.5000) .. (1327.5900,225.5000) .. controls (1327.9100,225.6570)
        and (1328.2500,225.7770) .. (1328.6000,225.8600) .. controls
        (1328.5000,225.7400) and (1328.4500,225.6200) .. (1328.3800,225.5000);

        % path6636
        \path[country]
        (1329.0300,224.5700) .. controls (1328.7700,224.5500) and
        (1328.5000,224.5700) .. (1328.2400,224.5700) .. controls (1328.7900,224.9900)
        and (1328.8300,224.6200) .. (1329.0300,224.5700);

        % path6638
        \path[country]
        (1332.9200,223.7700) .. controls (1333.1600,223.6020) and
        (1333.4000,223.4340) .. (1333.6400,223.2660) .. controls (1333.4700,222.9850)
        and (1333.2500,222.7450) .. (1332.9900,222.5460) .. controls
        (1333.0900,223.3700) and (1332.7900,223.5140) .. (1332.1300,222.9780) ..
        controls (1332.0200,223.5860) and (1332.2900,223.9180) ..
        (1332.9200,223.7700);

        % path6642
        \path[country]
        (1336.4500,220.6800) .. controls (1336.1300,219.6050) and
        (1334.7600,219.9430) .. (1334.2200,220.6100) .. controls (1334.9400,220.8260)
        and (1335.7300,221.1270) .. (1336.4500,220.6800);

        % path6644
        \path[country]
        (1335.7300,222.3300) .. controls (1335.9900,222.2800) and
        (1336.2500,222.2300) .. (1336.5200,222.1850) .. controls (1336.0600,221.6620)
        and (1335.4500,221.6340) .. (1335.0100,222.1850) .. controls
        (1335.2500,222.2350) and (1335.4900,222.2850) .. (1335.7300,222.3300);

        % path6648
        \path[country]
        (1337.0200,221.8300) .. controls (1337.4800,222.1500) and
        (1337.9800,222.2470) .. (1338.5300,222.1190) .. controls (1338.3900,221.1900)
        and (1337.5200,221.1750) .. (1337.0200,221.8300);

        % path6650
        \path[country]
        (1337.2400,219.8100) .. controls (1338.0700,220.7250) and
        (1341.4700,219.9820) .. (1341.8500,218.8020) .. controls (1341.3400,218.3570)
        and (1340.6100,218.3810) .. (1339.9900,218.5180) .. controls
        (1339.5200,218.6230) and (1337.7600,218.9210) .. (1339.5400,219.1630) ..
        controls (1338.6900,219.1620) and (1337.8200,219.0300) ..
        (1337.2400,219.8100);

        % path6652
        \path[country]
        (1340.3400,217.7300) .. controls (1339.5800,217.0520) and
        (1338.1600,218.0010) .. (1337.3800,218.1620) .. controls (1338.3900,218.1020)
        and (1339.5300,218.6050) .. (1340.3400,217.7300);

        % path6654
        \path[country]
        (1338.9700,220.4600) .. controls (1338.7300,220.4800) and
        (1338.4900,220.5100) .. (1338.2500,220.5300) .. controls (1338.5200,220.6880)
        and (1338.8100,220.8080) .. (1339.1100,220.8890) .. controls
        (1339.1100,220.7460) and (1339.0100,220.6020) .. (1338.9700,220.4580);

        % path6662
        \path[country]
        (1352.5800,208.4400) .. controls (1352.3100,208.6080) and
        (1352.0500,208.7760) .. (1351.7800,208.9440) .. controls (1352.3200,208.8170)
        and (1352.8500,208.6490) .. (1353.3700,208.4400) .. controls
        (1353.1000,208.4400) and (1352.8400,208.4400) .. (1352.5800,208.4400);

        % path6664
        \path[country]
        (1352.5000,208.8700) .. controls (1353.3500,208.6210) and
        (1354.0300,209.5840) .. (1354.7400,208.7250) .. controls (1353.9900,208.3970)
        and (1353.2200,208.6250) .. (1352.5000,208.8700);

        % path6666
        \path[country]
        (1354.7400,211.9700) .. controls (1354.9800,211.9500) and
        (1355.2100,211.9200) .. (1355.4500,211.9000) .. controls (1354.8300,211.7420)
        and (1354.2600,211.4060) .. (1353.8000,210.9640) .. controls
        (1353.7000,211.5870) and (1354.1200,211.9860) .. (1354.7400,211.9720);

        % path6668
        \path[country]
        (1354.8100,210.4500) .. controls (1354.5400,210.4700) and
        (1354.2800,210.5000) .. (1354.0100,210.5200) .. controls (1354.2400,210.7540)
        and (1354.5100,210.9460) .. (1354.8100,211.0960) .. controls
        (1354.8100,210.8810) and (1354.8100,210.6650) .. (1354.8100,210.4490);

        % path6670
        \path[country]
        (1355.1000,211.0300) .. controls (1354.8600,211.5300) and
        (1355.1000,211.6500) .. (1355.8200,211.3890) .. controls (1355.5800,211.2700)
        and (1355.3400,211.1510) .. (1355.1000,211.0300);

        % path6672
        \path[country]
        (1357.6200,207.1400) .. controls (1357.0400,207.0150) and
        (1356.4600,207.2520) .. (1356.1000,207.7160) .. controls (1356.6500,207.6560)
        and (1357.1600,207.4600) .. (1357.6200,207.1400);

        % path6674
        \path[country] (1357.4700,203.2500) .. controls (1357.7700,203.4690) and
        (1358.1100,203.5410) .. (1358.4800,203.4660) .. controls (1358.3400,202.4640)
        and (1357.9200,202.7170) .. (1357.4700,203.2500);

        % path6676
        \path[country]
        (1361.6500,201.3100) .. controls (1362.2400,200.9920) and
        (1362.8600,200.7750) .. (1363.5200,200.6620) .. controls (1362.5500,200.2190)
        and (1361.3900,200.3950) .. (1360.9300,201.4550) .. controls
        (1361.1700,201.4050) and (1361.4100,201.3550) .. (1361.6500,201.3100);

        % path6678
        \path[country]
        (1362.2200,199.3700) .. controls (1360.8000,198.2720) and
        (1361.0400,200.9500) .. (1362.5100,199.7290) .. controls (1362.4100,199.6100)
        and (1362.3100,199.4910) .. (1362.2200,199.3700);

        % path6680
        \path[country]
        (1363.8100,185.5400) .. controls (1363.6100,185.7610) and
        (1363.4400,186.0010) .. (1363.3000,186.2600) .. controls (1364.2300,186.8140)
        and (1365.1900,185.7320) .. (1364.8200,184.8200) .. controls
        (1364.4300,184.9850) and (1364.0900,185.2250) .. (1363.8100,185.5400);

        % path6682
        \path[country]
        (1364.2400,198.9300) .. controls (1364.0000,199.0300) and
        (1363.7600,199.1220) .. (1363.5200,199.2180) .. controls (1363.7700,199.1580)
        and (1364.0100,199.0580) .. (1364.2400,198.9300);

        % path6684
        \path[country]
        (1364.8200,198.5700) .. controls (1364.5200,198.4800) and
        (1364.2600,198.5500) .. (1364.0200,198.7870) .. controls (1364.2800,198.7170)
        and (1364.5500,198.6430) .. (1364.8200,198.5700);

        % path6686
        \path[country]
        (1365.1800,185.4700) .. controls (1365.8400,185.6090) and
        (1366.3800,185.1860) .. (1366.6200,184.6060) .. controls (1365.9800,184.2370)
        and (1365.0600,184.6660) .. (1365.1800,185.4700);

        % path6688
        \path[country]
        (1366.1800,194.4000) .. controls (1366.6900,194.3600) and
        (1367.1900,194.3100) .. (1367.7000,194.2560) .. controls (1367.1800,194.1360)
        and (1366.6700,194.1860) .. (1366.1800,194.4000);

        % path6690
        \path[country]
        (1367.3300,184.3900) .. controls (1367.1600,184.6300) and
        (1367.0000,184.8690) .. (1366.8300,185.1100) .. controls (1367.9100,184.3570)
        and (1369.6000,184.7280) .. (1370.5000,183.6710) .. controls
        (1369.8400,183.7870) and (1369.5900,183.1980) .. (1368.9900,183.1670) ..
        controls (1368.3900,183.1370) and (1368.0400,183.6260) .. (1367.4100,183.4550)
        .. controls (1367.8100,183.9320) and (1367.6400,184.1230) ..
        (1366.9000,184.0310) .. controls (1367.0400,184.1510) and (1367.1800,184.2700)
        .. (1367.3300,184.3900);

        % path6692
        \path[country]
        (1370.7200,183.6700) .. controls (1371.1900,183.1620) and
        (1370.3800,183.0210) .. (1370.0700,183.0220) .. controls (1370.2900,183.2380)
        and (1370.5000,183.4540) .. (1370.7200,183.6700);

        % path6694
        \path[country]
        (1370.3600,191.8800) .. controls (1370.5500,192.6710) and
        (1371.1500,192.9410) .. (1371.1500,191.8100) .. controls (1370.8800,191.8300)
        and (1370.6200,191.8600) .. (1370.3600,191.8800);

        % path6696
        \path[country]
        (1371.1500,183.8100) .. controls (1372.3800,184.6780) and
        (1375.0300,183.3440) .. (1375.6200,182.1540) .. controls (1375.0200,182.1540)
        and (1374.5100,182.3620) .. (1374.1000,182.8020) .. controls
        (1373.6800,181.2530) and (1371.7100,183.5050) .. (1371.1500,183.8100);

        % path6698
        \path[country]
        (1374.4600,181.2900) .. controls (1375.4000,181.2500) and
        (1376.5500,181.1110) .. (1377.2700,180.4260) .. controls (1376.5400,180.2390)
        and (1376.6700,180.0880) .. (1376.8700,179.5900) .. controls
        (1377.1000,179.0070) and (1375.6600,178.4400) .. (1375.3300,178.1950) ..
        controls (1375.3300,178.7160) and (1375.3300,179.2190) .. (1375.1100,179.7070)
        .. controls (1374.3200,178.7670) and (1372.7600,180.2270) ..
        (1371.7300,180.7150) .. controls (1372.8400,181.6530) and (1374.3000,179.8210)
        .. (1375.5400,180.3550) .. controls (1375.0600,180.5870) and
        (1374.5600,180.7320) .. (1374.0300,180.7880) .. controls (1374.1700,180.9540)
        and (1374.3100,181.1220) .. (1374.4600,181.2900);

        % path6700
        \path[country] (1373.6000,181.9400) .. controls (1374.0800,182.0000) and
        (1374.4900,181.8600) .. (1374.8200,181.5080) .. controls (1374.1700,181.2470)
        and (1373.4300,181.2390) .. (1372.8100,181.5780) .. controls
        (1373.0700,181.6980) and (1373.3300,181.8180) .. (1373.6000,181.9380);

        % path6702
        \path[country]
        (1374.7500,179.1300) .. controls (1374.8600,178.5510) and
        (1374.5900,178.5510) .. (1373.9600,179.1300) .. controls (1374.2200,179.1300)
        and (1374.4800,179.1300) .. (1374.7500,179.1300);

        % path6704
        \path[country]
        (1374.1000,183.8900) .. controls (1374.3700,183.7700) and
        (1374.6300,183.6500) .. (1374.9000,183.5300) .. controls (1374.5700,183.5300)
        and (1374.3000,183.6450) .. (1374.1000,183.8900);

        % path6706
        \path[country]
        (1375.0400,186.2600) .. controls (1375.5600,186.2600) and
        (1376.0600,186.1560) .. (1376.5500,185.9720) .. controls (1376.0500,185.5550)
        and (1375.2800,185.5450) .. (1375.0400,186.2600);

        % path6708
        \path[country]
        (1377.4100,180.4300) .. controls (1377.5100,180.6700) and
        (1377.5600,180.9090) .. (1377.6300,181.1500) .. controls (1377.1600,181.3230)
        and (1376.6800,181.4200) .. (1376.1900,181.4380) .. controls
        (1376.9400,182.2550) and (1375.6500,182.6380) .. (1375.6200,183.4550) ..
        controls (1376.2900,182.8640) and (1377.1300,182.5240) .. (1377.9900,182.3030)
        .. controls (1377.7600,182.5600) and (1377.5500,182.8240) ..
        (1377.3400,183.0950) .. controls (1377.7800,183.1150) and (1378.3400,183.5250)
        .. (1378.7800,183.3830) .. controls (1379.3200,183.2060) and
        (1379.5700,182.3460) .. (1380.0100,182.0150) .. controls (1379.9100,183.6770)
        and (1380.7100,182.2480) .. (1381.0900,181.8340) .. controls
        (1381.5100,181.3710) and (1382.1600,181.5650) .. (1382.7000,181.5430) ..
        controls (1383.6800,181.5030) and (1384.6000,180.1480) .. (1383.5600,179.4800)
        .. controls (1383.1200,179.1930) and (1382.1800,179.0290) ..
        (1381.7900,179.5100) .. controls (1381.2500,180.1920) and (1380.1100,180.7210)
        .. (1379.2900,181.5820) .. controls (1379.2900,181.3730) and
        (1381.5900,178.7320) .. (1379.6500,180.1420) .. controls (1380.3000,179.3080)
        and (1380.0600,178.0210) .. (1378.7500,178.6510) .. controls
        (1378.1200,178.9530) and (1377.8700,180.3870) .. (1378.7500,180.4300) ..
        controls (1378.2900,180.2710) and (1377.8300,180.2710) ..
        (1377.3800,180.4300);

        % path6710
        \path[country]
        (1378.7100,178.4100) .. controls (1379.7300,178.2240) and
        (1381.0400,177.3950) .. (1381.3000,176.3210) .. controls (1379.9200,175.5910)
        and (1377.8000,177.5640) .. (1377.4100,178.7690) .. controls
        (1377.9200,178.9270) and (1378.3500,178.8090) .. (1378.7100,178.4100);

        % path6712
        \path[country]
        (1378.7100,185.3200) .. controls (1378.4700,185.4200) and
        (1378.2300,185.5120) .. (1377.9900,185.6090) .. controls (1378.7300,185.7260)
        and (1379.4900,185.6390) .. (1380.2200,185.4640) .. controls
        (1379.7100,185.4240) and (1379.2100,185.3740) .. (1378.7100,185.3200);

        % path6714
        \path[country]
        (1381.3700,182.2300) .. controls (1383.5300,183.7430) and
        (1383.0300,180.2960) .. (1381.3700,182.2300);

        % path6716
        \path[country]
        (1383.3900,179.1300) .. controls (1383.6300,179.0100) and
        (1383.8700,178.8900) .. (1384.1100,178.7700) .. controls (1383.5700,178.4940)
        and (1383.0700,178.5410) .. (1382.6000,178.9150) .. controls
        (1382.8600,178.9850) and (1383.1200,179.0580) .. (1383.3900,179.1300);

        % path6722
        \path[country]
        (1385.9100,176.2500) .. controls (1386.1700,176.2300) and
        (1386.4400,176.2000) .. (1386.7000,176.1800) .. controls (1385.6500,176.4200)
        and (1385.6500,176.6600) .. (1386.7000,176.9000) .. controls
        (1386.2000,177.0940) and (1385.7000,177.2620) .. (1385.1900,177.4040) ..
        controls (1386.0900,177.9210) and (1387.1500,177.6950) .. (1388.0100,177.2290)
        .. controls (1389.0300,176.6770) and (1390.3000,177.2490) ..
        (1391.3800,176.9730) .. controls (1390.4700,176.7650) and (1390.4200,176.5380)
        .. (1391.2400,176.2920) .. controls (1391.7100,175.7770) and
        (1391.9800,174.5700) .. (1390.7400,175.2440) .. controls (1392.5000,174.7410)
        and (1390.6200,174.6210) .. (1390.0100,174.3180) .. controls
        (1388.1100,173.3690) and (1390.4400,175.8160) .. (1388.7900,174.0920) ..
        controls (1390.3500,175.4600) and (1387.6500,174.2280) .. (1386.9200,174.5960)
        .. controls (1387.3700,174.9990) and (1387.9000,175.1670) ..
        (1388.5000,175.1000) .. controls (1387.4100,175.4960) and (1386.2300,175.2960)
        .. (1385.1200,175.5330) .. controls (1385.8300,175.4630) and
        (1385.9900,175.5830) .. (1385.9100,176.2520);

        % path6724
        \path[country]
        (1386.7000,180.1400) .. controls (1386.6000,179.0140) and
        (1385.5100,179.6600) .. (1385.1900,180.2100) .. controls (1385.6900,180.1500)
        and (1386.1900,180.1200) .. (1386.7000,180.1400);

        % path6726
        \path[country]
        (1386.7800,179.2100) .. controls (1387.2300,179.6760) and
        (1387.8700,179.7990) .. (1388.4300,179.4260) .. controls (1388.1000,179.0140)
        and (1387.0700,178.3850) .. (1386.7800,179.2100);

        % path6728
        \path[country]
        (1395.7800,173.3000) .. controls (1396.2000,173.1210) and
        (1396.5800,172.8820) .. (1396.9300,172.5800) .. controls (1396.2400,172.2350)
        and (1395.5300,171.6520) .. (1394.7000,172.0040) .. controls
        (1395.6900,172.2990) and (1395.4400,172.7170) .. (1394.8400,173.1550) ..
        controls (1394.7000,172.8890) and (1394.5600,172.6250) .. (1394.4100,172.3640)
        .. controls (1393.8700,172.6600) and (1392.8400,173.2330) ..
        (1394.3100,173.2270) .. controls (1393.7800,173.0650) and (1391.6100,173.8820)
        .. (1393.5200,173.6590) .. controls (1392.9300,173.6790) and
        (1392.4000,173.8720) .. (1391.9400,174.2350) .. controls (1392.6500,174.5300)
        and (1395.9400,174.6540) .. (1395.7600,173.3000);

        % path6734
        \path[country]
        (1394.8400,171.0000) .. controls (1395.3200,170.7240) and
        (1395.8300,170.4840) .. (1396.3500,170.2800) .. controls (1395.8500,170.3600)
        and (1395.3400,170.3600) .. (1394.8400,170.2800) .. controls
        (1394.8400,170.5210) and (1394.8400,170.7600) .. (1394.8400,171.0000);

        % path6736
        \path[country]
        (1395.5600,171.0000) .. controls (1395.0800,174.0380) and
        (1399.8200,171.1200) .. (1400.3100,171.0000) .. controls (1399.6500,171.0600)
        and (1399.1000,170.9100) .. (1398.6700,171.0000) .. controls
        (1398.4400,171.0400) and (1398.1600,170.4550) .. (1397.8600,170.4300) ..
        controls (1397.0300,170.3600) and (1396.3300,170.7850) ..
        (1395.5600,171.0060);

        % path6746
        \path[country]
        (1396.7800,169.5600) .. controls (1397.0300,169.7300) and
        (1397.3000,169.8740) .. (1397.5800,169.9920) .. controls (1397.7400,169.3250)
        and (1396.9500,168.6420) .. (1396.7800,169.5600);

        % path6748
        \path[country]
        (1398.2200,169.9900) .. controls (1398.5400,170.0800) and
        (1398.8500,170.0500) .. (1399.1600,169.9200) .. controls (1398.8400,169.9400)
        and (1398.5300,169.9700) .. (1398.2200,169.9900);

        % path6750
        \path[country]
        (1400.7400,171.0000) .. controls (1400.2300,171.2950) and
        (1399.7700,171.6550) .. (1399.3700,172.0790) .. controls (1400.1400,171.9680)
        and (1401.1100,171.8990) .. (1401.3900,171.0000) .. controls
        (1401.1700,171.0000) and (1400.9500,171.0000) .. (1400.7400,171.0000);

        % path6752
        \path[country]
        (1401.6100,169.9200) .. controls (1400.9700,169.3830) and
        (1400.1700,169.2550) .. (1399.3700,169.2000) .. controls (1400.5600,169.8230)
        and (1400.8500,171.1590) .. (1402.4000,170.2800) .. controls
        (1402.1300,170.1600) and (1401.8700,170.0400) .. (1401.6100,169.9200);

        % path6756
        \path[country] (1403.9800,169.9200) .. controls (1404.4700,171.2540) and
        (1406.1600,170.6120) .. (1406.2900,169.4160) .. controls (1405.4800,169.1300)
        and (1404.6300,169.4260) .. (1403.9800,169.9200);

        % path6758
        \path[country]
        (1405.7800,172.3700) .. controls (1405.9200,172.1300) and
        (1406.0700,171.8900) .. (1406.2200,171.6490) .. controls (1405.6500,171.4200)
        and (1405.2100,171.6490) .. (1405.2100,172.2970) .. controls
        (1405.4000,172.3270) and (1405.5900,172.3470) .. (1405.7800,172.3670);

        % path6760
        \path[country]
        (1406.2200,171.0000) .. controls (1406.7400,171.3940) and
        (1407.4100,171.3940) .. (1407.9400,171.0000) .. controls (1407.4800,171.0600)
        and (1406.5900,170.5560) .. (1406.2200,171.0000);

        % path6762
        \path[country]
        (1411.1800,171.0000) .. controls (1411.1800,170.8270) and
        (1411.0800,170.8300) .. (1410.6800,170.7120) .. controls (1410.8400,170.8120)
        and (1411.0100,170.9050) .. (1411.1800,171.0000);

        % path6764
        \path[country]
        (1420.1100,165.5300) .. controls (1420.2100,165.4300) and
        (1420.3000,165.3380) .. (1420.4000,165.2420) .. controls (1419.6600,165.3220)
        and (1418.8900,165.4810) .. (1418.1700,165.1720) .. controls
        (1419.8000,167.0060) and (1414.5400,165.1920) .. (1416.9400,166.3230) ..
        controls (1416.1700,166.3330) and (1415.6300,165.6790) .. (1414.9800,166.2330)
        .. controls (1414.4200,166.7120) and (1413.0300,166.3460) ..
        (1412.3300,166.4680) .. controls (1412.8200,166.6890) and (1413.3300,166.8570)
        .. (1413.8500,166.9720) .. controls (1413.6200,167.1800) and
        (1413.3800,167.3720) .. (1413.1300,167.5480) .. controls (1414.0900,166.8200)
        and (1415.5600,167.4020) .. (1416.6500,167.2960) .. controls
        (1417.9600,167.1650) and (1419.0300,166.1830) .. (1420.1100,165.5310);

        % path6770
        \path[country]
        (1417.1600,169.2000) .. controls (1417.4200,169.2000) and
        (1417.6900,169.2000) .. (1417.9500,169.2000) .. controls (1417.5300,168.3630)
        and (1415.8600,168.0780) .. (1415.0700,168.4070) .. controls
        (1415.5800,169.1150) and (1416.3700,169.1110) .. (1417.1600,169.2000);

        % path6772
        \path[country]
        (1421.1900,166.8900) .. controls (1421.1900,166.7700) and
        (1421.0900,166.6510) .. (1421.0500,166.5310) .. controls (1420.0300,167.6930)
        and (1418.4300,167.1210) .. (1417.3000,168.0430) .. controls
        (1418.1000,168.6650) and (1419.1200,167.6660) .. (1419.1000,168.9790) ..
        controls (1419.6500,168.5690) and (1422.3200,167.9710) ..
        (1421.1900,166.8900);

        % path6774
        \path[country]
        (1423.4200,167.2500) .. controls (1424.2400,166.1340) and
        (1423.0800,165.9920) .. (1422.2100,165.9470) .. controls (1420.2800,165.8470)
        and (1422.1100,167.4820) .. (1423.4200,167.2500);

        % path6776
        \path[country]
        (1422.5600,163.9400) .. controls (1422.9800,164.3720) and
        (1423.4800,164.5160) .. (1424.0700,164.3730) .. controls (1423.8000,163.9790)
        and (1423.0000,163.2530) .. (1422.5600,163.9400);

        % path6778
        \path[country]
        (1423.0600,163.3700) .. controls (1423.2900,163.5110) and
        (1423.5300,163.4870) .. (1423.7800,163.3000) .. controls (1423.5400,163.3300)
        and (1423.3000,163.3500) .. (1423.0600,163.3700);

        % path6782
        \path[country]
        (1433.7200,163.9400) .. controls (1433.9800,163.9400) and
        (1434.2400,163.9400) .. (1434.5100,163.9400) .. controls (1433.4500,164.0000)
        and (1433.6600,163.5720) .. (1434.1500,163.0760) .. controls
        (1433.5800,162.9070) and (1433.0100,162.7630) .. (1432.4300,162.6440) ..
        controls (1431.6700,162.6440) and (1431.0800,163.1860) .. (1430.3300,163.2200)
        .. controls (1430.8300,163.3280) and (1431.1100,163.8480) ..
        (1431.4700,164.1480) .. controls (1431.9700,164.5550) and (1433.1800,164.0200)
        .. (1433.7200,163.9400);

        % path6794
        \path[country]
        (1317.0100,235.8700) .. controls (1318.5300,235.1340) and (1320.1900,235.7800)
        .. (1321.7600,235.2940) .. controls (1321.4000,235.2340) and
        (1321.0700,235.2740) .. (1320.7400,235.4320) .. controls (1320.0200,235.6700)
        and (1319.4600,235.1360) .. (1318.7400,235.1500) .. controls
        (1321.0600,234.4610) and (1317.2000,234.8120) .. (1319.4500,234.3580) ..
        controls (1318.6600,234.2340) and (1317.8700,234.3680) .. (1317.0800,234.4280)
        .. controls (1317.8700,234.2710) and (1318.6800,234.2760) ..
        (1319.4500,233.9960) .. controls (1318.7600,234.1560) and (1317.0000,234.6570)
        .. (1317.0100,233.4200) .. controls (1317.5700,233.4900) and
        (1318.0800,233.3500) .. (1318.5200,232.9870) .. controls (1316.5900,233.1810)
        and (1319.5200,231.9180) .. (1320.0300,231.9070) .. controls
        (1320.6400,231.8970) and (1320.9700,232.3720) .. (1321.5400,232.4830) ..
        controls (1322.1000,232.5930) and (1323.9200,232.0240) .. (1322.6200,233.2760)
        .. controls (1322.9300,232.4980) and (1326.9400,231.9760) ..
        (1327.7400,232.3390) .. controls (1326.8700,231.8660) and (1325.8300,232.4720)
        .. (1324.9100,232.2990) .. controls (1324.4300,232.2090) and
        (1320.4200,232.0420) .. (1322.4800,231.9740) .. controls (1321.2300,231.8840)
        and (1319.2300,232.4690) .. (1318.1600,231.6150) .. controls
        (1318.7500,231.6450) and (1319.2500,231.4580) .. (1319.6700,231.0390) ..
        controls (1319.3400,230.6780) and (1317.8600,230.4680) .. (1317.9200,229.8210)
        .. controls (1318.0200,228.8940) and (1320.0400,230.5410) ..
        (1320.1000,231.1110) .. controls (1320.3700,230.9870) and (1320.6100,230.8190)
        .. (1320.8200,230.6070) .. controls (1319.5000,230.6170) and
        (1320.5200,229.0440) .. (1321.6900,230.5370) .. controls (1321.7900,229.8320)
        and (1322.5900,229.3570) .. (1322.7000,230.1930) .. controls
        (1322.8000,230.7040) and (1324.7800,230.6050) .. (1325.1400,230.6090) ..
        controls (1324.5500,230.4790) and (1322.5500,229.6720) .. (1323.7800,228.9360)
        .. controls (1325.2500,228.0500) and (1325.4900,228.9360) ..
        (1326.5800,229.8160) .. controls (1324.6500,226.0270) and (1331.3300,228.7140)
        .. (1328.6700,230.4640) .. controls (1329.2400,230.6050) and
        (1329.7700,230.5140) .. (1330.2600,230.1760) .. controls (1329.6600,230.0480)
        and (1329.2200,229.5370) .. (1329.8200,229.0250) .. controls
        (1330.1300,228.7570) and (1331.0000,229.1490) .. (1331.4100,228.9550) ..
        controls (1329.7100,229.0150) and (1329.5400,228.1230) .. (1328.2100,227.6320)
        .. controls (1327.1600,227.2430) and (1325.9900,227.8730) ..
        (1324.9300,227.5820) .. controls (1325.7700,227.3030) and (1326.6600,227.4040)
        .. (1327.5200,227.2940) .. controls (1326.7300,226.8120) and
        (1325.8100,227.2040) .. (1325.0700,226.5740) .. controls (1326.4500,226.2690)
        and (1328.0900,225.8490) .. (1329.4700,226.3550) .. controls
        (1330.6500,226.7830) and (1332.5900,227.4070) .. (1333.7100,226.6460) ..
        controls (1333.1900,226.7840) and (1332.6600,226.8320) .. (1332.1300,226.7910)
        .. controls (1332.3200,225.1900) and (1335.0900,225.3440) ..
        (1336.1600,225.7110) .. controls (1334.8100,224.3270) and (1333.0000,226.5420)
        .. (1331.5500,225.4950) .. controls (1332.0500,225.3620) and
        (1332.5600,225.2190) .. (1333.0600,225.0640) .. controls (1331.9200,225.1240)
        and (1330.1900,226.1480) .. (1329.2500,225.0640) .. controls
        (1329.7100,224.8740) and (1330.1900,224.8010) .. (1330.6900,224.8460) ..
        controls (1330.0700,224.7160) and (1329.5400,224.4280) .. (1329.1000,223.9820)
        .. controls (1329.8600,223.4490) and (1330.7800,223.2550) ..
        (1331.6000,223.8260) .. controls (1332.4300,224.4080) and (1333.1900,223.5190)
        .. (1334.0700,223.6950) .. controls (1334.8700,223.8560) and
        (1335.5700,223.3970) .. (1335.9000,224.4200) .. controls (1336.1700,225.2790)
        and (1337.8200,225.3600) .. (1338.4600,225.8560) .. controls
        (1337.6800,224.4700) and (1335.6000,224.4850) .. (1335.2200,222.7590) ..
        controls (1335.8000,222.3920) and (1336.7000,223.1460) .. (1337.0300,223.5370)
        .. controls (1337.8400,224.4850) and (1337.4100,224.2910) ..
        (1338.8900,224.3430) .. controls (1337.4400,224.2020) and (1338.3900,223.6000)
        .. (1339.0400,223.4790) .. controls (1338.7400,223.4490) and
        (1336.1500,223.3710) .. (1338.2500,223.2630) .. controls (1337.9300,223.2830)
        and (1336.0100,222.6060) .. (1337.0700,222.3660) .. controls
        (1338.2900,222.0890) and (1339.7200,222.0380) .. (1340.9800,221.8230) ..
        controls (1340.2300,221.9230) and (1339.4400,222.0010) .. (1338.7500,221.6080)
        .. controls (1339.0400,221.3370) and (1339.2900,221.0360) ..
        (1339.5100,220.7070) .. controls (1339.9400,220.1790) and (1340.3500,220.5090)
        .. (1340.8900,220.2980) .. controls (1341.7200,219.9710) and
        (1342.5800,220.2880) .. (1341.7000,221.1760) .. controls (1342.4300,220.8400)
        and (1343.2200,220.6720) .. (1344.0100,220.5290) .. controls
        (1343.4500,220.6320) and (1342.9000,220.6090) .. (1342.3500,220.4590) ..
        controls (1342.8000,220.1380) and (1343.3100,219.9450) .. (1343.8600,219.8830)
        .. controls (1343.3600,219.8030) and (1342.8500,219.8030) ..
        (1342.3500,219.8830) .. controls (1343.1200,219.3620) and (1344.2200,219.1210)
        .. (1345.1100,218.8720) .. controls (1346.1600,218.5790) and
        (1347.6200,220.3710) .. (1346.1000,221.0350) .. controls (1346.8500,220.7580)
        and (1347.6300,220.9150) .. (1348.4000,220.8900) .. controls
        (1346.4400,220.4310) and (1348.8400,219.9810) .. (1349.3700,219.9860) ..
        controls (1350.2600,219.9960) and (1351.2000,220.2310) .. (1352.0700,220.0260)
        .. controls (1351.5300,219.3690) and (1351.6700,219.0810) ..
        (1352.5000,219.1620) .. controls (1351.9700,218.9740) and (1351.4700,219.0210)
        .. (1350.9900,219.3060) .. controls (1352.1700,218.3990) and
        (1353.5300,217.6780) .. (1355.0200,217.5060) .. controls (1354.9200,216.8590)
        and (1354.5000,216.6460) .. (1353.9400,216.9300) .. controls
        (1354.1700,215.9480) and (1355.2300,215.9870) .. (1355.9600,215.6340) ..
        controls (1355.3000,215.5540) and (1353.5000,215.9600) .. (1355.1700,214.9860)
        .. controls (1353.6600,215.0460) and (1352.7700,216.7320) ..
        (1351.2800,216.9300) .. controls (1351.8200,216.9300) and (1352.3300,216.7840)
        .. (1352.7900,216.4980) .. controls (1353.6600,217.6870) and
        (1350.8400,218.5690) .. (1350.1500,218.8140) .. controls (1347.8900,219.6210)
        and (1347.4000,220.0460) .. (1346.1000,218.1530) .. controls
        (1346.7300,218.1530) and (1347.2900,217.8430) .. (1347.7500,217.4330) ..
        controls (1346.7100,217.6830) and (1345.6500,217.9470) .. (1344.6600,218.3700)
        .. controls (1345.2200,217.9960) and (1345.8800,217.4980) ..
        (1344.5600,217.5060) .. controls (1345.7000,217.0030) and (1347.2100,215.9270)
        .. (1348.5200,216.4260) .. controls (1347.9800,216.0870) and
        (1347.4500,216.1120) .. (1346.9400,216.4960) .. controls (1347.1700,216.2860)
        and (1347.4100,216.0940) .. (1347.6600,215.9200) .. controls
        (1346.0200,216.2530) and (1347.7600,215.3290) .. (1348.1800,214.9860) ..
        controls (1348.7100,214.5600) and (1348.3900,214.0110) .. (1349.3200,214.3360)
        .. controls (1348.6000,212.3310) and (1353.0400,212.8530) ..
        (1352.6300,211.0960) .. controls (1353.4300,211.3350) and (1353.9000,212.1310)
        .. (1354.7200,212.3200) .. controls (1354.6200,212.5930) and
        (1354.4900,212.8570) .. (1354.3500,213.1130) .. controls (1355.0800,212.6370)
        and (1355.9300,212.2220) .. (1356.8000,212.1040) .. controls
        (1355.3900,212.2480) and (1356.2200,211.2430) .. (1356.9500,211.2400) ..
        controls (1356.4600,211.0550) and (1355.9500,210.9600) .. (1355.4300,210.9530)
        .. controls (1355.4300,209.8090) and (1357.0300,209.7890) ..
        (1357.8100,209.5850) .. controls (1357.4200,209.5750) and (1357.0400,209.5250)
        .. (1356.6600,209.4410) .. controls (1357.9700,208.4330) and
        (1359.8800,208.1690) .. (1361.4100,208.7930) .. controls (1358.8600,207.5360)
        and (1356.9900,209.9800) .. (1354.5000,209.9450) .. controls
        (1355.4800,209.6530) and (1355.4600,209.4620) .. (1354.4000,209.3690) ..
        controls (1355.1300,208.9860) and (1355.9800,209.2060) .. (1356.7000,208.7930)
        .. controls (1356.1300,209.0200) and (1355.5600,209.0440) ..
        (1354.9700,208.8630) .. controls (1355.4600,208.6650) and (1355.9600,208.5920)
        .. (1356.4800,208.6460) .. controls (1354.1700,208.1790) and
        (1359.0600,207.9710) .. (1356.4800,208.1420) .. controls (1357.1800,208.0820)
        and (1357.8800,207.9130) .. (1358.5000,207.5660) .. controls
        (1356.7100,207.6160) and (1358.5000,206.7530) .. (1359.1500,207.4220) ..
        controls (1359.2700,206.4990) and (1360.3300,206.4010) .. (1360.5200,207.3520)
        .. controls (1359.9400,207.5910) and (1359.3400,207.6390) ..
        (1358.7200,207.4970) .. controls (1360.4000,208.2760) and (1362.6800,207.0380)
        .. (1363.9000,205.9130) .. controls (1363.3600,206.1730) and
        (1362.8700,206.5180) .. (1362.3300,206.7610) .. controls (1361.8300,206.9820)
        and (1359.7900,206.9170) .. (1361.6000,206.7010) .. controls
        (1360.5900,206.6110) and (1360.7200,206.2010) .. (1361.2400,205.6930) ..
        controls (1360.6400,205.5790) and (1360.0900,205.8780) .. (1359.7300,206.3400)
        .. controls (1359.2100,205.6340) and (1359.8600,204.0620) ..
        (1360.8100,204.1090) .. controls (1361.0200,204.2860) and (1361.2000,204.4870)
        .. (1361.3600,204.7140) .. controls (1361.8800,205.2230) and
        (1362.6200,204.7840) .. (1363.1800,204.6130) .. controls (1362.9500,204.6830)
        and (1361.2500,204.0130) .. (1361.1800,203.9040) .. controls
        (1360.2600,202.4440) and (1362.1600,202.8470) .. (1362.8900,203.2450) ..
        controls (1361.0100,202.5000) and (1363.3100,199.6500) .. (1365.4800,201.8050)
        .. controls (1365.2200,200.6210) and (1363.4300,200.1170) ..
        (1362.4600,200.2210) .. controls (1363.4600,200.1910) and (1365.2200,199.2030)
        .. (1366.2100,198.8430) .. controls (1367.1300,198.5100) and
        (1366.8100,199.0220) .. (1367.3800,199.3730) .. controls (1367.7400,199.5970)
        and (1368.3900,199.2730) .. (1368.8000,199.3530) .. controls
        (1367.5800,199.0500) and (1370.2500,198.5560) .. (1370.8100,197.9850) ..
        controls (1368.7900,198.4670) and (1366.7100,198.6510) .. (1364.6900,199.1360)
        .. controls (1365.2000,198.3400) and (1366.0800,198.2640) ..
        (1366.9300,198.2000) .. controls (1366.1400,198.0710) and (1365.3300,198.2900)
        .. (1364.5500,198.0550) .. controls (1365.2100,197.5860) and
        (1365.1000,197.0220) .. (1364.4000,196.6880) .. controls (1365.1400,196.1830)
        and (1365.4300,197.0530) .. (1366.1300,197.0470) .. controls
        (1366.3700,197.0470) and (1368.3100,196.1040) .. (1368.4400,195.9670) ..
        controls (1367.2700,195.6180) and (1366.1100,197.0060) .. (1365.2700,195.6080)
        .. controls (1365.7900,195.4580) and (1366.3200,195.4340) ..
        (1366.8500,195.5380) .. controls (1366.4800,195.3920) and (1366.0900,195.2710)
        .. (1365.7000,195.1780) .. controls (1366.7100,194.9140) and
        (1367.7400,195.4690) .. (1368.7300,195.1080) .. controls (1368.4300,195.1380)
        and (1366.2400,195.0060) .. (1368.0800,194.8190) .. controls
        (1366.0700,194.6230) and (1369.2900,194.5520) .. (1369.5900,194.5320) ..
        controls (1368.7600,194.4040) and (1368.0800,193.8830) .. (1367.2800,193.6680)
        .. controls (1368.0700,193.2640) and (1369.1300,192.8940) ..
        (1370.0300,193.0550) .. controls (1371.1900,193.2630) and (1372.0200,192.2110)
        .. (1373.1900,192.8040) .. controls (1372.7100,192.5080) and
        (1372.1800,192.3640) .. (1371.6100,192.3720) .. controls (1371.9000,191.3580)
        and (1375.2000,190.8240) .. (1375.2000,191.5800) .. controls
        (1376.0600,191.0350) and (1377.3500,191.4220) .. (1378.0800,192.0120) ..
        controls (1378.0800,191.2090) and (1378.2200,191.0690) .. (1379.0200,191.3650)
        .. controls (1378.0300,191.1690) and (1377.0500,190.7880) ..
        (1376.0300,190.7500) .. controls (1374.6000,190.7000) and (1373.5600,191.3100)
        .. (1372.1100,190.7200) .. controls (1372.7000,190.5500) and
        (1373.0300,189.9470) .. (1373.6200,189.7840) .. controls (1374.2900,189.5990)
        and (1374.5800,190.4670) .. (1375.1300,189.6390) .. controls
        (1374.6100,189.6790) and (1374.1100,189.6090) .. (1373.6200,189.4230) ..
        controls (1374.3100,189.0370) and (1375.2000,188.4730) .. (1376.0000,188.9910)
        .. controls (1375.7100,189.1350) and (1375.4200,189.2790) ..
        (1375.1300,189.4230) .. controls (1375.8600,189.2450) and (1376.7100,189.1250)
        .. (1377.4400,189.3530) .. controls (1378.1000,189.5570) and
        (1378.5900,190.4580) .. (1379.3800,190.1450) .. controls (1377.7500,190.0850)
        and (1379.5600,188.7550) .. (1380.3200,188.7780) .. controls
        (1379.0400,188.6330) and (1377.8400,189.3180) .. (1376.5700,188.8480) ..
        controls (1379.0000,188.3150) and (1375.4300,188.8280) .. (1376.8500,187.8040)
        .. controls (1377.2900,187.4850) and (1378.0400,187.8840) ..
        (1378.5200,187.8440) .. controls (1376.6700,187.5480) and (1379.3400,187.5790)
        .. (1380.0300,187.9880) .. controls (1378.1800,186.1270) and
        (1376.3900,188.1570) .. (1374.3400,188.2050) .. controls (1374.6600,187.6810)
        and (1375.2300,187.3370) .. (1375.8500,187.3410) .. controls
        (1375.2700,187.3010) and (1374.7400,187.1050) .. (1374.2700,186.7650) ..
        controls (1374.7700,186.7050) and (1375.2700,186.6750) .. (1375.7800,186.6950)
        .. controls (1373.3300,186.5950) and (1377.7200,186.1400) ..
        (1378.1500,186.1010) .. controls (1378.8000,186.0410) and (1380.3500,186.4570)
        .. (1380.6100,185.5430) .. controls (1379.4100,184.8970) and
        (1378.1200,185.4730) .. (1376.8600,185.3260) .. controls (1377.3200,184.4490)
        and (1378.2700,184.7010) .. (1379.0200,184.3180) .. controls
        (1377.7800,185.9390) and (1380.3400,183.5510) .. (1381.1200,184.0440) ..
        controls (1382.0800,184.6590) and (1381.3600,186.6710) .. (1383.0500,186.5510)
        .. controls (1382.4600,186.4330) and (1382.0200,185.9900) ..
        (1381.9000,185.3990) .. controls (1382.2500,185.6800) and (1384.6800,186.6070)
        .. (1382.6200,185.3990) .. controls (1383.4700,185.8720) and
        (1383.6600,185.7040) .. (1383.2000,184.8950) .. controls (1383.7200,185.0450)
        and (1384.2500,185.0690) .. (1384.7800,184.9650) .. controls
        (1383.9500,184.9150) and (1383.1300,184.7800) .. (1382.3300,184.5330) ..
        controls (1382.7100,184.3660) and (1383.0900,184.2210) .. (1383.4800,184.1000)
        .. controls (1382.9400,183.9700) and (1382.3900,183.8980) ..
        (1381.8300,183.8840) .. controls (1382.8900,183.8040) and (1382.8900,183.5650)
        .. (1381.8300,183.1640) .. controls (1382.9400,183.4950) and
        (1383.9200,184.1810) .. (1385.0700,184.3880) .. controls (1384.1000,184.1290)
        and (1383.1400,183.4650) .. (1382.4000,182.8040) .. controls
        (1383.5900,182.7240) and (1384.7400,182.4100) .. (1385.8900,182.8740) ..
        controls (1386.3900,182.9240) and (1386.8900,182.9540) .. (1387.3900,182.9640)
        .. controls (1387.9200,183.1100) and (1387.7700,183.5630) ..
        (1388.4500,183.5960) .. controls (1388.0800,183.5660) and (1387.8700,183.4000)
        .. (1387.8100,183.0880) .. controls (1388.0100,182.5970) and
        (1389.1300,182.7680) .. (1389.4600,182.9480) .. controls (1387.4800,182.5020)
        and (1390.5400,182.4970) .. (1390.9700,182.5880) .. controls
        (1389.4100,182.1210) and (1388.4100,182.1330) .. (1386.8300,182.3270) ..
        controls (1385.8300,182.4500) and (1384.1300,182.5830) .. (1383.2700,181.9390)
        .. controls (1384.2900,181.7510) and (1383.8800,180.6730) ..
        (1385.2900,180.4590) .. controls (1386.6400,180.2540) and (1388.0500,180.3990)
        .. (1389.3900,180.5710) .. controls (1388.8700,180.3320) and
        (1388.3500,180.1160) .. (1387.8100,179.9240) .. controls (1388.5100,179.4680)
        and (1389.3100,179.7940) .. (1390.0400,179.9240) .. controls
        (1388.7800,179.7430) and (1389.3200,179.3780) .. (1389.9400,179.0600) ..
        controls (1387.9200,179.2560) and (1390.2000,176.9500) .. (1391.8900,177.2600)
        .. controls (1389.9700,175.8180) and (1394.4000,173.4070) ..
        (1394.0500,176.6840) .. controls (1394.2500,175.3470) and (1395.7100,175.6540)
        .. (1396.7900,176.1080) .. controls (1395.7700,175.6340) and
        (1394.5200,175.6120) .. (1393.9100,174.5240) .. controls (1394.8100,174.3140)
        and (1395.5800,174.5840) .. (1396.3600,175.0170) .. controls
        (1397.2400,175.5050) and (1399.1800,175.4750) .. (1398.5900,176.5400) ..
        controls (1399.1400,176.4800) and (1399.6100,175.4600) .. (1398.8100,175.4600)
        .. controls (1397.9500,175.4600) and (1397.1400,175.6400) ..
        (1396.6400,174.7390) .. controls (1397.0700,174.2860) and (1397.5700,174.1660)
        .. (1398.1500,174.3800) .. controls (1397.6300,174.1480) and
        (1397.1100,174.1230) .. (1396.5700,174.3100) .. controls (1396.4000,172.3380)
        and (1399.2100,172.5510) .. (1400.4600,172.2940) .. controls
        (1400.3400,173.3640) and (1400.5600,174.2390) .. (1400.0200,175.2450) ..
        controls (1400.7300,174.7750) and (1401.0300,173.4380) .. (1402.1100,173.9500)
        .. controls (1400.5400,173.8600) and (1401.7400,171.5770) ..
        (1402.0100,172.6530) .. controls (1402.3300,171.8120) and (1403.4400,172.1290)
        .. (1403.5200,171.1410) .. controls (1405.4200,171.9160) and
        (1402.8200,175.3870) .. (1402.0800,176.1810) .. controls (1402.8900,175.6320)
        and (1403.9100,175.4920) .. (1404.3200,174.4830) .. controls
        (1404.7300,173.4540) and (1406.2400,174.6080) .. (1406.9100,174.6700) ..
        controls (1404.5000,173.8370) and (1405.5400,171.7710) .. (1407.5600,171.3570)
        .. controls (1407.3000,171.5530) and (1407.0600,171.7690) ..
        (1406.8300,172.0050) .. controls (1407.7600,173.1810) and (1407.8700,171.4250)
        .. (1408.8500,172.1490) .. controls (1407.1200,169.6920) and
        (1413.4200,172.8130) .. (1413.8200,172.8700) .. controls (1413.4600,172.4540)
        and (1413.0000,172.2140) .. (1412.4500,172.1490) .. controls
        (1413.3300,172.1490) and (1413.4100,172.0790) .. (1412.6700,171.9150) ..
        controls (1412.2200,171.6030) and (1412.1800,170.5560) .. (1413.3100,171.4300)
        .. controls (1413.0100,170.6180) and (1411.0800,170.6550) ..
        (1412.8100,170.2060) .. controls (1411.6200,170.5620) and (1409.1900,170.3350)
        .. (1408.2700,169.3420) .. controls (1408.8000,169.1540) and
        (1409.3100,169.2020) .. (1409.7900,169.4860) .. controls (1409.8900,169.2220)
        and (1409.9300,168.9590) .. (1410.0000,168.6940) .. controls
        (1410.5500,168.9720) and (1411.0800,169.2840) .. (1411.5900,169.6310) ..
        controls (1411.8300,167.8600) and (1413.2300,169.6510) .. (1414.1100,168.9100)
        .. controls (1413.8900,169.8510) and (1414.9000,169.9700) ..
        (1415.5500,170.0620) .. controls (1414.9900,170.0220) and (1414.6300,169.6820)
        .. (1414.5400,169.1260) .. controls (1415.5300,168.9600) and
        (1416.5900,169.3340) .. (1417.5600,169.4850) .. controls (1417.3200,170.5900)
        and (1415.7200,170.4310) .. (1414.9000,170.4930) .. controls
        (1415.9600,170.5230) and (1417.1400,170.5130) .. (1418.0700,169.9180) ..
        controls (1418.1900,171.8100) and (1420.0100,171.0420) .. (1421.1600,170.9980)
        .. controls (1421.0300,170.5850) and (1419.9600,170.7170) ..
        (1419.5100,170.2780) .. controls (1420.1900,169.9240) and (1420.8000,169.5090)
        .. (1419.4100,169.3410) .. controls (1419.7400,169.3610) and
        (1422.2000,169.1530) .. (1420.1300,168.9810) .. controls (1420.9600,169.1500)
        and (1421.4500,168.0740) .. (1422.0500,167.7170) .. controls
        (1422.9500,167.1750) and (1423.9800,167.4310) .. (1424.9600,167.3970) ..
        controls (1423.5000,166.1760) and (1426.1900,166.3260) .. (1426.7600,165.9580)
        .. controls (1426.0400,165.5900) and (1425.2000,165.6610) ..
        (1424.5300,165.1660) .. controls (1425.3300,164.5030) and (1426.1600,165.5760)
        .. (1426.9000,164.7330) .. controls (1424.8200,164.3180) and
        (1428.0200,163.9510) .. (1428.7800,164.1120) .. controls (1428.7800,164.1220)
        and (1431.7200,166.0750) .. (1430.2900,164.2290) .. controls
        (1431.3200,164.1290) and (1432.2900,165.1290) .. (1433.3100,164.5890) ..
        controls (1432.6900,166.1590) and (1430.3800,166.2630) .. (1429.3500,167.4690)
        .. controls (1429.9300,167.3260) and (1430.2700,167.6040) ..
        (1430.2900,168.1890) .. controls (1429.9300,168.2290) and (1428.7700,169.3010)
        .. (1428.8500,170.0610) .. controls (1429.3500,169.7780) and
        (1430.3200,170.3300) .. (1430.5200,170.0010) .. controls (1430.7300,169.6430)
        and (1431.0200,169.3720) .. (1431.4000,169.1860) .. controls
        (1431.8500,168.8710) and (1431.1800,168.6590) .. (1431.4000,168.3350) ..
        controls (1432.6100,166.8490) and (1435.5400,164.5860) .. (1437.3700,164.0870)
        .. controls (1437.6900,165.2880) and (1437.7600,166.0020) ..
        (1436.2900,166.1030) .. controls (1437.6800,165.8600) and (1437.5900,167.5100)
        .. (1437.1600,168.3350) .. controls (1437.7700,168.3950) and
        (1437.8400,168.0800) .. (1438.1700,167.7060) .. controls (1438.6500,167.1630)
        and (1439.5100,167.5640) .. (1440.1100,167.5430) .. controls
        (1439.9200,167.2810) and (1439.7300,167.0170) .. (1439.5400,166.7510) ..
        controls (1440.0500,166.6510) and (1440.5600,166.6810) .. (1441.0500,166.8210)
        .. controls (1440.4900,166.6990) and (1440.1200,166.2480) ..
        (1440.1100,165.6700) .. controls (1440.9700,165.7300) and (1441.6200,164.8650)
        .. (1442.4900,165.2370) .. controls (1441.9100,164.5230) and
        (1440.9900,164.6220) .. (1440.1800,164.4460) .. controls (1440.7300,164.3560)
        and (1445.2400,161.9030) .. (1445.5900,163.5810) .. controls
        (1445.6900,163.8750) and (1447.0400,163.9330) .. (1447.3000,164.1870) ..
        controls (1448.0400,164.8940) and (1444.3400,165.3330) .. (1444.1400,165.4540)
        .. controls (1444.6900,165.3940) and (1445.2000,165.5140) ..
        (1445.6600,165.8130) .. controls (1444.8800,166.0200) and (1444.1500,166.3780)
        .. (1443.3500,166.5340) .. controls (1444.3500,166.5040) and
        (1445.7500,165.6600) .. (1446.6600,166.3890) .. controls (1445.9300,166.8840)
        and (1445.0900,167.1670) .. (1444.2900,167.5410) .. controls
        (1445.2500,167.6010) and (1446.2300,167.2270) .. (1447.1700,167.4710) ..
        controls (1446.6600,167.7710) and (1446.3200,168.3030) .. (1446.5200,168.9100)
        .. controls (1446.4200,167.8980) and (1447.4200,167.3110) ..
        (1448.3200,167.3980) .. controls (1446.4600,167.4180) and (1448.6100,165.2120)
        .. (1449.2200,164.8460) .. controls (1450.0300,164.3580) and
        (1453.0600,164.8160) .. (1452.2100,166.2450) .. controls (1452.9300,166.0300)
        and (1454.5600,165.2060) .. (1454.8100,166.4620) .. controls
        (1455.8300,165.4260) and (1458.3700,166.8900) .. (1456.6700,167.2540) ..
        controls (1458.2300,167.1360) and (1460.5500,166.9190) .. (1461.8200,168.1930)
        .. controls (1462.6300,169.0190) and (1459.9800,169.2990) ..
        (1459.6100,169.3740) .. controls (1457.9400,169.7090) and (1457.0000,170.7070)
        .. (1455.1300,170.4430) .. controls (1453.6300,170.2300) and
        (1450.7200,169.1370) .. (1449.4000,170.2780) .. controls (1450.3300,170.3380)
        and (1451.2400,170.4700) .. (1452.1500,170.6320) .. controls
        (1452.7900,170.7460) and (1456.0700,170.8400) .. (1454.0800,171.5730) ..
        controls (1454.9300,171.6840) and (1456.8600,172.1580) .. (1454.8700,173.0130)
        .. controls (1455.5500,172.9330) and (1456.2200,172.8330) ..
        (1456.9000,172.7250) .. controls (1457.0000,173.3070) and (1457.3200,173.3280)
        .. (1457.9000,173.3010) .. controls (1457.7900,172.9000) and
        (1457.7400,172.4910) .. (1457.7500,172.0760) .. controls (1458.5300,172.1160)
        and (1459.4300,172.2160) .. (1459.7000,173.0850) .. controls
        (1460.0800,171.7750) and (1461.9100,172.2480) .. (1462.2500,173.2680) ..
        controls (1462.9500,175.3550) and (1458.6700,174.0080) .. (1458.2500,173.5170)
        .. controls (1459.0200,174.9830) and (1457.3300,175.4480) ..
        (1456.2700,175.6280) .. controls (1455.7200,175.7180) and (1454.1300,175.7760)
        .. (1454.0500,176.4050) .. controls (1454.0500,176.8410) and
        (1454.3000,177.3410) .. (1453.1300,177.9780) .. controls (1452.5800,178.2800)
        and (1452.0700,177.9880) .. (1451.5900,177.6990) .. controls
        (1450.6100,177.0990) and (1451.8900,176.4900) .. (1452.2800,176.1090) ..
        controls (1453.3200,175.1070) and (1453.7900,173.6930) .. (1451.8600,173.1890)
        .. controls (1450.3800,172.8020) and (1448.8700,172.5850) ..
        (1447.4400,172.0230) .. controls (1445.8000,171.3820) and (1444.5800,169.7830)
        .. (1442.8400,170.9000) .. controls (1440.0000,172.7230) and
        (1435.7500,170.7260) .. (1434.7200,174.2750) .. controls (1434.4900,175.0930)
        and (1434.3100,175.8940) .. (1434.2200,176.7450) .. controls
        (1434.2200,177.2800) and (1434.6800,178.1930) .. (1434.2200,178.6530) ..
        controls (1433.6500,179.1590) and (1433.0400,178.9020) .. (1432.4200,179.2080)
        .. controls (1431.7900,179.5150) and (1431.4600,180.1850) ..
        (1431.0600,180.7120) .. controls (1430.1000,181.9490) and (1428.3400,180.5140)
        .. (1427.2000,180.2120) .. controls (1426.4200,180.0090) and
        (1425.6400,179.8510) .. (1424.8700,179.6200) .. controls (1423.9200,179.3360)
        and (1423.8800,180.1110) .. (1423.1700,180.4280) .. controls
        (1420.9900,181.4120) and (1418.6800,181.2170) .. (1416.3800,180.2640) ..
        controls (1415.4500,179.8800) and (1413.7800,178.1210) .. (1412.9100,177.4520)
        .. controls (1411.2900,176.2120) and (1409.9200,175.9690) ..
        (1408.1200,176.8990) .. controls (1408.3600,177.1210) and (1408.6000,177.3370)
        .. (1408.8400,177.5470) .. controls (1407.4100,178.3450) and
        (1405.0200,177.5570) .. (1403.4400,178.2670) .. controls (1405.5900,179.1400)
        and (1403.8900,180.8230) .. (1402.6500,181.5800) .. controls
        (1403.1700,181.6970) and (1403.6800,181.8650) .. (1404.1600,182.0840) ..
        controls (1401.7200,183.9530) and (1398.7700,181.7390) .. (1396.2500,181.9270)
        .. controls (1394.9900,182.0170) and (1394.1100,181.1770) ..
        (1392.8300,181.6670) .. controls (1391.9100,182.0160) and (1393.0200,183.4450)
        .. (1392.8300,184.1720) .. controls (1392.2900,186.7000) and
        (1389.0900,184.7220) .. (1387.5200,185.2450) .. controls (1384.9300,186.1080)
        and (1383.9700,188.7400) .. (1381.5200,189.8610) .. controls
        (1382.1100,190.3710) and (1383.6500,191.2530) .. (1383.4600,192.2120) ..
        controls (1383.3100,193.0200) and (1380.3600,194.7980) .. (1379.6700,195.5630)
        .. controls (1379.1900,196.0960) and (1378.8400,196.2750) ..
        (1378.2300,196.6090) .. controls (1377.5100,197.0050) and (1378.6200,197.8290)
        .. (1378.2300,198.3640) .. controls (1377.3200,199.5370) and
        (1374.2700,199.5580) .. (1372.9700,199.5090) .. controls (1373.1900,200.2900)
        and (1373.8700,205.3310) .. (1372.8500,205.8850) .. controls
        (1372.0400,206.3200) and (1371.7000,207.6900) .. (1370.9500,208.3540) ..
        controls (1369.9500,209.2350) and (1369.0000,210.2130) .. (1368.1500,211.2450)
        .. controls (1369.5600,211.7130) and (1372.1400,212.5990) ..
        (1371.0100,214.6420) .. controls (1370.2200,216.0620) and (1366.3000,215.0100)
        .. (1364.9000,215.2350) .. controls (1363.6100,215.4430) and
        (1359.8700,217.4830) .. (1359.8000,219.0280) .. controls (1359.8000,219.8370)
        and (1359.0200,220.4690) .. (1359.0800,221.1960) .. controls
        (1359.0800,221.7680) and (1360.3700,223.3260) .. (1359.9000,223.6500) ..
        controls (1358.8900,224.3430) and (1359.4800,226.3140) .. (1360.0000,227.3660)
        .. controls (1361.0200,229.4590) and (1359.8500,230.8260) ..
        (1360.1000,232.8950) .. controls (1360.2400,234.2090) and (1361.8500,234.6440)
        .. (1362.8500,235.0310) .. controls (1363.3500,235.2210) and
        (1364.1300,235.5000) .. (1364.3000,236.0700) .. controls (1364.4200,236.4340)
        and (1363.5700,238.5790) .. (1363.1400,238.5770) .. controls
        (1361.8200,238.5770) and (1360.5000,238.9340) .. (1361.0500,240.4780) ..
        controls (1361.3800,241.4000) and (1362.2700,241.9530) .. (1362.6400,242.8530)
        .. controls (1363.0700,243.9090) and (1362.1300,244.4350) ..
        (1362.2400,245.4470) .. controls (1362.3400,246.3070) and (1361.3600,247.0690)
        .. (1360.6600,247.3360) .. controls (1359.5100,247.7800) and
        (1358.4100,247.2190) .. (1358.5200,248.5770) .. controls (1358.5200,249.3080)
        and (1358.1200,249.7890) .. (1357.7900,250.3450) .. controls
        (1357.3800,251.0220) and (1358.0900,251.9970) .. (1358.0200,252.7540) ..
        controls (1357.9200,253.4780) and (1357.6100,256.0250) .. (1356.4400,255.8150)
        .. controls (1355.9100,255.7150) and (1355.5300,254.8130) ..
        (1355.2400,254.4540) .. controls (1354.9000,254.0240) and (1354.3300,254.1020)
        .. (1353.8400,253.8490) .. controls (1352.5400,253.1900) and
        (1351.6000,253.2550) .. (1351.1400,251.7210) .. controls (1350.9300,251.0390)
        and (1350.8200,250.3120) .. (1350.8300,249.5990) .. controls
        (1350.8300,249.1570) and (1351.3100,247.2660) .. (1351.4800,248.9750) ..
        controls (1352.2200,247.5960) and (1350.3400,247.1220) .. (1350.2000,248.5580)
        .. controls (1350.1000,249.3790) and (1351.1200,250.1190) ..
        (1350.2000,250.7750) .. controls (1350.0100,250.5390) and (1349.8200,250.2980)
        .. (1349.6300,250.0550) .. controls (1349.5100,250.6680) and
        (1349.0900,250.8170) .. (1348.5500,250.5590) .. controls (1349.6000,251.5220)
        and (1349.8000,252.1460) .. (1349.4100,253.5110) .. controls
        (1349.4100,252.0610) and (1349.3100,253.2880) .. (1348.8500,253.6980) ..
        controls (1348.4200,254.0470) and (1347.9000,254.2330) .. (1347.4400,254.5390)
        .. controls (1346.7000,255.0350) and (1347.2900,255.4790) ..
        (1346.1900,254.9470) .. controls (1345.5200,254.6280) and (1344.9100,254.2160)
        .. (1344.2200,253.9430) .. controls (1346.1200,254.7640) and
        (1343.8100,256.1090) .. (1342.7100,256.0320) .. controls (1342.8800,256.2710)
        and (1343.0500,256.5110) .. (1343.2200,256.7520) .. controls
        (1342.6100,256.9540) and (1341.9900,257.0510) .. (1341.3400,257.0400) ..
        controls (1341.4700,257.3030) and (1341.5900,257.5660) .. (1341.7100,257.8310)
        .. controls (1340.2700,258.0470) and (1339.7600,259.5330) ..
        (1338.6000,260.2260) .. controls (1337.1900,261.0750) and (1335.6600,261.4670)
        .. (1334.1300,262.0130) .. controls (1333.4800,262.2420) and
        (1332.6400,262.8540) .. (1331.9400,262.8490) .. controls (1331.2400,262.8490)
        and (1330.6000,262.4910) .. (1329.8900,262.4740) .. controls
        (1328.7600,262.4440) and (1326.7400,262.8820) .. (1325.9400,261.7920) ..
        controls (1326.4100,261.3580) and (1326.9300,261.0220) .. (1327.5200,260.7840)
        .. controls (1324.9900,262.3420) and (1316.9300,257.2840) ..
        (1320.3900,255.3840) .. controls (1320.1600,255.2000) and (1319.9200,255.0320)
        .. (1319.6700,254.8800) .. controls (1321.1700,254.7800) and
        (1322.2800,256.1830) .. (1323.7800,256.1040) .. controls (1323.5100,255.9000)
        and (1323.2500,255.6840) .. (1322.9900,255.4570) .. controls
        (1323.9300,254.9110) and (1325.0500,254.7910) .. (1326.0800,254.5200) ..
        controls (1324.8900,254.6200) and (1323.6800,254.8620) .. (1322.7000,255.6000)
        .. controls (1322.8400,254.9690) and (1322.4800,254.4090) ..
        (1321.9000,254.1600) .. controls (1322.4100,254.0070) and (1322.9100,253.8630)
        .. (1323.4200,253.7280) .. controls (1321.5700,253.3580) and
        (1325.0400,252.4660) .. (1325.6500,252.3600) .. controls (1325.1400,252.3400)
        and (1324.6400,252.4100) .. (1324.1600,252.5790) .. controls
        (1323.2700,252.8400) and (1322.8200,252.5090) .. (1324.0600,252.3600) ..
        controls (1323.5500,252.3900) and (1323.0400,252.3400) .. (1322.5400,252.2160)
        .. controls (1323.6000,251.5340) and (1324.5600,250.7840) ..
        (1325.7800,250.4160) .. controls (1325.0700,250.5880) and (1324.4200,249.9030)
        .. (1324.0100,250.6770) .. controls (1323.7100,251.2710) and
        (1322.7000,251.8230) .. (1322.1100,252.0730) .. controls (1322.1100,251.5090)
        and (1322.4900,251.1670) .. (1323.0500,251.1350) .. controls
        (1322.2600,251.1050) and (1321.3900,251.0850) .. (1320.7400,251.6390) ..
        controls (1321.3100,251.3720) and (1321.6500,251.5990) .. (1321.6800,252.2150)
        .. controls (1321.1400,252.1550) and (1320.6300,252.2750) ..
        (1320.1700,252.5760) .. controls (1320.1700,252.0230) and (1320.1700,251.4720)
        .. (1320.1700,250.9190) .. controls (1319.8300,251.0320) and
        (1319.5200,251.2000) .. (1319.2300,251.4230) .. controls (1321.1200,251.5840)
        and (1318.5600,253.8200) .. (1319.0900,251.7830) .. controls
        (1318.9700,253.3490) and (1317.9700,251.8630) .. (1318.0000,251.2440) ..
        controls (1318.0000,250.3510) and (1318.8400,249.5200) .. (1319.6600,249.2630)
        .. controls (1319.5600,249.9580) and (1319.4300,250.8720) ..
        (1318.5100,250.8470) .. controls (1319.2800,251.3290) and (1319.5700,250.7870)
        .. (1319.7800,250.1240) .. controls (1320.0600,249.2340) and
        (1321.4000,249.9800) .. (1322.1100,249.6230) .. controls (1320.1000,249.3740)
        and (1323.0700,248.9670) .. (1323.4800,248.6150) .. controls
        (1322.6400,249.1090) and (1321.5200,248.8230) .. (1320.7400,248.3260) ..
        controls (1321.4400,247.4260) and (1322.8400,246.0790) .. (1324.0600,246.0950)
        .. controls (1322.1400,245.5230) and (1325.7500,243.9780) ..
        (1326.3600,243.5760) .. controls (1326.6900,244.3680) and (1326.1100,245.0760)
        .. (1325.9300,245.8060) .. controls (1327.1500,244.4490) and
        (1327.5000,243.2440) .. (1329.5300,243.0720) .. controls (1327.9800,242.8160)
        and (1326.2400,243.1220) .. (1324.8000,243.6990) .. controls
        (1324.3700,243.8710) and (1322.9500,244.9110) .. (1322.6900,245.3570) ..
        controls (1320.7600,248.6760) and (1321.7700,245.1520) .. (1320.2400,245.3770)
        .. controls (1320.4000,244.9040) and (1320.5200,244.4240) ..
        (1320.6000,243.9370) .. controls (1320.3900,244.4230) and (1319.6500,245.9680)
        .. (1318.8500,245.6020) .. controls (1318.2000,245.3060) and
        (1318.4500,244.1010) .. (1317.6500,243.9370) .. controls (1318.1900,243.7900)
        and (1318.6200,243.3820) .. (1318.8000,242.8570) .. controls
        (1319.5200,244.9620) and (1321.4900,242.4520) .. (1321.0300,241.0570) ..
        controls (1320.0500,241.3020) and (1319.5500,242.4960) .. (1318.4800,242.4960)
        .. controls (1317.4300,242.4960) and (1317.4000,240.9290) ..
        (1316.5000,240.6250) .. controls (1317.3700,240.6250) and (1318.4000,241.0060)
        .. (1318.9400,241.7050) .. controls (1318.8400,241.0560) and
        (1318.6500,240.0090) .. (1319.6600,240.0490) .. controls (1318.7300,239.8230)
        and (1317.0800,241.2290) .. (1316.8500,239.5450) .. controls
        (1317.5100,240.0310) and (1317.6300,240.0280) .. (1317.9300,239.2570) ..
        controls (1317.1600,239.4580) and (1316.5600,238.2850) .. (1318.1500,238.5490)
        .. controls (1319.8400,238.8280) and (1320.9100,238.1630) ..
        (1322.5400,238.1050) .. controls (1323.7200,238.0650) and (1325.2600,238.8520)
        .. (1326.3500,238.1350) .. controls (1327.5000,237.3700) and
        (1329.7600,239.1510) .. (1328.1600,239.6170) .. controls (1328.6700,239.3250)
        and (1329.2000,239.2770) .. (1329.7400,239.4720) .. controls
        (1328.1000,238.2810) and (1332.0300,237.4730) .. (1332.7000,237.4560) ..
        controls (1330.5400,237.1860) and (1331.3500,236.3240) .. (1332.5500,235.2240)
        .. controls (1331.5700,235.6260) and (1330.3300,236.6200) ..
        (1331.2600,237.7440) .. controls (1330.4800,237.6840) and (1329.7300,238.0930)
        .. (1328.9500,237.8140) .. controls (1329.2000,237.5790) and
        (1329.4700,237.3630) .. (1329.7400,237.1670) .. controls (1329.0200,237.6300)
        and (1325.4700,237.8020) .. (1327.0800,236.4470) .. controls
        (1326.2000,236.5790) and (1326.3500,237.3260) .. (1325.8400,237.8340) ..
        controls (1325.1100,238.5740) and (1324.0500,237.8040) .. (1323.2600,237.6810)
        .. controls (1322.3500,237.5370) and (1320.7900,238.0430) ..
        (1319.9200,238.3030) .. controls (1318.9900,238.5790) and (1318.2700,237.7260)
        .. (1317.4300,237.5270) .. controls (1318.7900,237.5170) and
        (1318.0100,237.0080) .. (1317.4300,236.6630) .. controls (1318.3500,236.2330)
        and (1319.4500,236.0910) .. (1320.4500,236.1590) .. controls
        (1319.4700,235.8490) and (1318.3700,236.1990) .. (1317.4300,236.5190) ..
        controls (1318.0700,235.6750) and (1317.9100,235.4590) ..
        (1316.9300,235.8680);

        % path6796
        \path[country]
        (1317.0800,241.9900) .. controls (1316.8400,241.8460) and
        (1316.6000,241.7020) .. (1316.3600,241.5580) .. controls (1316.9200,241.2220)
        and (1317.4800,241.4780) .. (1317.8000,241.9900) .. controls
        (1317.5600,241.9900) and (1317.3200,241.9900) .. (1317.0800,241.9900);

        % path6798
        \path[country]
        (1317.8700,232.1300) .. controls (1318.1300,232.2500) and
        (1318.4000,232.3690) .. (1318.6600,232.4890) .. controls (1317.8700,232.6180)
        and (1317.0500,232.5390) .. (1316.2900,232.2730) .. controls
        (1316.7800,231.8970) and (1317.3100,231.8490) .. (1317.8700,232.1300);

        % path6800
        \path[country]
        (1320.2500,243.4300) .. controls (1319.7100,243.2630) and
        (1319.2300,242.9990) .. (1318.8100,242.6380) .. controls (1319.5400,242.2310)
        and (1320.3900,242.0450) .. (1321.0400,241.4860) .. controls
        (1321.1700,242.2530) and (1321.2300,243.2250) .. (1320.2500,243.4300);

        % path6802
        \path[country]
        (1323.7800,251.2800) .. controls (1324.0700,249.9310) and
        (1324.9000,250.6440) .. (1325.8600,250.4160) .. controls (1325.1400,250.6310)
        and (1324.3700,250.7760) .. (1323.7800,251.2800);

        % path6806
        \path[country]
        (1334.0000,223.2700) .. controls (1334.1000,223.0540) and
        (1334.1900,222.8380) .. (1334.2900,222.6230) .. controls (1334.5400,223.1930)
        and (1334.2900,222.9560) .. (1334.0000,223.2700);

        % path6812
        \path[country]
        (1456.9000,171.7200) .. controls (1455.4700,171.3660) and
        (1456.2000,173.4610) .. (1457.7700,172.1520) .. controls (1457.0900,172.5480)
        and (1456.8000,172.4040) .. (1456.9000,171.7200);

\end{scope}

    
    
    % //////// POLAND //////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (314.3784,208.1939) .. controls (314.3784,206.4769) and
    (316.8884,206.0279) .. (315.9484,204.0269) .. controls (315.6184,203.3339) and
    (314.8584,202.3009) .. (315.1484,201.4629) .. controls (315.2784,201.0749) and
    (316.6184,201.5709) .. (316.8984,201.5699) .. controls (316.7584,201.0039) and
    (316.8984,200.4999) .. (317.2584,200.0579) .. controls (317.1584,200.1769) and
    (317.1084,200.2969) .. (317.0384,200.4179) .. controls (316.5984,200.0429) and
    (316.0984,199.8269) .. (315.5284,199.7699) .. controls (315.8284,200.5339) and
    (314.6484,200.1009) .. (314.5884,199.4099) .. controls (316.2484,200.0329) and
    (318.8984,198.5969) .. (320.4084,197.9919) .. controls (322.2084,197.2649) and
    (326.6084,197.4629) .. (327.7384,195.9579) .. controls (329.1284,194.1199) and
    (332.3884,193.2729) .. (334.5784,192.6959) .. controls (337.3084,191.9739) and
    (341.0684,191.3939) .. (343.3884,193.3619) .. controls (342.7584,192.9309) and
    (342.0184,192.4899) .. (341.2284,192.7859) .. controls (342.1784,193.6789) and
    (342.4184,195.3949) .. (343.7984,195.7949) .. controls (345.4684,196.2759) and
    (347.6984,195.5539) .. (349.2984,195.0899) .. controls (348.5984,195.5139) and
    (347.7384,195.6249) .. (347.0484,196.0909) .. controls (346.0584,196.7609) and
    (348.1584,196.3769) .. (348.5384,196.1809) .. controls (351.1084,194.8659) and
    (353.3684,195.9229) .. (356.4284,195.8799) .. controls (360.4684,195.8199) and
    (366.1584,196.8209) .. (370.1684,196.2299) .. controls (373.1684,195.7899) and
    (373.8784,197.1929) .. (374.6284,199.9359) .. controls (375.3984,202.7559) and
    (378.8684,206.0699) .. (377.8684,209.1699) .. controls (377.3684,210.7389) and
    (375.3884,210.1759) .. (374.5584,211.3789) .. controls (373.7184,212.5829) and
    (372.9984,213.4949) .. (375.0284,213.8709) .. controls (378.2784,214.4729) and
    (375.5684,217.6559) .. (376.5384,219.4109) .. controls (377.5484,221.2579) and
    (377.9084,223.4719) .. (380.6884,224.8229) .. controls (380.2884,225.0269) and
    (379.8784,225.2189) .. (379.4684,225.3989) .. controls (380.6984,226.4869) and
    (381.0184,227.7219) .. (379.2684,228.3719) .. controls (377.4984,229.0249) and
    (375.9184,230.7349) .. (374.7084,232.1189) .. controls (373.6684,233.3139) and
    (371.4384,234.8699) .. (372.1284,236.7169) .. controls (372.4184,237.4899) and
    (372.3284,238.3109) .. (372.6184,239.0779) .. controls (372.8484,239.6869) and
    (373.5384,239.4779) .. (373.4184,240.3029) .. controls (372.2184,239.4579) and
    (370.4184,239.4729) .. (369.0584,238.9899) .. controls (367.7184,238.5139) and
    (367.0684,237.4899) .. (365.6884,237.1219) .. controls (364.3384,236.7589) and
    (362.8284,236.5469) .. (361.4984,237.1019) .. controls (359.7884,237.8169) and
    (359.5884,237.1619) .. (357.9284,236.9619) .. controls (356.6484,236.8049) and
    (356.1784,237.0519) .. (355.2484,237.8469) .. controls (354.8384,238.1889) and
    (354.3184,238.6259) .. (353.7584,238.6729) .. controls (352.8084,238.7529) and
    (353.1184,237.7419) .. (352.7484,237.2809) .. controls (352.3484,236.7849) and
    (351.4284,236.3739) .. (350.9184,235.7619) .. controls (350.0984,234.7759) and
    (348.0984,236.9399) .. (347.2084,237.0649) .. controls (347.4384,236.2909) and
    (344.1284,232.8159) .. (343.0184,232.5119) .. controls (341.7784,232.1719) and
    (341.1684,231.6589) .. (339.9584,232.0439) .. controls (338.6884,232.4449) and
    (338.5684,230.3259) .. (338.7084,229.5759) .. controls (336.6884,230.1829) and
    (334.9584,228.7669) .. (333.0984,228.2799) .. controls (333.0984,228.8929) and
    (333.4184,229.3969) .. (333.8884,229.7919) .. controls (333.1084,230.3139) and
    (331.6884,231.7409) .. (330.8084,230.5209) .. controls (330.0984,229.5239) and
    (329.6684,228.8579) .. (328.4184,228.4239) .. controls (328.7484,228.1379) and
    (329.9884,227.4759) .. (329.7184,226.8869) .. controls (329.3684,226.1159) and
    (327.6284,226.4439) .. (327.1884,226.9069) .. controls (327.0884,224.9349) and
    (323.4984,226.3489) .. (322.7384,225.2089) .. controls (322.0184,224.1239) and
    (322.7384,224.3049) .. (321.1084,223.6449) .. controls (319.8584,223.1359) and
    (320.8784,225.0589) .. (319.2684,224.7469) .. controls (320.3884,221.9529) and
    (321.1284,221.0569) .. (318.9884,219.6009) .. controls (318.0584,218.9739) and
    (318.7884,218.2689) .. (318.0684,217.6249) .. controls (317.1184,216.7859) and
    (318.1684,216.3939) .. (318.3284,215.4989) .. controls (318.4284,214.9489) and
    (318.2084,213.9569) .. (318.1384,213.3979) .. controls (318.0384,212.8349) and
    (316.9084,212.9759) .. (317.1284,212.0359) .. controls (317.2784,211.4199) and
    (318.0484,210.8089) .. (317.2284,210.3069) .. controls (316.2184,209.7029) and
    (315.2584,208.9979) .. (314.3984,208.1889);
    
    
    % //////// PORTUGAL ////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path3446
        \path[country]
        (1210.2300,419.6900) .. controls (1210.1300,419.4500) and (1210.0800,419.2110)
        .. (1210.0100,418.9700) .. controls (1212.3300,418.7940) and
        (1213.1300,415.0280) .. (1213.7900,413.3160) .. controls (1214.3800,411.8140)
        and (1214.7100,410.1510) .. (1215.1400,408.5910) .. controls
        (1215.2600,408.1690) and (1215.6600,408.0970) .. (1215.9200,407.8040) ..
        controls (1216.1300,407.5590) and (1216.1500,405.9640) .. (1215.5600,407.6660)
        .. controls (1215.8200,405.8230) and (1216.2800,404.7230) ..
        (1215.8800,402.8620) .. controls (1215.7500,402.2530) and (1214.8200,399.0530)
        .. (1216.0600,399.0250) .. controls (1214.2600,399.5730) and
        (1215.7000,396.9150) .. (1216.6600,396.5050) .. controls (1217.7500,396.0410)
        and (1219.2800,395.9810) .. (1220.1700,395.1370) .. controls
        (1220.0600,395.7380) and (1220.3300,396.0860) .. (1220.9600,396.0010) ..
        controls (1220.5600,396.2850) and (1219.2000,398.1070) .. (1220.4800,398.0730)
        .. controls (1221.5300,398.0430) and (1222.6200,397.2250) ..
        (1223.6600,397.3980) .. controls (1225.0300,397.6250) and (1225.5500,398.1690)
        .. (1226.9300,397.4380) .. controls (1227.3800,395.9640) and
        (1229.4500,397.0930) .. (1230.6800,396.9700) .. controls (1232.1100,396.8260)
        and (1231.3000,397.8620) .. (1231.4000,398.6340) .. controls
        (1231.5000,399.1340) and (1233.1600,399.4360) .. (1233.5400,399.7830) ..
        controls (1234.3700,400.5410) and (1229.1500,404.6730) .. (1228.4700,404.8390)
        .. controls (1229.0600,404.6960) and (1228.8000,408.5450) ..
        (1228.8100,408.8280) .. controls (1228.8100,409.3590) and (1229.0600,410.3370)
        .. (1228.8100,410.8300) .. controls (1228.4700,411.4840) and
        (1227.4900,411.2220) .. (1227.2700,412.0640) .. controls (1227.1500,412.5640)
        and (1228.9300,414.5910) .. (1227.3700,415.1130) .. controls
        (1226.7600,415.3110) and (1227.1100,416.0980) .. (1226.6100,416.3950) ..
        controls (1225.8700,416.8270) and (1224.0100,416.6630) .. (1223.2300,416.4450)
        .. controls (1223.4900,417.0270) and (1224.0400,417.3700) ..
        (1224.4900,417.7880) .. controls (1225.0700,418.3250) and (1224.5900,418.9140)
        .. (1224.9300,419.6030) .. controls (1225.3300,420.3140) and
        (1226.8900,421.4360) .. (1226.6200,422.2760) .. controls (1226.1600,423.7180)
        and (1224.5800,424.4430) .. (1224.1700,425.9020) .. controls
        (1223.8200,427.1840) and (1225.0300,429.5700) .. (1226.6200,429.0460) ..
        controls (1225.9300,430.7000) and (1224.8000,430.2910) .. (1223.9700,431.9550)
        .. controls (1223.5600,432.7770) and (1222.7700,433.3260) ..
        (1222.3900,434.1690) .. controls (1221.8700,435.3070) and (1223.0200,436.4290)
        .. (1222.3900,437.5690) .. controls (1221.5000,439.2820) and
        (1218.9300,439.4860) .. (1217.4300,438.8730) .. controls (1215.6200,438.1360)
        and (1213.2100,438.0570) .. (1211.6000,439.4140) .. controls
        (1211.3700,438.6750) and (1211.9100,437.6830) .. (1212.2100,437.0430) ..
        controls (1212.6900,436.0180) and (1212.6200,434.7070) .. (1213.0900,433.8070)
        .. controls (1213.6400,432.7440) and (1212.9000,431.9910) ..
        (1212.9600,430.9300) .. controls (1213.0600,429.3670) and (1214.0100,428.3060)
        .. (1213.0600,426.7410) .. controls (1213.5800,428.3890) and
        (1214.2000,426.5820) .. (1214.0700,425.9500) .. controls (1213.7500,426.7140)
        and (1211.3600,426.9580) .. (1210.5400,427.2460) .. controls
        (1210.9500,426.5500) and (1210.6900,425.7550) .. (1210.9000,425.0140) ..
        controls (1211.1900,425.1270) and (1211.4700,425.2470) .. (1211.7600,425.3740)
        .. controls (1211.8600,424.8200) and (1212.2500,424.7140) ..
        (1212.6400,424.4630) .. controls (1213.2000,424.0980) and (1212.5400,423.1290)
        .. (1212.5400,422.6380) .. controls (1212.0300,423.3130) and
        (1210.3100,425.7570) .. (1209.2500,424.9550) .. controls (1207.8900,423.9300)
        and (1210.2300,420.9830) .. (1210.2400,419.6870);

    \end{scope}
    
    
    % //////// ROMANIA /////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (357.2184,264.7139) .. controls (357.9984,264.1779) and
    (358.5984,264.2229) .. (359.3884,264.4269) .. controls (360.1484,264.6249) and
    (360.1984,263.6339) .. (360.8184,263.4179) .. controls (361.4984,263.1809) and
    (362.2284,263.3579) .. (362.9084,263.1389) .. controls (363.8984,262.8289) and
    (363.7084,261.6339) .. (364.1784,260.8939) .. controls (364.6184,260.1899) and
    (365.2084,259.5989) .. (365.7084,258.9359) .. controls (366.3484,258.0829) and
    (366.2684,257.3199) .. (366.8384,256.5489) .. controls (367.3484,255.8689) and
    (367.9284,255.0699) .. (368.2084,254.2569) .. controls (368.5284,253.3109) and
    (368.1084,252.8709) .. (368.8284,252.5129) .. controls (369.4884,252.1599) and
    (369.6884,251.9209) .. (370.1484,251.3339) .. controls (370.8684,250.4159) and
    (372.1784,251.0699) .. (373.0484,250.3469) .. controls (373.7584,249.7499) and
    (374.2484,248.9119) .. (375.0384,248.3979) .. controls (376.1184,247.6859) and
    (377.3484,248.5859) .. (378.4584,248.7309) .. controls (379.5184,248.8689) and
    (380.5584,249.0909) .. (381.6184,249.1989) .. controls (382.8884,249.3279) and
    (384.4884,248.7689) .. (385.6284,249.5049) .. controls (387.7884,250.8989) and
    (387.9884,251.7399) .. (389.9984,249.8219) .. controls (391.2584,248.6209) and
    (393.8784,249.2319) .. (395.4684,248.9649) .. controls (396.5184,248.7889) and
    (396.3284,248.0269) .. (396.9284,247.3639) .. controls (397.5784,246.6499) and
    (398.8184,246.6039) .. (399.7084,246.7049) .. controls (401.6884,246.9299) and
    (402.8184,249.0169) .. (403.6484,250.5939) .. controls (404.5684,252.3419) and
    (405.8684,253.8659) .. (407.2784,255.2189) .. controls (409.3384,257.1969) and
    (410.2984,258.6549) .. (411.1284,261.3739) .. controls (411.4284,262.3689) and
    (410.8384,263.3779) .. (410.6084,264.3179) .. controls (410.3584,265.3989) and
    (410.8284,266.5469) .. (410.9184,267.6379) .. controls (411.0484,269.4509) and
    (411.4884,270.1889) .. (412.9184,271.1979) .. controls (413.4684,271.5849) and
    (414.7784,272.5299) .. (415.6084,272.0529) .. controls (416.5184,271.5239) and
    (421.1884,268.9419) .. (421.8284,271.6619) .. controls (422.6584,275.1149) and
    (420.8084,276.4039) .. (417.6184,276.3779) .. controls (418.0084,276.0639) and
    (418.3484,274.1689) .. (417.5184,274.1969) .. controls (416.5284,274.2269) and
    (417.0584,276.5159) .. (416.3284,277.0979) .. controls (416.7984,276.9869) and
    (417.2784,276.9149) .. (417.7684,276.8819) .. controls (417.0384,277.1979) and
    (415.7484,277.2949) .. (416.6184,278.2489) .. controls (416.8784,278.0269) and
    (417.1184,277.7869) .. (417.3384,277.5289) .. controls (417.0284,278.6679) and
    (415.8084,279.2929) .. (415.6084,280.4809) .. controls (415.3884,281.7479) and
    (416.3484,283.8229) .. (415.5084,285.0059) .. controls (415.0284,284.5979) and
    (413.9584,285.0459) .. (413.4784,284.7989) .. controls (413.0984,284.6009) and
    (411.7084,283.5839) .. (410.9584,282.8999) .. controls (409.9384,282.5839) and
    (408.9684,283.0699) .. (407.5984,282.4119) .. controls (406.4884,281.8809) and
    (404.5884,281.1879) .. (402.4584,282.0489) .. controls (397.7884,282.5089) and
    (396.7784,285.1359) .. (394.6384,285.6209) .. controls (393.3284,285.9189) and
    (391.5084,285.2789) .. (389.6084,285.0359) .. controls (387.3284,284.7429) and
    (386.1084,285.3899) .. (384.8484,285.3599) .. controls (383.7984,285.3399) and
    (382.5084,284.2719) .. (380.6684,284.1999) .. controls (379.7284,284.1599) and
    (376.7084,284.9589) .. (376.0684,283.9389) .. controls (375.1284,282.4439) and
    (378.8784,282.3799) .. (375.4284,281.1329) .. controls (374.5784,280.8249) and
    (374.2884,280.8729) .. (373.1584,279.2879) .. controls (372.1784,277.9089) and
    (374.4784,278.2479) .. (374.9584,278.0129) .. controls (374.4184,277.3489) and
    (373.2684,276.6439) .. (372.3984,276.9539) .. controls (371.7984,277.1669) and
    (371.6384,278.7499) .. (370.9284,278.5949) .. controls (370.2084,278.4399) and
    (369.1784,277.2529) .. (368.2584,276.9889) .. controls (367.2584,276.7019) and
    (366.0984,276.4409) .. (365.3384,275.6579) .. controls (366.1684,275.4149) and
    (366.3684,274.3449) .. (365.3384,274.2189) .. controls (366.2984,273.3179) and
    (365.7784,272.6899) .. (364.6484,272.2929) .. controls (363.1184,271.7579) and
    (361.9584,270.8609) .. (360.6384,269.9709) .. controls (361.8184,267.6329) and
    (358.5484,266.2159) .. (357.2084,264.7139);
    
    
    % //////// RUSSIA //////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path2922
        \path[country]
        (1409.6600,291.9400) .. controls (1410.7700,291.1610) and (1411.6000,290.2150)
        .. (1411.7400,288.8240) .. controls (1411.8400,288.0370) and
        (1411.7400,287.7180) .. (1412.6300,287.6100) .. controls (1413.8200,287.4630)
        and (1415.1000,287.5900) .. (1416.1500,286.8800) .. controls
        (1417.0000,286.3080) and (1417.5200,284.6370) .. (1418.6700,284.5880) ..
        controls (1417.6800,285.5180) and (1416.4400,286.3910) .. (1415.7500,287.5920)
        .. controls (1418.2800,287.5920) and (1420.1700,288.9810) ..
        (1420.0400,285.9600) .. controls (1419.9200,283.2870) and (1423.4900,285.6490)
        .. (1424.4300,286.0730) .. controls (1426.5400,287.0190) and
        (1429.4700,285.6640) .. (1431.1700,287.5130) .. controls (1431.8600,288.2630)
        and (1432.5000,288.4210) .. (1431.6200,289.3940) .. controls
        (1430.8900,290.2070) and (1431.1100,292.1710) .. (1431.9600,292.8100) ..
        controls (1424.9300,293.5380) and (1417.8400,292.9870) .. (1410.8500,292.1780)
        .. controls (1411.4800,291.9150) and (1411.6800,291.2100) ..
        (1412.2700,290.9130) .. controls (1413.1400,290.4790) and (1414.0600,290.7420)
        .. (1414.7200,289.8850) .. controls (1413.8600,289.8250) and
        (1412.9600,289.6970) .. (1412.1000,289.7850) .. controls (1411.2100,289.8850)
        and (1410.8400,291.7640) .. (1409.6600,291.9350);
        
        % path2924
        \path[country]
        (1507.4500,238.4300) .. controls (1507.0800,238.5100) and (1506.2400,239.2320)
        .. (1506.0900,239.5280) .. controls (1505.9200,239.8700) and
        (1505.9200,240.0050) .. (1505.6500,240.1440) .. controls (1505.2200,240.3570)
        and (1505.1600,240.4070) .. (1504.6400,240.4070) -- (1503.8000,240.4070) ..
        controls (1503.5600,240.4070) and (1503.2200,240.4570) .. (1503.0100,240.3170)
        .. controls (1502.8300,240.1940) and (1502.5200,240.1370) ..
        (1502.4000,240.0100) .. controls (1502.3000,239.9200) and (1502.3000,239.4310)
        .. (1502.4000,239.3510) .. controls (1502.6200,239.1320) and
        (1502.9600,239.0500) .. (1503.1400,238.8670) .. controls (1503.2800,238.7350)
        and (1503.2800,238.3390) .. (1503.3200,238.2960) .. controls
        (1503.3200,238.2460) and (1503.4900,237.9320) .. (1503.4200,237.7690) ..
        controls (1503.2300,237.4000) and (1502.7300,237.1600) .. (1502.4900,236.8030)
        .. controls (1502.2600,236.4440) and (1501.9300,235.8850) ..
        (1501.6200,235.5730) .. controls (1501.3800,235.3410) and (1499.5900,235.3940)
        .. (1499.2400,235.2210) .. controls (1499.1400,235.1710) and
        (1498.9600,235.2610) .. (1498.8500,235.2210) .. controls (1498.5700,235.1310)
        and (1498.2800,235.0800) .. (1497.9700,235.0010) .. controls
        (1497.8700,234.9710) and (1497.7100,235.0510) .. (1497.6200,235.0010) ..
        controls (1497.1900,234.7850) and (1497.0100,234.6180) .. (1496.7000,234.2980)
        .. controls (1496.6000,234.2180) and (1496.4700,234.2480) ..
        (1496.3900,234.1670) -- (1496.3900,234.0770) .. controls (1496.2900,233.9970)
        and (1496.1000,234.0470) .. (1496.0400,233.9870) .. controls
        (1495.9400,233.9170) and (1495.7900,233.8710) .. (1495.6800,233.7670) ..
        controls (1495.5800,233.6970) and (1495.5800,233.6080) .. (1495.5100,233.5040)
        .. controls (1495.2600,232.8750) and (1495.3000,232.2440) ..
        (1494.8900,231.8340) .. controls (1494.7900,231.7340) and (1494.8900,231.5200)
        .. (1494.7200,231.4390) .. controls (1494.5300,231.3490) and
        (1494.5300,231.0610) .. (1494.4500,230.9120) .. controls (1494.4500,230.8820)
        and (1494.3100,230.7360) .. (1494.3200,230.7360) .. controls
        (1494.8400,230.7360) and (1495.1000,231.4760) .. (1495.5100,230.6460) ..
        controls (1495.6500,230.3630) and (1495.2800,230.1140) .. (1495.2000,230.0310)
        -- (1495.2000,229.0640) .. controls (1495.3300,228.9330) and
        (1495.5700,229.3610) .. (1495.5900,229.3720) .. controls (1495.8300,229.4880)
        and (1496.1500,229.6310) .. (1496.4300,229.7230) .. controls
        (1496.6700,229.8030) and (1496.9100,229.5880) .. (1497.1700,229.7630) ..
        controls (1497.3300,229.8690) and (1497.6400,230.1830) .. (1497.7500,230.2910)
        .. controls (1497.7500,230.3410) and (1500.2800,230.3910) ..
        (1500.2900,230.3810) .. controls (1500.2900,230.3510) and (1500.7000,230.2060)
        .. (1500.7800,230.2060) .. controls (1501.1100,229.7880) and
        (1501.0000,229.1950) .. (1500.7800,228.8000) .. controls (1500.6000,228.5270)
        and (1500.5600,228.1810) .. (1500.3400,227.9650) .. controls
        (1500.2400,227.8750) and (1499.5400,227.9650) .. (1499.4200,227.9650) ..
        controls (1499.1200,227.9650) and (1498.7400,227.9250) .. (1498.4500,227.8330)
        .. controls (1498.0100,227.6860) and (1497.6400,227.9760) ..
        (1497.1800,227.7430) .. controls (1497.0800,227.7130) and (1496.9900,227.7830)
        .. (1496.9200,227.7430) .. controls (1496.6700,227.6180) and
        (1496.0000,226.9170) .. (1495.7700,226.6890) .. controls (1495.5700,226.4830)
        and (1495.2200,226.5770) .. (1495.0300,226.3820) .. controls
        (1494.7100,226.0590) and (1494.1100,225.5140) .. (1494.1100,224.9320) ..
        controls (1494.1100,224.7690) and (1493.6600,224.2830) .. (1493.8400,224.0970)
        .. controls (1493.9400,224.0270) and (1495.1300,224.7120) ..
        (1495.3800,224.7120) .. controls (1495.5100,224.7120) and (1496.1100,225.1030)
        .. (1496.3500,225.1510) .. controls (1496.8500,225.2510) and
        (1499.0100,225.9700) .. (1499.2500,226.2060) .. controls (1499.3500,226.2960)
        and (1500.0900,226.3830) .. (1500.2600,226.4250) .. controls
        (1500.6400,226.5250) and (1500.9300,226.7130) .. (1501.3100,226.8650) ..
        controls (1501.4600,226.9250) and (1501.7000,226.8850) .. (1501.8400,226.9550)
        .. controls (1501.9400,226.9950) and (1502.0600,227.1100) ..
        (1502.1000,227.1300) .. controls (1502.3800,227.2700) and (1502.7200,227.2200)
        .. (1502.9800,227.3940) .. controls (1503.1200,227.4840) and
        (1503.1500,227.6050) .. (1503.2000,227.7020) .. controls (1503.2000,227.7920)
        and (1503.5600,228.1060) .. (1503.6400,228.1850) .. controls
        (1503.7400,228.2850) and (1503.4500,229.5230) .. (1503.4200,229.6780) ..
        controls (1503.4200,229.8860) and (1503.5200,230.4860) .. (1503.4200,230.6010)
        .. controls (1503.2600,230.9290) and (1502.9700,231.3430) ..
        (1503.1200,231.7870) .. controls (1503.2200,232.0610) and (1503.3500,232.1740)
        .. (1503.4700,232.4020) -- (1503.4700,232.5780) .. controls
        (1503.5900,232.8250) and (1503.8900,233.1790) .. (1504.1300,233.4130) ..
        controls (1504.4400,233.7240) and (1504.8800,233.7900) .. (1505.2700,233.9840)
        .. controls (1505.8400,234.2710) and (1506.5600,235.0530) ..
        (1506.9800,235.4780) .. controls (1507.0800,235.5680) and (1507.1200,235.7470)
        .. (1507.2000,235.8290) .. controls (1507.3900,236.0160) and
        (1507.7800,236.2000) .. (1507.9500,236.5320) .. controls (1508.0500,236.7440)
        and (1508.0500,237.5720) .. (1507.8500,237.7180) .. controls
        (1507.6900,237.8830) and (1507.8500,238.2030) .. (1507.4600,238.4210) --
        cycle(1482.7700,237.4960) .. controls (1482.4800,237.3060) and
        (1481.0700,237.3620) .. (1480.8400,237.2470) .. controls (1480.4600,237.0560)
        and (1480.1400,236.9050) .. (1479.6000,236.6880) .. controls
        (1479.0600,236.4740) and (1478.5200,236.2320) .. (1478.1700,235.8810) ..
        controls (1478.0700,235.8310) and (1477.9700,235.8710) .. (1477.9200,235.8210)
        .. controls (1477.6800,235.5810) and (1477.3900,235.1500) ..
        (1477.1200,235.0130) .. controls (1476.7000,234.8040) and (1476.3000,234.5080)
        .. (1475.9300,234.1430) .. controls (1475.9300,234.1330) and
        (1474.5600,233.8710) .. (1474.4400,233.8320) .. controls (1474.2200,233.7620)
        and (1473.3600,233.3800) .. (1473.2000,233.4600) .. controls
        (1473.0500,233.5400) and (1473.1000,233.7800) .. (1473.0800,233.8950) ..
        controls (1472.8100,234.4250) and (1472.3600,234.9040) .. (1471.9600,235.5100)
        .. controls (1471.8600,235.6420) and (1471.8100,235.5700) ..
        (1471.7100,235.6340) .. controls (1471.4800,235.7860) and (1471.3100,236.0210)
        .. (1471.0900,236.1310) .. controls (1470.6300,236.3630) and
        (1469.8400,236.3810) .. (1469.5400,236.6900) .. controls (1469.5400,236.7300)
        and (1469.5400,236.9080) .. (1469.4400,236.9390) .. controls
        (1469.1400,237.2420) and (1469.3400,237.2920) .. (1469.1900,237.6220) ..
        controls (1468.8600,238.2940) and (1469.7100,238.6790) .. (1470.3100,238.6790)
        .. controls (1470.6400,238.9170) and (1472.2000,239.6610) ..
        (1472.2400,239.7350) .. controls (1472.3600,239.9720) and (1472.5600,240.1340)
        .. (1472.6700,240.3560) -- (1472.6700,240.6050) .. controls
        (1472.8400,240.8530) and (1472.7800,240.4600) .. (1472.8600,240.7910) ..
        controls (1473.0800,241.6620) and (1472.9800,242.1490) .. (1473.5400,242.7170)
        .. controls (1473.7700,242.9440) and (1474.0700,242.9800) ..
        (1474.4100,243.1520) .. controls (1474.5800,243.2320) and (1474.8600,243.0920)
        .. (1475.0400,243.1520) .. controls (1475.1900,243.2020) and
        (1475.4900,243.5440) .. (1475.6600,243.7110) .. controls (1475.8500,243.9070)
        and (1476.0300,244.9460) .. (1476.1500,245.2020) .. controls
        (1476.3500,245.5970) and (1476.7800,245.8870) .. (1476.9600,246.2580) ..
        controls (1477.0800,246.4890) and (1477.1500,247.3220) .. (1477.2100,247.4390)
        .. controls (1477.3100,247.6110) and (1477.6600,248.0100) ..
        (1477.7700,248.1220) .. controls (1477.7700,248.1720) and (1478.1800,248.1820)
        .. (1478.2700,248.1820) .. controls (1478.7400,248.1820) and
        (1479.1900,247.8780) .. (1479.5100,247.5610) .. controls (1479.6100,247.4810)
        and (1479.6100,247.3060) .. (1479.6300,247.2500) .. controls
        (1479.7300,247.1800) and (1480.0200,246.9810) .. (1480.0700,246.8780) ..
        controls (1480.1700,246.7780) and (1480.1700,246.3900) .. (1480.1900,246.3180)
        .. controls (1480.4400,246.0740) and (1480.6500,245.6240) ..
        (1480.8800,245.5110) .. controls (1481.0700,245.4110) and (1481.4000,245.4510)
        .. (1481.6800,245.4510) .. controls (1481.8900,245.4510) and
        (1482.5100,245.2800) .. (1482.6800,245.4510) .. controls (1483.0100,245.7860)
        and (1483.4100,246.4250) .. (1483.9800,246.5690) .. controls
        (1484.2600,246.6390) and (1484.5700,246.5990) .. (1484.8500,246.6930) ..
        controls (1485.1600,246.7960) and (1485.5700,246.7730) .. (1485.8500,246.6330)
        .. controls (1486.2300,246.4430) and (1486.5000,245.2550) ..
        (1486.7200,244.8310) .. controls (1486.8300,244.6070) and (1486.7200,243.7940)
        .. (1486.9000,243.4650) .. controls (1487.1100,243.0400) and
        (1487.4900,243.2000) .. (1487.8300,243.0300) .. controls (1487.9300,242.9800)
        and (1487.9700,242.8340) .. (1488.0200,242.7810) .. controls
        (1488.3600,242.4380) and (1487.9200,241.5010) .. (1487.7700,241.2280) ..
        controls (1487.5800,240.9320) and (1486.9200,240.5250) .. (1486.6500,240.4200)
        .. controls (1486.5400,240.3700) and (1486.3900,240.4200) ..
        (1486.2800,240.3600) .. controls (1486.1400,240.2900) and (1485.9200,240.0580)
        .. (1485.7800,239.9250) .. controls (1485.6800,239.8550) and
        (1484.8700,239.4040) .. (1484.7900,239.3660) .. controls (1484.4400,239.1930)
        and (1484.0100,238.1040) .. (1483.8600,237.8750) .. controls
        (1483.7200,237.6710) and (1483.3800,237.7110) .. (1483.3000,237.6260) ..
        controls (1483.1000,237.4310) and (1483.1300,237.4250) .. (1482.7400,237.5020)
        -- cycle(1671.4100,182.4400) .. controls (1668.3900,181.6870) and
        (1665.6500,179.4160) .. (1662.6400,179.0130) .. controls (1661.3100,178.8340)
        and (1660.0300,178.5680) .. (1658.7100,178.3070) .. controls
        (1658.2100,178.2070) and (1654.3600,177.2610) .. (1656.3900,177.2990) ..
        controls (1655.4500,177.1960) and (1651.9500,175.8420) .. (1651.5600,176.7950)
        .. controls (1651.1400,177.8050) and (1649.7200,176.3440) ..
        (1651.2500,175.9890) .. controls (1648.3000,175.3770) and (1645.5400,174.1550)
        .. (1642.5800,173.5700) .. controls (1639.7500,173.0080) and
        (1636.7900,172.9450) .. (1633.9200,172.8640) .. controls (1632.3000,172.8140)
        and (1630.6600,172.7640) .. (1629.0800,172.3610) .. controls
        (1628.1300,172.1180) and (1627.1100,171.7640) .. (1626.2600,172.4610) ..
        controls (1626.1300,172.7480) and (1626.0100,173.0620) .. (1625.9500,173.3680)
        .. controls (1625.6900,173.3880) and (1625.4100,173.4480) ..
        (1625.1500,173.4690) .. controls (1624.5100,173.8400) and (1624.0900,173.2490)
        .. (1623.6400,174.0740) .. controls (1624.8500,174.7940) and
        (1626.3100,175.4060) .. (1627.1600,176.5940) .. controls (1627.9700,177.7160)
        and (1628.9600,176.7240) .. (1629.5800,177.7030) .. controls
        (1631.6200,180.9380) and (1625.3500,179.9840) .. (1624.6400,181.0290) ..
        controls (1625.0900,181.1950) and (1626.4400,182.0070) .. (1626.1600,182.6410)
        .. controls (1625.7600,183.5440) and (1623.7800,182.9510) ..
        (1623.1300,182.8430) .. controls (1621.5000,182.5720) and (1619.9800,180.7200)
        .. (1622.3300,180.1220) .. controls (1621.7700,179.7570) and
        (1618.2700,178.4790) .. (1620.2100,178.3070) .. controls (1618.6600,178.5610)
        and (1616.8400,178.1460) .. (1615.5700,179.3150) .. controls
        (1615.7500,179.5710) and (1615.9600,179.7960) .. (1616.1800,180.0210) ..
        controls (1616.0600,179.9710) and (1613.6900,178.6950) .. (1613.8600,179.6180)
        .. controls (1613.9700,180.2650) and (1613.1700,180.3170) ..
        (1612.6500,180.3230) .. controls (1611.8200,180.3330) and (1611.4000,181.1860)
        .. (1610.6300,181.4320) .. controls (1609.8800,181.6720) and
        (1609.0400,181.4220) .. (1608.3100,181.2300) .. controls (1606.0800,180.6470)
        and (1597.9100,180.3790) .. (1598.6400,184.2540) .. controls
        (1597.7100,184.6440) and (1596.9100,183.1050) .. (1596.2200,183.4480) ..
        controls (1595.6400,183.7380) and (1594.5500,184.6300) .. (1594.6100,183.3470)
        .. controls (1593.6200,184.5640) and (1590.5800,184.0940) ..
        (1589.2600,183.8510) .. controls (1589.2600,182.1510) and (1591.8100,183.3090)
        .. (1592.5900,182.4400) .. controls (1592.3100,181.9750) and
        (1589.9000,179.6070) .. (1591.9900,179.4160) .. controls (1591.2100,179.1490)
        and (1590.3400,179.1820) .. (1589.5700,178.9120) .. controls
        (1591.0400,178.4790) and (1592.7400,179.1990) .. (1594.1000,178.3070) ..
        controls (1591.0600,178.1970) and (1585.5500,178.7220) .. (1583.4200,181.3310)
        .. controls (1584.3500,181.2810) and (1585.1000,181.8320) ..
        (1585.7400,182.4400) .. controls (1585.2500,182.5400) and (1583.3700,183.9030)
        .. (1583.0200,183.1450) .. controls (1582.7000,182.4540) and
        (1583.5800,182.0640) .. (1582.6100,181.7340) .. controls (1581.5800,181.3840)
        and (1580.2600,181.8830) .. (1579.3900,182.4400) .. controls
        (1578.4700,183.0260) and (1577.1800,182.7700) .. (1576.1600,182.8430) ..
        controls (1574.2300,182.9800) and (1572.6400,184.8310) .. (1571.0200,185.2620)
        .. controls (1568.7300,185.8710) and (1567.1000,187.0030) ..
        (1564.5700,186.4720) .. controls (1565.6300,186.8610) and (1566.6600,187.6510)
        .. (1567.4900,188.3870) .. controls (1566.5700,187.8500) and
        (1563.6600,187.6180) .. (1562.7600,188.2860) .. controls (1561.8900,188.9220)
        and (1561.1100,188.1400) .. (1560.4400,188.7900) .. controls
        (1561.7800,189.4410) and (1561.0100,190.3810) .. (1560.7400,191.4100) ..
        controls (1560.4900,192.3640) and (1562.0300,193.0600) .. (1560.6400,193.8290)
        .. controls (1560.1000,194.1290) and (1558.5900,193.9190) ..
        (1557.9200,194.0310) .. controls (1556.8700,194.2070) and (1555.3600,194.1310)
        .. (1554.4900,194.8370) .. controls (1554.7200,194.6070) and
        (1554.8900,194.3820) .. (1555.1000,194.1320) .. controls (1553.7000,194.0420)
        and (1551.9200,194.5650) .. (1550.6600,193.7290) .. controls
        (1549.7700,193.1370) and (1549.3200,192.0870) .. (1548.3400,191.6120) ..
        controls (1547.2900,191.1060) and (1545.7500,191.4530) .. (1544.9200,190.5030)
        .. controls (1543.8900,189.3390) and (1545.5000,188.7160) ..
        (1546.4300,188.4870) .. controls (1546.3300,188.2230) and (1546.2200,187.9450)
        .. (1546.1300,187.6810) .. controls (1548.5700,186.8300) and
        (1551.2200,187.5910) .. (1553.6800,186.8750) .. controls (1552.8800,184.9770)
        and (1550.7500,184.4680) .. (1549.1500,183.4480) .. controls
        (1547.4000,182.3320) and (1546.2900,181.6320) .. (1544.1100,181.4320) ..
        controls (1541.8300,181.2240) and (1539.3500,182.1100) .. (1537.1500,181.5330)
        .. controls (1536.0900,181.2530) and (1533.8700,180.0610) ..
        (1532.9200,181.1300) .. controls (1534.6500,181.6600) and (1536.8100,182.3040)
        .. (1538.3600,183.2460) .. controls (1539.3000,183.8120) and
        (1538.3600,185.2120) .. (1539.5700,185.3630) .. controls (1538.4900,185.5390)
        and (1538.8900,185.9790) .. (1539.4700,186.3710) .. controls
        (1538.2400,186.4310) and (1539.1400,186.8540) .. (1539.0700,187.5800) ..
        controls (1538.9700,188.1680) and (1538.7800,188.7500) .. (1538.5700,189.2940)
        .. controls (1538.2900,189.9960) and (1537.6800,191.2060) ..
        (1538.6700,191.6120) .. controls (1540.0800,192.1940) and (1541.4100,191.9500)
        .. (1542.6000,193.2250) .. controls (1543.2700,193.9430) and
        (1542.8500,195.3410) .. (1544.0100,195.6440) .. controls (1541.4300,196.4590)
        and (1542.4600,200.1530) .. (1543.6100,201.5910) .. controls
        (1542.6600,200.8420) and (1542.2000,199.4960) .. (1540.8800,199.2720) ..
        controls (1540.1900,199.1530) and (1538.8900,199.2720) .. (1538.9700,200.2800)
        .. controls (1538.6700,200.1630) and (1538.3900,199.9950) ..
        (1538.1600,199.7760) .. controls (1538.5900,199.3650) and (1539.0900,199.0870)
        .. (1539.6700,198.9700) .. controls (1539.4100,197.7250) and
        (1537.2600,197.4010) .. (1536.2500,197.3570) .. controls (1534.6600,197.2870)
        and (1533.9500,197.2970) .. (1532.4200,196.8530) .. controls
        (1530.9100,196.4110) and (1530.0000,197.4670) .. (1529.0900,198.4660) ..
        controls (1527.9700,199.6930) and (1526.7300,200.0240) .. (1525.1600,200.3810)
        .. controls (1523.5700,200.7440) and (1522.6600,201.7500) ..
        (1521.3300,202.5980) .. controls (1520.6000,203.0620) and (1518.4700,203.6300)
        .. (1518.6100,204.8160) .. controls (1518.7500,205.9560) and
        (1521.3200,207.1170) .. (1522.1400,207.8400) .. controls (1523.3600,208.9150)
        and (1524.4200,210.1670) .. (1525.0600,211.6700) .. controls
        (1524.1200,211.3870) and (1521.9600,210.7470) .. (1521.0300,210.9640) ..
        controls (1519.6100,211.2940) and (1519.0000,211.3440) .. (1517.6000,210.7630)
        .. controls (1516.1300,210.1530) and (1514.4700,209.7120) ..
        (1512.8600,209.8560) .. controls (1511.8500,209.9460) and (1510.6600,211.2460)
        .. (1510.3400,209.8560) .. controls (1510.9400,209.9060) and
        (1511.5600,209.5880) .. (1511.9600,209.1500) .. controls (1509.5600,209.8520)
        and (1507.9600,207.4630) .. (1505.8100,207.0330) .. controls
        (1504.9900,206.8700) and (1503.4300,206.0460) .. (1502.8900,207.1340) ..
        controls (1502.3000,208.3060) and (1502.2300,208.7310) .. (1500.5700,208.6460)
        .. controls (1501.8200,210.3400) and (1503.7900,211.2890) ..
        (1505.4000,212.5770) .. controls (1506.1600,213.1800) and (1507.1700,213.0360)
        .. (1508.0300,212.7790) .. controls (1509.1400,212.4470) and
        (1509.8600,213.1830) .. (1510.8500,213.4840) .. controls (1510.0400,214.5250)
        and (1513.1600,216.8620) .. (1509.6400,216.5080) .. controls
        (1508.6800,216.4080) and (1508.3900,217.4290) .. (1507.0200,217.0120) ..
        controls (1505.5700,216.5740) and (1504.0100,216.4590) .. (1502.5800,216.0040)
        .. controls (1501.4100,215.6310) and (1500.8000,214.5760) ..
        (1499.7600,213.9880) .. controls (1499.2100,213.6730) and (1499.2600,214.7160)
        .. (1498.6500,213.8870) .. controls (1498.3900,213.5490) and
        (1498.0600,213.2950) .. (1497.6400,213.1820) .. controls (1496.4500,212.6010)
        and (1495.7600,213.6340) .. (1494.6200,213.0810) .. controls
        (1493.7000,212.6330) and (1492.7700,211.9900) .. (1491.8000,211.6700) ..
        controls (1492.0200,211.4320) and (1492.1900,211.2070) .. (1492.4000,210.9640)
        .. controls (1492.1400,210.7920) and (1491.8600,210.6240) ..
        (1491.6000,210.4600) .. controls (1491.8800,210.2790) and (1492.2100,210.1110)
        .. (1492.5000,209.9560) .. controls (1491.4800,209.8860) and
        (1491.4500,208.4870) .. (1490.3900,208.3440) .. controls (1491.4300,207.1880)
        and (1488.8600,206.2360) .. (1488.2700,205.6220) .. controls
        (1487.6800,205.0030) and (1490.6100,204.2340) .. (1489.5800,202.8000) ..
        controls (1491.6300,203.2890) and (1488.4700,200.3950) .. (1487.9700,200.0790)
        .. controls (1485.8100,198.7300) and (1482.8900,198.3920) ..
        (1480.4100,198.2640) .. controls (1481.1400,198.0130) and (1482.3500,198.1530)
        .. (1482.0200,196.9540) .. controls (1481.1100,197.1330) and
        (1479.0100,196.9540) .. (1478.0900,196.7520) .. controls (1478.9400,196.3090)
        and (1480.0100,196.3030) .. (1480.9100,196.5510) .. controls
        (1479.9900,195.6050) and (1478.5000,196.4230) .. (1477.3800,196.1480) ..
        controls (1478.2300,196.2940) and (1478.9500,195.4910) .. (1479.8000,195.8450)
        .. controls (1478.9300,195.1400) and (1477.6800,195.3720) ..
        (1476.6800,195.0390) .. controls (1478.5600,195.2370) and (1475.2100,193.8050)
        .. (1474.4600,193.9300) .. controls (1474.7100,193.6750) and
        (1474.9400,193.4980) .. (1475.1700,193.2250) .. controls (1473.9000,192.3400)
        and (1472.4000,192.4910) .. (1471.0300,191.9140) .. controls
        (1472.0100,192.0660) and (1473.0100,191.5350) .. (1473.9600,191.9140) ..
        controls (1474.9700,192.3160) and (1476.2100,192.4600) .. (1477.2800,192.4180)
        .. controls (1475.1300,192.4980) and (1479.4500,194.6450) ..
        (1480.0100,194.8370) .. controls (1480.6700,195.0660) and (1481.9600,194.5660)
        .. (1482.4200,194.9380) .. controls (1483.1100,195.4860) and
        (1483.9000,195.5660) .. (1484.4400,194.7370) .. controls (1484.1700,196.0270)
        and (1485.9900,195.2830) .. (1486.6600,196.4500) .. controls
        (1486.7600,196.5800) and (1489.2100,196.1850) .. (1489.7800,196.4500) ..
        controls (1492.4500,197.6890) and (1495.0000,198.2360) .. (1497.9500,198.3650)
        .. controls (1501.4300,198.5170) and (1504.5900,199.6280) ..
        (1508.0300,199.9780) .. controls (1511.1100,200.2930) and (1513.8100,199.8780)
        .. (1516.7900,199.1720) .. controls (1519.5200,198.5270) and
        (1521.2000,197.5090) .. (1523.2500,195.6440) .. controls (1524.6000,194.4070)
        and (1526.1300,191.9420) .. (1523.6500,191.3100) .. controls
        (1523.1400,191.1810) and (1522.5100,189.5930) .. (1522.3400,189.0920) ..
        controls (1521.9000,187.8290) and (1521.4400,188.0930) .. (1520.4200,187.5800)
        .. controls (1519.2900,187.0140) and (1518.0800,187.1680) ..
        (1517.1000,186.2700) .. controls (1516.2200,185.4750) and (1515.1000,184.7290)
        .. (1513.9700,184.3550) .. controls (1514.1700,184.6100) and
        (1514.3000,184.8890) .. (1514.4800,185.1610) .. controls (1511.9900,185.4630)
        and (1509.2100,184.0170) .. (1507.1200,182.8430) .. controls
        (1507.3900,183.0520) and (1507.6700,183.2240) .. (1507.9200,183.4480) ..
        controls (1505.2400,182.9710) and (1503.1400,180.9950) .. (1500.5700,180.2220)
        .. controls (1497.5600,179.3210) and (1494.5100,178.4520) ..
        (1491.6000,177.2990) .. controls (1488.9900,176.2700) and (1486.7100,177.0140)
        .. (1484.1400,176.5940) .. controls (1483.0300,176.4140) and
        (1481.9300,175.9170) .. (1480.8100,175.8880) .. controls (1479.8000,175.8580)
        and (1478.6800,176.2420) .. (1477.6900,175.8880) .. controls
        (1477.6900,176.5580) and (1477.3600,176.8470) .. (1476.9800,177.0980) ..
        controls (1476.3000,177.5540) and (1475.3000,177.7000) .. (1474.8600,178.6100)
        .. controls (1474.2700,177.4220) and (1476.3900,177.5070) ..
        (1476.9800,177.0980) .. controls (1476.4400,176.9320) and (1475.5300,176.5880)
        .. (1476.8800,176.3920) .. controls (1475.8600,176.1890) and
        (1476.1900,176.0660) .. (1476.8800,175.6870) .. controls (1476.0500,174.7050)
        and (1474.6400,175.2040) .. (1473.7600,175.7870) .. controls
        (1473.9400,175.5330) and (1474.1100,175.3550) .. (1474.2600,175.0820) ..
        controls (1473.4100,175.0620) and (1472.5800,174.7540) .. (1471.7400,174.6790)
        .. controls (1471.3700,174.6490) and (1471.0700,174.7690) ..
        (1470.7300,174.8800) .. controls (1470.8700,174.8400) and (1470.9900,174.7190)
        .. (1471.1400,174.6790) .. controls (1470.2200,174.1990) and
        (1469.2700,173.9540) .. (1468.3100,173.5700) .. controls (1468.4100,173.3010)
        and (1468.5300,173.0750) .. (1468.7200,172.8640) .. controls
        (1469.5400,173.8600) and (1474.0900,175.0320) .. (1474.3600,173.0660) ..
        controls (1473.1200,172.5340) and (1471.7800,172.7980) .. (1470.5300,172.1590)
        .. controls (1469.6800,171.7270) and (1468.3800,171.0780) ..
        (1467.4100,171.4530) .. controls (1467.6500,171.6690) and (1467.8700,171.8430)
        .. (1468.1100,172.0580) .. controls (1467.6900,172.1080) and
        (1466.6200,171.9190) .. (1466.5000,172.5620) .. controls (1466.4000,172.9670)
        and (1465.3600,173.5260) .. (1465.0900,173.3680) .. controls
        (1464.1700,172.8420) and (1462.7900,172.7540) .. (1461.7600,172.5620) ..
        controls (1462.5000,173.0860) and (1462.9100,173.9800) .. (1461.7600,174.2760)
        .. controls (1460.5900,174.5800) and (1459.4800,174.0200) ..
        (1458.4400,173.5700) .. controls (1459.3500,175.6320) and (1456.2300,175.6400)
        .. (1455.0100,175.8880) .. controls (1453.5900,176.1740) and
        (1454.6000,176.8770) .. (1453.8000,177.6020) .. controls (1452.7100,178.5790)
        and (1450.8000,178.6350) .. (1449.4600,179.1140) .. controls
        (1450.2500,179.2170) and (1452.4200,179.3930) .. (1451.0800,180.6260) ..
        controls (1449.9200,181.7180) and (1450.1000,182.7410) .. (1451.4800,183.6490)
        .. controls (1452.8200,184.5270) and (1454.4900,184.5580) ..
        (1455.8100,185.4640) .. controls (1456.8500,186.1750) and (1458.7500,186.9450)
        .. (1459.5400,187.8830) .. controls (1461.3100,189.9630) and
        (1453.7800,191.6180) .. (1456.1200,194.5350) .. controls (1458.3700,197.3550)
        and (1461.7300,199.1590) .. (1462.9700,202.8000) .. controls
        (1462.2100,202.8400) and (1461.5000,203.0690) .. (1460.7500,203.2030) ..
        controls (1461.7300,203.4790) and (1461.2000,204.9780) .. (1460.7500,205.7230)
        .. controls (1460.3300,206.4260) and (1461.8300,206.6250) ..
        (1462.0600,207.1340) .. controls (1460.5000,207.4690) and (1460.8100,209.2140)
        .. (1462.1600,209.6540) .. controls (1463.0600,209.9450) and
        (1464.0600,209.4040) .. (1464.5800,210.4600) .. controls (1461.8200,211.7070)
        and (1465.8000,213.1330) .. (1466.9000,213.6860) .. controls
        (1469.3500,214.9110) and (1465.6200,217.2430) .. (1464.4800,217.8180) ..
        controls (1467.4500,219.4700) and (1470.4700,221.0280) .. (1473.3500,222.7570)
        .. controls (1474.5600,223.4780) and (1475.0400,223.7580) ..
        (1474.4600,225.0750) .. controls (1473.7900,226.6110) and (1473.3300,227.6570)
        .. (1471.9400,228.7040) .. controls (1468.9600,230.9570) and
        (1466.6500,233.8680) .. (1463.7800,236.2630) .. controls (1461.0000,238.5770)
        and (1457.5000,240.0620) .. (1455.0100,242.7140) .. controls
        (1456.4200,242.7340) and (1457.1200,242.7140) .. (1458.3300,241.9080) ..
        controls (1458.7900,241.6070) and (1459.9200,240.9430) .. (1460.4500,241.5050)
        .. controls (1459.7300,241.9270) and (1460.2700,242.7710) ..
        (1460.4500,243.3190) .. controls (1459.9400,243.0720) and (1459.4300,242.7940)
        .. (1458.9400,242.5130) .. controls (1459.8000,243.4700) and
        (1461.8700,245.1060) .. (1463.0700,245.5360) .. controls (1464.7900,246.1490)
        and (1466.2200,244.9830) .. (1467.9100,246.1410) .. controls
        (1468.0100,246.1910) and (1471.4600,248.0560) .. (1469.9300,248.0560) ..
        controls (1468.2500,248.0560) and (1466.7000,246.9960) .. (1464.9900,246.9480)
        .. controls (1463.5000,246.9080) and (1463.1900,248.5720) ..
        (1461.8600,248.6610) .. controls (1461.1100,248.7110) and (1460.1500,247.6480)
        .. (1459.6400,248.6610) .. controls (1459.4900,248.9630) and
        (1459.4600,249.4650) .. (1459.0400,249.4670) .. controls (1458.3300,249.4670)
        and (1456.9800,248.0740) .. (1457.2300,249.4670) .. controls
        (1457.3400,250.1250) and (1457.9400,250.4000) .. (1457.4300,251.0800) ..
        controls (1457.9300,251.2740) and (1458.4400,251.5450) .. (1458.6400,252.0880)
        .. controls (1456.9200,252.0680) and (1457.0300,253.2910) ..
        (1456.4200,254.5070) .. controls (1455.9800,255.3790) and (1454.6800,255.7580)
        .. (1454.7100,256.8250) .. controls (1454.7100,257.8930) and
        (1455.6100,258.7760) .. (1455.4100,259.8490) .. controls (1455.2900,260.4660)
        and (1455.1500,261.0840) .. (1455.7100,261.5630) .. controls
        (1456.4000,262.1470) and (1456.9100,263.7720) .. (1457.7300,263.8810) ..
        controls (1455.5900,265.5730) and (1454.4500,266.6030) .. (1457.6300,268.0130)
        .. controls (1459.0100,268.6250) and (1458.5400,270.9920) ..
        (1457.7300,272.0450) .. controls (1459.3200,271.8520) and (1460.6400,274.0110)
        .. (1461.3600,275.2700) .. controls (1461.6300,275.7490) and
        (1461.9500,278.9920) .. (1462.8700,278.5970) .. controls (1464.4600,277.9140)
        and (1465.2600,279.4570) .. (1466.9000,279.1010) .. controls
        (1467.6700,278.9340) and (1468.5900,278.8640) .. (1469.3200,279.2010) ..
        controls (1470.1000,279.5610) and (1469.7200,280.0660) .. (1469.8200,280.7130)
        .. controls (1470.0900,282.3150) and (1474.1100,279.8900) ..
        (1475.1700,280.2090) .. controls (1475.8200,280.4070) and (1479.8600,282.1890)
        .. (1479.9000,282.7290) .. controls (1480.0000,283.8460) and
        (1479.4800,284.3630) .. (1480.2100,285.4510) .. controls (1480.5700,285.9900)
        and (1481.0500,287.0740) .. (1480.3100,287.5670) .. controls
        (1479.0200,288.4230) and (1482.2500,290.6280) .. (1482.8300,291.5990) ..
        controls (1483.4200,292.6040) and (1484.0600,293.6990) .. (1485.1500,294.2200)
        .. controls (1485.9400,294.6010) and (1487.3100,294.4490) ..
        (1487.5600,295.5300) .. controls (1487.7200,296.1750) and (1486.6300,297.4640)
        .. (1488.1700,297.1430) .. controls (1489.2600,296.9150) and
        (1489.6200,297.0830) .. (1490.6900,297.3440) .. controls (1492.5300,297.8010)
        and (1490.9200,297.9470) .. (1491.9000,298.6540) .. controls
        (1492.5300,299.1050) and (1493.7900,299.5430) .. (1494.0200,300.3680) ..
        controls (1494.1700,300.9310) and (1491.0500,302.7300) .. (1490.3900,302.7870)
        .. controls (1488.5400,302.9470) and (1487.0600,301.0860) ..
        (1485.2500,302.5850) .. controls (1484.3800,303.3030) and (1485.7300,304.2730)
        .. (1486.2500,304.7020) .. controls (1487.3000,305.5530) and
        (1486.9400,305.5980) .. (1487.1600,306.8190) .. controls (1487.5000,308.6500)
        and (1488.0300,310.5890) .. (1489.9800,311.2540) .. controls
        (1491.5600,311.7900) and (1492.9200,310.9440) .. (1492.8100,309.2380) ..
        controls (1494.6300,309.3650) and (1495.6800,310.0450) .. (1497.4400,309.3390)
        .. controls (1499.0500,308.6950) and (1500.1800,309.8230) ..
        (1501.5700,309.2380) .. controls (1503.0400,308.6200) and (1504.0500,310.7820)
        .. (1504.5000,311.7580) .. controls (1504.9800,312.8040) and
        (1506.5500,312.9320) .. (1507.0200,313.9750) .. controls (1506.3800,314.3710)
        and (1505.4100,314.1150) .. (1505.0000,314.8820) .. controls
        (1504.8000,315.2580) and (1507.2300,317.4500) .. (1506.1100,318.1080) ..
        controls (1507.0600,318.4240) and (1509.4000,319.1840) .. (1510.3400,318.7120)
        .. controls (1511.8300,317.9690) and (1512.4600,319.9980) ..
        (1513.8700,319.9220) .. controls (1513.4500,320.7130) and (1514.6700,323.0320)
        .. (1514.9800,323.8530) .. controls (1515.5100,325.2340) and
        (1516.5600,325.9060) .. (1517.9000,325.1630) .. controls (1519.1300,324.4870)
        and (1519.8100,325.3270) .. (1520.8300,325.8690) .. controls
        (1520.9700,325.9490) and (1522.8800,326.7790) .. (1522.9400,326.7760) ..
        controls (1524.6700,326.6960) and (1526.2300,324.8660) .. (1528.1800,325.0620)
        .. controls (1529.3100,325.1760) and (1529.8500,326.8570) ..
        (1530.5000,327.5820) .. controls (1531.2200,328.3810) and (1532.4600,328.4170)
        .. (1532.9200,329.4970) .. controls (1534.6000,328.5300) and
        (1533.8100,327.8270) .. (1535.8400,328.8920) .. controls (1536.9000,329.4440)
        and (1539.8100,330.6210) .. (1540.6800,329.5980) .. controls
        (1541.4400,331.1020) and (1542.5500,330.1930) .. (1543.4000,331.2110) ..
        controls (1544.0100,331.9280) and (1545.0000,332.2780) .. (1545.9200,332.2190)
        .. controls (1546.5600,332.1790) and (1546.7000,331.6640) ..
        (1547.4400,332.0170) .. controls (1546.3300,333.0730) and (1548.9700,335.4200)
        .. (1546.4300,336.4520) .. controls (1545.7700,336.7190) and
        (1545.2100,336.7840) .. (1545.7200,337.6610) .. controls (1546.3800,338.7890)
        and (1547.3900,337.2390) .. (1547.5400,338.7700) .. controls
        (1546.6800,338.5140) and (1545.2400,339.3040) .. (1545.7200,340.3830) ..
        controls (1545.8900,340.7520) and (1548.5400,341.6730) .. (1547.1300,342.7010)
        .. controls (1547.4300,342.9430) and (1547.7700,343.0020) ..
        (1548.1400,342.9030) .. controls (1548.3300,343.8120) and (1547.6700,346.7410)
        .. (1546.6300,346.8340) .. controls (1545.5300,346.9340) and
        (1544.2800,346.5190) .. (1543.2000,346.7330) .. controls (1542.2600,346.9210)
        and (1541.2200,346.1190) .. (1540.5800,347.2370) .. controls
        (1540.2700,347.7960) and (1539.9200,348.2600) .. (1539.2700,348.4460) ..
        controls (1538.0000,348.8130) and (1536.5600,351.0490) .. (1538.1600,351.3690)
        .. controls (1537.1200,352.2820) and (1538.0000,353.1600) ..
        (1539.0700,352.6800) .. controls (1539.3400,352.5590) and (1539.5400,352.4180)
        .. (1539.7800,352.2770) .. controls (1539.6400,352.4080) and
        (1539.4500,352.5990) .. (1539.3700,352.7800) .. controls (1540.7400,352.9360)
        and (1542.0000,352.0020) .. (1543.3000,351.7730) .. controls
        (1544.9600,351.4840) and (1544.2100,353.2810) .. (1545.5200,352.8810) ..
        controls (1544.5100,353.7690) and (1542.6900,354.7960) .. (1541.1900,354.9980)
        .. controls (1538.1700,355.4030) and (1540.4300,355.4940) ..
        (1540.0800,356.9130) .. controls (1539.1600,356.9730) and (1538.4900,356.4300)
        .. (1537.5600,356.7110) .. controls (1536.7100,356.9640) and
        (1536.0200,357.2730) .. (1535.1400,356.9130) .. controls (1535.7900,358.9900)
        and (1536.9600,358.6260) .. (1538.4700,359.5340) .. controls
        (1539.0600,359.8920) and (1541.3200,361.1430) .. (1541.0900,362.0530) ..
        controls (1540.3500,362.1030) and (1539.5700,360.9460) .. (1538.8700,361.2470)
        .. controls (1538.2700,361.5050) and (1538.3400,362.8800) ..
        (1537.9600,363.3640) .. controls (1537.8600,362.8850) and (1537.7500,362.4340)
        .. (1537.6600,361.9530) .. controls (1536.7600,362.5160) and
        (1536.7100,366.3020) .. (1535.2400,365.3800) .. controls (1535.1400,365.8620)
        and (1535.5700,367.8410) .. (1536.0500,366.0850) .. controls
        (1536.1500,366.8240) and (1536.7500,367.5340) .. (1536.3500,368.3030) ..
        controls (1535.8300,368.1480) and (1532.5200,367.7940) .. (1532.8200,368.4030)
        .. controls (1531.8200,367.5870) and (1529.7800,366.2600) ..
        (1529.2900,368.0000) .. controls (1529.5200,367.8140) and (1529.7500,367.6460)
        .. (1530.0000,367.4960) .. controls (1530.0000,368.1000) and
        (1530.4000,368.5040) .. (1531.0100,368.5040) .. controls (1530.3500,368.8890)
        and (1529.5200,369.0130) .. (1529.1900,369.8150) .. controls
        (1531.2300,370.7120) and (1533.3400,370.4150) .. (1534.6300,372.5360) ..
        controls (1535.2800,373.5880) and (1538.6000,374.4560) .. (1537.5600,373.1410)
        .. controls (1539.0500,373.5580) and (1539.7800,375.2420) ..
        (1541.0900,375.9630) .. controls (1542.5000,376.7470) and (1544.1700,376.9720)
        .. (1545.6200,377.7770) .. controls (1548.9400,379.6160) and
        (1551.1100,382.9380) .. (1554.4900,384.6310) .. controls (1554.3300,381.1740)
        and (1562.0400,384.3540) .. (1563.5600,385.0340) .. controls
        (1564.7800,385.5760) and (1566.0800,385.9420) .. (1567.3900,386.1430) ..
        controls (1568.6200,386.3310) and (1569.5600,385.8940) .. (1570.7200,385.9410)
        .. controls (1571.5500,385.9710) and (1572.1800,386.5150) ..
        (1573.0400,386.5460) .. controls (1573.8200,386.5760) and (1574.6700,386.4760)
        .. (1575.3600,386.9490) .. controls (1576.2000,387.5230) and
        (1582.0300,389.9750) .. (1581.2000,390.8800) .. controls (1583.4200,392.5250)
        and (1587.0700,388.0980) .. (1588.5600,391.1830) .. controls
        (1588.6700,389.5820) and (1591.0100,390.1550) .. (1591.6800,390.9810) ..
        controls (1592.8200,392.3820) and (1593.5300,391.2560) .. (1594.9100,391.9890)
        .. controls (1595.7900,392.4600) and (1595.1300,393.6370) ..
        (1595.2100,394.4080) .. controls (1595.3100,395.1760) and (1597.0300,395.7810)
        .. (1597.6300,396.0210) .. controls (1599.9000,396.9290) and
        (1602.5600,397.1140) .. (1604.2800,398.8430) .. controls (1605.0200,399.5850)
        and (1605.6400,399.8990) .. (1606.5000,400.3550) .. controls
        (1607.4200,400.8420) and (1607.4100,402.1190) .. (1608.4200,402.5720) ..
        controls (1609.2400,402.9460) and (1610.9400,403.6900) .. (1611.8400,403.2780)
        .. controls (1612.3400,403.0490) and (1612.7500,401.8040) ..
        (1613.1500,401.3630) .. controls (1613.9700,400.4680) and (1614.9500,399.8140)
        .. (1615.5700,398.7420) .. controls (1616.2300,397.6060) and
        (1615.2600,397.3530) .. (1614.4600,396.5250) .. controls (1613.5300,395.5630)
        and (1612.8800,394.4010) .. (1611.8400,393.5010) .. controls
        (1610.9400,392.7160) and (1609.7700,392.0080) .. (1609.1200,390.9810) ..
        controls (1608.4300,389.8760) and (1608.0800,388.7770) .. (1606.9000,388.0580)
        .. controls (1606.0600,387.5460) and (1606.3300,385.7730) ..
        (1607.0000,385.2360) .. controls (1605.1700,384.9080) and (1606.3400,381.3610)
        .. (1606.9000,380.3980) .. controls (1605.5500,379.5550) and
        (1605.6800,382.4810) .. (1605.8000,383.2200) .. controls (1604.4900,383.0260)
        and (1605.4400,382.3750) .. (1605.3900,381.5070) .. controls
        (1605.2900,380.5940) and (1604.6800,379.7950) .. (1604.1800,379.0880) ..
        controls (1603.3500,377.9110) and (1602.7400,377.3410) .. (1601.4600,376.6680)
        .. controls (1600.5100,376.1650) and (1598.8200,375.8610) ..
        (1598.9400,374.4510) .. controls (1599.0400,373.4660) and (1601.1500,372.6700)
        .. (1600.3500,371.6290) .. controls (1600.5300,371.8830) and
        (1600.7500,372.1080) .. (1600.9600,372.3340) .. controls (1601.7500,369.5830)
        and (1604.1400,367.0430) .. (1601.8600,364.4730) .. controls
        (1602.7900,364.4730) and (1603.2500,365.4060) .. (1603.6800,366.0850) ..
        controls (1603.4800,365.4680) and (1603.4200,364.7120) .. (1602.8700,364.2710)
        .. controls (1603.7100,364.5070) and (1604.4300,365.0820) ..
        (1605.1900,365.4800) .. controls (1604.8800,363.8820) and (1606.3600,364.9770)
        .. (1607.3100,364.4730) .. controls (1607.7700,364.2250) and
        (1608.0000,363.7030) .. (1608.6200,363.7670) .. controls (1607.3800,362.2250)
        and (1610.6100,363.4910) .. (1610.9400,363.6660) .. controls
        (1611.0400,363.0540) and (1610.7300,362.7620) .. (1610.1300,362.7590) ..
        controls (1610.4900,362.2520) and (1610.3900,361.7850) .. (1609.7300,361.6500)
        .. controls (1610.2400,361.3890) and (1610.7500,361.4410) ..
        (1611.2400,361.7510) .. controls (1611.2400,360.7690) and (1612.3700,360.7650)
        .. (1612.9500,361.1460) .. controls (1612.8500,360.6460) and
        (1612.8000,360.1420) .. (1612.7500,359.6340) .. controls (1613.0200,359.7740)
        and (1613.2900,359.8890) .. (1613.5600,360.0380) .. controls
        (1613.3200,358.5600) and (1607.5100,357.2010) .. (1607.9100,356.4090) ..
        controls (1608.4300,355.4010) and (1611.4200,357.0800) .. (1611.0400,355.7030)
        .. controls (1610.7600,354.7200) and (1609.5700,353.9060) ..
        (1608.9200,353.1840) .. controls (1606.7100,350.7520) and (1605.2000,347.8810)
        .. (1601.7600,347.2370) .. controls (1600.9200,347.0790) and
        (1599.1700,346.6940) .. (1598.5400,347.5390) .. controls (1597.8000,348.5310)
        and (1596.7700,345.7550) .. (1596.3200,345.3220) .. controls
        (1596.5600,345.1520) and (1596.7900,344.9840) .. (1597.0300,344.8180) ..
        controls (1595.9800,343.8730) and (1596.1600,343.2000) .. (1594.6100,342.8020)
        .. controls (1593.7500,342.5820) and (1592.6800,342.3240) ..
        (1592.1900,341.4920) .. controls (1591.2800,339.9420) and (1592.4800,337.6540)
        .. (1593.7000,336.7540) .. controls (1595.3800,335.5060) and
        (1592.3000,334.4480) .. (1592.0900,333.3270) .. controls (1591.6200,330.8910)
        and (1592.1900,329.9600) .. (1593.9000,328.6910) .. controls
        (1594.9800,327.9150) and (1592.8500,324.9320) .. (1595.5100,324.9620) ..
        controls (1597.8200,324.9920) and (1599.4000,328.7750) .. (1601.3600,329.6990)
        .. controls (1602.3900,330.1820) and (1603.9300,329.5500) ..
        (1604.6900,328.7920) .. controls (1605.3300,328.1460) and (1604.2800,327.5280)
        .. (1603.9800,326.9770) .. controls (1603.4300,325.9740) and
        (1603.0100,323.5420) .. (1601.7600,323.1470) .. controls (1603.5100,323.6060)
        and (1605.1100,322.7600) .. (1606.5000,321.6350) .. controls
        (1607.0000,321.2300) and (1606.2000,320.4220) .. (1606.3000,319.9220) ..
        controls (1606.4500,319.1470) and (1607.5800,319.4180) .. (1608.1100,319.4180)
        .. controls (1609.0700,319.4180) and (1609.3800,318.4500) ..
        (1610.2300,318.2080) .. controls (1611.0100,317.9850) and (1612.0000,318.0330)
        .. (1612.4500,317.2000) .. controls (1613.1400,315.9130) and
        (1612.6000,314.5090) .. (1614.4600,315.3860) .. controls (1614.2700,314.9070)
        and (1614.1500,314.3530) .. (1613.9600,313.8740) .. controls
        (1615.0800,314.1130) and (1617.8100,314.3270) .. (1618.0900,315.4870) ..
        controls (1618.5200,317.2280) and (1619.8300,315.0890) .. (1620.6100,316.3940)
        .. controls (1621.0000,315.9130) and (1620.9900,314.9620) ..
        (1621.6200,314.6810) .. controls (1622.5000,314.2840) and (1623.3000,314.2960)
        .. (1624.2400,313.7730) .. controls (1625.3500,317.3430) and
        (1628.5500,315.8560) .. (1631.3000,316.1930) .. controls (1632.8900,316.3890)
        and (1633.0900,317.8800) .. (1634.3200,318.4100) .. controls
        (1635.4300,318.8860) and (1636.3700,318.5840) .. (1637.2400,319.6190) ..
        controls (1637.8800,320.3700) and (1640.3600,321.3340) .. (1640.2700,321.8370)
        .. controls (1640.1400,322.5430) and (1640.2700,323.5660) ..
        (1640.8700,324.0540) .. controls (1641.8500,324.8900) and (1642.0900,323.0360)
        .. (1641.7800,322.4420) .. controls (1641.3700,321.6820) and
        (1640.5400,321.0430) .. (1640.2700,320.2240) .. controls (1641.5500,319.3410)
        and (1643.3800,321.0660) .. (1644.3000,321.7360) .. controls
        (1645.3000,322.4680) and (1646.8000,322.6170) .. (1647.6200,323.3490) ..
        controls (1648.6100,324.2240) and (1650.5300,323.8560) .. (1650.9500,322.3410)
        .. controls (1651.2500,321.2580) and (1652.8400,320.9960) ..
        (1652.7600,319.8210) .. controls (1653.3300,319.8510) and (1653.8300,320.0770)
        .. (1654.2800,320.4260) .. controls (1654.2800,319.4520) and
        (1657.3600,319.2050) .. (1657.6000,319.8210) .. controls (1657.8400,320.4210)
        and (1659.2300,321.1560) .. (1659.8200,321.3330) .. controls
        (1660.4800,321.5310) and (1660.8100,320.7010) .. (1661.5300,321.0310) ..
        controls (1661.4300,317.7230) and (1662.3100,320.6610) .. (1664.1500,319.3170)
        .. controls (1665.6100,318.2560) and (1666.8300,320.4800) ..
        (1667.3800,321.3330) .. controls (1668.1600,322.5320) and (1669.9900,322.8220)
        .. (1671.3100,322.9460) .. controls (1670.8136,228.0063) and
        (1671.5223,182.5050) .. (1671.4100,182.4400) -- cycle;
    
    \end{scope}
    
    
    % //////// SERBIA & COSOVO /////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]

        \path[country]
        (1412.8700,360.8400) .. controls (1411.7100,360.3470) and (1410.6800,362.1140)
        .. (1410.2800,362.2760) .. controls (1409.5700,362.5620) and
        (1408.3500,362.3460) .. (1406.9000,362.8310) .. controls (1407.3100,363.8390)
        and (1407.6100,364.4230) .. (1407.8300,365.4770) .. controls
        (1407.9800,366.1420) and (1408.1800,366.3340) .. (1408.8700,366.3590) ..
        controls (1406.9000,367.7280) and (1410.5700,368.5670) .. (1411.1900,369.1810)
        .. controls (1411.0900,369.0910) and (1409.1900,369.6090) ..
        (1408.9400,369.7100) .. controls (1409.5500,370.9130) and (1408.9400,371.5290)
        .. (1408.7300,371.8770) .. controls (1409.6300,371.5230) and
        (1410.4500,371.2880) .. (1410.6600,371.7510) .. controls (1411.1500,372.8370)
        and (1411.2600,372.7540) .. (1409.6000,375.2790) .. controls
        (1409.0500,376.1100) and (1410.8200,377.3480) .. (1412.3200,378.4030) ..
        controls (1413.9500,379.9160) and (1411.1600,379.1900) .. (1410.7300,379.5370)
        .. controls (1410.4700,379.5970) and (1413.0200,382.4100) ..
        (1412.4900,382.6660) .. controls (1411.0800,383.3380) and (1409.6100,383.4690)
        .. (1408.5700,383.4950) .. controls (1409.0700,383.4150) and
        (1410.3200,384.9490) .. (1412.2000,386.4520) .. controls (1412.8000,386.9300)
        and (1412.9400,387.4300) .. (1414.2800,387.8860) .. controls
        (1415.3500,388.5220) and (1417.2800,387.9160) .. (1417.6000,389.1640) ..
        controls (1417.7400,389.2540) and (1416.1200,390.0560) .. (1416.2200,390.0960)
        .. controls (1416.3600,390.1560) and (1417.2000,391.5260) ..
        (1416.9000,391.6740) .. controls (1418.8300,392.2950) and (1416.5200,393.4790)
        .. (1419.9000,394.1220) .. controls (1420.9200,394.3160) and
        (1420.8900,398.8660) .. (1421.0000,397.7640) .. controls (1422.4600,396.5330)
        and (1422.3400,394.3040) .. (1425.7300,395.5250) .. controls
        (1425.7300,394.4370) and (1426.9000,394.6180) .. (1427.5000,394.1940) ..
        controls (1428.1900,394.8940) and (1428.9500,393.4760) .. (1430.0100,393.8000)
        .. controls (1430.6700,394.0010) and (1435.1400,393.5180) ..
        (1434.0200,391.8590) .. controls (1433.3700,390.9040) and (1433.2100,389.7820)
        .. (1433.7600,389.1880) .. controls (1434.3000,388.6160) and
        (1434.9800,389.2480) .. (1435.5800,388.4830) .. controls (1436.1700,387.7360)
        and (1436.6400,387.0030) .. (1436.9600,386.2400) .. controls
        (1435.9700,385.9260) and (1434.7000,384.6330) .. (1433.9400,383.9220) ..
        controls (1431.5000,381.6340) and (1432.7200,379.7860) .. (1434.0900,377.4960)
        .. controls (1433.7800,377.2090) and (1432.0800,375.4820) ..
        (1432.7300,375.0520) .. controls (1433.2800,374.6930) and (1433.9900,374.9200)
        .. (1434.5500,374.6490) .. controls (1434.0000,373.9770) and
        (1432.5600,373.0720) .. (1431.7200,373.7420) .. controls (1431.4600,373.9550)
        and (1430.6900,375.2670) .. (1430.4100,375.2540) .. controls
        (1430.0400,375.2340) and (1429.3200,374.2170) .. (1428.9000,374.0440) ..
        controls (1427.9200,373.6400) and (1426.8200,373.3220) .. (1425.8800,372.8350)
        .. controls (1425.1800,372.4740) and (1425.6000,372.6010) ..
        (1424.8900,372.3440) .. controls (1425.7900,371.8570) and (1426.1700,371.0740)
        .. (1424.8900,370.9200) .. controls (1426.2900,369.6010) and
        (1425.1500,369.3280) .. (1423.9700,368.8910) .. controls (1422.7600,368.4430)
        and (1421.2100,367.3470) .. (1420.1500,366.6360) .. controls
        (1421.4700,364.0270) and (1418.6600,364.0110) .. (1418.2900,362.2010) ..
        controls (1417.9600,360.5840) and (1414.5600,360.5560) .. (1412.8400,360.8400)
        -- cycle;

        \begin{scope}

            \path[country]
            (1416.3600,389.9480) .. controls (1416.7500,389.6600) and (1417.5600,389.1390)
            .. (1417.9700,389.3200) .. controls (1418.0700,388.6330) and
            (1418.1400,389.4200) .. (1418.4100,388.9590) .. controls (1418.8500,388.2160)
            and (1419.3900,388.3200) .. (1419.8700,388.1110) .. controls
            (1420.8700,387.6820) and (1420.8400,387.2270) .. (1420.3700,386.1340) ..
            controls (1420.8400,386.0740) and (1421.4400,385.7420) .. (1421.8300,385.4700)
            .. controls (1422.1300,387.4320) and (1426.9600,386.7430) ..
            (1426.6200,388.6940) .. controls (1426.4500,389.6800) and (1428.3600,390.0310)
            .. (1428.5700,390.8410) .. controls (1428.8800,392.0270) and
            (1426.6500,393.2400) .. (1427.5300,394.1980) .. controls (1426.7300,394.5640)
            and (1425.5100,394.6150) .. (1425.8100,395.5770) .. controls
            (1424.6100,395.4280) and (1424.8100,394.7570) .. (1423.0600,395.4640) ..
            controls (1421.6600,396.0280) and (1421.7500,397.6630) .. (1421.0300,397.8810)
            .. controls (1420.5500,397.7490) and (1421.2300,395.4880) ..
            (1420.2400,394.7190) .. controls (1420.0000,393.8550) and (1419.1400,394.1620)
            .. (1418.2800,393.5070) .. controls (1417.7100,392.5930) and
            (1418.1200,392.1270) .. (1417.0700,391.7940) .. controls (1416.8500,391.3010)
            and (1415.8900,390.3430) .. (1416.3600,389.9480);

        \end{scope}
    
    \end{scope}
    
    
    % //////// SLOVAKIA ////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (333.9584,243.5459) .. controls (334.7384,241.5159) and
    (335.7184,241.8749) .. (337.5884,241.8549) .. controls (338.3084,241.8549) and
    (341.3384,240.3509) .. (341.4184,239.6879) .. controls (341.7284,237.1419) and
    (347.7684,235.1899) .. (347.2084,237.0649) .. controls (347.9984,236.9559) and
    (349.6384,235.2209) .. (350.4884,235.5389) .. controls (351.8284,236.0339) and
    (353.2084,237.4499) .. (352.8984,238.0009) .. controls (354.0484,238.9139) and
    (354.4484,238.3429) .. (355.7484,237.3879) .. controls (356.1984,237.0589) and
    (357.4284,236.6559) .. (358.0784,236.8899) .. controls (360.4684,237.7459) and
    (361.4484,236.7379) .. (363.2584,236.7579) .. controls (365.2984,236.7779) and
    (366.2684,236.7579) .. (367.9884,238.4029) .. controls (368.6684,239.0459) and
    (370.3984,239.2389) .. (370.9484,239.4419) .. controls (371.3884,239.5119) and
    (371.3084,239.4319) .. (370.7784,240.9899) .. controls (370.3084,242.3529) and
    (369.0284,243.6889) .. (368.8384,244.8829) .. controls (368.8384,245.1189) and
    (369.3184,245.5219) .. (368.5284,245.4559) .. controls (365.9584,246.8379) and
    (364.6084,244.0289) .. (364.0484,244.2029) .. controls (363.4584,244.3859) and
    (363.3684,244.6839) .. (362.6684,244.5489) .. controls (361.8384,244.3879) and
    (360.8984,244.0699) .. (360.0584,243.9859) .. controls (358.0684,243.7869) and
    (357.6184,244.1779) .. (357.4184,246.0769) .. controls (357.2884,247.3469) and
    (354.1984,248.1129) .. (353.1384,247.5339) .. controls (350.5384,246.1169) and
    (351.6584,247.2479) .. (350.5684,248.1879) .. controls (349.6184,249.0149) and
    (344.7284,248.5099) .. (347.0484,250.3439) .. controls (345.4684,250.5369) and
    (343.8684,251.0989) .. (342.1684,250.9799) .. controls (341.5884,250.9399) and
    (340.5484,251.0699) .. (339.7184,250.8529) .. controls (338.9684,250.6589) and
    (338.1584,250.0089) .. (337.4484,249.6599) .. controls (336.3784,249.1279) and
    (335.0084,248.2199) .. (334.4184,247.1359) .. controls (334.1684,246.6759) and
    (334.4184,246.0989) .. (334.2484,245.6019) .. controls (333.9584,244.6749) and
    (334.1284,244.3869) .. (333.9584,243.5459);
    
    
    % //////// SLOWENIA ////////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country]
    (311.4884,265.9299) .. controls (311.3584,265.3119) and
    (311.9484,264.5569) .. (312.3584,264.2099) .. controls (311.6784,264.0589) and
    (311.0884,263.6829) .. (310.4884,263.3459) .. controls (311.9984,261.6999) and
    (311.2784,260.6959) .. (313.1584,261.1469) .. controls (313.8584,261.3159) and
    (318.0484,262.7919) .. (318.6484,262.2599) .. controls (319.8384,261.1999) and
    (320.9084,260.0309) .. (322.6384,260.1389) .. controls (323.5484,260.1989) and
    (324.6484,260.6459) .. (325.5084,260.1189) .. controls (326.3884,259.5829) and
    (327.4484,259.5349) .. (328.3484,260.0989) .. controls (327.5784,259.1319) and
    (328.7784,257.6119) .. (329.8284,258.4489) .. controls (330.6384,259.0999) and
    (331.6384,260.7319) .. (332.2484,261.6109) .. controls (331.4384,261.4879) and
    (328.7984,260.8119) .. (330.2184,262.4749) .. controls (329.4184,262.4449) and
    (328.9684,261.9159) .. (328.6384,262.8419) .. controls (328.4484,263.3589) and
    (326.4584,263.8279) .. (325.8684,264.1839) .. controls (325.4184,264.4609) and
    (326.2584,265.8269) .. (326.2184,266.4169) .. controls (326.1184,267.3379) and
    (324.0184,267.4069) .. (323.1584,268.1619) .. controls (323.5084,268.2779) and
    (323.8084,268.5849) .. (324.1684,268.6659) .. controls (323.5284,268.7969) and
    (323.9884,271.1049) .. (322.7584,270.3139) .. controls (321.3384,269.4059) and
    (319.9684,269.8229) .. (318.6184,268.5219) .. controls (318.1584,269.6259) and
    (316.5684,270.5709) .. (315.3584,270.0259) .. controls (314.8584,269.8019) and
    (314.8684,269.7869) .. (314.4684,270.1789) .. controls (313.8684,270.7739) and
    (312.6084,270.2689) .. (311.9284,270.1089) .. controls (312.6884,269.4419) and
    (314.2384,269.1899) .. (313.6584,268.1649) .. controls (313.1984,267.3539) and
    (311.1184,267.5669) .. (312.1484,266.2219);

    
    
    % //////// SPAIN ///////////////////////////////////////////////////////////////////////////////

    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path5998
        \path[country]
        (1214.1200,389.0900) .. controls (1214.2200,388.9700) and (1214.2700,388.8500)
        .. (1214.3400,388.7300) .. controls (1213.4100,388.8100) and
        (1213.3800,388.0210) .. (1213.6400,387.3640) .. controls (1214.0500,386.3050)
        and (1214.8000,386.5880) .. (1215.4700,385.8720) .. controls
        (1216.7500,384.4860) and (1219.5300,385.1390) .. (1221.3200,384.3390) ..
        controls (1219.8700,384.3990) and (1220.8000,383.9850) .. (1221.3200,383.6910)
        .. controls (1221.0100,383.8040) and (1220.7000,383.9000) ..
        (1220.3800,383.9790) .. controls (1220.1600,383.0340) and (1223.3400,380.6120)
        .. (1223.3400,382.1790) .. controls (1223.8200,381.8910) and
        (1224.3000,381.6030) .. (1224.7800,381.3150) .. controls (1224.9000,382.3780)
        and (1229.0700,381.8930) .. (1229.1000,383.6910) .. controls
        (1230.3700,382.0470) and (1234.1000,383.3240) .. (1235.8600,383.0440) ..
        controls (1237.3700,382.8040) and (1237.7600,382.7150) .. (1239.3500,383.0940)
        .. controls (1241.0400,383.4970) and (1242.7600,383.8730) ..
        (1244.4800,384.1640) .. controls (1246.8200,384.5610) and (1248.9700,384.3410)
        .. (1251.1200,383.8250) .. controls (1252.4800,383.4990) and
        (1254.0900,383.8050) .. (1255.2800,384.5230) .. controls (1256.9000,385.4990)
        and (1256.6600,384.1460) .. (1258.1600,384.2540) .. controls
        (1259.4900,384.3440) and (1260.7900,384.8770) .. (1262.0900,385.1270) ..
        controls (1262.8700,385.2780) and (1265.4000,384.4360) .. (1265.7400,384.9850)
        .. controls (1266.1200,385.5820) and (1268.4700,384.8570) ..
        (1268.0500,386.2980) .. controls (1267.9500,386.6030) and (1267.5900,386.9680)
        .. (1267.8600,387.2650) .. controls (1268.4700,387.9580) and
        (1268.2800,387.1850) .. (1268.9300,387.2150) .. controls (1270.9800,387.3200)
        and (1273.6900,389.2510) .. (1274.5300,389.5770) .. controls
        (1274.9400,389.7330) and (1275.4200,389.3300) .. (1275.8400,389.4870) ..
        controls (1276.3800,389.6840) and (1276.7400,390.4720) .. (1277.2500,390.3670)
        .. controls (1278.6600,390.0720) and (1280.4500,390.1390) ..
        (1282.1600,390.6070) .. controls (1281.9300,389.9810) and (1282.1600,389.5390)
        .. (1282.5200,389.0950) .. controls (1283.3900,389.1150) and
        (1284.0100,389.1850) .. (1285.5500,390.1360) .. controls (1286.8200,390.1760)
        and (1288.0000,390.5950) .. (1287.7000,392.6950) .. controls
        (1289.4400,392.4180) and (1289.3300,391.1650) .. (1289.4500,392.0290) ..
        controls (1289.7800,392.2160) and (1291.5200,393.2730) .. (1291.9300,393.1380)
        .. controls (1292.4200,392.9810) and (1292.8800,392.6200) ..
        (1293.4400,392.8430) .. controls (1294.5000,393.2680) and (1295.6400,393.6860)
        .. (1296.5200,392.9740) .. controls (1297.1900,392.4300) and
        (1297.8200,392.5080) .. (1299.4300,392.6800) .. controls (1300.0500,392.7500)
        and (1299.5500,393.7410) .. (1300.3000,393.6320) .. controls
        (1300.3000,394.4000) and (1299.8200,394.1650) .. (1299.3800,394.5140) ..
        controls (1298.7400,395.0310) and (1299.3800,396.3080) .. (1299.3800,396.9770)
        .. controls (1299.2800,398.8270) and (1295.2500,400.1630) ..
        (1293.8900,400.7280) .. controls (1292.8600,401.1520) and (1292.5900,402.1170)
        .. (1291.7400,402.5210) .. controls (1290.7100,403.0090) and
        (1289.3000,402.9940) .. (1288.2000,403.2710) .. controls (1285.5300,403.9430)
        and (1283.9100,405.1030) .. (1281.7600,406.5920) .. controls
        (1283.4300,407.9290) and (1281.8600,408.1840) .. (1280.7100,408.8370) ..
        controls (1279.0300,409.7960) and (1278.7100,412.1080) .. (1277.0700,413.1570)
        .. controls (1274.2700,414.9460) and (1273.2800,420.0720) ..
        (1275.5800,422.5210) .. controls (1276.9800,424.0120) and (1278.1100,424.4650)
        .. (1275.8000,425.9090) .. controls (1274.4700,426.7450) and
        (1273.4500,427.0970) .. (1272.3700,428.2890) .. controls (1271.7200,428.9950)
        and (1271.1400,430.0760) .. (1270.6900,431.1040) .. controls
        (1270.4100,431.7490) and (1270.0900,432.4720) .. (1270.0800,433.1880) ..
        controls (1270.0800,433.7850) and (1271.0400,434.5930) .. (1270.4500,433.1580)
        .. controls (1271.3700,434.6700) and (1267.6400,434.7840) ..
        (1266.9200,434.8700) .. controls (1265.1800,435.0790) and (1262.7700,436.6580)
        .. (1262.3500,438.3730) .. controls (1261.9900,439.8470) and
        (1260.7700,442.4740) .. (1259.1900,441.2000) .. controls (1258.2200,440.4200)
        and (1257.5000,441.4700) .. (1256.7000,441.7990) .. controls
        (1255.5400,442.2750) and (1254.2900,441.5590) .. (1253.0600,441.7590) ..
        controls (1250.5000,442.1790) and (1247.9500,441.8850) .. (1245.3300,441.9360)
        .. controls (1243.9300,441.9660) and (1243.6200,442.2240) ..
        (1242.6100,443.1730) .. controls (1241.4500,444.2580) and (1239.9200,443.8130)
        .. (1238.5800,444.4830) .. controls (1237.9200,444.8160) and
        (1237.2600,447.0650) .. (1236.6600,447.0060) .. controls (1235.9200,446.9360)
        and (1236.1100,448.1610) .. (1234.9600,448.1330) .. controls
        (1234.0300,448.1130) and (1233.3200,446.5100) .. (1232.4300,446.6070) ..
        controls (1231.4600,446.7130) and (1230.7200,444.6830) .. (1230.4900,443.9580)
        .. controls (1231.7700,443.7330) and (1230.1800,442.8090) ..
        (1229.8000,442.5170) .. controls (1228.8900,441.8140) and (1229.9700,440.6090)
        .. (1230.8500,440.3570) .. controls (1230.3000,440.1810) and
        (1230.0300,440.4770) .. (1229.9900,441.0050) .. controls (1229.5200,440.5040)
        and (1225.6800,437.9040) .. (1226.5300,437.1160) .. controls
        (1225.2000,436.9700) and (1226.5300,437.6710) .. (1225.0800,437.7030) ..
        controls (1224.4400,437.7130) and (1223.6500,437.9590) .. (1223.0300,437.7330)
        .. controls (1222.1300,437.4070) and (1222.1700,435.1220) ..
        (1222.2900,434.3830) .. controls (1222.4000,433.7370) and (1222.9100,433.2530)
        .. (1223.3400,432.8080) .. controls (1223.8700,432.2610) and
        (1223.9400,431.4010) .. (1224.4000,430.9420) .. controls (1225.4800,429.8870)
        and (1225.9200,430.7010) .. (1226.6100,429.0550) .. controls
        (1225.2400,429.5090) and (1224.1300,427.6870) .. (1224.0900,426.5340) ..
        controls (1223.9900,424.7420) and (1226.1100,423.8680) .. (1226.6200,422.2850)
        .. controls (1226.8900,421.4280) and (1225.2600,420.2820) ..
        (1224.8800,419.5250) .. controls (1224.5600,418.8860) and (1224.8800,418.5130)
        .. (1224.4100,417.9650) .. controls (1224.0100,417.5050) and
        (1223.4800,417.0130) .. (1223.2200,416.4530) .. controls (1224.1300,416.7080)
        and (1225.0900,416.5230) .. (1226.0200,416.5230) .. controls
        (1226.9800,416.5230) and (1226.7200,415.9580) .. (1227.0500,415.3610) ..
        controls (1227.4700,414.6160) and (1228.3100,414.5140) .. (1227.3900,412.2470)
        .. controls (1227.1200,411.5780) and (1228.3500,411.2300) ..
        (1228.4700,411.1710) .. controls (1229.1200,410.8630) and (1228.8900,409.9470)
        .. (1228.8600,409.3920) .. controls (1228.8600,408.9630) and
        (1229.0600,404.7070) .. (1228.5000,404.8440) .. controls (1229.5100,404.6000)
        and (1229.9800,403.5060) .. (1230.9400,402.8980) .. controls
        (1231.5000,402.5470) and (1233.9000,400.4960) .. (1233.6100,399.9180) ..
        controls (1233.2600,399.2070) and (1231.4200,399.3580) .. (1231.3500,398.9220)
        .. controls (1231.2400,398.2460) and (1231.7400,396.3800) ..
        (1231.0200,397.0050) .. controls (1230.5300,397.4290) and (1227.1500,396.4900)
        .. (1227.0700,397.0750) .. controls (1226.9100,398.2960) and
        (1224.9400,397.8460) .. (1224.2500,397.5680) .. controls (1223.1600,397.1210)
        and (1222.0400,397.6380) .. (1221.0100,398.0070) .. controls
        (1218.9000,398.7670) and (1220.1900,396.5800) .. (1221.0100,395.9990) ..
        controls (1220.3800,396.0790) and (1220.1200,395.7350) .. (1220.2200,395.1350)
        .. controls (1219.6000,395.7260) and (1218.7600,395.7470) ..
        (1217.9800,395.8900) .. controls (1216.9900,396.0700) and (1216.4100,396.8730)
        .. (1215.5400,397.2950) .. controls (1214.7500,395.2320) and
        (1217.0400,395.0080) .. (1217.5500,393.4060) .. controls (1217.1800,394.1100)
        and (1216.4200,394.3310) .. (1215.6800,394.3430) .. controls
        (1215.8400,393.5200) and (1216.6200,393.1920) .. (1217.2700,392.8310) ..
        controls (1216.6100,393.1200) and (1215.6300,393.1930) .. (1215.6800,392.1830)
        .. controls (1215.6800,391.4630) and (1216.8500,391.1880) ..
        (1216.9800,390.4550) .. controls (1216.3400,391.0510) and (1215.3300,390.9920)
        .. (1214.9600,391.8940) .. controls (1214.2400,390.8540) and
        (1215.3900,390.0170) .. (1216.1100,389.4460) .. controls (1215.3800,390.0340)
        and (1214.4500,390.1960) .. (1214.1700,389.0900);

        % path6006
        \path[country]
        (1285.8300,423.6500) .. controls (1284.3900,423.3890) and
        (1284.9400,422.0700) .. (1285.9300,421.5720) .. controls (1286.3900,421.3370)
        and (1286.9800,421.2600) .. (1287.3900,421.6320) .. controls
        (1288.0800,422.2650) and (1286.1500,423.0010) .. (1285.8600,423.6470);

        % path6008
        \path[country]
        (1285.9000,425.3000) .. controls (1285.6700,424.4730) and
        (1285.9000,424.3280) .. (1286.6200,424.8680) .. controls (1286.3800,425.0120)
        and (1286.1400,425.1560) .. (1285.9000,425.3000);

        % path6010
        \path[country]
        (1299.5100,418.6100) .. controls (1298.1600,420.1300) and
        (1298.2900,419.3680) .. (1296.6700,419.1050) .. controls (1294.9500,418.8260)
        and (1296.1000,416.9750) .. (1294.1300,417.8220) .. controls
        (1292.3800,418.5730) and (1293.8200,416.4620) .. (1294.3200,416.0980) ..
        controls (1295.8300,415.0050) and (1297.4000,414.5150) .. (1299.1500,413.9310)
        .. controls (1298.4200,414.1390) and (1298.1200,415.0560) ..
        (1298.8200,415.5590) .. controls (1299.3600,415.9510) and (1300.1300,415.4090)
        .. (1300.6400,415.8090) .. controls (1301.3300,416.3570) and
        (1299.5600,418.0040) .. (1299.5100,418.6100);

        % path6012
        \path[country]
        (1303.2600,413.6400) .. controls (1304.5500,412.4160) and
        (1306.7100,413.3520) .. (1306.8600,415.0800) .. controls (1305.9400,415.2270)
        and (1303.7500,414.4760) .. (1303.2600,413.6400);
    
    \end{scope}
    
    
    % //////// SWEDEN //////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path3388
        \path[country]
        (1357.4700,260.9300) .. controls (1356.9900,261.1700) and
        (1356.5100,261.4100) .. (1356.0300,261.6500) .. controls (1356.4400,262.2120)
        and (1358.0700,262.4800) .. (1358.3900,261.6400) .. controls
        (1358.5900,261.1150) and (1357.9400,260.2440) .. (1357.4700,260.9340);

        % path3390
        \path[country]
        (1357.1100,262.5100) .. controls (1356.9600,262.7500) and
        (1356.8200,262.9890) .. (1356.6800,263.2300) .. controls (1357.2800,263.3200)
        and (1357.8000,262.9850) .. (1358.0500,262.4380) .. controls
        (1357.7300,262.4580) and (1357.4200,262.4880) .. (1357.1100,262.5080);

        % path3392
        \path[country]
        (1387.3500,275.5400) .. controls (1387.4700,275.9880) and
        (1387.5100,276.4440) .. (1387.4900,276.9070) .. controls (1388.7000,276.6590)
        and (1389.2100,274.3760) .. (1389.4800,273.4060) .. controls
        (1390.0000,271.5720) and (1390.8900,269.9530) .. (1391.6000,268.1960) ..
        controls (1390.4100,268.1660) and (1390.0700,270.3530) .. (1389.6000,271.1120)
        .. controls (1388.7400,272.4860) and (1386.9500,273.6380) ..
        (1387.3500,275.5400);

        % path3394
        \path[country]
        (1397.4300,254.7300) .. controls (1397.1900,254.8500) and
        (1396.9500,254.9700) .. (1396.7100,255.0900) .. controls (1396.9800,255.0400)
        and (1397.2200,254.9170) .. (1397.4300,254.7300);

        % path3396
        \path[country]
        (1399.4500,270.9300) .. controls (1399.1500,270.1120) and
        (1401.9300,267.8450) .. (1402.5400,267.4020) .. controls (1399.8000,267.1390)
        and (1405.8300,262.8660) .. (1401.3800,263.7910) .. controls
        (1400.1300,264.0520) and (1398.9700,265.1040) .. (1398.1400,266.0460) ..
        controls (1397.4100,266.8900) and (1397.7300,269.9990) .. (1399.0100,270.2110)
        .. controls (1398.6000,270.6640) and (1398.2600,271.1680) ..
        (1398.0100,271.7230) .. controls (1398.6400,271.8540) and (1399.1600,271.4660)
        .. (1399.4500,270.9300);

        % path3398
        \path[country]
        (1398.0800,243.8600) .. controls (1398.3900,244.2030) and
        (1398.7700,244.3470) .. (1399.2300,244.2920) .. controls (1398.9000,243.7640)
        and (1398.4300,243.3240) .. (1397.8600,243.0690) .. controls
        (1397.9600,243.3320) and (1398.0000,243.5960) .. (1398.0800,243.8600);

        % path3400
        \path[country]
        (1399.0100,254.1600) .. controls (1398.8400,254.4000) and
        (1398.6800,254.6400) .. (1398.5100,254.8810) .. controls (1399.0000,254.7060)
        and (1399.0200,254.6010) .. (1399.0100,254.1600);

        % path3402
        \path[country]
        (1399.7400,251.2100) .. controls (1399.9800,251.0650) and
        (1400.2100,250.9220) .. (1400.4500,250.7770) .. controls (1399.8600,250.5440)
        and (1399.4700,250.7970) .. (1399.4500,251.4250) .. controls
        (1399.5500,251.3550) and (1399.6400,251.2830) .. (1399.7400,251.2100);

        % path3404
        \path[country]
        (1403.3300,263.7300) .. controls (1403.8700,263.9420) and
        (1404.3600,263.8460) .. (1404.7800,263.4430) .. controls (1404.2500,262.8040)
        and (1403.6100,263.0260) .. (1403.3300,263.7300);

        % path3452
        \path[country]
        (1354.5900,254.1600) .. controls (1355.6500,253.9750) and (1355.9800,255.9660)
        .. (1356.7400,255.7610) .. controls (1357.9400,255.4350) and
        (1358.2600,252.6800) .. (1357.8500,251.7890) .. controls (1357.1300,250.2010)
        and (1358.8100,249.8450) .. (1358.5700,248.4930) .. controls
        (1358.2200,246.5530) and (1361.7100,247.8340) .. (1362.1700,245.8190) ..
        controls (1362.5000,244.3370) and (1362.9800,243.3100) .. (1362.0000,241.9700)
        .. controls (1361.4600,241.2300) and (1360.1100,239.3800) ..
        (1361.6000,238.7440) .. controls (1363.1000,238.1100) and (1363.5700,238.7740)
        .. (1364.1100,236.7300) .. controls (1364.4800,235.3470) and
        (1362.8900,235.0940) .. (1361.9600,234.7490) .. controls (1360.2600,234.1080)
        and (1359.8000,232.8250) .. (1360.2300,231.2460) .. controls
        (1360.7500,229.3550) and (1360.4600,228.3630) .. (1359.8100,226.6210) ..
        controls (1359.5600,225.9360) and (1359.1500,224.8620) .. (1359.5400,224.1720)
        .. controls (1359.8500,223.6130) and (1360.2500,223.7220) ..
        (1360.0600,223.1640) .. controls (1359.8200,222.4760) and (1359.2900,222.0740)
        .. (1359.1700,221.3100) .. controls (1359.0300,220.3860) and
        (1359.8900,219.9110) .. (1359.8600,219.2040) .. controls (1359.7600,217.9030)
        and (1361.9700,216.7700) .. (1362.5900,216.2650) .. controls
        (1364.4300,214.7750) and (1366.1600,214.9840) .. (1368.0700,215.2580) ..
        controls (1369.3400,215.4400) and (1371.5900,215.5020) .. (1371.2500,213.7340)
        .. controls (1370.9000,211.9790) and (1369.0400,211.8020) ..
        (1368.2700,211.2480) .. controls (1368.9600,210.3970) and (1369.7400,209.6260)
        .. (1370.5200,208.8520) .. controls (1371.2300,208.1440) and
        (1372.1500,206.3270) .. (1372.9600,205.8880) .. controls (1373.9900,205.3340)
        and (1373.3100,200.2930) .. (1373.0900,199.5120) .. controls
        (1374.6600,199.5720) and (1376.7500,199.4520) .. (1378.1200,198.5820) ..
        controls (1378.7700,198.1670) and (1378.1200,197.5510) .. (1378.1200,197.0810)
        .. controls (1378.0200,196.5670) and (1379.0200,196.3800) ..
        (1379.3000,196.0800) .. controls (1380.5800,194.7200) and (1381.8700,193.8080)
        .. (1383.2900,192.6440) .. controls (1384.4600,191.6910) and
        (1382.2200,190.3110) .. (1381.7100,189.8640) .. controls (1384.0200,188.8040)
        and (1384.6700,186.5890) .. (1386.9000,185.5440) .. controls
        (1388.3300,184.8740) and (1389.2200,185.0580) .. (1390.6800,185.3870) ..
        controls (1391.4200,185.5530) and (1393.0600,185.0260) .. (1392.9600,184.0470)
        .. controls (1392.8600,183.3940) and (1392.3100,182.4600) ..
        (1392.5900,181.8020) .. controls (1392.9400,180.9710) and (1395.5600,181.9870)
        .. (1396.1600,181.8720) .. controls (1397.6600,181.5810) and
        (1402.0900,183.5940) .. (1404.3200,182.0870) .. controls (1403.8300,181.8680)
        and (1403.3300,181.7000) .. (1402.8100,181.5830) .. controls
        (1404.0400,180.8270) and (1405.7400,179.1440) .. (1403.6000,178.2700) ..
        controls (1406.8700,176.8050) and (1410.5100,180.0560) .. (1413.3200,181.2940)
        .. controls (1415.2300,182.1400) and (1417.6200,182.1600) ..
        (1419.5100,183.0100) .. controls (1420.1300,183.2880) and (1423.4500,185.2900)
        .. (1423.8100,186.0140) .. controls (1424.1100,186.6370) and
        (1423.2100,186.6150) .. (1423.0700,186.9860) .. controls (1422.9700,187.1260)
        and (1423.1700,187.3100) .. (1423.2100,189.0310) .. controls
        (1423.2100,189.4600) and (1424.0400,189.5650) .. (1424.4200,189.6660) ..
        controls (1425.8700,190.0580) and (1424.8300,190.7110) .. (1424.3200,191.3450)
        .. controls (1423.7700,192.0420) and (1425.5000,193.1290) ..
        (1425.9200,193.4660) .. controls (1426.8700,194.2210) and (1426.5900,195.7040)
        .. (1425.8000,196.5860) .. controls (1424.1700,198.3900) and
        (1428.1800,200.1820) .. (1428.6900,201.9120) .. controls (1427.0800,202.1320)
        and (1424.2800,203.0010) .. (1422.9000,201.7400) .. controls
        (1423.1300,201.9670) and (1423.3400,202.2070) .. (1423.5400,202.4610) ..
        controls (1422.3800,202.4610) and (1421.4300,202.2110) .. (1420.4500,201.5970)
        .. controls (1420.2600,203.5680) and (1418.4700,200.6970) ..
        (1418.0700,202.0920) .. controls (1417.8800,202.7550) and (1418.6900,203.4270)
        .. (1418.7900,204.0450) .. controls (1418.0600,204.0250) and
        (1417.3700,203.7630) .. (1416.7100,203.4690) .. controls (1416.9600,203.6260)
        and (1417.2300,203.7700) .. (1417.5000,203.9010) .. controls
        (1416.9800,204.2590) and (1416.4300,204.3310) .. (1415.8400,204.1180) ..
        controls (1418.1700,204.8060) and (1414.0600,205.1390) .. (1413.6100,205.1980)
        .. controls (1414.0900,206.0110) and (1415.2700,206.3300) ..
        (1414.2600,207.6450) .. controls (1413.9100,208.1000) and (1411.9800,209.4520)
        .. (1411.3800,209.1570) .. controls (1411.7800,209.6160) and
        (1412.2900,209.9040) .. (1412.8900,210.0210) .. controls (1410.8400,210.4520)
        and (1414.5800,211.7400) .. (1414.9800,212.3970) .. controls
        (1413.5700,213.0760) and (1411.5900,213.8620) .. (1411.0300,215.4760) ..
        controls (1410.7000,216.4030) and (1408.1500,217.4790) .. (1408.3500,218.3010)
        .. controls (1408.2000,218.0280) and (1408.0300,217.7640) ..
        (1407.8500,217.5090) .. controls (1407.4800,218.4440) and (1406.1900,218.7540)
        .. (1405.3200,218.9120) .. controls (1404.3900,219.0780) and
        (1404.1000,220.9580) .. (1403.2400,219.3080) .. controls (1403.4700,220.5220)
        and (1403.2400,219.8670) .. (1402.3700,219.8960) .. controls
        (1401.9000,219.9160) and (1401.5100,220.9980) .. (1401.0900,221.2900) ..
        controls (1399.5700,222.3450) and (1397.6300,222.2120) .. (1396.0400,223.4130)
        .. controls (1396.5400,223.4730) and (1397.0400,223.5030) ..
        (1397.5500,223.4830) .. controls (1397.5500,224.2870) and (1396.9100,224.8190)
        .. (1396.1500,224.4410) .. controls (1395.7400,224.2340) and
        (1395.5100,225.3680) .. (1394.7500,224.9960) .. controls (1396.5800,224.8070)
        and (1394.3300,224.6340) .. (1394.0300,224.7080) .. controls
        (1394.2000,223.8930) and (1393.1600,223.5380) .. (1393.0900,222.7640) ..
        controls (1392.8300,223.9190) and (1394.1600,224.5850) .. (1394.3300,225.6390)
        .. controls (1394.5900,227.2660) and (1392.3700,228.3790) ..
        (1391.2900,227.0840) .. controls (1390.7300,228.3720) and (1391.4600,229.2990)
        .. (1392.8000,229.3880) .. controls (1391.9200,229.5060) and
        (1391.4600,230.9100) .. (1391.2900,231.6200) .. controls (1391.0300,232.7090)
        and (1392.4400,233.2670) .. (1392.0800,234.2120) .. controls
        (1391.5000,233.6280) and (1390.6900,233.1920) .. (1389.8500,233.4200) ..
        controls (1392.5800,234.0370) and (1388.3000,233.8190) .. (1390.6400,234.2840)
        .. controls (1388.6300,234.0960) and (1390.0100,234.5220) ..
        (1390.5400,234.7160) .. controls (1388.4400,234.3370) and (1391.7700,235.5910)
        .. (1389.7500,235.7960) .. controls (1390.7800,236.1540) and
        (1390.2000,237.5400) .. (1390.2700,238.3050) .. controls (1390.3700,239.4320)
        and (1391.0700,240.0590) .. (1391.6200,240.9800) .. controls
        (1391.3600,241.1090) and (1391.0900,241.2290) .. (1390.8300,241.3400) ..
        controls (1391.2000,241.5590) and (1392.9400,241.6640) .. (1393.0800,241.9770)
        .. controls (1393.6900,243.3250) and (1394.5900,242.3280) ..
        (1395.5800,242.1320) .. controls (1395.0300,244.1130) and (1398.4700,243.8310)
        .. (1399.2500,244.9400) .. controls (1397.4300,245.3030) and
        (1399.8900,245.9770) .. (1400.4700,246.0920) .. controls (1400.8900,246.1720)
        and (1403.1000,249.0810) .. (1401.3400,247.6760) .. controls
        (1401.8400,248.0940) and (1402.2600,248.6110) .. (1402.5600,249.1880) ..
        controls (1401.4500,249.2280) and (1400.6200,249.8350) .. (1399.7700,250.4730)
        .. controls (1399.0200,251.0390) and (1396.8400,251.3680) ..
        (1398.2400,251.8520) .. controls (1397.6900,251.9980) and (1397.2100,251.8820)
        .. (1396.8000,251.4920) .. controls (1396.6800,252.3770) and
        (1399.4300,252.9040) .. (1399.1100,251.5620) .. controls (1399.6100,251.8380)
        and (1400.6400,253.5160) .. (1399.2100,252.7140) .. controls
        (1401.1100,253.3680) and (1398.4200,252.6840) .. (1398.0600,252.5710) ..
        controls (1398.1700,253.1630) and (1398.6200,253.6040) .. (1399.2100,253.7210)
        .. controls (1398.6100,254.0390) and (1397.9300,254.0860) ..
        (1397.3100,254.3170) .. controls (1396.4400,254.6380) and (1396.3400,255.5070)
        .. (1395.6300,255.9490) .. controls (1395.1500,256.2450) and
        (1394.8100,254.3290) .. (1394.0300,254.3700) .. controls (1394.4900,254.7410)
        and (1394.6800,255.2210) .. (1394.6000,255.8090) .. controls
        (1394.3600,255.6410) and (1394.1200,255.4730) .. (1393.8800,255.3050) ..
        controls (1394.1000,255.9710) and (1394.1000,256.4570) .. (1393.1600,256.0260)
        .. controls (1393.2900,256.2620) and (1393.4100,256.5020) ..
        (1393.5200,256.7460) .. controls (1392.5800,257.2670) and (1391.5900,257.2080)
        .. (1390.5700,257.1050) .. controls (1390.8200,257.2860) and
        (1391.0600,257.4780) .. (1391.2900,257.6810) .. controls (1389.6900,258.5310)
        and (1387.6700,257.0030) .. (1386.1800,258.1140) .. controls
        (1387.3900,257.8130) and (1389.1300,257.9480) .. (1389.7800,259.1940) ..
        controls (1388.8100,259.7250) and (1387.8300,259.2440) .. (1386.8300,259.1940)
        .. controls (1388.3500,259.7240) and (1390.9800,262.1650) ..
        (1388.3400,263.1530) .. controls (1388.9800,263.0040) and (1389.2100,263.3410)
        .. (1389.0600,263.9460) .. controls (1388.5600,263.6690) and
        (1388.0300,263.5960) .. (1387.4700,263.7290) .. controls (1387.8100,264.1700)
        and (1389.6100,265.1770) .. (1388.3700,265.6710) .. controls
        (1387.2800,266.1090) and (1389.3200,266.7570) .. (1388.6900,267.5830) ..
        controls (1387.2500,269.4750) and (1388.5900,271.4470) .. (1387.0300,273.4200)
        .. controls (1386.0200,274.6920) and (1385.5000,278.3740) ..
        (1383.1900,277.6820) .. controls (1381.8100,277.2680) and (1380.3700,277.9160)
        .. (1378.9700,277.8260) .. controls (1378.1900,277.7760) and
        (1376.1900,277.6060) .. (1377.2500,278.9220) .. controls (1375.8900,279.4520)
        and (1374.7100,278.6300) .. (1373.9200,280.3850) .. controls
        (1373.4600,281.3880) and (1374.5500,282.1650) .. (1374.6500,283.1240) ..
        controls (1374.8300,284.9270) and (1372.3500,283.7340) .. (1371.6200,283.7990)
        .. controls (1369.3200,284.0060) and (1367.4500,284.0850) ..
        (1365.1500,283.9620) .. controls (1365.8900,283.9320) and (1366.4100,281.6450)
        .. (1365.7200,280.9120) .. controls (1364.9500,280.1030) and
        (1363.0600,277.9100) .. (1363.1400,276.7620) .. controls (1365.6000,277.6240)
        and (1364.1700,276.7620) .. (1364.0000,275.3940) .. controls
        (1367.3500,274.8400) and (1364.1000,273.7280) .. (1363.2500,272.5840) ..
        controls (1362.4600,271.4820) and (1361.3300,270.5830) .. (1360.8300,269.2950)
        .. controls (1360.5100,268.4700) and (1360.1500,267.3880) ..
        (1359.0300,267.7610) .. controls (1359.0300,267.2100) and (1359.1300,266.6380)
        .. (1359.0300,266.0910) .. controls (1358.8200,265.1460) and
        (1357.2600,265.0170) .. (1358.6900,264.5210) .. controls (1357.3100,265.0130)
        and (1358.6900,260.7300) .. (1358.7900,260.2020) .. controls
        (1357.8700,260.0090) and (1357.4000,261.0400) .. (1356.4800,260.9220) ..
        controls (1356.8900,260.4370) and (1357.2700,259.9330) .. (1357.6300,259.4100)
        .. controls (1356.2900,259.2740) and (1357.3600,260.1750) ..
        (1356.1200,260.5610) .. controls (1355.9900,259.8850) and (1355.5100,259.7330)
        .. (1354.9700,260.1290) .. controls (1355.5400,258.7750) and
        (1353.4500,255.0020) .. (1354.6800,254.1570);

    \end{scope}
    
    
    % //////// SWITZERLAND /////////////////////////////////////////////////////////////////////////
    
    \path[shift={(-12.49595,1.66613)}, country, we]
    (260.0184,264.4979) .. controls (260.2384,264.0629) and
    (260.4884,263.6409) .. (260.7484,263.2289) .. controls (261.0784,262.5819) and
    (260.5684,262.0619) .. (260.7484,261.4539) .. controls (261.0884,260.5449) and
    (262.6484,259.8379) .. (262.7084,259.5479) .. controls (262.9184,258.3819) and
    (263.4984,257.6409) .. (265.1584,256.6939) .. controls (266.0584,256.1829) and
    (266.6284,255.1219) .. (267.4884,254.2749) .. controls (265.8784,254.4679) and
    (266.8584,251.9419) .. (268.1784,253.1409) .. controls (269.6084,254.4309) and
    (270.2484,252.3099) .. (271.6284,252.1149) .. controls (270.9084,252.9559) and
    (274.5484,252.3099) .. (275.2184,252.3449) .. controls (276.5184,252.4149) and
    (277.5484,252.4539) .. (277.8284,251.6279) .. controls (276.8284,251.9989) and
    (276.6284,251.0729) .. (277.5284,250.7629) .. controls (277.8984,250.6369) and
    (278.2684,250.7729) .. (278.8284,250.9949) .. controls (279.7784,251.3659) and
    (280.9784,251.3889) .. (281.1784,251.4609) .. controls (282.2884,251.8789) and
    (283.6784,252.0359) .. (284.5784,252.8279) .. controls (285.7684,253.8689) and
    (283.9984,255.5649) .. (283.7984,256.7229) .. controls (286.0984,256.4339) and
    (286.2784,258.0969) .. (288.1584,258.4609) .. controls (288.9684,258.6179) and
    (289.2884,257.0869) .. (290.1684,257.3379) .. controls (291.2084,257.6309) and
    (290.3184,258.7919) .. (290.2684,259.3249) .. controls (290.1684,259.7389) and
    (291.1084,261.0329) .. (290.1684,261.0579) .. controls (289.5084,261.0779) and
    (288.9884,259.8829) .. (288.3584,260.4389) .. controls (288.1284,260.6389) and
    (287.3484,261.8149) .. (287.8984,262.0649) .. controls (288.8584,262.5059) and
    (288.2884,262.8409) .. (288.1384,263.7779) .. controls (287.1984,263.4019) and
    (287.1584,262.3899) .. (285.9784,262.6259) .. controls (284.8184,262.8559) and
    (284.6984,263.1009) .. (283.7484,262.1939) .. controls (283.6484,262.1039) and
    (282.6284,260.3519) .. (282.4884,261.7849) .. controls (282.3584,263.0989) and
    (282.3884,263.4189) .. (281.4284,264.4119) .. controls (280.2184,265.6779) and
    (281.3084,268.6459) .. (279.3784,265.8119) .. controls (278.9384,265.1809) and
    (278.4284,264.8719) .. (277.8384,264.4259) .. controls (276.9284,263.7459) and
    (277.2884,262.4539) .. (276.3984,261.8329) .. controls (275.8884,262.4749) and
    (275.2784,263.1239) .. (274.4584,263.3459) .. controls (275.3584,264.3929) and
    (273.3784,266.2349) .. (272.2684,266.1319) .. controls (270.1684,265.9379) and
    (268.4284,267.2679) .. (266.8284,265.5779) .. controls (266.2584,264.9819) and
    (265.4784,264.3559) .. (265.6684,263.4179) .. controls (265.9484,262.1069) and
    (264.9084,261.7919) .. (263.7884,261.9049) .. controls (261.9084,262.0959) and
    (262.2284,264.4409) .. (259.9884,264.4979);
    
    
    % //////// TURKEY //////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path3456
        \path[country]
        (1459.2400,407.0520) .. controls (1459.9900,406.6960) and
        (1461.0200,405.6750) .. (1461.2400,404.8640) .. controls (1461.5900,403.6000)
        and (1460.6200,402.6510) .. (1462.3800,401.8600) .. controls
        (1463.3300,401.4270) and (1462.9800,401.4210) .. (1462.7400,400.4140) ..
        controls (1462.6000,399.8230) and (1462.3700,399.2320) .. (1461.7300,399.0240)
        .. controls (1459.4300,398.2730) and (1462.2700,397.9110) ..
        (1462.1400,396.9910) .. controls (1462.1400,396.7350) and (1464.5900,396.0240)
        .. (1465.0000,395.8920) .. controls (1466.3200,395.4610) and
        (1467.1000,395.0170) .. (1468.0600,396.1070) .. controls (1468.9600,397.1240)
        and (1469.4600,396.4720) .. (1470.6000,396.3590) .. controls
        (1471.1300,396.3090) and (1471.7500,396.3590) .. (1472.1800,396.7180) ..
        controls (1472.9100,397.3240) and (1471.8200,397.5340) .. (1472.3300,398.1990)
        .. controls (1474.2600,400.6800) and (1476.5100,401.7580) ..
        (1479.5700,402.6760) .. controls (1480.7500,403.0300) and (1479.7700,404.7530)
        .. (1479.0400,405.0240) .. controls (1477.6400,405.5420) and
        (1475.6100,404.1860) .. (1474.1800,404.1030) .. controls (1473.4800,404.0630)
        and (1473.0500,404.5530) .. (1472.4700,404.8510) .. controls
        (1471.7500,405.2170) and (1471.0000,404.5820) .. (1470.1800,404.8310) ..
        controls (1469.1900,405.1290) and (1468.7800,406.1990) .. (1468.1000,406.9440)
        .. controls (1466.9800,408.1540) and (1465.4900,408.4960) ..
        (1464.2100,409.4300) .. controls (1463.1200,410.2220) and (1462.0700,412.4320)
        .. (1460.9000,412.8870) .. controls (1460.5400,411.4850) and
        (1461.1400,410.0270) .. (1462.5200,409.5360) .. controls (1462.7600,409.4460)
        and (1465.4100,408.6470) .. (1464.5400,407.9290) .. controls
        (1463.1200,406.7620) and (1459.9300,409.8890) .. (1459.2400,407.0550);
        
        % path3458
        \path[country]
        (1460.1800,417.9240) .. controls (1460.2800,417.1790) and
        (1460.3700,413.4920) .. (1460.9200,413.2810) .. controls (1462.2900,412.7600)
        and (1462.7300,410.7800) .. (1464.1400,410.0750) .. controls
        (1464.8900,409.7000) and (1465.8600,410.3620) .. (1466.5600,409.8730) ..
        controls (1467.4300,409.2610) and (1467.8100,409.7270) .. (1468.5800,410.1870)
        .. controls (1469.6800,410.8480) and (1473.2400,410.5670) ..
        (1470.9800,409.2110) .. controls (1471.7000,408.9190) and (1472.4700,408.9570)
        .. (1473.2100,409.1410) .. controls (1472.8400,409.2730) and
        (1472.6700,409.5070) .. (1472.6700,409.8420) .. controls (1473.1000,410.4320)
        and (1475.2400,410.0840) .. (1475.7800,410.0340) .. controls
        (1477.4600,409.8810) and (1479.8800,410.8590) .. (1481.2800,409.6450) ..
        controls (1480.6100,408.9900) and (1479.7400,409.5650) .. (1479.0400,408.9980)
        .. controls (1479.9400,406.6940) and (1484.0900,407.5620) ..
        (1485.9600,407.1260) .. controls (1484.3400,406.3310) and (1482.0400,406.9990)
        .. (1480.6800,405.6090) .. controls (1479.1600,404.0490) and
        (1480.6800,402.7550) .. (1482.3200,402.9090) .. controls (1484.1100,403.0780)
        and (1485.9000,403.9110) .. (1487.7200,403.5140) .. controls
        (1490.1500,402.9850) and (1492.1200,404.3100) .. (1494.6000,404.0650) ..
        controls (1495.7400,403.9520) and (1495.9100,403.3650) .. (1496.3400,402.4710)
        .. controls (1496.8000,401.4860) and (1498.5500,401.0550) ..
        (1499.4400,400.5340) .. controls (1502.0100,399.0300) and (1504.0500,397.7080)
        .. (1506.9500,396.9230) .. controls (1509.9800,396.1040) and
        (1512.3000,396.5410) .. (1515.3700,396.5410) .. controls (1516.6100,396.5410)
        and (1517.9200,397.0510) .. (1519.1500,396.6850) .. controls
        (1519.7200,396.5150) and (1519.9000,395.8380) .. (1520.4500,395.6770) ..
        controls (1521.0100,395.5140) and (1521.4900,395.8440) .. (1522.0300,395.8930)
        .. controls (1521.1100,397.0000) and (1522.6800,398.5050) ..
        (1523.6900,398.8100) .. controls (1524.4500,399.0410) and (1525.2300,399.2320)
        .. (1526.0300,399.1270) .. controls (1526.9100,399.0130) and
        (1527.6500,398.0280) .. (1527.6500,399.2770) .. controls (1527.8500,397.4210)
        and (1529.0400,399.6790) .. (1529.2200,400.2100) .. controls
        (1529.4500,400.9120) and (1531.3600,403.2870) .. (1532.1200,402.4800) ..
        controls (1533.1100,401.4140) and (1534.1700,401.6490) .. (1535.2400,402.5000)
        .. controls (1536.5400,403.5410) and (1538.1400,403.7290) ..
        (1539.5900,404.4560) .. controls (1540.4100,404.8680) and (1540.5500,403.1770)
        .. (1541.6700,404.4060) .. controls (1542.5800,405.3980) and
        (1544.3300,405.3740) .. (1545.5700,405.4980) .. controls (1547.2900,405.6710)
        and (1549.0500,404.4810) .. (1550.7800,404.3110) .. controls
        (1552.2600,404.1650) and (1553.0700,403.9710) .. (1554.4800,404.4770) ..
        controls (1556.4600,405.1860) and (1557.9300,405.6700) .. (1559.9600,404.7160)
        .. controls (1562.4100,403.5710) and (1564.6400,402.2660) ..
        (1566.7300,400.5850) .. controls (1567.5700,399.9120) and (1568.3400,401.0510)
        .. (1569.1900,401.0690) .. controls (1569.7100,401.0790) and
        (1569.6600,400.3720) .. (1570.2700,400.4930) .. controls (1570.6600,400.5730)
        and (1571.0500,400.6600) .. (1571.4400,400.7400) .. controls
        (1572.0100,400.8570) and (1573.6300,401.4950) .. (1573.9800,400.7300) ..
        controls (1574.4000,399.7920) and (1576.4400,399.0100) .. (1575.8100,400.4220)
        .. controls (1576.4500,400.3010) and (1577.0100,400.7140) ..
        (1577.4700,401.0980) .. controls (1577.8000,401.3980) and (1578.1500,401.6810)
        .. (1578.5100,401.9450) .. controls (1579.0800,402.0150) and
        (1579.2200,402.2850) .. (1578.9000,402.7510) .. controls (1579.1700,403.5570)
        and (1580.2600,402.7710) .. (1580.7000,403.4310) .. controls
        (1580.9900,403.8600) and (1581.1800,405.1320) .. (1581.6100,405.4780) ..
        controls (1582.9700,406.5790) and (1584.0800,407.6790) .. (1583.3000,408.8040)
        .. controls (1582.5300,409.9150) and (1584.6100,411.5650) ..
        (1583.5200,412.3020) .. controls (1585.2700,413.1870) and (1586.1700,412.9850)
        .. (1588.0000,413.0530) .. controls (1589.5700,413.1130) and
        (1591.7800,415.1950) .. (1592.3700,416.5500) .. controls (1591.5100,415.8460)
        and (1590.2100,414.8250) .. (1589.8500,416.5500) .. controls
        (1589.7400,417.0820) and (1589.8500,417.6410) .. (1589.7200,418.1710) ..
        controls (1589.5000,418.8570) and (1587.6900,418.4940) .. (1587.1200,418.7100)
        .. controls (1587.5400,419.2080) and (1588.3800,420.4920) ..
        (1588.5400,421.1170) .. controls (1588.8100,422.1600) and (1589.2700,422.7030)
        .. (1589.6400,423.6690) .. controls (1590.1900,425.0900) and
        (1589.6400,427.1670) .. (1591.5100,427.7820) .. controls (1590.8900,428.3630)
        and (1590.5300,429.5280) .. (1590.3400,430.3240) .. controls
        (1589.9500,431.9220) and (1591.6100,431.6880) .. (1592.4500,432.4620) ..
        controls (1593.2900,433.2390) and (1593.1200,434.2640) .. (1593.3900,435.2800)
        .. controls (1593.5300,435.7880) and (1594.4200,436.0130) ..
        (1594.7800,436.3260) .. controls (1595.1700,436.6720) and (1594.7800,437.4930)
        .. (1595.0400,437.9330) .. controls (1593.3600,436.7500) and
        (1592.6700,439.6900) .. (1591.7000,439.3720) .. controls (1590.4600,438.9600)
        and (1591.4800,437.3200) .. (1590.5700,436.7090) .. controls
        (1590.1100,436.4040) and (1589.3500,436.4320) .. (1588.9400,436.8090) ..
        controls (1588.1900,437.4810) and (1587.1000,437.3240) .. (1586.2200,437.0480)
        .. controls (1584.7900,436.5980) and (1583.6800,436.1250) ..
        (1582.1700,436.1470) .. controls (1581.0900,436.1670) and (1580.4200,435.8640)
        .. (1579.8600,436.8090) .. controls (1579.1800,437.9530) and
        (1577.8200,438.9810) .. (1577.3500,437.2750) .. controls (1576.9400,435.7880)
        and (1575.0700,437.5770) .. (1574.2500,437.8430) .. controls
        (1572.1300,438.5270) and (1570.3600,438.5070) .. (1568.2200,438.2240) ..
        controls (1564.3700,437.7160) and (1561.0500,441.5900) .. (1557.1500,441.8610)
        .. controls (1555.6000,441.9690) and (1552.7900,442.3530) ..
        (1551.4800,441.3650) .. controls (1550.0600,440.2870) and (1549.1700,439.6680)
        .. (1547.4100,440.5220) .. controls (1545.5300,441.4340) and
        (1541.4400,443.5850) .. (1539.8200,441.5810) .. controls (1539.0100,440.5760)
        and (1537.2900,440.2270) .. (1537.0400,441.8090) .. controls
        (1536.8000,443.3650) and (1537.3400,444.4540) .. (1538.0100,445.7860) ..
        controls (1537.3000,445.8260) and (1536.5500,446.0270) .. (1535.8500,445.8560)
        .. controls (1535.7300,446.4720) and (1536.1400,447.1230) ..
        (1535.9500,447.7280) .. controls (1535.6900,448.4460) and (1534.7400,448.5970)
        .. (1534.5100,449.3840) .. controls (1533.9700,449.0210) and
        (1533.4200,448.6110) .. (1532.7800,448.4480) .. controls (1533.4000,447.6410)
        and (1532.5400,446.5920) .. (1532.0600,445.9880) .. controls
        (1531.1500,444.8620) and (1532.1600,444.1990) .. (1533.0700,443.3840) ..
        controls (1534.0300,442.5470) and (1534.6600,441.9570) .. (1533.7200,440.6900)
        .. controls (1533.3400,440.1840) and (1532.5600,439.5590) ..
        (1532.0200,440.2520) .. controls (1531.2800,441.2100) and (1530.5300,441.0590)
        .. (1529.6100,441.7520) .. controls (1531.1400,441.5960) and
        (1529.6100,443.1390) .. (1528.4300,442.9310) .. controls (1527.0200,442.6730)
        and (1525.7600,441.8430) .. (1524.5000,441.2100) .. controls
        (1521.4900,439.7030) and (1519.9300,444.1250) .. (1518.5200,445.9280) ..
        controls (1518.3000,445.6870) and (1518.0900,445.4470) .. (1517.8700,445.2080)
        .. controls (1517.3300,445.7770) and (1516.9700,446.7890) ..
        (1516.0900,446.4560) .. controls (1515.3200,446.1670) and (1513.1600,446.6980)
        .. (1512.4400,447.0580) .. controls (1511.1400,447.7120) and
        (1509.6000,447.6140) .. (1508.3300,447.0580) .. controls (1506.3700,446.1930)
        and (1505.6700,444.0220) .. (1503.8000,443.1100) .. controls
        (1501.7500,442.1080) and (1499.6900,440.9630) .. (1497.4300,440.5620) ..
        controls (1496.2400,440.3520) and (1493.8200,439.8720) .. (1493.8200,441.7590)
        .. controls (1493.8200,442.8420) and (1494.0200,444.8110) ..
        (1493.2300,445.6760) .. controls (1492.8000,446.1470) and (1492.2200,445.2740)
        .. (1491.8100,445.2180) .. controls (1490.7700,445.0750) and
        (1489.6900,446.3110) .. (1488.6600,446.4840) .. controls (1487.4700,446.6840)
        and (1485.6600,445.9160) .. (1484.6800,445.2870) .. controls
        (1483.9300,444.8090) and (1483.9000,443.2460) .. (1482.8800,443.1980) ..
        controls (1483.6700,442.0780) and (1481.8200,440.8620) .. (1481.5900,442.3350)
        .. controls (1480.8200,441.6610) and (1478.8700,441.4080) ..
        (1478.6300,440.2460) .. controls (1478.4500,441.0860) and (1476.4200,442.4700)
        .. (1475.7500,442.9820) .. controls (1475.9900,442.4790) and
        (1475.8500,442.1680) .. (1475.2500,442.0460) .. controls (1475.8200,441.9240)
        and (1476.1800,441.4720) .. (1476.1800,440.8940) .. controls
        (1475.4500,441.5070) and (1472.0100,442.2410) .. (1471.0700,441.9740) ..
        controls (1471.8200,441.0580) and (1473.2200,441.0030) .. (1474.2900,441.0310)
        .. controls (1475.3900,441.0610) and (1475.2700,441.3480) ..
        (1475.7200,440.5040) .. controls (1476.0300,439.9170) and (1476.7000,439.6510)
        .. (1477.1200,439.1660) .. controls (1475.7900,438.5730) and
        (1471.2300,438.4960) .. (1470.1400,439.5980) .. controls (1468.4900,437.6650)
        and (1471.6200,438.6860) .. (1471.8600,438.1870) .. controls
        (1472.0500,437.7720) and (1472.0300,437.1920) .. (1471.7600,436.7980) ..
        controls (1471.2100,435.8750) and (1470.6000,437.1560) .. (1470.9000,435.7100)
        .. controls (1469.3100,437.7390) and (1469.4300,433.5570) ..
        (1467.9500,433.6220) .. controls (1468.9800,433.0650) and (1470.1500,432.5280)
        .. (1469.2700,431.1360) .. controls (1468.6300,430.1320) and
        (1466.8300,430.6520) .. (1466.3900,429.9060) .. controls (1465.9400,429.1340)
        and (1465.4800,428.0530) .. (1464.8000,429.4040) .. controls
        (1464.5000,430.0030) and (1462.3700,428.3920) .. (1462.3300,427.8620) ..
        controls (1464.4800,428.3760) and (1462.6200,426.1030) .. (1462.7000,425.2170)
        .. controls (1462.8000,424.4840) and (1463.9200,425.0190) ..
        (1464.1400,425.3790) .. controls (1464.5900,426.1250) and (1464.4400,427.3480)
        .. (1465.1400,427.9340) .. controls (1464.9900,426.3380) and
        (1467.4700,428.3350) .. (1468.1600,426.7100) .. controls (1466.7300,426.5330)
        and (1466.1500,425.8380) .. (1465.2800,424.7660) .. controls
        (1466.0300,424.3520) and (1466.4200,423.4450) .. (1467.3000,423.2540) ..
        controls (1466.9100,422.0860) and (1465.7000,423.2940) .. (1465.8100,421.9760)
        .. controls (1465.9200,420.6620) and (1465.2300,420.4930) ..
        (1464.2700,419.6540) .. controls (1464.9100,418.9210) and (1465.6400,418.2770)
        .. (1466.2200,417.4940) .. controls (1464.1700,416.4490) and
        (1462.2300,418.6040) .. (1460.1700,417.9290);

        % path3606
        \path[country]
        (1457.4500,412.5960) .. controls (1456.8700,411.6470) and
        (1458.7200,410.6290) .. (1459.0800,411.6170) .. controls (1459.2900,412.1910)
        and (1457.8000,412.5720) .. (1457.4500,412.5960);
    
    \end{scope}
    
    
    % //////// UKRAINE /////////////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        \path[country]
        (1498.1345,309.0368) .. controls (1495.6646,309.8438) and (1496.5113,309.6936)
        .. (1492.8014,309.1726) .. controls (1492.5014,311.8666) and
        (1491.0143,311.4589) .. (1489.5743,311.1089) .. controls (1488.8444,310.9359)
        and (1487.8006,310.8929) .. (1487.0607,311.0749) .. controls
        (1486.8307,311.1329) and (1485.8500,311.6395) .. (1485.6000,311.5165) ..
        controls (1484.0300,310.7385) and (1482.8391,312.2966) .. (1482.1691,313.5886)
        .. controls (1481.2291,315.4066) and (1482.6410,315.9429) ..
        (1482.2710,317.5969) .. controls (1481.9610,318.9369) and (1479.8157,316.3801)
        .. (1479.3157,316.2721) .. controls (1478.5257,316.1001) and
        (1477.5799,316.8299) .. (1476.8700,316.4759) .. controls (1476.3199,316.2029)
        and (1475.9232,316.2309) .. (1475.4432,316.5779) .. controls
        (1473.7732,317.7828) and (1473.8557,316.1228) .. (1472.7256,315.5248) ..
        controls (1471.6557,314.9558) and (1469.8862,315.4265) .. (1470.0762,316.8836)
        .. controls (1469.5261,316.6356) and (1469.4991,315.8038) ..
        (1468.9892,315.5928) .. controls (1468.4591,315.3678) and (1467.8186,315.9567)
        .. (1467.3586,315.6268) .. controls (1466.7286,315.1618) and
        (1466.0604,315.2071) .. (1465.3205,315.2871) .. controls (1464.3305,315.3991)
        and (1463.8539,314.7315) .. (1463.7239,315.9325) .. controls
        (1462.9339,315.7315) and (1462.3041,314.8902) .. (1461.4140,315.1852) ..
        controls (1460.3840,315.5281) and (1459.7921,314.7842) .. (1459.1721,314.0981)
        .. controls (1458.5820,313.4432) and (1455.9258,313.7287) ..
        (1455.0958,313.5207) .. controls (1453.4158,313.0957) and (1451.9803,312.4316)
        .. (1450.1702,312.5016) .. controls (1448.1402,312.5796) and
        (1446.0619,312.7634) .. (1444.0219,312.7734) .. controls (1443.1218,312.7774)
        and (1441.6086,312.5188) .. (1440.9987,313.4188) .. controls
        (1440.5187,314.1328) and (1439.8324,314.7462) .. (1439.0624,315.1512) ..
        controls (1438.2324,315.5862) and (1436.1731,314.0608) .. (1436.0731,315.5588)
        .. controls (1435.9531,317.2978) and (1438.4233,321.0674) ..
        (1440.1834,321.4694) .. controls (1439.7834,321.6734) and (1439.4045,321.8669)
        .. (1438.9945,322.0469) .. controls (1441.0944,323.9109) and
        (1439.1957,324.5917) .. (1437.6357,325.5457) .. controls (1436.2257,326.4037)
        and (1435.0631,327.7956) .. (1433.9331,328.9766) .. controls
        (1432.5731,330.4086) and (1430.8750,331.7681) .. (1431.7251,333.8342) ..
        controls (1431.9851,334.4712) and (1431.6246,335.6201) .. (1432.2346,336.0421)
        .. controls (1432.6546,336.3351) and (1433.0140,336.3973) ..
        (1432.9139,336.9593) .. controls (1431.9940,336.3083) and (1430.9841,335.9460)
        .. (1430.6041,336.2120) .. controls (1430.2141,336.4790) and
        (1430.4106,337.4752) .. (1430.0606,338.1822) .. controls (1429.4406,339.4452)
        and (1428.1661,340.4667) .. (1428.3961,341.9867) -- (1428.4301,341.9867) ..
        controls (1429.2902,342.1827) and (1429.4267,342.8345) .. (1430.0267,343.2775)
        .. controls (1430.5568,343.6695) and (1430.8695,343.4249) ..
        (1431.4194,344.0249) .. controls (1432.1894,344.8759) and (1433.6954,344.2792)
        .. (1433.6954,345.8252) .. controls (1435.0253,345.4842) and
        (1435.2247,344.1938) .. (1436.6847,345.2138) .. controls (1437.5647,345.8248)
        and (1438.5241,345.4884) .. (1439.5041,345.6554) .. controls
        (1440.4641,345.8204) and (1440.9878,346.1510) .. (1442.0177,346.0290) ..
        controls (1442.8378,345.9290) and (1443.7554,345.6621) .. (1444.5655,345.9271)
        .. controls (1446.2855,346.4821) and (1447.2833,348.9412) ..
        (1449.0833,346.9122) .. controls (1450.3134,345.5352) and (1452.1011,345.8733)
        .. (1453.7711,345.7233) .. controls (1455.1211,345.6023) and
        (1455.8248,345.7125) .. (1456.2847,344.3985) .. controls (1456.4847,343.8295)
        and (1457.1575,343.5694) .. (1457.6775,343.4474) .. controls
        (1458.2075,343.3204) and (1459.2059,343.4348) .. (1459.5458,343.0058) ..
        controls (1459.3459,342.2168) and (1460.0188,342.0625) .. (1460.5989,342.1905)
        .. controls (1463.5689,342.8425) and (1464.3445,341.0892) ..
        (1465.3545,341.4092) .. controls (1466.6245,341.8112) and (1468.2665,344.6809)
        .. (1469.7365,343.9909) .. controls (1469.9765,345.2369) and
        (1470.8413,343.6160) .. (1471.0613,344.9081) .. controls (1471.3813,343.4520)
        and (1472.9750,344.5897) .. (1473.5750,345.2817) .. controls
        (1475.0150,346.9357) and (1474.4191,344.5316) .. (1475.7490,346.5386) ..
        controls (1476.2691,347.3366) and (1476.4140,348.1145) .. (1476.9040,348.8485)
        .. controls (1477.0940,349.1355) and (1478.0268,351.8860) ..
        (1478.2967,351.5320) .. controls (1479.1967,350.3580) and (1479.2163,352.8272)
        .. (1478.8063,353.4683) .. controls (1480.3862,353.6812) and
        (1483.6855,356.7384) .. (1481.7955,357.6804) .. controls (1482.4556,357.9544)
        and (1482.7260,358.5864) .. (1483.4260,358.8014) .. controls
        (1481.8161,360.5054) and (1478.8332,356.8232) .. (1477.7532,359.0392) ..
        controls (1477.5733,358.6112) and (1477.4037,358.1853) .. (1477.2437,357.7483)
        .. controls (1475.3737,358.4283) and (1475.6070,358.8160) ..
        (1475.8170,360.3300) .. controls (1476.0670,362.0560) and (1475.0145,362.9386)
        .. (1474.0845,364.1005) .. controls (1473.2446,365.1545) and
        (1473.7724,366.1764) .. (1472.0124,366.4784) .. controls (1470.3025,366.7714)
        and (1472.5856,367.9678) .. (1472.8956,368.1768) .. controls
        (1474.9356,369.5468) and (1475.3317,368.2491) .. (1477.1418,367.8032) ..
        controls (1478.5518,367.4552) and (1481.1019,365.9830) .. (1481.4218,369.0600)
        .. controls (1482.5719,368.6990) and (1482.0342,366.7613) ..
        (1481.0142,366.6143) .. controls (1481.1742,366.3663) and (1481.3098,366.1339)
        .. (1481.4899,365.9009) .. controls (1480.0498,366.5599) and
        (1480.7001,364.9372) .. (1481.1501,364.4402) .. controls (1481.3501,366.6602)
        and (1483.0874,363.5251) .. (1484.0375,363.4551) .. controls
        (1483.9125,363.9746) and (1483.5770,364.3700) .. (1483.1882,364.7120) ..
        controls (1484.5429,363.7982) and (1486.2847,362.4936) .. (1486.0077,361.5529)
        .. controls (1485.6977,360.4899) and (1484.0338,360.4029) ..
        (1483.6639,359.3449) .. controls (1484.6738,358.6089) and (1486.1055,360.8978)
        .. (1486.2455,361.6548) .. controls (1487.7655,360.0608) and
        (1487.3721,357.5879) .. (1489.9820,357.1369) .. controls (1490.5920,357.0309)
        and (1491.7800,357.5770) .. (1492.1900,357.0010) .. controls
        (1492.4801,356.5910) and (1492.5952,355.7992) .. (1493.1752,355.6762) ..
        controls (1492.8452,356.1422) and (1492.8132,356.6089) .. (1493.0732,357.1029)
        .. controls (1493.5433,356.8039) and (1495.4851,357.3425) ..
        (1495.4851,356.4915) .. controls (1495.4751,355.9355) and (1495.5211,355.4307)
        .. (1495.4851,354.9289) .. controls (1495.5631,355.5934) and
        (1495.6396,356.2729) .. (1496.1305,356.7632) .. controls (1497.3304,357.9452)
        and (1499.1385,357.2811) .. (1500.4785,356.8991) .. controls
        (1498.4985,358.3761) and (1495.3553,358.6975) .. (1493.0053,357.5445) ..
        controls (1493.9253,358.8605) and (1498.6336,358.3045) .. (1494.8735,359.7865)
        .. controls (1496.1436,359.4155) and (1497.3324,360.3325) ..
        (1498.3724,360.9075) .. controls (1499.5824,361.5765) and (1500.4153,361.4370)
        .. (1501.7354,361.4170) .. controls (1502.9553,361.3970) and
        (1504.4299,360.8021) .. (1505.5399,361.3491) .. controls (1506.2148,361.6846)
        and (1506.4938,361.8178) .. (1506.7288,361.7907) .. controls
        (1506.7718,361.7857) and (1506.8559,361.7041) .. (1506.8987,361.6888) --
        (1508.3593,360.8056) .. controls (1508.2803,360.7173) and (1508.0260,360.5702)
        .. (1507.9857,360.4999) .. controls (1511.9257,361.1909) and
        (1511.3127,360.6753) .. (1511.2127,359.9903) .. controls (1511.1927,359.8653)
        and (1512.5756,361.5210) .. (1512.4356,361.4510) .. controls
        (1512.5656,360.3120) and (1512.8948,360.9494) .. (1513.2849,361.0094) ..
        controls (1513.5748,361.0514) and (1514.0641,360.9635) .. (1513.9642,360.8735)
        .. controls (1513.9641,359.8715) and (1514.0022,360.9038) ..
        (1513.8623,361.6888) .. controls (1512.4623,360.6398) and (1513.8053,364.9186)
        .. (1514.7455,360.8396) .. controls (1516.0054,361.3526) and
        (1514.9852,361.8814) .. (1515.0852,362.0964) .. controls (1515.1552,361.8224)
        and (1516.4138,362.7932) .. (1516.6137,363.4892) .. controls
        (1516.6537,363.2442) and (1515.8482,360.6989) .. (1516.1383,360.4999) ..
        controls (1516.9582,359.9509) and (1518.7866,359.6919) .. (1517.8366,358.3259)
        .. controls (1520.5466,358.6799) and (1517.1214,361.3048) ..
        (1517.0213,361.7228) .. controls (1519.4514,361.1038) and (1519.8427,357.7251)
        .. (1522.2527,357.0011) .. controls (1523.6926,356.5691) and
        (1524.6532,356.9309) .. (1526.0232,356.1518) .. controls (1526.8332,355.6888)
        and (1528.0648,355.6155) .. (1528.6048,356.5255) .. controls
        (1528.9049,355.2545) and (1530.3122,354.6453) .. (1531.4923,354.5553) ..
        controls (1532.4922,354.4793) and (1532.6283,353.4425) .. (1533.5982,353.2645)
        .. controls (1534.5783,353.0875) and (1536.6508,353.5666) ..
        (1537.4708,353.0946) .. controls (1538.1207,352.7086) and (1537.5658,351.9142)
        .. (1538.1162,351.4301) .. controls (1537.6561,351.4021) and
        (1536.3990,350.1549) .. (1539.3390,348.4409) .. controls (1540.3291,348.1049)
        and (1540.3375,347.1884) .. (1541.0375,346.8104) .. controls
        (1541.7875,346.4054) and (1542.4755,346.8965) .. (1543.2454,346.7425) ..
        controls (1544.5655,346.4795) and (1546.6277,347.6179) .. (1547.4576,346.2669)
        .. controls (1547.7176,345.8369) and (1548.4189,343.5010) ..
        (1548.2389,342.9040) .. controls (1547.8589,343.0020) and (1547.5199,342.9422)
        .. (1547.2199,342.7002) .. controls (1548.6298,341.6722) and
        (1545.8952,340.7253) .. (1545.7252,340.3563) .. controls (1545.2452,339.2773)
        and (1546.7095,338.5037) .. (1547.5596,338.7597) .. controls
        (1547.5296,337.1877) and (1546.2233,338.7169) .. (1545.6234,337.4689) ..
        controls (1545.1733,336.5109) and (1546.4042,336.6550) .. (1546.9141,336.2800)
        .. controls (1548.6942,334.9640) and (1546.4477,332.8590) ..
        (1547.4576,331.8980) .. controls (1546.6377,331.6000) and (1546.3357,332.4827)
        .. (1545.2157,332.2037) .. controls (1544.5857,332.0447) and
        (1543.8693,331.7206) .. (1543.4494,331.2186) .. controls (1542.5893,330.2016)
        and (1541.3899,331.0921) .. (1540.6299,329.5881) .. controls
        (1539.7598,330.6111) and (1536.9243,329.4268) .. (1535.8742,328.8748) ..
        controls (1533.8342,327.8088) and (1534.5989,328.4852) .. (1532.9188,329.4522)
        .. controls (1532.5089,328.2642) and (1530.5836,327.9618) ..
        (1529.9636,326.6328) .. controls (1529.5836,325.8158) and (1528.7178,324.6563)
        .. (1527.5178,324.9683) .. controls (1525.4178,325.5103) and
        (1524.0060,326.7687) .. (1522.9660,326.7687) .. controls (1521.3460,326.2657)
        and (1519.9979,324.8004) .. (1518.6179,324.9344) .. controls
        (1517.8379,325.0144) and (1516.8167,326.1313) .. (1515.6966,324.9684) ..
        controls (1513.2566,320.4674) and (1513.8623,320.2910) .. (1513.8623,319.9070)
        .. controls (1512.5123,319.9800) and (1511.7594,317.9661) ..
        (1510.4993,318.6501) .. controls (1509.3893,319.2521) and (1507.0074,318.3407)
        .. (1506.1173,318.0387) .. controls (1507.1874,317.4047) and
        (1504.7903,315.0356) .. (1505.0303,314.7776) .. controls (1505.4404,314.3376)
        and (1506.4705,314.3274) .. (1507.0005,313.9964) .. controls
        (1506.3305,312.6103) and (1505.1052,313.3423) .. (1504.0453,310.8033) ..
        controls (1503.7553,310.1023) and (1502.4453,308.6988) .. (1501.7354,309.1048)
        .. controls (1500.4753,309.8178) and (1499.3046,308.9569) ..
        (1498.1346,309.0369) -- cycle;
    
    \end{scope}
    
    
    % //////// UNITED KINGDOM //////////////////////////////////////////////////////////////////////
    
    \begin{scope}[shift={(-1072.0076,-94.98601)}]
    
        % path2690
        \path[country]
        (1230.6100,291.9600) .. controls (1231.2200,290.9900) and (1232.5900,291.0090)
        .. (1233.4900,290.4480) .. controls (1233.1600,290.2050) and
        (1232.8400,289.9400) .. (1232.5500,289.6550) .. controls (1234.4000,290.2320)
        and (1235.1100,288.1660) .. (1235.9900,287.1550) .. controls
        (1236.8300,286.1940) and (1238.5700,287.4580) .. (1238.8200,285.6950) ..
        controls (1240.4500,286.4500) and (1242.4900,284.5670) .. (1244.1200,285.6940)
        .. controls (1244.7800,286.1500) and (1245.1700,287.2160) ..
        (1245.4800,287.9030) .. controls (1245.3800,287.7790) and (1246.6900,289.2530)
        .. (1246.6600,288.9910) .. controls (1246.6600,289.2690) and
        (1245.2700,289.9650) .. (1245.0800,290.1590) .. controls (1245.5800,290.1090)
        and (1247.0700,289.4710) .. (1247.4000,290.1290) .. controls
        (1247.7400,290.7970) and (1248.3800,292.1570) .. (1247.2400,292.4630) ..
        controls (1247.4200,291.7550) and (1247.1400,290.8110) .. (1246.2300,291.0230)
        .. controls (1246.7900,291.3540) and (1246.7200,291.9360) ..
        (1246.3700,292.3910) .. controls (1246.6600,292.2370) and (1246.9100,292.2580)
        .. (1247.1200,292.4510) .. controls (1247.2200,292.9440) and
        (1246.0700,293.5820) .. (1245.6900,293.6220) .. controls (1244.7100,293.7250)
        and (1244.7100,295.3610) .. (1243.5200,295.0080) .. controls
        (1242.5200,294.7110) and (1242.3400,294.3990) .. (1241.4800,294.9580) ..
        controls (1240.7600,295.4340) and (1239.5700,294.9480) .. (1239.8900,293.9720)
        .. controls (1239.4900,293.9920) and (1236.7400,290.9260) ..
        (1236.5500,292.8940) .. controls (1236.2300,296.3730) and (1231.9600,293.0820)
        .. (1230.6100,291.9550);

        % path2640
        \path[country]
        (1238.8900,270.2100) .. controls (1237.9400,269.8700) and
        (1238.4900,268.9040) .. (1239.3200,268.6260) .. controls (1238.1000,266.2470)
        and (1236.8800,270.6660) .. (1238.8900,270.2100);

        % path2642
        \path[country]
        (1239.2500,266.9700) .. controls (1239.2500,266.7510) and
        (1240.5800,265.8670) .. (1239.9900,265.6910) .. controls (1239.3300,265.4930)
        and (1237.7500,265.3690) .. (1237.8100,266.4660) .. controls
        (1238.3500,266.4560) and (1238.8300,266.6210) .. (1239.2500,266.9700);

        % path2644
        \path[country]
        (1238.8900,267.7700) .. controls (1239.0900,267.0000) and
        (1238.8900,266.8800) .. (1238.1700,267.4100) .. controls (1238.4100,267.5300)
        and (1238.6500,267.6500) .. (1238.8900,267.7700);

        % path2646
        \path[country]
        (1240.4000,275.5400) .. controls (1240.7200,275.2500) and
        (1241.0800,275.0100) .. (1241.4800,274.8190) .. controls (1240.9000,274.6890)
        and (1240.5200,274.9720) .. (1240.4000,275.5400);

        % path2648
        \path[country]
        (1243.0600,263.0900) .. controls (1244.2300,264.7130) and
        (1245.5600,261.6730) .. (1244.2200,262.1530) .. controls (1244.9200,262.0630)
        and (1247.2500,261.0890) .. (1245.7300,260.7860) .. controls
        (1247.0700,260.1770) and (1246.8100,258.3970) .. (1245.4000,259.3740) ..
        controls (1244.7000,259.8540) and (1243.8800,259.9660) .. (1243.1600,260.3940)
        .. controls (1242.3900,260.8590) and (1243.0600,261.6690) ..
        (1242.0600,262.0100) .. controls (1242.0600,261.7450) and (1242.0600,261.4810)
        .. (1241.9600,261.2180) .. controls (1241.4100,261.3240) and
        (1240.9300,261.5650) .. (1240.5200,261.9380) .. controls (1241.1300,262.3730)
        and (1241.4900,262.8470) .. (1240.4200,263.0900) .. controls
        (1240.9400,263.2010) and (1241.4200,263.4170) .. (1241.8600,263.7370) ..
        controls (1241.3600,263.9680) and (1240.8800,264.2320) .. (1240.4200,264.5290)
        .. controls (1241.2100,265.8440) and (1242.8300,263.9560) ..
        (1243.0100,263.0900);

        % path2650
        \path[country]
        (1241.9800,274.5300) .. controls (1242.5300,274.3460) and
        (1242.9600,274.0100) .. (1243.2800,273.5210) .. controls (1242.7300,273.6640)
        and (1242.2500,274.0310) .. (1241.9800,274.5300);

        % path2652
        \path[country]
        (1243.5700,282.6000) .. controls (1244.7600,282.0710) and
        (1245.7800,280.9180) .. (1244.1600,280.0130) .. controls (1243.1200,279.4330)
        and (1242.5500,281.1770) .. (1242.2000,281.8080) .. controls
        (1242.6800,281.5150) and (1243.1800,281.2750) .. (1243.7100,281.0880) ..
        controls (1243.8100,281.6060) and (1243.8100,282.1100) ..
        (1243.5700,282.6000);

        % path2654
        \path[country]
        (1246.5200,270.8600) .. controls (1247.3500,270.6310) and
        (1248.6700,269.8910) .. (1248.5300,268.8430) .. controls (1245.3700,269.9580)
        and (1246.7100,266.1380) .. (1245.0100,265.5310) .. controls
        (1244.8300,265.9950) and (1244.7300,266.4740) .. (1244.7200,266.9700) ..
        controls (1243.2900,266.6350) and (1243.4800,267.5410) .. (1242.4100,267.3300)
        .. controls (1242.2300,268.7770) and (1243.9900,267.8790) ..
        (1244.6500,268.5540) .. controls (1243.0100,268.6720) and (1244.6500,269.6970)
        .. (1245.3100,269.6910) .. controls (1246.0000,269.6910) and
        (1246.7800,269.3340) .. (1247.4500,269.6310) .. controls (1246.8600,269.7720)
        and (1246.4700,270.2380) .. (1246.5200,270.8570);

        % path2656
        \path[country]
        (1245.7300,328.6100) .. controls (1246.6100,328.8100) and
        (1247.8700,327.0930) .. (1248.5500,326.5530) .. controls (1249.7900,325.5590)
        and (1252.2300,326.3840) .. (1253.0700,324.8660) .. controls
        (1253.0700,325.7970) and (1254.9300,326.6980) .. (1255.6900,326.7570) ..
        controls (1257.1200,326.8680) and (1258.0500,324.0490) .. (1258.0400,322.9930)
        .. controls (1258.4900,323.8330) and (1260.0600,322.9930) ..
        (1260.6300,322.7820) .. controls (1262.1500,322.2470) and (1263.7000,322.9440)
        .. (1264.8100,324.0020) .. controls (1264.9100,323.0720) and
        (1265.8500,323.3530) .. (1266.4700,323.4660) .. controls (1267.1500,323.5900)
        and (1269.0900,322.9900) .. (1267.2600,322.6340) .. controls
        (1268.0900,322.6340) and (1273.3300,322.6040) .. (1271.8600,321.1940) ..
        controls (1272.7400,322.0890) and (1273.8500,321.3890) .. (1274.8900,321.6270)
        .. controls (1275.1600,321.6770) and (1275.2800,321.8300) ..
        (1275.2500,322.0790) .. controls (1275.2500,322.5060) and (1276.9900,322.0390)
        .. (1276.9800,322.0390) .. controls (1278.5100,321.8450) and
        (1279.9700,321.7750) .. (1281.4700,322.2180) .. controls (1282.7300,322.5900)
        and (1284.5000,321.6220) .. (1285.7400,321.2970) .. controls
        (1286.8300,321.0100) and (1287.0700,320.6500) .. (1287.8000,319.9790) ..
        controls (1288.5900,319.2570) and (1290.1200,319.4170) .. (1290.5900,318.3290)
        .. controls (1291.1100,317.1220) and (1285.4800,316.9550) ..
        (1284.8900,316.8740) .. controls (1285.2900,316.7670) and (1285.6800,316.6220)
        .. (1286.0500,316.4410) .. controls (1285.3200,316.2720) and
        (1284.5500,316.0930) .. (1283.8900,316.5860) .. controls (1284.5400,315.8930)
        and (1285.4200,316.1690) .. (1286.2400,316.0110) .. controls
        (1287.6100,315.7440) and (1287.5600,314.3590) .. (1286.1400,314.2100) ..
        controls (1286.6700,314.3200) and (1287.0100,313.8770) .. (1287.4300,313.6720)
        .. controls (1288.2600,313.2650) and (1288.8900,314.0960) ..
        (1289.8100,313.2730) .. controls (1289.5800,312.7790) and (1289.2000,312.4910)
        .. (1288.6600,312.4090) .. controls (1289.2300,312.3020) and
        (1290.6100,312.3890) .. (1289.0900,311.8340) .. controls (1291.1900,312.4640)
        and (1291.4900,311.1060) .. (1292.3800,309.6110) .. controls
        (1293.5500,307.6730) and (1293.3400,305.8000) .. (1291.0900,304.6860) ..
        controls (1289.7900,304.0400) and (1286.8100,303.1380) .. (1285.5300,304.2430)
        .. controls (1285.0800,304.6220) and (1284.9300,305.4430) ..
        (1284.3400,305.6410) .. controls (1283.4400,305.9420) and (1282.9000,304.4960)
        .. (1281.9600,304.7050) .. controls (1283.1300,302.9400) and
        (1285.5400,302.8300) .. (1283.5200,300.2510) .. controls (1281.8500,298.1160)
        and (1280.0100,298.2410) .. (1277.6500,297.9360) .. controls
        (1279.2200,297.2570) and (1282.0000,297.8460) .. (1283.2600,298.8730) ..
        controls (1282.9700,297.8680) and (1279.7600,295.1120) .. (1282.0400,294.4800)
        .. controls (1280.5600,294.1020) and (1280.2800,292.6160) ..
        (1279.3000,291.6720) .. controls (1278.3800,290.7900) and (1276.9700,290.8180)
        .. (1275.8200,290.6380) .. controls (1273.8900,290.3360) and
        (1273.3600,285.7390) .. (1273.2400,284.2480) .. controls (1273.0400,281.7670)
        and (1269.9300,279.6170) .. (1267.5500,279.1810) .. controls
        (1266.9300,279.0670) and (1266.4000,278.1980) .. (1265.7200,278.8080) ..
        controls (1265.2900,279.2020) and (1264.8800,279.3910) .. (1264.2900,279.3820)
        .. controls (1262.7400,279.3620) and (1260.5900,279.4520) ..
        (1259.4300,278.2080) .. controls (1261.8400,280.0000) and (1263.4800,277.4870)
        .. (1265.9100,277.4870) .. controls (1267.2900,277.4870) and
        (1266.8000,276.4200) .. (1266.0700,275.8470) .. controls (1265.0400,275.0370)
        and (1264.0000,276.3240) .. (1262.8800,276.1910) .. controls
        (1265.7200,275.6380) and (1268.0400,274.3160) .. (1269.8700,272.0630) ..
        controls (1270.6900,271.0500) and (1270.9400,269.8530) .. (1271.6400,268.8160)
        .. controls (1272.1200,268.0950) and (1273.4500,267.6260) ..
        (1273.0800,266.5600) .. controls (1272.4000,264.6360) and (1268.6000,265.3710)
        .. (1267.0200,265.5470) .. controls (1265.3800,265.7300) and
        (1263.8000,265.0840) .. (1262.2000,265.5570) .. controls (1260.8600,265.9600)
        and (1259.3300,266.7970) .. (1257.9900,267.0420) .. controls
        (1258.1900,266.3580) and (1258.9800,266.2970) .. (1259.2100,265.6020) ..
        controls (1258.4200,265.5320) and (1257.7100,265.9030) .. (1256.9800,266.1060)
        .. controls (1257.8500,265.2120) and (1260.0400,265.8330) ..
        (1260.4400,264.4510) .. controls (1259.4000,264.2080) and (1258.1600,264.4510)
        .. (1257.2700,263.7300) .. controls (1258.9800,264.3840) and
        (1258.6500,263.9540) .. (1259.7700,263.2040) .. controls (1260.6900,262.5850)
        and (1261.8000,262.3240) .. (1262.7400,261.7280) .. controls
        (1263.1200,261.4830) and (1268.0100,258.2930) .. (1265.4600,257.7800) ..
        controls (1263.9100,257.4670) and (1261.9800,258.2150) .. (1260.4600,258.5100)
        .. controls (1259.6200,258.6750) and (1258.7200,258.8820) ..
        (1257.8600,258.8120) .. controls (1257.6400,258.7920) and (1257.3500,258.7520)
        .. (1257.2100,258.5690) .. controls (1256.9700,258.2700) and
        (1255.9600,259.0260) .. (1255.6100,259.1950) .. controls (1256.3800,257.9430)
        and (1255.7100,258.8070) .. (1255.1500,258.4720) .. controls
        (1254.9300,258.3380) and (1254.5500,257.8530) .. (1254.2400,257.9250) ..
        controls (1253.6100,258.0710) and (1253.8500,259.9040) .. (1252.9500,260.3470)
        .. controls (1253.2300,260.4970) and (1253.8100,260.7020) ..
        (1253.8100,260.9950) .. controls (1251.6300,259.9940) and (1252.2900,262.3730)
        .. (1251.2200,262.7230) .. controls (1251.7700,262.9510) and
        (1252.2200,263.3930) .. (1252.4400,263.9480) .. controls (1251.7400,264.2210)
        and (1249.2300,263.2860) .. (1249.4200,264.7390) .. controls
        (1249.2000,263.4040) and (1247.5800,265.6670) .. (1249.3200,266.7560) ..
        controls (1248.8400,266.6960) and (1248.3600,266.6660) .. (1247.8800,266.6860)
        .. controls (1247.7700,268.0800) and (1248.9200,268.0870) ..
        (1249.9700,267.9820) .. controls (1249.4400,268.1490) and (1248.9600,268.4130)
        .. (1248.5300,268.7740) .. controls (1249.1700,268.5360) and
        (1249.8800,268.6700) .. (1250.2600,269.2790) .. controls (1249.3200,268.1910)
        and (1248.0600,270.2850) .. (1250.1600,270.1420) .. controls
        (1249.9400,270.2220) and (1246.4900,270.3720) .. (1248.8700,271.2220) ..
        controls (1247.8400,270.3010) and (1246.6800,272.0250) .. (1248.0800,272.3020)
        .. controls (1247.5000,272.2220) and (1247.1600,272.5130) ..
        (1247.1400,273.0940) .. controls (1246.3600,272.7220) and (1245.3500,272.8170)
        .. (1244.6900,273.3820) .. controls (1245.8300,273.6480) and
        (1247.4100,272.8850) .. (1248.4300,273.5980) .. controls (1247.6200,273.2260)
        and (1247.0900,274.1860) .. (1246.2700,273.8140) .. controls
        (1246.9500,276.7800) and (1250.6300,273.1830) .. (1251.8200,272.5180) ..
        controls (1251.3500,273.0390) and (1251.0700,273.8640) .. (1252.2500,273.3820)
        .. controls (1251.6700,273.4990) and (1248.6500,274.8740) ..
        (1250.6000,274.6780) .. controls (1250.3600,274.9150) and (1250.1100,275.1560)
        .. (1249.8700,275.3980) .. controls (1250.3900,275.4280) and
        (1250.8900,275.3780) .. (1251.3900,275.2540) .. controls (1251.0900,275.4150)
        and (1249.7300,275.4710) .. (1249.6500,275.5790) .. controls
        (1249.4000,275.8850) and (1249.0300,276.1460) .. (1248.7000,276.3550) ..
        controls (1248.3200,276.6000) and (1248.5900,277.2980) .. (1248.5400,277.6870)
        .. controls (1248.5400,278.1080) and (1246.5200,280.8560) ..
        (1248.2200,278.8540) .. controls (1247.3700,279.4460) and (1247.5200,281.6850)
        .. (1248.7200,280.6540) .. controls (1247.4000,281.3980) and
        (1247.3600,282.8340) .. (1246.5000,283.9240) .. controls (1245.8900,284.6870)
        and (1247.7900,285.2520) .. (1247.9800,283.7280) .. controls
        (1248.1200,282.6370) and (1249.5700,281.3730) .. (1249.2000,280.3330) ..
        controls (1248.6800,278.8540) and (1250.9000,277.9490) .. (1251.8200,277.4150)
        .. controls (1251.2100,277.9490) and (1249.5900,278.7610) ..
        (1249.7600,279.7870) .. controls (1249.8800,280.2720) and (1250.1600,280.3930)
        .. (1250.6000,280.1500) .. controls (1250.8400,280.6130) and
        (1251.1500,281.0220) .. (1251.5300,281.3750) .. controls (1251.7000,280.7620)
        and (1251.3400,280.1510) .. (1250.8100,279.8630) .. controls
        (1251.3800,279.0970) and (1251.6800,279.6030) .. (1251.8200,280.2220) ..
        controls (1252.8300,279.3250) and (1252.1300,277.6070) .. (1253.3300,277.8460)
        .. controls (1252.8300,278.2650) and (1252.7600,278.7450) ..
        (1253.1200,279.2860) .. controls (1252.9700,277.9250) and (1253.8000,279.3660)
        .. (1254.6300,279.7180) .. controls (1254.0700,279.6880) and
        (1252.7800,279.2080) .. (1252.5400,280.0350) .. controls (1252.0800,281.6170)
        and (1253.1400,281.5890) .. (1253.6400,282.7070) .. controls
        (1254.4800,284.6120) and (1250.1900,285.7210) .. (1251.0300,287.9980) ..
        controls (1250.9300,287.8370) and (1249.9900,286.9660) .. (1249.8600,287.4610)
        .. controls (1249.6100,288.4100) and (1251.1500,289.7080) ..
        (1251.6800,290.3020) .. controls (1251.1200,288.6450) and (1251.7800,288.3170)
        .. (1253.3300,289.0200) .. controls (1254.6100,289.6010) and
        (1254.8600,289.5590) .. (1254.9100,287.9990) .. controls (1256.4100,289.4790)
        and (1257.3400,288.8860) .. (1259.0200,288.3990) .. controls
        (1259.5400,288.2480) and (1260.3500,288.0800) .. (1260.2400,287.3510) ..
        controls (1261.3900,287.4920) and (1262.5500,287.4110) .. (1263.7000,287.4950)
        .. controls (1262.4100,288.3550) and (1260.8500,288.4670) ..
        (1260.1000,290.0160) .. controls (1259.6300,290.9960) and (1260.5200,294.2740)
        .. (1261.9700,293.4720) .. controls (1261.7600,294.0130) and
        (1261.8600,294.4930) .. (1262.2600,294.9110) .. controls (1262.5700,294.5040)
        and (1262.8300,294.0730) .. (1263.0500,293.6160) .. controls
        (1263.2600,294.5020) and (1264.0200,294.0640) .. (1264.4900,293.7600) ..
        controls (1264.0200,294.4020) and (1264.0300,295.2210) .. (1263.4800,295.9200)
        .. controls (1263.1700,296.3260) and (1261.8900,297.9840) ..
        (1263.6300,297.7200) .. controls (1261.8800,298.5930) and (1262.4300,301.5860)
        .. (1264.5600,300.8880) .. controls (1263.5900,301.5980) and
        (1260.6400,298.8840) .. (1262.1200,301.8240) .. controls (1260.1300,300.1260)
        and (1257.2900,301.8840) .. (1255.1300,301.8240) .. controls
        (1255.9300,300.8430) and (1253.4200,299.9270) .. (1252.7800,300.4660) ..
        controls (1251.4900,301.5560) and (1253.5900,303.0820) .. (1254.8400,301.9690)
        .. controls (1253.6700,303.2860) and (1252.0000,304.0560) ..
        (1250.8800,305.4250) .. controls (1252.3400,305.5390) and (1253.6700,303.8890)
        .. (1255.1300,304.6330) .. controls (1254.7700,305.2340) and
        (1255.1300,305.8250) .. (1255.6400,306.1450) .. controls (1254.7800,306.5430)
        and (1255.0100,307.6490) .. (1256.0000,307.5130) .. controls
        (1255.1900,307.6290) and (1255.1300,308.4040) .. (1254.8200,309.0010) ..
        controls (1254.4100,309.7840) and (1253.3800,310.2520) .. (1252.6000,310.5420)
        .. controls (1250.8600,311.1860) and (1248.3500,311.6270) ..
        (1247.2100,313.0570) .. controls (1247.8300,313.3050) and (1248.0600,313.8210)
        .. (1247.5700,314.3530) .. controls (1248.3500,314.5170) and
        (1249.1300,314.4230) .. (1249.6600,313.7770) .. controls (1249.2900,314.4710)
        and (1248.5300,314.6920) .. (1247.7900,314.6410) .. controls
        (1248.7700,315.8810) and (1251.7600,314.4700) .. (1252.7600,313.7770) ..
        controls (1252.7600,314.8200) and (1253.9100,314.8570) .. (1254.6300,314.6410)
        .. controls (1254.3300,315.0840) and (1253.9200,315.2040) ..
        (1253.4000,315.0010) .. controls (1253.6000,316.2520) and (1254.5300,315.6420)
        .. (1255.2700,315.2960) .. controls (1256.4100,314.7650) and
        (1257.0400,316.5180) .. (1258.0300,316.9530) .. controls (1259.8500,317.7450)
        and (1260.1500,316.1030) .. (1261.6300,315.8880) .. controls
        (1263.2500,315.6530) and (1264.3500,314.8100) .. (1265.6400,313.8480) ..
        controls (1264.4100,315.3280) and (1262.6700,316.3510) .. (1261.3200,317.7360)
        .. controls (1260.9700,318.0970) and (1261.4900,318.5320) ..
        (1260.7400,318.6280) .. controls (1259.9000,318.7360) and (1259.0400,318.7880)
        .. (1258.2000,318.6180) .. controls (1257.0100,318.3720) and
        (1255.0100,317.9590) .. (1253.8700,318.6480) .. controls (1253.1800,319.0600)
        and (1253.1400,319.8770) .. (1252.4400,320.2960) .. controls
        (1251.4800,320.8720) and (1251.2900,319.4400) .. (1250.9500,321.1470) ..
        controls (1250.8100,321.8330) and (1249.1200,324.4290) .. (1248.2500,324.2310)
        .. controls (1247.7100,324.1090) and (1247.5700,324.1310) ..
        (1247.3700,324.7310) .. controls (1247.0400,325.6860) and (1245.6900,326.1200)
        .. (1244.8500,326.4650) .. controls (1244.1700,326.7400) and
        (1243.4300,327.0390) .. (1242.8500,327.5010) .. controls (1242.6200,327.6910)
        and (1242.9500,328.3500) .. (1243.1800,328.2940) .. controls
        (1244.0800,328.0970) and (1245.1800,327.3180) .. (1245.6300,328.6140);

        % path2658
        \path[country]
        (1244.5000,271.5100) .. controls (1244.6400,271.4400) and
        (1244.7800,271.3660) .. (1244.9300,271.2940) .. controls (1244.7400,270.6090)
        and (1244.2600,270.4910) .. (1243.7800,271.0060) .. controls
        (1244.0200,271.1740) and (1244.2600,271.3420) .. (1244.5000,271.5100);

        % path2660
        \path[country]
        (1244.4300,276.8400) .. controls (1245.6900,276.7500) and
        (1246.8700,276.2300) .. (1248.1000,275.9760) .. controls (1247.8500,274.6190)
        and (1244.9900,273.2900) .. (1244.1400,274.7520) .. controls
        (1244.7200,274.8020) and (1245.2000,275.0370) .. (1245.5800,275.4720) ..
        controls (1245.0800,275.8580) and (1244.3900,276.4150) .. (1245.7300,276.1920)
        .. controls (1245.2100,276.2420) and (1244.7800,276.4620) ..
        (1244.4300,276.8400);

        % path2662
        \path[country]
        (1245.6600,280.8000) .. controls (1246.2700,279.8590) and
        (1247.3300,279.0900) .. (1247.5300,277.9200) .. controls (1246.5700,278.4950)
        and (1246.0400,279.6160) .. (1245.0100,280.0790) .. controls
        (1245.2000,280.3460) and (1245.4100,280.5860) .. (1245.6600,280.8000);

        % path2664
        \path[country]
        (1246.5200,268.4100) .. controls (1246.7400,267.9280) and
        (1246.8800,267.4240) .. (1246.9500,266.8970) .. controls (1246.5000,267.3150)
        and (1246.3500,267.8190) .. (1246.5200,268.4100);

        % path2666
        \path[country]
        (1250.4100,283.7500) .. controls (1251.3700,283.3610) and
        (1251.0700,281.3030) .. (1249.9700,281.3740) .. controls (1248.6900,281.4540)
        and (1249.2800,283.8220) .. (1250.4100,283.7500);

        % path2670
        \path[country]
        (1265.2400,256.7500) .. controls (1265.3800,256.1690) and
        (1265.2400,255.5910) .. (1264.5200,255.5250) .. controls (1264.3700,256.1100)
        and (1264.7100,256.5520) .. (1265.2400,256.7500);

        % path2672
        \path[country]
        (1265.2400,255.1700) .. controls (1265.9900,255.8490) and
        (1267.9900,256.1910) .. (1268.6200,255.1700) .. controls (1267.8400,255.1200)
        and (1266.5100,255.1700) .. (1266.2300,254.2040) .. controls
        (1266.0000,253.4220) and (1264.0300,254.1840) .. (1265.2400,255.1700);

        % path2674
        \path[country]
        (1266.9700,257.1100) .. controls (1267.2100,256.8740) and
        (1267.3300,256.5860) .. (1267.3300,256.2460) .. controls (1266.5600,256.1960)
        and (1266.4400,256.4800) .. (1266.9700,257.1100);

        % path2676
        \path[country]
        (1267.7600,253.1500) .. controls (1267.8600,252.6540) and
        (1267.6600,252.3180) .. (1267.1800,252.1420) .. controls (1266.9200,252.7090)
        and (1267.1800,253.0740) .. (1267.7600,253.1500);

        % path2678
        \path[country]
        (1268.9100,253.5100) .. controls (1269.3300,253.1670) and
        (1269.7900,252.8790) .. (1270.2800,252.6460) .. controls (1269.6400,252.5560)
        and (1269.1300,252.9310) .. (1268.9100,253.5100);

        % path2776
        \path[country]
        (1277.7700,246.9600) .. controls (1277.6500,247.2240) and
        (1277.5300,247.4880) .. (1277.4100,247.7520) .. controls (1278.9800,247.7520)
        and (1279.0600,245.0650) .. (1279.6400,244.0790) .. controls
        (1279.0400,244.0290) and (1278.7100,243.6850) .. (1278.8500,243.0730) ..
        controls (1278.6100,243.2410) and (1278.3700,243.4090) .. (1278.1300,243.5770)
        .. controls (1278.0300,243.0680) and (1278.1300,242.5870) ..
        (1278.4100,242.1360) .. controls (1277.5100,242.0130) and (1277.6700,243.1540)
        .. (1276.7600,242.9280) .. controls (1277.1500,243.4150) and
        (1277.6300,243.7990) .. (1278.2000,244.0790) .. controls (1277.5200,244.4600)
        and (1276.7500,244.6320) .. (1275.9700,244.5840) .. controls
        (1276.2200,245.8530) and (1276.3100,244.9150) .. (1277.2800,245.2430) ..
        controls (1278.0700,245.5120) and (1278.4700,246.3240) ..
        (1277.7700,246.9600);

        % path2778
        \path[country]
        (1279.4200,243.1400) .. controls (1279.9400,242.7370) and
        (1280.7200,241.5310) .. (1279.5200,241.4840) .. controls (1279.6200,242.0190)
        and (1279.1200,242.6400) .. (1279.4200,243.1400);

        % path2780
        \path[country]
        (1281.2200,241.7000) .. controls (1282.2700,239.9470) and
        (1279.1600,241.4350) .. (1281.2200,241.7000);

        % path2782
        \path[country]
        (1280.9300,242.5700) .. controls (1281.1700,242.4700) and
        (1281.4200,242.3790) .. (1281.6600,242.2830) .. controls (1280.9400,241.8930)
        and (1280.6900,241.9890) .. (1280.9300,242.5700);

        % path5354
        \path[country]
        (1272.3700,323.7800) .. controls (1272.9900,323.7200) and
        (1273.5300,323.3510) .. (1273.8800,322.8430) .. controls (1272.7000,322.1880)
        and (1272.0300,322.3960) .. (1270.9300,323.0590) .. controls
        (1271.4400,323.2320) and (1271.9200,323.4720) .. (1272.3700,323.7800);

    \end{scope}

}

